Rank-one matrix estimation: analysis of algorithmic and information theoretic limits by the spatial coupling method

Factorizing low-rank matrices is a problem with many applications in machine learning and statistics, ranging from sparse PCA to community detection and sub-matrix localization. For probabilistic models in the Bayes optimal setting, general expressions for the mutual information have been proposed using powerful heuristic statistical physics computations via the replica and cavity methods, and proven in few specific cases by a variety of methods. Here, we use the spatial coupling methodology developed in the framework of error correcting codes, to rigorously derive the mutual information for the symmetric rank-one case. We characterize the detectability phase transitions in a large set of estimation problems, where we show that there exists a gap between what currently known polynomial algorithms (in particular spectral methods and approximate message-passing) can do and what is expected information theoretically. Moreover, we show that the computational gap vanishes for the proposed spatially coupled model, a promising feature with many possible applications. Our proof technique has an interest on its own and exploits three essential ingredients: the interpolation method first introduced in statistical physics, the analysis of approximate message-passing algorithms first introduced in compressive sensing, and the theory of threshold saturation for spatially coupled systems first developed in coding theory. Our approach is very generic and can be applied to many other open problems in statistical estimation where heuristic statistical physics predictions are available.

==> sections/concentration_jean.tex <==
\section{Concentration} \label{app:concentration}
%
In this appendix we prove a concentration equality that is necessary to show formula ?? linking the signal and matrix MMSE.

\section{Concentration of the overlap w.r.t the posterior}
%
In order to show the connection between the matrix-mmse and the vector-mmse, it turns out that we need some concentration properties on the overlap $q \defeq 1/n \sum_i x_i^{(1)}x_i^{(2)}$ between the two independent replicas $x_i^{(1)}$ and $x_i^{(2)}$. For this end, we consider a \emph{perturbed} system with the following Hamiltonian
\begin{align}\label{eq:perturbed_hamiltonian}
\mathcal{H}(\bx,h) &= \frac{1}{\Delta} \sum_{1 \le i\le j\le n}\bigg[ \frac{x_{i}^2x_{j}^2}{2n} -  \frac{s_{i}s_{j}x_{i}x_{j}}{n} - \frac{x_{i}x_{j}z_{i j} \sqrt{\Delta}}{\sqrt{n}} \bigg] + h \sum_i x_i^{(1)}x_i^{(2)},
\end{align}
where a perturbation term $h \sum_i x_i^{(1)}x_i^{(2)}$ is added to the original Hamiltonian (again, the dependence of the Hamiltonian on $\bs,\bz,\Delta$ and $n$ is implicit and dropped from the notation of $\mathcal{H}(\bx,h)$ for readability). Note that $\mathcal{H}(\bx,0)$ corresponds to the Hamiltonian of the original system. However, for some technical reasons that will become clear in the sequel, we work with the perturbed system (\ref{eq:perturbed_hamiltonian}) and then let $h \rightarrow 0$ at the end of the analysis.

Let $Z(h)$ be the partition function associated with $\mathcal{H}(\bx,h)$ and denote by $f_{h,n}$ the free energy of the perturbed system at fixed signal and noise realization with $f_{h,n} =  - \ln \big( Z(h) \big)/n$. Moreover, we denote by $\langle \cdot \rangle_{h}$ the expectation over the posterior distribution associated with $\mathcal{H}(\bx, h)$. Note the the perturbation term has been chosen so that the following lemma holds.
\begin{lemma}\label{lemma:pertubed_energy_concave}
$f_{h,n}$ is concave in $h$.
\end{lemma}
\begin{proof}
By using the dominated convergence theorem, one obtains the following
\begin{align}
\label{eq:perturbed_energy_derivative1}
\frac{d}{dh} f_{h,n} &=  \langle q \rangle_{h} \\
\label{eq:perturbed_energy_derivative2}
\frac{d^2}{dh^2} f_{h,n} &= - n \Big( \langle q^2 \rangle_{h} - \langle q \rangle_{h}^2 \Big) \le 0. 
\end{align}
\end{proof}
Furthermore, it turns out the the overlap $q$ satisfies some concentration properties.
\begin{lemma}\label{lemma:concentration_q}
Concentration of $q$: For any $a >\epsilon>0$ fixed
\begin{align*}
\int_{\epsilon}^{a} dh \mathbb{E} \Big[ \Big\langle \big(q - \langle q \rangle_{h} \big)^2 \Big\rangle_{h} \Big] = \mathcal{O}\Big(\frac{1}{n}\Big).
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
\int_{\epsilon}^{a} dh \mathbb{E} \Big[ \Big\langle \big(q - \langle q \rangle_{h} \big)^2 \Big\rangle_{h} \Big]
&= \int_{\epsilon}^{a} dh \mathbb{E} \big[ \langle q^2 \rangle_{h} - \langle q \rangle_{h}^2 \big]
= - \int_{\epsilon}^{a} dh \frac{1}{n} \frac{d^2}{dh^2} \mathbb{E} \big[f_{h,n} \big]\\
&= \frac{1}{n} \Big( \frac{d}{dh} \mathbb{E} \big[f_{\epsilon,n}\big] - \frac{d}{dh} \mathbb{E} \big[f_{a,n}\big] \Big) = \mathcal{O}\Big(\frac{1}{n}\Big),
\end{align*}
where the second equality follows from (\ref{eq:perturbed_energy_derivative2}) and the dominated convergence theorem. The last equality uses the fact that the derivative of $\mathbb{E} \big[f_{h,n}\big]$ is $\mathcal{O}(1)$ for $h\ge\epsilon$, which is valid, by Nishimori condition, for all signal's prior distribution with bounded second moment
\begin{align*}
\frac{d}{dh} \mathbb{E} \big[f_{h,n}\big] =  \frac{1}{n} \sum_i \mathbb{E} \big[ \langle x_i^{(1)}x_i^{(2)} \rangle_{h} \big] = \mathbb{E} \big[ \langle s_i x_i \rangle_{h} \big] \le \mathbb{E} \big[  s_i^2 \big] = v. 
\end{align*} 
\end{proof} 
%
\subsection{Concentration of the overlap w.r.t the disorder}
%
Call the perturbed signal $\tilde \bs = [\tilde s_1, s_2, \ldots,s_n]$, where the first signal component is modified w.r.t $\bs$. It is easy to show that the difference between the Hamiltonian evaluated at $\bs$ and $\tilde\bs$ is simply
%
\begin{align}
\delta \mathcal{H}(\bx,\tilde \bs, \bs) \defeq \mathcal{H}(\bx,\bs, \bz) - \mathcal{H}(\bx,\tilde \bs,\bz) = \frac{x_1(\tilde s_1 - s_1)}{\Delta n}\sum_{j=1}^n s_jx_j \label{eq:deltaH_concentration}
\end{align}
%
Call $\mathcal{Z}(\bs,\bz)=\int d\bx P_0(\bx)\exp(-\mathcal{H}(\bx,\bs,\bz))$ the partition associated with $\mathcal{H}(\bx,\bs)$, and $f(\bs,\bz) = -\ln(\mathcal{Z}(\bs,\bz) )/n$ the associated free energy at fixed signal and noize realizations. We now use similar steps as in Section~\ref{sec:subadditivitystyle} in order to evaluate the difference between the free energy associated with $\mathcal{H}(\bx,\bs, \bz)$ and $\mathcal{H}(\bx,\tilde \bs,\bz)$. Exactly as we obtained \eqref{eq:Z_openVSclosed}, \eqref{eq:Z_openVSclosed_2}, we get
%
\begin{align}
f(\bs,\bz) &= f(\tilde \bs,\bz) - \frac{1}{n}\ln(\langle e^{-\delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)}\rangle_{\mathcal{H}}),\\ 
f(\tilde \bs,\bz) &= f(\bs,\bz) - \frac{1}{n}\ln(\langle e^{\delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)}\rangle_{\tilde{\mathcal{H}}}),
\end{align}
%
where $\langle A(\mathbf{X}) \rangle_{\mathcal{H}} \defeq \mathcal{Z}(\bs,\bz)^{-1}\int d\bx A(\bx) P_0(\bx)\exp(-\mathcal{H}(\bx,\bs,\bz))$ is the expectation w.r.t the posterior associated with $\mathcal{H}(\bx,\bs,\bz)$, and similarly, $\langle A(\mathbf{X}) \rangle_{\tilde{\mathcal{H}}}$ is the the expectation w.r.t the posterior associated with $\mathcal{H}(\bx,\tilde \bs,\bz)$. Combining these two identites and using the convexity of the exponential, we get
%
\begin{align}
f(\tilde \bs,\bz) + \frac{\langle \delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)\rangle_{\mathcal{H}}}{n} \le f(\bs,\bz) \le f(\tilde \bs,\bz) + \frac{\langle \delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)\rangle_{\tilde{\mathcal{H}}}}{n}.
\end{align}
%
Let us now estimate $\langle \delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)\rangle_{\mathcal{H}}/n$. From \eqref{eq:deltaH_concentration} we get
%
\begin{align}
\frac{\langle \delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)\rangle_{\mathcal{H}}}{n} = \frac{(\tilde s_1-s_1)}{\Delta n^2} \sum_{j=1}^n s_j \langle X_1 X_j\rangle_{\mathcal{H}}
\end{align}
%


==> sections/interpolation_subadditivity_style.tex <==
\section{Invariance of the optimal threshold under spatial coupling}\label{sec:subadditivitystyle}
%
In this section, we prove that the Bayesian optimal threshold (defined in (\ref{Deltaopt}) in terms of the mutual information) remains intact under spatial coupling, i.e. $\Delta_{\rm opt}^{\rm c} = \Delta_{\rm opt}$. Note that for a Gaussian noise, the normalized mutual information of the underlying system is equal to the free energy $f^{\rm u}_n$, a fundamental quantity in statistical physics, up to a trivial term
\begin{align}\label{eq:mutual_Information_free_Energy}
\frac{1}{n} I(\tbf{S} \tbf{S}^T ; \tbf{W}) = f^{\rm u}_n + \frac{v^2}{4\Delta}.
\end{align}
Therefore, we will perform our analysis for this section in terms of the free energy.

In statistical physics language, for an underlying system with a given Hamiltonian $\mathcal{H^{\rm u}}$, the posterior probability distribution $p(\bx\vert \bs,\bz)$ and the corresponding partition function $Z$ are
%
\begin{align}\label{eq:posterior_partition}
&p(\bx\vert \bs,\bz) = \frac{P_0(\bx) e^{-\mathcal{H}_{\rm u}}}{Z},\nonumber \\
%
&Z = \int d\bx P_0(\bx) e^{-\mathcal{H}_{\rm u}}.
\end{align}
%
The free energy is then defined as
\begin{align}
f_{n}^{\rm u} = \frac{-\mathbb{E} [\ln (Z)]}{n},
\end{align}
where $\mathbb{E}[\cdot]$ is the average over all the disorders.
In order to prove that $\Delta_{\rm opt}^{\rm c} = \Delta_{\rm opt}$, we introduce four systems of the form (\ref{eq:def_coupledSyst}) having all the same size $n(L+1)$:
\begin{itemize}
\item $S_1$: the fully connected (homogeneous) system having the optimal threshold $\Delta_{\rm opt}^{\rm h}$ and the free energy $f_{ L,n}^{\rm h} = \frac{-\mathbb{E} [\ln (Z_1)]}{n(L+1)}$, where $Z_1$ is the partition function associated to $S_1$, with  coupling window $w_1 = L/2$.
\item $S_2$: the SC system, previously used to show threshold saturation with pinning conditions at the boundaries, having $\Delta_{\rm opt}^{\rm c}$ and $f_{ L,n}^{\rm c}$ with $1<w_2<L/2$. We will refer to this system as the actual SC system.
\item $S_3$: the unpinned SC system (similar to $S_2$ but without pinning conditions) having $\Delta_{\rm opt}^{\rm p}$ and $f_{L,n}^{\rm p}$ with $1<w_3<L/2$.
\item $S_4$: the decoupled system having $\Delta_{\rm opt}^{\rm dec}$ and $f_{L,n}^{\rm dec}$ with $w_4 = 0$.
\end{itemize}
By using the interpolation method twice, between $S_1$ and $S_3$ then between $S_4$ and $S_3$, and knowing that $S_1$ and $S_4$ have the same asymptotic free energy $f^{\rm u} = \lim_{n \rightarrow \infty}f_{n}^{\rm u}$ as the underlying system (and thus the same threshold $\Delta_{\rm opt}$), we prove that $\lim_{n \rightarrow \infty}f_{L,n}^{\rm p} = f^{\rm u}$. Furthermore, we show that pinning the closed chain in $S_2$ results in an energy loss that vanishes with $L$. Therefore, one can deduce that $f_{L,n}^{\rm c} = f_{L,n}^{\rm p}$ by taking $n \rightarrow \infty$ then $L \rightarrow \infty$. Hence, the results $\lim_{L,n \rightarrow \infty}f_{L,n}^{\rm c} = f^{\rm u}$ and $\Delta_{\rm opt}^{\rm c} = \Delta_{\rm opt}$ follow directly. Note that the reason why we used $S_3$ as an intermediate step to proof the result for $S_2$ is because the former is more convenient to perform the interpolation method.
        
In full generality, let us consider two SC systems of size $n(L+1)$ with coupling windows $w$ and $w_0$ respectively. Furthermore, we assume that the two systems are coupled using the matrices $\bold{\Lambda}$ and $\bold{\Lambda}^0$ respectively. We consider that the noise of the first and second SC systems are respectively $\Delta / t$ and $\Delta / (1 - t)$ and we define an interpolated system which Hamiltonian is just the sum of those of the two SC systems, $\mathcal{H}_{\rm int}(t,\bold{\Lambda},\bold{\Lambda}^0) = \mathcal{H}(t,\bold{\Lambda}) + \mathcal{H}(1-t,\bold{\Lambda}^0)$, with
\begin{align*}
\mathcal{H}(t,\bold{\Lambda}) &= \frac{t}{\Delta} \sum_{\mu} \Lambda_{\mu,\mu} \sum_{i_\mu\le j_\mu}\bigg[ \frac{x_{i_\mu}^2x_{j_\mu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\mu}x_{i_\mu}x_{j_\mu}}{n} - \frac{x_{i_\mu}x_{j_\mu}z_{i_\mu j_\mu} \sqrt{\Delta}}{\sqrt{n t\Lambda_{\mu,\mu}}}\bigg]\nonumber\\
%
&+ \frac{t}{\Delta} \sum_{\mu}\sum_{\nu\in \{\mu+1:\mu+w\}}\Lambda_{\mu,\nu}\sum_{i_\mu\le j_\nu}\bigg[ \frac{x_{i_\mu}^2x_{j_\nu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n} - \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu} \sqrt{\Delta}}{\sqrt{nt\Lambda_{\mu,\nu}}}\bigg]\nonumber\\
%
&+ \frac{t}{\Delta} \sum_{\mu}\sum_{\nu\in \{\mu-w:\mu-1\}}\Lambda_{\mu,\nu}\sum_{j_\nu < i_\mu}\bigg[ \frac{x_{i_\mu}^2x_{j_\nu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n} - \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu} \sqrt{\Delta}}{\sqrt{nt\Lambda_{\mu,\nu}}}\bigg].
\end{align*}
In this setting, at $t=1$ the interpolated system is the first SC one as the noise is infinitely large in the second SC one and no information is available about it, while at $t=0$ the opposite happens. 
In order to compare any two systems, one is normally interested in computing the derivative of $\mathbb{E}[\ln \big(Z(t)\big)]$ w.r.t. the interpolation parameter $t$. Following the lines of [\cite{krzakala2016mutual}], we obtain
\begin{align} \label{eq:derivative_interpolation}
\partial_t \mathbb{E}[\ln \big(Z(t)\big)] &= \frac{1}{4\Delta n} \Big( \sum_{\mu}\sum_{\nu\in \mathcal{S}_{\mu}^{w}} \Lambda_{\mu,\nu} \sum_{i_\mu, j_\nu}\mathbb{E}[x_{i_\mu}x_{j_\nu}s_{i_\mu}s_{j_\nu}] + \sum_{\mu} \Lambda_{\mu,\mu} \sum_{ i_\mu} \mathbb{E}[x_{i_\mu}^2 s_{i_\mu}^2] \Big) \nonumber \\
&- \frac{1}{4\Delta n} \Big( \sum_{\mu}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} \Lambda_{\mu,\nu}^0 \sum_{i_\mu, j_\nu}\mathbb{E}[x_{i_\mu}x_{j_\nu}s_{i_\mu}s_{j_\nu}] + \sum_{\mu} \Lambda_{\mu,\mu}^0 \sum_{ i_\mu} \mathbb{E}[x_{i_\mu}^2 s_{i_\mu}^2] \Big),
\end{align}  
%
where $\mathcal{S}_{\mu}^{w} = \{\mu-w:\mu+w\}$. We define the overlaps per block as $q_\mu \defeq \frac{1}{n} \sum_{i_\mu} x_{i_\mu}s_{i_\mu}$ and $\tilde{q}_\mu \defeq \frac{1}{n} \sum_{i_\mu} x_{i_\mu}^2 s_{i_\mu}^2$. Hence, (\ref{eq:derivative_interpolation}) can be rewritten as
\begin{align} \label{eq:derivative_interpolation_overlap}
\frac{4\Delta}{ n} \partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E} \Big[ \mathbf{q}^{\intercal} \mathbf{\Lambda} \, \mathbf{q} + \frac{1}{n} \, \tilde{\mathbf{q}}^{\intercal} diag ({\mathbf{\Lambda}})
- \mathbf{q}^{\intercal} \mathbf{\Lambda}^0 \, \mathbf{q} - \frac{1}{n} \, \tilde{\mathbf{q}}^{\intercal} diag ({\mathbf{\Lambda}}^0)
\Big],
\end{align} 
where $\mathbf{q}^{\intercal}  = [q_0:q_L]$, $\tilde{\mathbf{q}}^{\intercal}  = [\tilde{q}_0:\tilde{q}_L]$ and $diag ({\mathbf{\Lambda}})$ represents the column vector with entries $\Lambda_{\mu,\mu}$.  Moreover, the symmetry of the coupling matrix rewrites (\ref{eq:derivative_interpolation_overlap}) as 
\begin{align} \label{eq:derivative_interpolation_diagonalization}
\frac{4\Delta}{ n} \partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E} \Big[ (\mathbf{Uq})^{\intercal}\mathbf{D} \, (\mathbf{Uq}) + \frac{1}{n} \, \tilde{\mathbf{q}}^{\intercal} diag ({\mathbf{\Lambda}})
- ({\mathbf{U}^0\mathbf{q}})^{\intercal} \mathbf{D}^0 \, (\mathbf{U}^0\mathbf{q}) - \frac{1}{n} \, \tilde{\mathbf{q}}^{\intercal} diag ({\mathbf{\Lambda}}^0)
\Big],
\end{align}
where $\mathbf{U}$ and $\mathbf{U}^0$ are the orthogonal matrices obtained by eigenvalue decomposition of $\mathbf{\Lambda}$ and $\mathbf{\Lambda}^0$ respectively, while $\mathbf{D}$ and $\mathbf{D}^0$ are the  corresponding diagonal matrices. Furthermore, since the coupling matrices are doubly-stochastic, the leading eigenvalue in $\mathbf{D}$ and $\mathbf{D}^0$ is always equal to $1$ while the remaining eigenvalues are $\le 1$ in absolute value.

\subsection{The homogeneous VS the coupled systems}
%
We interpolate between $S_1$ (recovered at $t=1$) and $S_3$ (recovered at $t=0$). We represent $S_1$ by setting $w = w_1=L/2$  in (\ref{eq:derivative_interpolation_diagonalization}) and taking a homogeneous coupling matrix with elements $\Lambda_{\mu,\nu} = \frac{1}{L+1}$ for $\nu\in \mathcal{S}_{\mu}^{w}$. $S_3$ is represented by setting $1<w_0=w_3<L/2$ and taking a triangular shape coupling window wiht $\Lambda_{\mu,\nu}^0 = \frac{(w_0+1) - |\mu - \nu|}{(w_0+1)^2}$ for $\nu\in \mathcal{S}_{\mu}^{w_0}$. 

Due to the periodicity of the closed-chain, the coupling matrices are also circulant. Hence, the corresponding eigenvalue decomposition in (\ref{eq:derivative_interpolation_diagonalization}) is nothing but the Discrete Fourier Transform (DFT) given by
\begin{align} \label{eq:derivative_homogeneousVScoupled}
\frac{4\Delta}{ n} \partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E} \Big[ \hat{\mathbf{q}}^{\intercal} \mathbf{D} \, \hat{\mathbf{q}} + \frac{1}{n(L+1)} \sum_{\mu}\tilde{q}_{\mu}
- \hat{\mathbf{q}}^{\intercal} \mathbf{D}^0 \, \hat{\mathbf{q}} - \frac{1}{n(w_0+1)} \sum_{\mu}\tilde{q}_{\mu}
\Big],
\end{align}
where $\hat{\mathbf{q}}$ is the DFT of $\mathbf{q}$. Notice that the fully connected system $S_1$ yields a diagonal matrix $\mathbf{D}$ with a single non-zero eigenvalue (which is the unity one). For $\mathbf{D}^0$, beside the unity leading eigenvalue, all the remaining eigenvalues are non-negative. This is because of the triangular shape coupling window used in the construction of $S_3$. The triangular window corresponds to a discrete-time convolution between two rectangular windows, and thus a quadratic value in the DFT domain.
%Following the lines of [\cite{krzakala2016mutual}], we obtain
%%
%\begin{align}  \label{eq:derivative_homogeneousVScoupled}
%\partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \frac{1}{4\Delta} \Big[ \frac{1}{n(L+1)} \sum_{\mu,\nu, i_\mu, j_\nu} \mathbb{E}[x_{i_\mu}x_{j_\nu}s_{i_\mu}s_{j_\nu}] -  \frac{1}{ n(2w_0+1)} \sum_{\mu}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} \sum_{i_\mu, j_\nu}\mathbb{E}[x_{i_\mu}x_{j_\nu}s_{i_\mu}s_{j_\nu}] \Big]
%\end{align}
%%
%where  $\mathbb{E}[\cdot]$ is the average over all the disorders. We define the overlap per block as $q_\mu \defeq \frac{1}{n} \sum_{i_\mu} x_{i_\mu}s_{i_\mu}$. Note that due to the periodic boundary condition of the closed-chain SC system of length $L+1$, any quantity $U_\mu$ indexed by the spatial index satisfies $U_\mu = U_{\bar{\mu}}$, with $\bar{\mu} = \text{mod}(\mu -1, L+1) +1$. This induces the following identities
%%
%\begin{align} \label{eq:periodicBound}
%\sum_{\mu} U_\mu &= \sum_{\mu} \frac{1}{l+1}\sum_{\nu \in \bar{\mathcal{S}}_{\mu}} U_\nu, \nonumber \\
%\sum_{\mu} U_{\mu} \sum_{\nu \in \bar{\mathcal{S}}_{\mu}\backslash \mu} U_\nu &= \sum_{\mu} \frac{1}{l+1}\sum_{\underset{\eta \neq \nu }{\eta , \nu \in \bar{\mathcal{S}}_{\mu}}} U_{\eta}  U_\nu,
%\end{align}
%%
%where $\bar{\mathcal{S}}_{\mu}=\{k+\mu:k+\mu+l\}$ and $\forall k,l \in \mathbb{N}$. Furthermore, the periodicity at the boundaries yields the following property
%\begin{align}\label{eq:periodicBound_2}
%\sum_{\mu} U_\mu\sum_{\nu \in \bar{\mathcal{S}}_{\mu}} U_{\nu} = \sum_{\mu} \frac{1}{l+1}  \Big(\sum_{\nu\in \bar{\mathcal{S}}_{\mu}} U_\nu\Big)^2 .
%\end{align}
%\begin{proof}
%\textbf{(\ref{eq:periodicBound_2}):} By combining the two identities in (\ref{eq:periodicBound}), one obtains
%\begin{align*}
%\sum_{\mu} \frac{1}{l+1}\sum_{\underset{\eta \neq \nu }{\eta , \nu \in \bar{\mathcal{S}}_{\mu}}} U_{\eta}  U_\nu = \sum_{\mu} \frac{1}{l+1}\sum_{\eta \in \bar{\mathcal{S}}_{\mu}} U_{\eta} \sum_{\nu \in \bar{\mathcal{S}}_{\eta}\backslash \eta}U_\nu.
%\end{align*}
%Thus, the property (\ref{eq:periodicBound_2}) follows
%\begin{align*}
%&\sum_{\mu} U_\mu\sum_{\nu \in \bar{\mathcal{S}}_{\mu}} U_{\nu} = \sum_{\mu} U_{\mu}^2 + \sum_{\mu} U_{\mu} \sum_{\nu \in \bar{\mathcal{S}}_{\mu}\backslash \mu} U_\nu = \frac{1}{l+1} \Big( \sum_{\mu}  \sum_{\nu\in \bar{\mathcal{S}}_{\mu}} U_\nu^{2} + \sum_{\mu} \sum_{\eta \in \bar{\mathcal{S}}_{\mu}} U_{\eta} \sum_{\nu \in \bar{\mathcal{S}}_{\eta} \backslash \eta} U_\nu \Big) \nonumber \\
%%
%=&\frac{1}{l+1} \Big( \sum_{\mu}  \sum_{\nu\in \bar{\mathcal{S}}_{\mu}} U_\nu^{2} + \sum_{\mu}  \sum_{\underset{\eta \neq \nu }{\eta , \nu \in \bar{\mathcal{S}}_{\mu}}} U_{\eta}  U_\nu \Big) = \frac{1}{l+1}  \sum_{\mu} \Big(\sum_{\nu\in \bar{\mathcal{S}}_{\mu}} U_\nu\Big)^2 . 
%\end{align*}
%\end{proof}
%Hence, (\ref{eq:derivative_homogeneousVScoupled}) can be rewritten as
%%
%\begin{align}  \label{eq:derivativeNeg_homogeneousVScoupled}
%&\frac{4\Delta}{n}\partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E}\Big[\frac{1}{L+1} \sum_{\mu,\nu} q_\mu q_\nu -  \frac{1}{2w_0+1} \sum_{\mu}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} q_\mu q_\nu \Big] \nonumber\\
%%
%&= (L+1) \mathbb{E}\Big[\Big(\frac{1}{L+1} \sum_{\mu} q_\mu\Big)^2 - \frac{1}{L+1}\sum_{\mu} q_\mu\frac{1}{2w_0+1}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} q_\nu \Big]\nonumber \\
%%
%&= (L+1) \mathbb{E}\Big[\Big(\frac{1}{L+1} \sum_{\mu} \frac{1}{2w_0+1}\sum_{\nu\in S{\mu}} q_\nu\Big)^2 - \frac{1}{L+1}\sum_{\mu} \Big(\frac{1}{2w_0+1}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} q_\nu \Big)^2 \Big]\le 0,
%\end{align}
%%
%where the inequality is obtained using the convexity of the quadratic function and the last equality using the property (\ref{eq:periodicBound_2}). 
Therefore, we can assert that $\frac{\partial_t \mathbb{E}[\ln \big(Z(t)\big)]}{ n} \le 0$.  Hence, $f_{L,n}^{\rm {p}}\le f_{L,n}^{\rm h}$ as  the interpolated free energy $\frac{-\mathbb{E}[\ln (Z(t))]}{n(L+1)}$ is non-decreasing in $t$.
%
\subsection{The decoupled VS the coupled systems}
%
We now interpolate between $S_4$ (recovered at $t=1$) and $S_3$ (recovered at $t=0$) by setting $w = w_4=0$ and using the same parameters for $S_3$ as before. Using similar arguments as for the previous case, one obtains
\begin{align} \label{eq:derivativeNeg_decoupledVScoupled}
\frac{4\Delta}{ n} \partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E} \Big[ \hat{\mathbf{q}}^{\intercal} \mathbf{D} \, \hat{\mathbf{q}} + \frac{1}{n} \sum_{\mu}\tilde{q}_{\mu}
- \hat{\mathbf{q}}^{\intercal} \mathbf{D}^0 \, \hat{\mathbf{q}} - \frac{1}{n(w_0+1)} \sum_{\mu}\tilde{q}_{\mu}
\Big] \ge 0,
\end{align}
%
%\begin{align}
%\frac{4\Delta}{n}\partial_t \mathbb{E}[\ln \big(Z(t)\big)] &= \mathbb{E}\Big[\sum_{\mu} q_\mu^2 -  \frac{1}{2w_0+1} \sum_{\mu}\sum_{\nu\in\{\mu:\mu+w_0\}} q_\mu q_\nu \Big] \nonumber\\
%%
%&= \mathbb{E}\Big[\sum_{\mu} \frac{1}{2w_0+1}\sum_{\nu\in\{\mu:\mu+w_0\}} q_\nu^2 - \sum_{\mu} \Big(\frac{1}{2w_0+1}\sum_{\nu\in\{\mu:\mu+w_0\}} q_\nu \Big)^2 \Big] \ge 0, \label{eq:derivativeNeg_decoupledVScoupled}
%\end{align}
%
where the inequality is obtained by noticing that $\mathbf{D}$ is the identity matrix in this case. This proves that $f_{L,n}^{\rm{dec}}\le f_{L,n}^{\rm{p}}$. Combining the previous two results, we have that 
%
\begin{lemma}\label{lemma:freeEnergy_sandwich}
$ f_{L,n}^{\rm{dec}} \le f_{L,n}^{\rm{p}}\le f_{L,n}^{\rm h}$.
\end{lemma}
%
\subsection{Existence of the free energy's infinite limit}
%
Consider now the underlying system of the form (\ref{eq:mainProblem}) with size $N$ and free energy $f_N^{\rm u}$. By dividing this system into two similar but independent subsystems of sizes $N_1$ and $N_2$, with $N_1 + N_2 = N$, it turns out that the free energy $f_N^{\rm u}$ is superadditive w.r.t. $N$.
%
\begin{lemma}\label{lemma:superadditivity}
$N f_N^{\rm u} \geq N_1 f_{N_1}^{\rm u} + N_2 f_{N_2}^{\rm u}$.
\end{lemma}
%
\begin{proof}
Using the interpolation method again, as done in [\cite{guerra_toninelli_2008}], between the underlying system and the two subsystems, one gets the following partition function
\begin{align*}
Z(t) =& \int d\bx P_0(\bx) \exp\Bigg(-\frac{t}{\Delta} \sum_{1 \le i\le j\le N}\bigg[ \frac{x_{i}^2x_{j}^2}{2N} -  \frac{s_{i}s_{j}x_{i}x_{j}}{N} - \frac{x_{i}x_{j}z_{i j} \sqrt{\Delta/t}}{\sqrt{N}}\bigg]\\
%
&-\frac{(1-t)}{\Delta}  \sum_{1 \le i\le j\le N_1}\bigg[ \frac{x_{i}^2x_{j}^2}{2N_1} -  \frac{s_{i}s_{j}x_{i}x_{j}}{N_1} - \frac{x_{i}x_{j}z_{i j} \sqrt{\Delta/t}}{\sqrt{N_1}}\bigg] \\
&-\frac{(1-t)}{\Delta}  \sum_{N_1 \le i\le j\le N_2}\bigg[ \frac{x_{i}^2x_{j}^2}{2N_2} -  \frac{s_{i}s_{j}x_{i}x_{j}}{N_2} - \frac{x_{i}x_{j}z_{i j} \sqrt{\Delta/t}}{\sqrt{N_2}}\bigg]\Bigg).
\end{align*}
The derivative of $\mathbb{E}[\ln \big(Z(t)\big)]$ w.r.t. the interpolation parameter $t$ gives
\begin{align*}
\frac{4\Delta}{N}\partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E}\Big[  q^2 -  \frac{N_1}{N} q_1^2 - \frac{N_2}{N} q_2^2 \Big] \le 0
\end{align*}
where $q = \frac{1}{N} \sum_{i=1}^{N}x_i s_i$, $q_1= \frac{1}{N_1} \sum_{i=1}^{N_1}x_i s_i$ and $q_2 = \frac{1}{N_2} \sum_{i=N_1+1}^{N}x_i s_i$. The inequality is due to the convexity of the quadratic. Hence, Lemma \ref{lemma:superadditivity} follows.
\end{proof}
%
Lemma \ref{lemma:superadditivity} implies, by Fekete's Lemma of superadditive sequences, that the asymptotic free energy of the underlying system exists $\lim_{N\rightarrow \infty}\frac{1}{N}f_N^{\rm u} = f^{\rm u}$. Note that the  homogeneous system $S_1$ is nothing but the underlying system at $N= n(L+1)$. Moreover, the decoupled system $S_4$ consists of $L+1$ non-interacting copies of the underlying system.  Therefore, in the limit $n\rightarrow \infty$, the three quantities of Lemma \ref{lemma:freeEnergy_sandwich} exist and the following lemma holds
\begin{lemma}\label{lemma:freeEnergy_sandwich_limit}
$ \lim_{n\rightarrow \infty} f_{L,n}^{\rm{dec}} = \lim_{n\rightarrow \infty} f_{L,n}^{\rm{p}} = \lim_{n\rightarrow \infty} f_{L,n}^{\rm h} = f^{\rm u}$.
\end{lemma}
%
\subsection{The unpinned VS the actual SC systems}
The only difference between the free energy of the unpinned SC system $f_{L,n}^{\rm{p}}$ and that of the actual SC system $f_{L,n}^{\rm{c}}$ comes from the boundary condition (the blocks in $\mathcal{B}= \{0:w\} \cup \{L-w+1:L\}$). In the sequel, we prove that the contribution of the pinned boundary conditions of the actual SC systems to the free energy is $\mathcal{O}(\frac{w}{L})$ for a wide range of parameters. Therefore, by taking the asymptotic limit in the proper order, we have that
\begin{lemma}\label{lemma:openVSclosed}
$\lim_{L,n \rightarrow \infty}f_{L,n}^{\rm{c}} = \lim_{L,n \rightarrow \infty}f_{L,n}^{\rm{p}} = f^{\rm{u}}$ and $\Delta_{\rm opt}^{\rm c} = \Delta_{\rm opt}$.
\end{lemma}
\begin{proof}
The Hamiltonians of the unpinned and the actual SC systems, $\mathcal{H}^{\rm p}$ and $\mathcal{H}^{\rm c}$ respectively, satisfy the identity $\mathcal{H}^{\rm c} = \mathcal{H}^{\rm p} - \delta \mathcal{H}$ with
\begin{align}\label{eq:H_openVSclosed}
\delta \mathcal{H} &=  \sum_{\mu \in \mathcal{B}} \Lambda_{\mu,\mu} \sum_{i_\mu\le j_\mu}\bigg[ \frac{x_{i_\mu}^2x_{j_\mu}^2 + s_{i_\mu}^2s_{j_\mu}^2}{2n\Delta} -  \frac{s_{i_\mu}s_{j_\mu}x_{i_\mu}x_{j_\mu}}{n\Delta} - \frac{(x_{i_\mu}x_{j_\mu}-s_{i_\mu}s_{j_\mu})z_{i_\mu j_\mu}}{\sqrt{n \Delta \Lambda_{\mu,\mu}}}\bigg]\nonumber\\
%
&+ \sum_{\mu \in \mathcal{B}}\sum_{\nu\in \{\mu+1:\mu+w\}\cap \mathcal{B}}\Lambda_{\mu,\nu}\sum_{i_\mu\le j_\nu}\bigg[ \frac{x_{i_\mu}^2x_{j_\nu}^2 + s_{i_\mu}^2s_{j_\nu}^2}{2n\Delta} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n \Delta} - \frac{(x_{i_\mu}x_{j_\nu}-s_{i_\mu}s_{j_\nu})z_{i_\mu j_\nu} }{\sqrt{n \Delta \Lambda_{\mu,\nu}}}\bigg]\nonumber\\
%
&+ \sum_{\mu \in \mathcal{B}}\sum_{\nu\in \{\mu-w:\mu-1\}\cap \mathcal{B}}\Lambda_{\mu,\nu}\sum_{j_\nu < i_\mu}\bigg[ \frac{x_{i_\mu}^2x_{j_\nu}^2 + s_{i_\mu}^2s_{j_\nu}^2}{2n\Delta} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n\Delta} - \frac{(x_{i_\mu}x_{j_\nu}-s_{i_\mu}s_{j_\mu})z_{i_\mu j_\nu} }{\sqrt{n\Delta\Lambda_{\mu,\nu}}}\bigg]
%
\end{align}
% old $\delta \mathcal{H}$
%\begin{align}
%\delta \mathcal{H} &=  \sum_{\mu \in \mathcal{B}} \sum_{i_\mu\le j_\mu} \frac{x_{i_\mu}x_{j_\mu}z_{i_\mu j_\mu} \sqrt{\Lambda_{\mu,\mu}} }{\sqrt{\Delta n}}
%%
%+ \sum_{\mu \in \mathcal{B}}\sum_{\nu\in \{\mu+1:\mu+w\} \cap \mathcal{B}}\sum_{i_\mu\le j_\nu} \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu}\sqrt{\Lambda_{\mu,\nu}}}{\sqrt{\Delta n}}\nonumber\\
%%
%&+ \sum_{\mu \in \mathcal{B}}\sum_{\nu\in \{\mu-w:\mu-1\} \cap \mathcal{B}}\sum_{j_\nu < i_\mu} \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu}\sqrt{\Lambda_{\mu,\nu}}}{\sqrt{ \Delta n}}.
%\end{align}
Let $Z^{\rm p}$ and $Z^{\rm c}$ be the partition functions associated with $\mathcal{H}^{\rm p}$ and $\mathcal{H}^{\rm c}$ (where $Z^{\rm p}=\int d\bx P_0(\bx) e^{- \mathcal{H^{\rm p}}}$ and $Z^{\rm c}= \int d\bx P_0(\bx)e^{- \mathcal{H^{\rm c}}}$). Hence, one obtains the following identities
\begin{align}\label{eq:Z_openVSclosed}
\begin{cases}
\ln(Z^{\rm p}) &= \ln\Big( Z^{\rm c} \int d\bx \frac{P_0(\bx)e^{- \mathcal{H}^{\rm c}}}{Z^{\rm c}} e^{-\delta \mathcal{H}} \Big) \\
\ln(Z^{\rm c}) &= \ln\Big( Z^{\rm p}  \int d\bx \frac{P_0(\bx)e^{- \mathcal{H}^{\rm p}}}{Z^{\rm p}} e^{\delta \mathcal{H}} \Big),
\end{cases}
\end{align}
where the integrals can be seen as expectations over two posterior distributions, of the form (\ref{eq:posterior_partition}), associated to $\mathcal{H}^{\rm c}$ and $\mathcal{H}^{\rm p}$ respectively. Denote by $\langle \cdot \rangle_{\rm c}$ and $\langle \cdot \rangle_{\rm p}$ these expectations. In terms of free energy, (\ref{eq:Z_openVSclosed}) translates to
\begin{equation}\label{eq:energy_openVSclosed}
\begin{cases}
 f_{L,n}^{\rm{p}} = f_{L,n}^{\rm{c}} - \frac{\mathbb{E}\big[\ln \big( \langle e^{ -\delta \mathcal{H}} \rangle_{\rm c} \big)\big]}{n(L+1)}\\
  f_{L,n}^{\rm{c}} = f_{L,n}^{\rm{p}} - \frac{\mathbb{E}\big[\ln \big( \langle e^{ \delta \mathcal{H}} \rangle_{\rm p} \big)\big]}{n(L+1)}.
 \end{cases}
\end{equation}
Using the convexity of exponential, we get
%where the left-hand side inequality is obtained by noticing that the extra energy term is non-negative for a Hamiltonian with complete square, while the right-hand side inequality is due to the convexity of exponential. Furthermore, for bounded second and forth moments of the signal's prior distribution, $\frac{\mathbb{E} [ \langle \delta \mathcal{H} \rangle_{\rm c} ]}{n(L+1)}=\mathcal{O}(\frac{w}{L})$.
\begin{equation}\label{eq:openVSclosed_sandwich}
f_{L,n}^{\rm{c}} + \frac{\mathbb{E}\big[ \langle \delta \mathcal{H} \rangle_{\rm p} \big]}{n(L+1)} \le f_{L,n}^{\rm{p}} \le f_{L,n}^{\rm{c}} + \frac{\mathbb{E}\big[ \langle \delta \mathcal{H} \rangle_{\rm c} \big]}{n(L+1)}.
\end{equation}
Recall that due to the pinning condition used in the construction of the SC system in section \ref{sec:thresh-sat} (Remark \ref{remark:pinning}), we assume perfect knowledge of the variables at the boundaries where $x_{i_\mu} = s_{i_\mu}\, \forall \mu \in \mathcal{B}$. Thus, the expectation $\langle \cdot \rangle_{\rm c}$ associated with the actual SC system yields
\begin{align}
\frac{\mathbb{E}[ \langle \delta \mathcal{H} \rangle_{\rm c} ]}{n(L+1)} = 0 . 
\end{align}
Moreover, following the lines of [\cite{krzakala2016mutual}] by using a Gaussian integration by part and Nishimori conditions, we obtain
\begin{align}\label{eq:openVSclosed_order}
\frac{\Big|\mathbb{E}[ \langle \delta \mathcal{H} \rangle_{\rm p} ]\Big|}{n(L+1)} &\le \frac{n(n+1)(2w+1)^2}{n^2(L+1)(w+1)} \Big|\mathbb{E} [\langle x_{i_\mu}^2x_{j_\nu}^2 \rangle_{\rm p}]\Big|  + \frac{n(n-1)(2w+1)}{2n^2(L+1)(w+1)} \Big|\mathbb{E} [\langle x_{i_\mu}^2x_{j_\mu}^2 \rangle_{\rm p}]\Big| \nonumber \\
%
&+ \frac{(2w+1)}{n(L+1)(w+1)}\Big|\mathbb{E} [\langle x_{i_\mu}^4\rangle_{\rm p}]\Big| \nonumber\\
%
&= \mathcal{O}\Big(\frac{w}{L}\Big) \Big|\mathbb{E} [\langle x_{i_\mu}^2x_{j_\nu}^2 \rangle_{\rm p}]\Big|  + \mathcal{O}\Big(\frac{1}{L}\Big)  \Big|\mathbb{E} [\langle x_{i_\mu}^2x_{j_\mu}^2 \rangle_{\rm p}]\Big| + \mathcal{O}\Big(\frac{1}{nL}\Big) \Big|\mathbb{E} [\langle x_{i_\mu}^4\rangle_{\rm p}]\Big|,
\end{align}
for $ \Lambda_{\mu,\nu} \le \frac{1}{w+1}$. Furthermore, for bounded second and fourth moments of the signal's prior distribution, all the expectations in (\ref{eq:openVSclosed_order}) are bounded too (by Nishimori conditions). Therefore, Lemma \ref{lemma:openVSclosed} holds by taking $n\rightarrow \infty$ then $L\rightarrow \infty$ in (\ref{eq:openVSclosed_sandwich}).

\end{proof}
 
%

==> sections/low_noise_regime.tex <==
\section{Proof of Theorem \ref{thm1} for $\Delta <\Delta_{\rm opt}$}\label{sec:delta-less-delta-opt}
%
We first show the following Lemma.

\begin{lemma}\label{small-noise-lemma}
Let $\Delta < \Delta_{\rm amp}$. Then the limit of the mutual information per variable exists and is given by the replica symmetric formula \eqref{eq:RSformula}.
\end{lemma}

\begin{proof}
Let us apply \eqref{eq:subopt} to the AMP estimator $\hat{\tbf{s}}^t$. By definition of the MMSE estimator as being optimal in the MSE sense,
% 
\begin{align}\label{startingpoint}
{\rm MSE}_{n, \rm amp}^t(\Delta^{-1}) \geq {\rm MMSE}_n(\Delta^{-1}).
\end{align}
%
Taking limits in the order $\lim_{t\to +\infty}\limsup_{n\to +\infty}$ and using \eqref{eq:mseampmatriciel} we find
\begin{align}
v^2 - (v-E_{\infty})^2 \geq \limsup_{n\to +\infty}{\rm MMSE}_n(\Delta^{-1}),
\end{align}
and in view of \eqref{eq:GSV} we obtain 
\begin{align}\label{thisineq}
\frac{1}{4}(v^2 - (v-E_{\infty})^2) \geq  \limsup_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\Delta^{-1}}.
\end{align}
Now, for $\Delta < \Delta_{\rm amp}$ we have $E_{\infty} = E_{\rm good}(\Delta)$ which is the unique and hence {\it global} minimum of $i_{\rm RS}(E; \Delta)$. Hence, by exactly the same calculation done in equations
\eqref{first} -\eqref{third}, we conclude that the left hand of \eqref{thisineq} is a {\it total derivative}, namely
$$
\frac{d}{d\Delta^{-1}}\{\min_{E}i_{\rm RS}(E; \Delta)\}.
$$
In other words
\begin{align}
\frac{d}{d\Delta^{-1}}\{\min_{E}i_{\rm RS}(E; \Delta)\} \geq 
\limsup_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\Delta^{-1}},
\end{align}
which is also equivalent to 
\begin{align}\label{middlepoint}
\frac{d}{d\Delta}\{\min_{E}i_{\rm RS}(E; \Delta)\} \leq 
\liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\Delta}.
\end{align}
We now integrate this inequality over an interval 
$[0, \Delta] \subset [0, \Delta_{\rm amp}]$
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) - \min_{E}i_{\rm RS}(E; 0) 
& \leq 
\int_0^\Delta d\tilde{\Delta}\,\liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\tilde{\Delta}}
\nonumber \\ &
\leq 
\liminf_{n\to +\infty}\int_0^\Delta d\tilde{\Delta}\,\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\tilde{\Delta}}
\nonumber \\ &
= \liminf_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W}) - H(S).
\end{align}
The second inequality uses Fatou's Lemma and the last equality uses that for zero noise 
$I(\tbf{S}\tbf{S}^T\vert \tbf{W}) = H(\tbf{S}\tbf{S}^T) - H(\tbf{S}\tbf{S}^T\vert \tbf{W}) = H(\tbf{S}\tbf{S}^T) = H(\tbf{S}) = nH(S)$. 
In appendix \ref{appendix_smallnoise} an explicit calculation shows that $\min_{E}i_{\rm RS}(E; 0) = H(S)$.  Therefore
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) \leq \liminf_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W}).
\end{align}
The final step combines this inequality with the interpolation bound \eqref{eq:guerrabound}
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) & \leq 
\liminf_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})
\leq 
\limsup_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})
\leq 
\min_{E}i_{\rm RS}(E; \Delta)
\end{align}
This shows that the limit of the mutual information exists and is equal to the replica symmetric formula for $\Delta <\Delta_{\rm amp}$.
\end{proof}

This proof already shows the existence of the thermodynamic limit for 
$\Delta < \Delta_{\rm amp}$. In hindsight this is perhaps not so surprising. Indeed it crucially uses the interpolation bound \eqref{eq:guerrabound} which itself is based on an interpolation which does not per se show the existence of this limit, but which is quite similar to another interpolation used for showing the existence of the limit for {\it all} $\Delta$ (this other type of interpolation is used in section \ref{sec:subadditivitystyle}). 

One can try to apply the same proof idea to the regime $\Delta > \Delta_{\rm pot}$. 
Equations \eqref{startingpoint} - \eqref{middlepoint} work out exactly in the same way
because the AMP fixed point $E_{\infty} = E_{\rm bad}(\Delta)$ which is the {\it global} minimum of $i_{\rm RS}(E; \Delta)$.
Then when one integrates on $[\Delta, +\infty[$ one finds 
$$
\limsup_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W}) \leq \min_{E}i_{\rm RS}(E; \Delta).
$$
This essentially gives an alternative proof of \eqref{eq:guerrabound} for $\Delta > \Delta_{\rm pot}$. However the result is {\it weaker} because \eqref{eq:guerrabound} is valid at finite size.

For the rest of this section we need the following Lemma. The proof is deferred to section 
\ref{sec:subadditivitystyle} because it uses similar interpolation arguments together with 
standard limiting arguments for sequences of concave/convex functions. 

\begin{lemma}\label{existence-thermo-limit}
The limit $\lim_{n\to +\infty}\frac{1}{n} I(\tbf{S}\tbf{S}^T\vert \tbf{W})$ exists 
and is a continuous function of $\Delta$. 
\end{lemma}

A crucial step in our analysis is the following Lemma.

\begin{lemma}\label{analyticity-argument-lemma}
We necessarily have $\Delta_{\rm pot} \geq \Delta_{\rm opt}$. 
\end{lemma}

\begin{proof}
If $\Delta_{\rm pot} =+\infty$ then we are done; so we suppose it is finite. The proof 
proceeds by contradiction: suppose $\Delta_{\rm pot} < \Delta_{\rm opt}$. Notice first that it not possible to have $\Delta_{\rm pot} < \Delta_{\rm amp}$ because in the range $]0, \Delta_{\rm amp}[$, as a function of $E$, the function $i_{\rm RS}(E;\Delta)$ has a unique critical point. So we assume $\Delta_{\rm pot}\in [\Delta_{\rm amp}, \Delta_{\rm opt}[$. 
For $\Delta \in ]0, \Delta_{\rm pot}[$ we have $\min_{E\in [0, v]}i_{\rm RS}(E; \Delta)
= i_{\rm RS}(E_{\rm good}(\Delta); \Delta)$ which by hypothesis is an analytic function  in this interval. By definition of $\Delta_{\rm opt}$, the function 
$\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})$ is analytic in $]0, \Delta_{\rm opt}[$. Therefore {\it both functions are analytic on} $]0, \Delta_{\rm pot}[$ and since by Lemma~\ref{small-noise-lemma} they are equal for $]0, \Delta_{\rm amp}[\subset ]0, \Delta_{\rm pot}[$, {\it they must 
be equal on the whole range} $]0, \Delta_{\rm pot}[$. This implies that the two functions are equal at $\Delta_{\rm pot}$ because they are continuous. Explicitly,
\begin{align}\label{eq:equalityatpoint}
\min_{E}i_{\rm RS}(E; \Delta_{\rm pot}) = \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta_{\rm pot}}.
\end{align}

Now, fix some $\Delta \in ]\Delta_{\rm pot}, \Delta_{\rm opt}[$. Since this $\Delta$ is greater than $\Delta_{\rm pot}$ the fixed point of state evolution is $E_{\infty} = E_{\rm bad}(\Delta)$ and this is also the global minimum of $i_{\rm RS}(E;\Delta)$. Hence 
exactly as in \eqref{startingpoint} - \eqref{middlepoint} we can show that for 
$\Delta \in ]\Delta_{\rm pot}, \Delta_{\rm opt}[$,
\begin{align}\label{contra}
\frac{d}{d\Delta}\{\min_{E}i_{\rm RS}(E; \Delta)\} \leq 
\liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\Delta}.
\end{align}
This time \eqref{eq:guerrabound}, \eqref{contra} and the assumption $\Delta_{\rm pot}\in [\Delta_{\rm amp}, \Delta_{\rm opt}[$, taken together, lead to a 
contradiction, and hence we must have $\Delta_{\rm pot} \geq \Delta_{\rm opt}$. 

To see explicitly how the contradiction appears, integrate \eqref{contra} 
on $]\Delta_{\rm pot}, \Delta[\subset\Delta \in ]\Delta_{\rm pot}, \Delta_{\rm opt}[$, and use Fatou's Lemma, to obtain
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) - \min_{E}i_{\rm RS}(E; \Delta_{\rm pot})
& 
\leq \liminf_{n\to +\infty}\biggl\{\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta} - \frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta_{\rm pot}}\biggr\}
\nonumber \\ &
= 
\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta} - 
\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta_{\rm pot}}
\end{align}
From \eqref{eq:equalityatpoint} and \eqref{eq:guerrabound} we obtain 
$
\min_{E}i_{\rm RS}(E; \Delta) = \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})
$
{\it when} $\Delta_{\rm amp} \leq \Delta_{\rm pot} < \Delta < \Delta_{\rm opt}$. But by 
the previous results this equality is also 
true for $0 < \Delta \leq \Delta_{\rm pot}$. So the equality is valid 
in the whole interval $]0, \Delta_{\rm opt}[$ and therefore $\min_{E}i_{\rm RS}(E; \Delta)$ is analytic at $\Delta_{\rm pot}$. But this is impossible by the definition of 
$\Delta_{\rm pot}$. 
\end{proof} 

\begin{corollary}
Let $\Delta < \Delta_{\rm opt}$. Then the thermodynamic limit of the mutual information per variable is given by the replica symmetric formula \eqref{eq:RSformula}.
\begin{align}
\lim_{n\to +\infty} \frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W}) = \min_{E}i_{\rm RS}(E; \Delta)
\end{align}
\end{corollary}

\begin{proof}
Lemma~\ref{small-noise-lemma} says that the two functions are equal  for $\Delta <\Delta_{\rm amp}$ and Lemma~\ref{analyticity-argument-lemma} implies that {\it both} functions are analytic for $\Delta <\Delta_{\rm opt}$. Thus they must be equal on the whole range $\Delta < \Delta_{\rm opt}$.
\end{proof}

==> sections/threshold_saturation.tex <==
\section{Threshold saturation}\label{sec:thresh-sat}
%
Let us now prove that for a proper spatially coupled system, threshold saturation occurs, that is $\Delta_{\rm pot} \le \Delta_{\rm amp, c}$, where $\Delta_{\rm amp, c}$ is the algorithmic AMP threshold of the coupled system that we will define in the next. First, define the following average
%
\begin{align}
\langle A \rangle_E \defeq \frac{\int dx A(x) P_0(x)e^{-\frac{x^2}{2\Sigma(E,\Delta)^{2}} + x\big(\frac{s}{\Sigma(E,\Delta)^{2}} + \frac{z}{\Sigma(E,\Delta)} \big)} }{\int dx P_0(x)
e^{-\frac{x^2}{2\Sigma(E,\Delta)^{2}} + x\big(\frac{s}{\Sigma(E,\Delta)^{2}} + \frac{z}{\Sigma(E,\Delta)} \big)}}. \label{eq:defBracket_posteriorMean}
\end{align}
%
where $s,z$ and $\Delta$ are fixed and the dependence in these is implicit for sake of brevity. The AMP algorithm asymptotic perfomance can be tracked thanks to the SE analysis. Let us define the following operator.
%
\begin{definition}[SE operator] 
The state evolution operator associated with the underlying system is
%
\begin{align}
T_{\rm u}(E) \defeq \mathbb{E}_{S,Z}[(S - \langle x\rangle_E)^2], \label{def:SEop_underlying}
\end{align}
%
where $S \sim P_0(s)$, $Z\sim \mathcal{N}(z|0,1)$.
%
\end{definition}
%
Note that this operator is nothing else than the MMSE of a scalar AWGN channel with effective noise variance equal to $\Sigma(E,\Delta)^2$. Call $\hat{\tbf{s}}^{(t)}$ the estimate at iteration $t$ of the signal by the AMP algorithm. The AMP averaged scalar MSE is $E^{(t)}\defeq \mathbb{E}_{S,Z}[n^{-1}\sum_{i=1}^n(s_i - \hat s_i^{(t)})^2]$ is tracked iterating the SE recursion
%
\begin{align} \label{eq:SEiteration}
E^{(t+1)}=T_{\rm u}(E^{(t)}), \quad t\geq 0, \quad E^{(0)} = v, 
\end{align}
%
i.e. initializing the iteration without any knowledge about the signal other than its prior distribution.
%
\begin{remark}
Note that using this operator, $i)$ the good solution is given by $E_{\rm good}(\Delta) = T_{\rm u}^{(\infty)}(0)$ and $ii)$ the AMP threshold of Definition~\ref{amp-thresh} is given by $\Delta_{{\rm amp}} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm u}}^{(\infty)}(v) = E_{\rm good}(\Delta)\}$. 
\end{remark}
%
% In the next we will need the following definition.
%
% \begin{definition}[scalar MSE Floor] The scalar MSE floor $E_{\rm good}(\Delta)$ is defined as the fixed point reached from the initial condition $E^{(0)} = 0$. In other words $E_{\rm good}(\Delta) = T_{\rm u}^{(\infty)}(0)$. 
% \end{definition}
%
\begin{definition}[Bassin of attraction]
The basin of attraction of the good solution $E_{\rm good}(\Delta)$ is 
$\mathcal{V}_{\rm good} \defeq \{ E \ \! |\ \! T_{\rm u}^{(\infty )}(E) = E_{\rm good}(\Delta) \}$.
\end{definition}
%
% \begin{definition} [AMP threshold of the underlying ensemble]
% The AMP threshold of the underlying system is $\Delta_{{\rm u}} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm u}}^{(\infty)}(v) = E_{\rm good}(\Delta)\}$. 
% \end{definition}
%
For this section, it is more convenient to work with the free energy $f_{\rm u}(E)$, simply related to the replica potential \eqref{eq:potentialfunction} by $f_{\rm u}(E;\Delta) = i_{\rm RS}(E;\Delta) - \frac{v^2}{4\Delta}$. In Appendix~\ref{app:nishi}, we show the following Lemma linking the SE and potential analysies.
%
% \begin{align}
% 0=\frac{\partial f_{\rm{u}}(E)}{\partial E}\Big|_{\mathring E} \Leftrightarrow \mathring E = \mathbb{E}[(s - \langle x\rangle_{\mathring E})^2] = T_{\rm{u}}(\mathring E).
% \end{align}
% %
% We recognize the SE operator (\ref{def:SEop_underlying}), so that we can assert the follwing Lemma that links the SE and potential formulations.
%
\begin{lemma}\label{lemma:fixedpointSE_extPot_underlying}
% If $\mathring{E}$ is a fixed point of \eqref{eq:SEiteration}, i.e., $T_{{\rm u}}(\mathring E) = \mathring E$, then $\frac{\partial F_{{\rm u}}(E)}{\partial E}\big|_{\mathring E} =0$ and vice-versa.
$\mathring E = T_{{\rm u}}(\mathring E) \Leftrightarrow \frac{\partial f_{{\rm u}}(E)}{\partial E}\big|_{\mathring E} =0$.
\end{lemma} 
%
\begin{definition}[Free energy gap] \label{def:fgap}
Define $\delta f_{{\rm u}}(\Delta) \defeq {\rm inf} _{E \notin \mathcal{V}_{\rm good} } (f_{{\rm u}}( E) - f_{{\rm u}}(E_{\rm good}(\Delta)))$ as the free energy gap, with the convention that the infimum over the empty set is $\infty$ (this happens for $\Delta < \Delta_{{\rm amp}}$).
\end{definition}
%
\begin{remark}\label{remark:potThresh}
An equivalent definition of the potential threshold, Definition~\ref{def:pot-thresh}, but in terms of the free energy gap is $\Delta_{\rm pot} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! \delta f_{{\rm u}}(\Delta) > 0\}$. (HERE IS $\Delta_{\rm pot}$ is such that $\delta f_{{\rm u}}(\Delta_{\rm pot}) = 0$ BETTER?? TO HOMOGENEIZE WITH Definition~\ref{def:pot-thresh})
\end{remark}
%
In order to prove threshold saturation, formally given by Theorem~\ref{th:mainth_thsat} and Corollary~\ref{cor:maincorollary_thsat}, we need to define a proper spatially coupled (SC) version of the original problem (\ref{eq:mainProblem}). 
%
\subsection{The spatially coupled system}
%
We consider a chain of length $L+1$ where each \emph{block} of the chain, each of size $n$, is coupled to itself and $w \in\{1:L\}$ blocks in front and $w$ blocks before itself, thus to $2w+1$ blocks in total. The SC system is naturally defined, similarly to (\ref{eq:mainProblem}), as
%
\begin{align} \label{eq:def_coupledSyst}
W_{i_\mu j_\nu} = \frac{s_{i_\mu} s_{j_\nu}}{\sqrt{n(2w+1)}} + z_{i_\mu j_\nu} \sqrt{\Delta},
\end{align}
%
where the notation $u_{i_\mu j_\nu}$ means that the index $i_\mu \in \{1:n\}$ (resp. $j_\nu$) belongs to the block $\mu \in \{0:L\}$ (resp. $\nu$) along the coupled chain. In the case $w=L$, one recovers the original (or underlying) problem where the signal $\bf s$ has $n(L+1)$ components. In this construction, the performance of the AMP decoder is tracked by a \emph{scalar MSE profile} (or just \emph{profile}) $\tbf{E}^{(t)}$, defined componentwise by 
%
\begin{align}
E^{(t)}_\mu \defeq \mathbb{E}_{S,Z}[n^{-1}\sum_{i_\mu=1}^n(s_{i_\mu} - \hat s_{i_\mu}^{(t)})^2].
\end{align}
%
It has $L+1$ components and describes the scalar MSE in each block. Let us introduce the SE associated with the AMP algorithm for the inference over this SC system but first, denote the following average at fixed $s,z$ and $\Delta$
%
\begin{align}
% \langle f(x) \rangle_\mu = \frac{\int dx f(x)P_0(x)e^{\frac{\Sigma_\mu({\tbf E})^{-2}}{2} (2 xs - x^2) + \Sigma_\mu({\tbf E})^{-1} zx}}{\int dx P_0(x)e^{\frac{\Sigma_\mu({\tbf E})^{-2}}{2} (2 xs - x^2) + \Sigma_\mu({\tbf E})^{-1} zx}},
\langle A \rangle_\mu \defeq \frac{\int dx A(x) P_0(x)e^{-\frac{x^2}{2\Sigma_\mu({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu({\tbf E},\Delta)} \big)} }{\int dx P_0(x)
e^{-\frac{x^2}{2\Sigma_\mu({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu({\tbf E},\Delta)} \big)}},
\end{align}
%
where the \emph{effective noise variance} of the SC system is defined as
%
\begin{align} \label{eq:defSigma_mu}
\Sigma_\mu(\tbf{E},\Delta)^2 \defeq \Delta \Big(v-\sum_{\nu \in \mu^w} \frac{E_\nu}{2w+1}\Big)^{-1}.
\end{align}
%
\begin{definition}
The state evolution operator associated with the coupled system (\ref{eq:def_coupledSyst}) is defined component-wise as
%
\begin{align}
[T_{\rm c}({\tbf E})]_\mu \defeq \mathbb{E}_{S,Z}[(S - \langle x\rangle_\mu)^2]. \label{def:SEop_SC}
\end{align}
%
$T_{\rm c}({\tbf E})$ is vector valued and here we have written its $\mu$-th component. 
\end{definition}
%
\begin{remark} \label{remark:pinning}
We assume perfect knowledge at the boundaries, i.e. $z_{i_\mu j_\nu} = 0$ if $\mu$ and $\nu$ both belong to $\mathcal{B} \defeq \{0:w\}\cup \{L-w:L\}$ (TO DOUBLE CHECK THIS) or equivalently, $E_\mu=0 \ \forall \ \mu \in \mathcal{B}$. We refer to this as the pinning condition. 
\end{remark}
%
The SE iteration tracking the scalar MSE profile of the SC system then read for $\mu\notin \mathcal{B}$
%
\begin{equation}\label{equ:statevolutioncoupled}
E_\mu^{(t+1)} = [T_{\rm c}({\tbf E}^{(t)})]_\mu, \quad t\geq 0, \quad E^{(0)}_\mu = v \ \forall \ \mu\notin \mathcal{B}.
\end{equation}
%
Let us introduce a suitable notion of degradation that will be useful in the next.
%
\begin{definition}[Degradation] \label{def:degradation}
A profile ${\tbf{E}}$ is degraded (resp. strictly degraded) w.r.t another one ${\tbf{G}}$, denoted as ${\tbf{E}} \succeq {\tbf{G}}$ (resp. ${\tbf{E}} \succ {\tbf{G}}$), if $E_\mu \ge  G_\mu \ \forall \ \mu$ 
(resp. if ${\tbf{E}} \succeq {\tbf{G}}$ and there exists some $\mu$ such that $E_\mu > G_\mu$).
\end{definition}
%
Similarly as for the underlying system, see Definition~\ref{amp-thresh}, we define the AMP threshold for the SC system. Define the good error profile $\tbf{E}_{\rm good}(\Delta)$ as the vector with $L+1$ components equal to $E_{\rm good}(\Delta)$.
%
\begin{definition} [Threshold of coupled ensemble]\label{def:AMPcoupled}
The AMP threshold of the coupled system is defined as $\Delta_{\rm amp, c} \defeq {\liminf}_{L, w\to \infty}\, {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm c}}^{(\infty)}(\boldsymbol{v}) \prec \tbf{E}_{\rm good}(\Delta)\}$
where $\boldsymbol{v}$ is the all $v$ vector. The ${\liminf}_{L, w \to \infty}$ is taken along sequences where {\it first} $L \to \infty$ and {\it then} $w\to\infty$. 
\end{definition}
%
% Define the ensemble $\mu^{w} \defeq \{\mu - w,\ldots, \mu + w\} = \{\mu - w : \mu + w\}$. 
% The replica symmetric free energy for the SC system \eqref{eq:def_coupledSyst} can be computed by the replica symmetric replica method. It gives
% %
% \begin{align} 
% f_{\rm{c}}(\{E_\mu, \hat m_\mu\}) = &\sum_{\mu=0}^{L}\frac{v - E_\mu}{2} \Big(\hat m_\mu - \sum_{\nu \in \mu^{w}} \frac{v - E_\nu}{2\Delta(2w+1)} \Big) \nonumber \\
% -&\sum_{\mu=0}^L \mathbb{E}_{S,Z}\Big[\ln\Big(\int P_0(x)e^{-x^2\frac{\hat m_\mu}{2} + x \big(S\hat m_\mu + Z\sqrt{\hat m_\mu} \big)}\Big)\Big], \label{eq:coupledF}
% \end{align}
% %
% where $Z\sim \mathcal{N}(z|0,1)$ and $S \sim P_0(s)$. We define the \emph{effective noise variance} of the SC system as
% %
% \begin{align} \label{eq:defSigma_mu}
% \Sigma_\mu(\tbf{E},\Delta)^2 \defeq \Delta \Big(v-\sum_{\nu \in \mu^w} \frac{E_\nu}{2w+1}\Big)^{-1}.
% \end{align}
% %
% The fixed point conditions giving the extrema of this potential are
% %
% \begin{align}
% 0=\frac{\partial f_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {\hat m_\mu}} &\Rightarrow E_\mu = \mathbb{E}[(s - \langle x\rangle_\mu)^2] = [T_{\rm c}({\tbf E})]_\mu, \label{eq:fixedPointPotSC_isSE}\\
% %
% 0=\frac{\partial f_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {E_\mu}} &\Rightarrow \hat m_\mu = \Sigma_\mu({\tbf E})^{-2}.
% \end{align}
% %
% Plugging these relations with (\ref{eq:defSigma_mu}) in (\ref{eq:coupledF}), we obtain the RS free energy for the SC system. 
%
\begin{definition}[RS free energy of the coupled system]
%
The replica symmetric free energy of the SC system, or SC potential, is
%
\begin{align}
f_{\rm{c}}(\tbf{E}) = &\sum_{\mu=0}^L\sum_{\nu \in \mu^{w}} \frac{(v\!-\!E_\mu) (v\!-\!E_\nu)}{4\Delta(2w+1)} \nonumber \\
- &\sum_{\mu=0}^L \mathbb{E}_{S,Z}\Big[\ln\Big(\int P_0(x)
 e^{-\frac{x^2}{2\Sigma_\mu(\tbf E,\Delta)^{2}} +x\big(\frac{S}{\Sigma_\mu(\tbf E, \Delta)^{2} } + \frac{Z}{\Sigma_\mu(\tbf E,\Delta)}\big)} dx\Big)\Big], \label{def:RSf_SC}
\end{align}
%
where $\mu^{w} \defeq \{\mu - w,\ldots, \mu + w\} = \{\mu - w : \mu + w\}$, $Z\sim \mathcal{N}(z|0,1)$ and $S \sim P_0(s)$.
\end{definition}
%
As for the underlying system, we obtain from similar relations as in Appendix~\ref{app:nishi} the following Lemma linking SE and potential formulations.
%
\begin{lemma}\label{lemma:fixedpointSE_extPot}
$\mathring E_\mu = [T_{\rm c}(\mathring {\tbf E})]_\mu \Leftrightarrow \frac{\partial f_{{\rm c}}({\tbf E})}{\partial E_\mu}\big|_{\mathring{{\tbf E}}} = 0 \ \forall \ \mu\in \mathcal{B}^{\rm c}=\{w+1:L-w-1\}$.
\end{lemma}
%
The proof presented in the next subsection uses extensively the following monotonicity properties of the SE operators. 
%
\begin{lemma}
The SE operator of the SC system maintains degradation in space, i.e. ${\tbf E} \succeq  {\tbf G} \Rightarrow T_{\rm{c}}({\tbf E}) \succeq T_{\rm{c}}({\tbf{G}})$. This property is verified by $T_{\rm{u}}(E)$ for a scalar error as well.
\label{lemma:spaceDegrad}
\end{lemma}
%
\begin{proof}
From \eqref{eq:defSigma_mu} it is immediately seen that ${\tbf E} \succeq  {\tbf G} \Rightarrow \Sigma_\mu({\tbf E},\Delta) \geq \Sigma_\mu({\tbf G},\Delta)\ \forall \ \mu$. Now, the SE operator \eqref{def:SEop_SC} can be interpreted as an average over the chain blocks of local MMSE's. The local MMSE's are the ones of random variables $S\sim P_0(s)$ sent through AWGN channels with effective noise distributed as $\mathcal{N}(\cdot | 0,\Sigma_\mu^2)$. The MMSE's are increasing functions of $\Sigma_\mu^2$: this is intuitively clear but we provide an explicit formula for the derivative below. Thus $[T_{{\rm c}}( {\tbf E})]_\mu \geq [T_{{\rm c}}( {\tbf G})]_\mu \ \forall \ \mu$, which means $T_{{\rm c}}({\tbf E}) \succeq T_{{\rm c}}({\tbf{G}})$.

The derivative of the scalar MMSE of the Gaussian channel with i.i.d noise $\mathcal{N}(\cdot|0, \Sigma^2)$ can be computed as 
%
\begin{align}
 \frac{d \,{\rm Smmse}(\Sigma^{-2})}{d\,\Sigma^{-2}} = - 2\, \mathbb{E}_{X,Y}\big[\|X - \mathbb{E}[X\vert Y]\|_2^2 \, {\rm Var}[X\vert Y]\big].
\end{align}
%
This formula explicitly confirms that $T_{\rm u}(E)$ (resp. $[T_{{\rm c}}(\tbf E)]_\mu$) is an increasing function of $\Sigma$ (resp. $\Sigma_\mu$).
\end{proof}
%
\begin{corollary}
\label{cor:timeDegrad}
The SE operator of the coupled 
system maintains degradation in time, 
i.e., $T_{{\rm c}}({\tbf E}^{(t)}) \preceq  {\tbf E}^{(t)}\Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \preceq  {\tbf E}^{(t+1)}$. 
Similarly $T_{{\rm c}}({\tbf E}^{(t)}) \succeq  {\tbf E}^{(t)} \Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \succeq  {\tbf E}^{(t+1)}$. 
Furthermore, the limiting error profile ${\tbf E}^{(\infty)} \defeq T_{{\rm c}}^{(\infty)}({\tbf E}^{(0)})$
exists. This property is verified by $T_{{\rm u}}(E)$ for a scalar error as well.
\end{corollary}
%
\begin{proof}
The degradation statements are a consequence of Lemma~\ref{lemma:spaceDegrad}. The existence 
of the limits follows from the monotonicity of the operator and boundedness of the scalar MSE.
\end{proof}
%
Now that we have settled the required definitions and properties, we can prove threshold saturation. 
%
\subsection{Proof of threshold saturation}
%
The pinning condition together with the monotonicity properties of the coupled SE operator ensure that any fixed point point profile ${\tbf E}^*$ of the SE iteration \eqref{equ:statevolutioncoupled} must adopt a shape similar to Fig.~\ref{fig:errorProfile}. From now on we work with a \emph{saturated profile} $\tbf E$, which construction is described in detail in Fig.~\ref{fig:errorProfile}. It verifies ${\tbf E} \succeq {\tbf E}^{*}$ and thus serves as an upper bound in the proof. In the next, we will need the following operator.
%
\begin{figure}[!t]
\centering
\includegraphics[width=0.65\textwidth]{figs/profile_E_2}
\vspace*{-5pt}
\caption{A fixed point profile $\tbf{E}^{*}$ of the coupled SE iteration (solid) is null $\forall \ \mu \le w$ by the pinning condition and increases until $E_{{\rm max}} \in [0,v]$ at $\mu_{\rm max}\in \{w+1:L-w-1\}$. Then it decreases and is again null $\forall \ \mu \ge L-w$. The associated \emph{saturated} profile $\tbf E$ (dashed) starts at $E_{\rm good}(\Delta) \ \forall \ \mu \le \mu_*$, where $\mu_*$ is defined by: $E^{*}_{\mu}\le E_{\rm good}(\Delta) \ \forall \ \mu\le \mu_*$ and $E^{*}_{\mu'} > E_{\rm good}(\Delta) \ \forall \ \mu' > \mu_*$. Then it matches $\tbf E^{*} \ \forall \ \mu \in\{\mu_*:\mu_{\rm max}\}$ and saturates at $E_{{\rm max}} \ \forall \ \mu \ge \mu_{\rm max}$. By construction ${\tbf E}$ is non decreasing and is degraded w.r.t the fixed point profile ${\tbf E} \succeq {\tbf E}^{*}$.}
\label{fig:errorProfile}
\end{figure}
%
\begin{definition}[Shift operator]
The shift operator is defined componentwise as $[{\rm S}({\tbf E})]_1 \defeq E_{\rm good}(\Delta), \ [{\rm S}({\tbf E})]_\mu \defeq  E_{\mu-1}$.
\end{definition}
%
\subsubsection{Taylor expansion of the RS free energy of the SC system}
%
The first main step in the proof of threshold saturation is based on the Taylor expansion of the RS free energy of the SC system. It starts with the following Lemma.
%
\begin{lemma}\label{leminterp}
Let ${\tbf E}$ be a saturated profile. If ${\tbf E}_\lambda \defeq (1-\lambda) {\tbf E} + \lambda {\rm S}({\tbf E})$ and $\delta {E}_{\mu} \defeq {E}_{\mu} -{E}_{\mu-1}$, then for a proper $\lambda\in[0,1]$,
%
\begin{align}
f_{{\rm c}}({\rm S}({\tbf E})) &-f_{{\rm c}}({\tbf E}) = \frac{1}{2} \sum_{\mu,\mu'=1}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 f_{{\rm c}}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}. \label{eq:lemma_secondDerivativeFsc}
\end{align}
%
\label{lemma:Fdiff_quadraticForm}
\end{lemma}
%
\begin{proof}
%
The free energy difference can be expressed as
%
\begin{align}
f_{{\rm c}}({\rm S}({\tbf E})) -f_{{\rm c}}({\tbf E}) = \frac{1}{2}\sum_{\mu,\mu'=1}^{L} \delta {E}_{\mu} \delta {E}_{\mu'}  \frac{\partial^2 f_{{\rm c}}({\tbf E})}{\partial E_{\mu}\partial  E_{\mu'}}\Big|_{ {\tbf E}_\lambda} - \sum_{\mu=1}^{L} \delta {E}_{\mu} \frac{\partial f_{{\rm c}}({\tbf E})}{\partial  E_\mu}\Big|_{{\tbf E}}. \label{eq:expFbsminusFb}
\end{align}
%
By saturation of $\tbf E$ at the boundaries, $\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{1:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$. Moreover for $r\notin\mathcal{A}$, $E_\mu=[T_{\rm c}(\tbf E)]_\mu$, and thus by Lemma~\ref{lemma:fixedpointSE_extPot} the potential derivative cancels at these positions. Hence the last sum in (\ref{eq:expFbsminusFb}) cancels.
\end{proof}
%
From the previous Lemma, in order to compute the free energy difference between those of the shifted and non-shifted profiles, we need to compute the Hessian associated with this free energy.
%
\begin{align}
\frac{\partial f_{\rm{c}}({\tbf E})}{\partial {E_\mu}} &= \sum_{\nu \in \mu^{w}} \frac{E_\nu}{2\Delta(2w+1)} -\frac{1}{2} \sum_\nu \frac{\partial \Sigma_\nu(\tbf E)^{-2}}{\partial E_\mu} [T_{\rm{c}}({\tbf E})]_\nu - \frac{v}{2\Delta} \nonumber\\
%
&= \frac{1}{2\Delta(2w+1)}\Big(\sum_{\nu \in \mu^{w}} E_\nu-\sum_{\nu \in \mu^w} [T_{\rm{c}}({\tbf E})]_\nu\Big)- \frac{v}{2\Delta},\\
%
\Rightarrow\frac{\partial^2 f_{\rm{c}}({\tbf E})}{\partial {E_\mu}\partial {E_{\mu'}}} &= \frac{1}{2\Delta(2w+1)}\Big( \mathbb{I}(\mu' \in \mu^w) - \frac{1}{\Delta(2w+1)}\sum_{\nu \in \mu^w\cap {\mu'}^w} \frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \, \Sigma_\nu^{-2}} \Big). \label{eq:hessian_explicit}
\end{align}
%
We can now compute the r.h.s of \eqref{eq:lemma_secondDerivativeFsc}. Define $\delta E^* \defeq {\rm{max}} \,|\delta E_\mu|$. Due to the indicator function, the first term of the r.h.s of \eqref{eq:hessian_explicit} can be bounded as
%
\begin{align}
\frac{1}{2\Delta(2w+1)} \Big|\sum_{\mu=1}^L\sum_{\mu'\in \mu^w}\delta E_{\mu}\delta E_{\mu'}\Big| \le \frac{\delta E^*}{2\Delta} \Big|\sum_{\mu}\delta E_{\mu}\Big| \le \frac{\delta E^*}{2\Delta} |E_L - E_{\rm good}(\Delta)|,
\end{align}
%
where we have used the fact that the sum is telescopic for the last inequality. Notice now the following important smoothness property verified by the saturated profile.
%
\begin{lemma}
The saturated profile ${\tbf E}$ is smooth, i.e. $\delta E^* \le K^*/w$ for some $K^*=\mathcal{O}(1)$.
\end{lemma}
%
\begin{proof}
By saturation of $\tbf E$, $\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{1:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$. For $\mu \notin\mathcal{A}$, we can replace the fixed point profile component $E_\mu$ by $[T_{\rm c}(\tbf E)]_\mu$ and Taylor expand the SE operator. Define $\delta \Sigma_\mu^{-2} \defeq \Sigma_{\mu+1}({\tbf E})^{-2} - \Sigma_\mu({\tbf E})^{-2}$. From \eqref{eq:defSigma_mu} we get $\delta \Sigma_\mu^{-2} = (E_{\mu - w}-E_{\mu+w+1})/(\Delta(2w+1))$, where $E_{\mu - w}-E_{\mu+w+1} \le v$. We assume that the coupled SE operator is Lipshitz continuous with Lipshitz constant $K_T$ independent of the coupling window $w$. Then we obtain (TO DOUBLE CHECK THIS STEP)
%
\begin{align} \label{eq:deltamstar}
|\delta E_{\mu+1}| &= |[T_{\rm{c}}({\tbf E})]_{\mu +1} - [T_{\rm{c}}({\tbf E})]_{\mu}| \le K \delta \Sigma_\mu^{-2} \Big|\frac{\partial [T_{\rm{c}}({\tbf E})]_{\mu}}{\partial \Sigma_\mu^{-2}}\Big| \le K^*/w \eqdef \delta E^* \ \forall\ \mu,
\end{align}
%
where $K, K^*=\mathcal{O}(1)$ are independent of $w$.
% which is the desired result. Thus ${\tbf E}$ is smooth in the sense that its closeby variations are getting smaller as $w$ increases.
%
\end{proof}
%
Let us now study the second term of the r.h.s of \eqref{eq:hessian_explicit} (without considering the boundaries for sake of simplicity, despite they can be included easily) (TO INCLUDE)
%
\begin{align}
-&\frac{1}{2\Delta^2(2w+1)^2} \sum_{\mu, \mu'=1}^L \delta E_\mu \delta E_{\mu '} \sum_{\nu \in \mu^w\cap {\mu'}^w} \frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \Sigma_{\nu}^{-2}} \nonumber\\ 
%
\le \ &\frac{K_T \delta E^*}{2\Delta^2(2w+1)^2} \sum_{\mu=1}^L \delta E_\mu \sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mu^w\cap {\mu'}^w). \label{eq:last_secondTerm_boudHessian}
\end{align}
%
One can show that for a fixed $\mu$, $\sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mu^w\cap {\mu'}^w) = (2w+1)^2$. Thus \eqref{eq:last_secondTerm_boudHessian} can be upper bounded, using (\ref{eq:deltamstar}), by $K_T \delta E^* |E_L-E_{\rm good}(\Delta)|/(2\Delta^2) = K'/w$ for some constant $K'=\mathcal{O}(1)$ independent of $w$. From this analysis and using the triangle inequality for the last step, we obtain
%
\begin{align}
\frac{1}{2}\Big| \sum_{\mu,\mu'=1}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 f_{{\rm c}}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}\Big| \le U / w, \quad U=\mathcal{O}(1),
\end{align}
%
$U$ independent of $w.$ Combining this inequality with Lemma~\ref{leminterp} proves the following Lemma.
%
\begin{lemma} \label{lemma:dF_ge_Uoverw}
For a saturated profile $\tbf E$, $|f_{{\rm c}}({\rm S}({\tbf E})) -f_{{\rm c}}({\tbf E})|\le U / w$, where $U=\mathcal{O}(1)$ is independent of $w,L$.
\end{lemma}
%
\subsubsection{Direct evalutation of the free energy change}
%
The second main step in the proof is based on a direct evaluation of the free energy change when shifting the saturated profile. For this step, we will need the following Lemmas.
%
\begin{lemma}
Let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_{\rm good}(\Delta)$. Then $ E_{\rm max} \notin \mathcal{V}_{\rm good}$.
\label{lemma:outside_basin}
\end{lemma}
%
\begin{proof}
The fact that the error profile is non decreasing and the assumption that ${\tbf E} \succ {\tbf E}_{\rm good}(\Delta)$ imply that $E_{\rm max} > E_{0}$. Moreover,
%
$E_{\rm max} \le [T_{\rm c}({\tbf E})]_{\mu_{\rm max}} \le T_{\rm u}(E_{\rm max})$
%
where the first inequality follows from $\tbf E\succ \tbf E^*$ and the monotonicity of $T_{\rm c}$, while the second comes from the fact that $\tbf E$ is non decreasing. Combining these with the 
monotonicity of $T_{\rm u}$ gives $T_{\rm u}(E_{\rm max}) \ge  E_{\rm max} \Rightarrow T_{\rm u}^{(\infty)}( E_{\rm max}) \ge  E_{\rm max}> E_{\rm good}(\Delta) \Rightarrow  E_{\rm max} \notin \mathcal {V}_{\rm good}$.
\end{proof}
%
\begin{lemma}\label{lemma:FcSE_minus_FcE_le_deltaF}
Fix $\Delta < \Delta_{\rm pot}$ and let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_0$. Then $|f_{\rm{c}}(S(\tbf{E})) - f_{\rm{c}}(\tbf{E})| \ge \delta f_{\rm{u}}(\Delta)$, where $\delta f_{\rm{u}}(\Delta)$ is the free energy gap, see Definition~\ref{def:fgap}.
\end{lemma}
%
\begin{proof}
Call $\mathcal{I}(\Sigma) \defeq \mathbb{E}_{S,Z}[\ln(\int P_0(x)\exp\big(\frac{\Sigma^{-2}}{2}(2 Sx - x^2) + \Sigma^{-1} Zx\big)dx)]$. Then \eqref{def:RSf_SC} gives
%$f_{\rm{c}}(S(\tbf{E})) - f_{\rm{c}}(\tbf{E})$ is equal to
\begin{align}
% \delta F_{\rm{c}}&=\sum_{\mu=1}^L \Big[\sum_{\nu \in \mu^{w}} \frac{(v-E_{\mu-1}) (v-m_{\nu-1}) }{4\Delta(2w+1)} - I(\hat \Sigma_{\mu-1})\Big] - \sum_{\mu=1}^L \Big[\sum_{\nu \in \mu^{w}} \frac{(v-E_{\mu})(v- E_{\nu})}{4\Delta(2w+1)} - I(\hat \Sigma_{\mu}) \Big] \nonumber \\
%
f_{\rm{c}}({\rm S}(\tbf{E})) - f_{\rm{c}}(\tbf{E})=\sum_{\nu \in 0^{w}} \frac{(v\!-\!E_{0}) (v\!-\!E_{\nu}) }{4\Delta(2w+1)} - \mathcal{I}(\Sigma_{0}) - \sum_{\nu \in L^{w}} \frac{(v\!-\!E_{L})(v\!-\!E_{\nu}) }{4\Delta(2w+1)} + \mathcal{I}(\Sigma_{L}), \label{eq:lastFcSE_minus_FcE}
\end{align}
%
using the fact that the sum is telescoping. Recall $\Sigma(E,\Delta)^2= \Delta/ (v - E)$. Now looking at \eqref{eq:defSigma_mu}, one notices that thanks to the saturation of ${\tbf E}$ at the boundaries, $\Sigma_{0}({\tbf E}) = \Sigma(E_{\rm good}(\Delta))$, $\Sigma_{L}({\tbf E}) = \Sigma(E_L)$ where $E_L = E_{\rm{max}}$. So finally, we can write from \eqref{eq:lastFcSE_minus_FcE} that
%
\begin{align}
f_{\rm{c}}({\rm S}(\tbf{E})) - f_{\rm{c}}(\tbf{E}) &= \Big[\frac{(v\!-\!E_{0})^2 }{4\Delta} - \mathcal{I}(\Sigma(E_{\rm good}(\Delta))) \Big] - \Big[\frac{(v\!-\!E_{L})^2 }{4\Delta} - \mathcal{I}(\Sigma(E_L)) \Big] \nonumber\\
%
&= f_{\rm{u}}(E_{\rm good}(\Delta)) - f_{\rm{u}}(E_L) \le -\delta f_{\rm{u}}(\Delta),
\end{align}
%
where we recognized the free energy of the underlying system $f_{\rm u}(E;\Delta) = i_{\rm RS}(E;\Delta) - \frac{v^2}{4\Delta}$ and the last inequality is a direct application of Lemma~\ref{lemma:outside_basin}. Finally, using the positivity of $\delta f_{\rm{u}}(\Delta)$ as $\Delta<\Delta_{\txt{pot}}$, we obtain the desired result.
\end{proof}
%
We now have all the necessary Lemmas in order to prove threshold saturation.
%
\begin{theorem} \label{th:mainth_thsat}
Assume a spatially coupled instance of rank one matrix estimation is to be solved. Fix $\Delta<\Delta_{\rm{pot}}$, $w>U/\delta f_{\rm{u}}(\Delta)$ ($U$ being independent of $w,L$) and $L>2w$ (such that the problem is well defined, due to the pinning condition, see remark~\ref{remark:pinning}). Then any fixed point profile ${\tbf{E}^*}$ of the coupled state evolution iteration \eqref{equ:statevolutioncoupled} satisfies ${\tbf{E}}^* \prec {\tbf{E}}_{\rm good}(\Delta)$.
\end{theorem}
%
\begin{proof}
Assume that, under these hypotheses, there exists 
a saturated profile $\tbf E$ associated with $\tbf E^*$ such 
that $\tbf E\succ {\tbf{E}}_{\rm good}(\Delta)$. Combining Lemmas~\ref{lemma:dF_ge_Uoverw} and \ref{lemma:FcSE_minus_FcE_le_deltaF} we get $\delta f_{\rm{u}}(\Delta)\le U/w \Rightarrow w \le U/\delta f_{\rm{u}}(\Delta)$, a contradiction. 
Hence, ${\tbf{E}} \preceq {\tbf{E}}_{\rm good}(\Delta)$. Since $\tbf E \succ {\tbf E}^*$, then ${\tbf E}^* \prec {\tbf{E}}_{\rm good}(\Delta)$.
\end{proof}
%
\begin{corollary}\label{cor:maincorollary_thsat}
By first taking $L \to \infty$ and then $w\to\infty$, the AMP threshold of the coupled ensemble satisfies $\Delta_{\rm amp, c}\geq \Delta_{\rm{pot}}$.
\end{corollary}
%
This corollary follows from Theorem~\ref{th:mainth_thsat} and Definition~\ref{def:AMPcoupled}. It says that the AMP threshold of the SC system saturates the potential threshold. 

==> sections/threshold_saturation_old.tex <==
\section{Threshold saturation}\label{sec:thresh-sat}
%
%The replica symmetric solution is intimately related to an effective scalar denoising problem given by $y = s + \Sigma(E) z$
%where $s\sim P_0$ and $z\sim \mathcal{N}(0,1)$. Define the function 
%\begin{align}
%{\rm mmse}(\Sigma(E)^{-2}) = \mathbb{E}_{s, y}\bigl[ s - \mathbb{E}[x\vert y]\bigr]
%\end{align}
%where 
%\begin{align}
%\mathbb{E}[x\vert y] = \frac{\int dx\, x P_0(x) e^{-\frac{(y-x)^2}{2\Sigma(E)^2}}}{\int dx\,  P_0(x) e^{-\frac{(y-x)^2}{2\Sigma(E)^2}}}
%\end{align}
%In appendix \ref{appendixA} we show that the critical points of $h_{\rm RS}(E;\Delta)$ satisfy the fixed point equation
%\begin{align}
%E = {\rm mmse}(\Sigma(E)^{-2})
%\end{align}
%On the other hand, this is nothing else than the fixed point equation of state evolution 
%associated to the Approximate Message Passing (AMP) algorithm
%
Let us now introduce the main objects used in this paper, namely the state evolution and potential analysies. First define the \emph{effective noise variance} as
%
\begin{align}
\Sigma(E)^2 = \frac{\Delta}{v-E}. \label{eq:effNoise}
\end{align}
%
Using this definition, we can define the potential of the underlying system.
%
\begin{definition}[RS free energy] \label{def:RSf}
The replica symmetric (RS) free energy for the underlying system, or potential, obtained from the replica method of statistical physics, is
%
\begin{align}
% F_{\rm{u}}(\tilde m) = \frac{{\tilde m}^2}{4\Delta} - \mathbb{E}\Big[\ln\int P_0(x)\exp\Big(-\frac{\tilde m}{2\Delta} x^2+\frac{\tilde m}{\Delta} xs + \sqrt{\frac{\tilde m}{\Delta}} zx\Big)dx\Big],\\
%
% F_{\rm{u}}(\tilde E) = \frac{(v-\tilde E)^2}{4\Delta} - \mathbb{E}\ln\Big(\mathbb{E}_x\exp\Big(-\frac{v-\tilde E}{2\Delta}(x^2+ 2xs) + \sqrt{\frac{v-\tilde E}{\Delta}} zx\Big)\Big),
%
F_{\rm{u}}(E) = \frac{(v-E)^2}{4\Delta} - \mathbb{E}\ln\int P_0(x)\exp\Big(\frac{\Sigma(E)^{-2}}{2}(2xs -x^2) + \Sigma(E)^{-1} zx\Big)dx, \label{eq:RSf}
\end{align}
%
where the expectation $\mathbb{E}[\cdot]$ is w.r.t $z\sim \mathcal{N}(z|0,1)$ and $s \sim P_0(s)$.
\end{definition}
%
Define $\langle\cdot\rangle_E$ as the average w.r.t 
%
\begin{align}
\langle f(x) \rangle_E \defeq \frac{\int dx f(x) P_0(x)e^{\frac{\Sigma(E)^{-2}}{2}(2xs - x^2) + \Sigma(E)^{-1} zx} }{\int dx P_0(x)e^{\frac{\Sigma(E)^{-2}}{2}(2xs - x^2) + \Sigma(E)^{-1} zx}}. \label{eq:defBracket_posteriorMean}
\end{align}
%
Keep in mind that this distribution depends on $s$, $z$ too. The inference of the signal is performed by approximate message passing (AMP), which asymptotic perfomance can be tracked thanks to the state evolution (SE) analysis.
%
\begin{definition}[SE operator] 
The state evolution operator associated with the underlying system is
%
\begin{align}
T_{\rm u}(E) \defeq \mathbb{E}[(s - \langle x\rangle_E)^2]. \label{def:SEop_underlying}
\end{align}
%
\end{definition}
%
Call $\hat{\tbf{s}}^{(t)}$ the estimate at iteration $t$ of the signal by the AMP algorithm. The AMP averaged mean squarre error (MSE) is $E^{(t)}\defeq \mathbb{E}[n^{-1}\sum_{i=1}^n(s_i - \hat s_i^{(t)})^2]$, where $\mathbb{E}[\cdot]$ is the average w.r.t the observation $W$, i.e. w.r.t the noise and signal instances. It can then be tracked iterating the SE recursion
%
\begin{align} \label{eq:SEiteration}
E^{(t+1)}=T_{\rm u}(E^{(t)}), \qquad t\geq 0,
\end{align}
%
with initialization $E^{(0)} = v$, that is without any knowledge about the signal other than its prior distribution.
%
\begin{definition}[MSE Floor] The MSE floor $E_0$ is defined as the fixed point reached from the initial condition $E^{(0)} = 0$. In other words $E_0 = T_{\rm u}^{(\infty)}(0)$. 
\end{definition}
%
\begin{definition}[Bassin of attraction]
The basin of attraction of the MSE floor $E_0$ is 
$\mathcal{V}_0 \defeq \{ E \ \! |\ \! T_{\rm u}^{(\infty )}(E) = E_0 \}$.
\end{definition}
%
\begin{definition} [AMP threshold of the underlying ensemble]
The AMP threshold is $\Delta_{{\rm u}} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm u}}^{(\infty)}(v) = E_0\}$. 
\end{definition}
%
The replica method suggests that the free energy is the minimum of (\ref{eq:RSf}). Using an integration by part for $z$ and the so-called Nishimori conditions (TO PROVE??) $v = \mathbb{E}[\langle x^2\rangle_E]$, $\mathbb{E}[s \langle x \rangle_E] = \mathbb{E}[\langle x\rangle_E^2]\ \forall \ E$, one obtains
%
\begin{align}
0=\frac{\partial F_{\rm{u}}(E)}{\partial E}\Big|_{\mathring E} \Rightarrow \mathring E = \mathbb{E}[(s - \langle x\rangle_{\mathring E})^2] = T_{\rm{u}}(\mathring E).
\end{align}
%
We recognize the SE operator (\ref{def:SEop_underlying}), so that we can assert the follwing Lemma that links the SE and potential formulations.
%
\begin{lemma}\label{lemma:fixedpointSE_extPot_underlying}
% If $\mathring{E}$ is a fixed point of \eqref{eq:SEiteration}, i.e., $T_{{\rm u}}(\mathring E) = \mathring E$, then $\frac{\partial F_{{\rm u}}(E)}{\partial E}\big|_{\mathring E} =0$ and vice-versa.
$\mathring E = T_{{\rm u}}(\mathring E) \Leftrightarrow \frac{\partial F_{{\rm u}}(E)}{\partial E}\big|_{\mathring E} =0$.
\end{lemma} 
%
\begin{definition}[Free energy gap] \label{def:fgap}
The free energy gap is $\delta F_{{\rm u}} \defeq {\rm inf} _{E \notin \mathcal{V}_0 } (F_{{\rm u}}( E) - F_{{\rm u}}(E_0))$, with the convention that the infimum over the empty set is $\infty$ (this happens for $\Delta < \Delta_{{\rm u}}$).
\end{definition}
%
\begin{definition}[Potential threshold] \label{def:potThresh}
The potential threshold is defined as $\Delta_{\rm pot} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! \delta F_{{\rm u}} > 0\}$. 
\end{definition} 

THIS ENDS THE DEFINITIONS THAT I MOVED, N

THE PROOF OF THRSHOLD SATURATION STARTS HERE.

%
A fundamental step in the proof is based on the Theorem~\ref{th:mainth_thsat} and Corollary~\ref{cor:maincorollary_thsat}. Let us now prove this Theorem. It starts by defining a proper spatially coupled (SC) version of the original problem (\ref{eq:mainProblem}). 
%
\subsection{The spatially coupled system}
%
We consider a chain of length $L+1$ where each \emph{block} of size $n$ is connected to itself and $w \in\{1:L\}$ blocks in front and before itself, thus to $2w+1$ blocks in total. The SC system is naturally defined similarly to (\ref{eq:mainProblem}) as
%
\begin{align} \label{eq:def_coupledSyst}
W_{i_\mu j_\nu} = \frac{s_{i_\mu} s_{j_\nu}}{\sqrt{n(2w+1)}} + z_{i_\mu j_\nu} \sqrt{\Delta},
\end{align}
%
where the notation $x_{i_\mu j_\nu}$ means that the index $i$ (resp. $j$) belongs to the block $\mu$ (resp. $\nu$) along the $1$-d spatial dimension, i.e. along the coupled chain. In the case $w=L$, one recovers the original (or homogeneous) problem with $n(L+1)$ variables. In this construction, the performance of the AMP decoder is tracked by an \emph{MSE profile} (or just \emph{profile}) $\tbf{E}$ with $L+1$ components, describing the MSE in each block.

Let us introduce the state evolution associated with the AMP algorithm for the inference over this SC system. First, define the \emph{effective noise variance} of the SC system as
%
\begin{align} \label{eq:defSigma_mu}
\Sigma_\mu(\tbf{E})^2 \defeq \Delta \Big(v-\sum_{\nu \in \mu^w} \frac{E_\nu}{2w+1}\Big)^{-1},
\end{align}
%
and denote
%
\begin{align}
\langle f(x) \rangle_\mu = \frac{\int dx f(x)P_0(x)e^{\frac{\Sigma_\mu({\tbf E})^{-2}}{2} (2 xs - x^2) + \Sigma_\mu({\tbf E})^{-1} zx}}{\int dx P_0(x)e^{\frac{\Sigma_\mu({\tbf E})^{-2}}{2} (2 xs - x^2) + \Sigma_\mu({\tbf E})^{-1} zx}},
\end{align}
%
than depends on $z, s$. Before defining the SE operator associated with the AMP algorithm for this SC system, we introduce a suitable notion of degradation that will be useful in the next.
%
\begin{definition}[Degradation] \label{def:degradation}
A profile ${\tbf{E}}$ is degraded (resp. strictly degraded) w.r.t another one ${\tbf{G}}$, denoted as ${\tbf{E}} \succeq {\tbf{G}}$ (resp. ${\tbf{E}} \succ {\tbf{G}}$), if $E_\mu \ge  G_\mu \ \forall \ \mu$ 
(resp. if ${\tbf{E}} \succeq {\tbf{G}}$ and there exists some $\mu$ such that $E_\mu > G_\mu$).
\end{definition}
%
\begin{definition}
The state evolution operator associated with the coupled system (\ref{eq:def_coupledSyst}) is defined component-wise as
%
\begin{align}
[T_{\rm c}({\tbf E})]_\mu \defeq \mathbb{E}[(s - \langle x\rangle_\mu)^2]. \label{def:SEop_SC}
\end{align}
%
$T_{\rm c}({\tbf E})$ is vector valued and here we have written its $\mu$-th component. 
\end{definition}
%
We assume perfect knowledge at the boundaries, i.e. $E_\mu=0 \ \forall \ \mu \in \mathcal{B} \defeq \{0:w\}\cup \{L-w:L\}$. We refer to this as the \emph{pinning condition}. The SE iterations for the SC system then read for $\mu\notin \mathcal{B}$
%
\begin{equation}\label{equ:statevolutioncoupled}
E_\mu^{(t+1)} = [T_{\rm c}({\tbf E}^{(t)})]_\mu, \qquad t\geq 0,
\end{equation}
%
with initialization $E^{(0)}_\mu = v \ \forall \ \mu\notin \mathcal{B}$. Similarly for the underlying system, we define an AMP threshold for the SC system.
%
\begin{definition} [Threshold of coupled ensemble]\label{def:AMPcoupled}
The AMP threshold of the coupled system is defined as $\Delta_{\text c} \defeq {\liminf}_{L, w\to \infty} {\rm sup}\,\{\Delta>0\ \! |\ \! T_{\text{c}}^{(\infty)}(\boldsymbol{1}) \prec \tbf E_0\}$
where $\boldsymbol{1}$ is the all ones vector. The ${\liminf}_{L, w \to \infty}$ is taken along sequences where {\it first} $L \to \infty$ and {\it then} $w\to\infty$. 
\end{definition}
%
Define the ensemble $\mu^{w} \defeq \{\mu - w,\ldots, \mu + w\}\eqdef \{\mu - w : \mu + w\}$. The RS free energy under the Nishimori conditions for this SC system can be computed by the replica symmetric replica method, which gives
%
\begin{align} 
F_{\rm{c}}(\{E_\mu, \hat m_\mu\}) = &\sum_{\mu=0}^{L}\frac{v - E_\mu}{2} \Big(\hat m_\mu - \sum_{\nu \in \mu^{w}} \frac{v - E_\nu}{2\Delta(2w+1)} \Big) \nonumber \\
-&\sum_{\mu=0}^L \mathbb{E}\ln\int P_0(x)\exp\Big(\frac{\hat m_\mu}{2} (2xs - x^2) + \sqrt{\hat m_\mu} zx\Big)dx, \label{eq:coupledF}
\end{align}
%
where the expectation $\mathbb{E}[\cdot]$ is w.r.t $z\sim \mathcal{N}(z|0,1)$ and $s \sim P_0(s)$. The fixed point conditions givieng the extrema of this potential are
%
\begin{align}
0=\frac{\partial F_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {\hat m_\mu}} &\Rightarrow E_\mu = \mathbb{E}[(s - \langle x\rangle_\mu)^2] = [T_{\rm c}({\tbf E})]_\mu, \label{eq:fixedPointPotSC_isSE}\\
%
0=\frac{\partial F_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {E_\mu}} &\Rightarrow \hat m_\mu = \Sigma_\mu({\tbf E})^{-2}.
\end{align}
%
Plugging these relations with (\ref{eq:defSigma_mu}) in (\ref{eq:coupledF}), we obtain the RS free energy for the SC system.
%
\begin{definition}[RS free energy of the coupled system]
%
The replica symmetric free energy of the SC system, or SC potential, is
%
\begin{align}
F_{\rm{c}}(\tbf{E}) = &\sum_{\mu=0}^L\sum_{\nu \in \mu^{w}} \frac{(v-E_\mu) (v-E_\nu)}{4\Delta(2w+1)} \nonumber \\
- &\sum_{\mu=0}^L \mathbb{E}\ln\int P_0(x)\exp\Big(\frac{\Sigma_\mu(\tbf E)^{-2}}{2}(2 xs - x^2) + \Sigma_\mu(\tbf E)^{-1} zx\Big)dx. \label{def:RSf_SC}
\end{align}
\end{definition}
%
As for the underlying system, we obtain from (\ref{eq:fixedPointPotSC_isSE}) the following Lemma linking SE and potential formulations.
%
\begin{lemma}\label{lemma:fixedpointSE_extPot}
$\mathring E_\mu = [T_{\rm c}(\mathring {\tbf E})]_\mu \Leftrightarrow \frac{\partial F_{{\rm c}}({\tbf E})}{\partial E_\mu}\big|_{\mathring{{\tbf E}}} = 0 \ \forall \ \mu\in \mathcal{B}^{\rm c}=\{w+1:L-w-1\}$.
\end{lemma}
%
\subsection{Proof of threshold saturation}
%
The next monotonicity properties of the SE operators are essential in the proof. 
%
\begin{lemma}
The SE operator of the SC system maintains degradation in space, i.e. ${\tbf E} \succeq  {\tbf G} \Rightarrow T_{\rm{c}}({\tbf E}) \succeq T_{\rm{c}}({\tbf{G}})$. This property is verified by $T_{\rm{u}}(E)$ for a scalar error as well.
\label{lemma:spaceDegrad}
\end{lemma}
%
\begin{proof}
From \eqref{eq:defSigma_mu} it is immediately seen that ${\tbf E} \succeq  {\tbf G} \Rightarrow \Sigma_\mu({\tbf E}) \geq \Sigma_\mu({\tbf G})\ \forall \ \mu$. Now, the SE operator \eqref{def:SEop_SC} can be interpreted as an average over the spatial dimension of local MMSE's. The local MMSE's are the ones of random variables $s\sim P_0(s)$ sent through AWGN channels with effective noise $\mathcal{N}(\cdot | 0,\Sigma_\mu^2)$. The MMSE's are increasing functions of $\Sigma_\mu^2$: this is intuitively clear but we provide an explicit formula for the derivative below. Thus $[T_{{\rm c}}( {\tbf E})]_\mu \geq [T_{{\rm c}}( {\tbf G})]_\mu \ \forall \ \mu$, which means $T_{{\rm c}}({\tbf E}) \succeq T_{{\rm c}}({\tbf{G}})$.

The derivative of the MMSE of the Gaussian channel with i.i.d noise $\mathcal{N}(\cdot|0, \Sigma^2)$ can be computed as 
%
\begin{align}
 \frac{d \ \! {\rm mmse}(\Sigma)}{d(\Sigma^{-2})} = - 2 \mathbb{E}_{X,Y}\big[\|X - \mathbb{E}[X\vert Y]\|_2^2 \, {\rm Var}[X\vert Y]\big].
\end{align}
%
This formula explicitly confirms that $T_{\rm u}(E)$ (resp. $[T_{{\rm c}}(\tbf E)]_\mu$) is an increasing function of $\Sigma$ (resp. $\Sigma_\mu$).
\end{proof}
%
\begin{corollary}
\label{cor:timeDegrad}
The SE operator of the coupled 
system maintains degradation in time, 
i.e., $T_{{\rm c}}({\tbf E}^{(t)}) \preceq  {\tbf E}^{(t)}\Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \preceq  {\tbf E}^{(t+1)}$. 
Similarly $T_{{\rm c}}({\tbf E}^{(t)}) \succeq  {\tbf E}^{(t)} \Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \succeq  {\tbf E}^{(t+1)}$. 
Furthermore, the limiting error profile ${\tbf E}^{(\infty)} \defeq T_{{\rm c}}^{(\infty)}({\tbf E}^{(0)})$
exists. This property is verified by $T_{{\rm u}}(E)$ for the underlying system as well.
\end{corollary}
%
\begin{figure}[!t]
\centering
\includegraphics[width=0.65\textwidth]{figs/profile_E}
\vspace*{-5pt}
\caption{A fixed point profile $\tbf{E}^{*}$ of the coupled SE (solid) is null $\forall \ \mu \le w$ and increases until $E_{{\rm max}} \in [0,v]$ at $\mu_{\rm max}\in \{w+1:L-w-1\}$. Then it decreases and is again null $\forall \ \mu \ge L-w$. The associated \emph{saturated} profile $\tbf E$ (dashed) starts at $E_0 \ \forall \ \mu \le \mu_*$, where $\mu_*$ is defined by: $E^{*}_{\mu}\le E_0 \ \forall \ \mu\le \mu_*$ and $E^{*}_{\mu'} > E_0 \ \forall \ \mu' > \mu_*$. Then it matches $\tbf E^{*} \ \forall \ \mu \in\{\mu_*:\mu_{\rm max}\}$ and saturates $E_{{\rm max}} \ \forall \ \mu \ge \mu_{\rm max}$. By construction ${\tbf E}$ is non decreasing and ${\tbf E} \succeq {\tbf E}^{*}$.}
\label{fig:errorProfile}
\end{figure}
%
\begin{proof}
The degradation statements are a consequence of Lemma~\ref{lemma:spaceDegrad}. The existence 
of the limits follows from the monotonicity of the operator and boundedness of the MSE.
\end{proof}
%
The pinning condition together with the monotonicity properties of the coupled SE operator ensures that any fixed point point profile ${\tbf E}^*$ must adopt a shape similar to Fig.~\ref{fig:errorProfile}. 
From now on we work with a \emph{saturated profile} $\tbf E$, which construction is described in detail in Fig.~\ref{fig:errorProfile}. The associated saturated profile verifies ${\tbf E} \succeq {\tbf E}^{*}$, where ${\tbf E}^{*}$ is the fixed point profile of the coupled SE operator \eqref{def:SEop_SC}. In the next, we will need the following operator.
%
\begin{definition}[Shift operator]
The shift operator is defined componentwise as $[\text{S}({\tbf E})]_1 \defeq E_0, \ [\text{S}({\tbf E})]_\mu \defeq  E_{\mu-1}$.
\end{definition}
%
The first main step in the proof of threshold saturation is based on the Taylor expansion of the RS free energy of the SC system. It starts with the following Lemma.
%
\begin{lemma}\label{leminterp}
Let ${\tbf E}$ be a saturated profile. If ${\tbf E}_\lambda \defeq (1-\lambda) {\tbf E} + \lambda \text{S}({\tbf E})$ and $\delta {E}_{\mu} \defeq {E}_{\mu} -{E}_{\mu-1}$, then for a proper $\lambda\in[0,1]$,
%
\begin{align}
F_{{\rm c}}(\text{S}({\tbf E})) &-F_{{\rm c}}({\tbf E}) = \frac{1}{2} \sum_{\mu,\mu'=1}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 F_{{\rm c}}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}. \label{eq:lemma_secondDerivativeFsc}
\end{align}
%
\label{lemma:Fdiff_quadraticForm}
\end{lemma}
%
\begin{proof}
%
$F_{{\rm c}}(\text{S}({\tbf E})) - F_{{\rm c}}({\tbf E})$ can be expressed as
%
\begin{align}
F_{{\rm c}}(\text{S}({\tbf E})) -F_{{\rm c}}({\tbf E}) = \frac{1}{2}\sum_{\mu,\mu'=1}^{L} \delta {E}_{\mu} \delta {E}_{\mu'}  \frac{\partial^2 F_{{\rm c}}({\tbf E})}{\partial E_{\mu}\partial  E_{\mu'}}\Big|_{ {\tbf E}_\lambda} - \sum_{\mu=1}^{L} \delta {E}_{\mu} \frac{\partial F_{{\rm c}}({\tbf E})}{\partial  E_\mu}\Big|_{{\tbf E}}. \label{eq:expFbsminusFb}
\end{align}
%
By saturation of $\tbf E$, $\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{1:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$. Moreover for $r\notin\mathcal{A}$, $E_\mu=[T_{\rm c}(\tbf E)]_\mu$, and thus by Lemma~\ref{lemma:fixedpointSE_extPot} the potential derivative cancels at these positions. Hence the last sum in (\ref{eq:expFbsminusFb}) cancels.
\end{proof}
%
We thus need to compute the Hessian associated with this free energy.
%
\begin{align}
\frac{\partial F_{\rm{c}}({\tbf E})}{\partial {E_\mu}} &= \sum_{\nu \in \mu^{w}} \frac{E_\nu}{2\Delta(2w+1)} -\frac{1}{2} \sum_\nu \frac{\partial \Sigma_\nu(\tbf E)^{-2}}{\partial E_\mu} [T_{\rm{c}}({\tbf E})]_\nu - \frac{v}{2\Delta} \nonumber\\
%
&= \frac{1}{2\Delta(2w+1)}\Big(\sum_{\nu \in \mu^{w}} E_\nu-\sum_{\nu \in \mu^w} [T_{\rm{c}}({\tbf E})]_\nu\Big)- \frac{v}{2\Delta},\\
%
\Rightarrow\frac{\partial^2 F_{\rm{c}}({\tbf E})}{\partial {E_\mu}\partial {E_{\mu'}}} &= \frac{1}{2\Delta(2w+1)}\Big( \mathbb{I}(\mu' \in \mu^w) - \frac{1}{\Delta(2w+1)}\sum_{\nu \in \mu^w\cap {\mu'}^w} \frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \, \Sigma_\nu^{-2}} \Big). \label{eq:hessian_explicit}
\end{align}
%
We can now compute the r.h.s of \eqref{eq:lemma_secondDerivativeFsc}. Define $\delta E^* = {\rm{max}} \,|\delta E_\mu|$. Due to the indicator function, the first term in \eqref{eq:hessian_explicit} can be bounded as
%
\begin{align}
\frac{1}{2\Delta(2w+1)} \Big|\sum_{\mu, \mu'\in \mu^w}\delta E_{\mu}\delta E_{\mu'}\Big| \le \frac{\delta E^*}{2\Delta} \Big|\sum_{\mu}\delta E_{\mu}\Big| \le \frac{\delta E^*}{2\Delta} |E_L - E_0|,
\end{align}
%
where we have used the fact that the sum is telescopic for the last inequality. Notice now the following important smoothness property verified by a saturated profile.
%
\begin{lemma}
A saturated profile ${\tbf E}$ is smooth, i.e. $\delta E^* \le K^*/w$ for some $K^*=\mathcal{O}(1)$.
\end{lemma}
%
\begin{proof}
By saturation of $\tbf E$, $\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{1:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$. For $\mu \notin\mathcal{A}$, we can replace $E_\mu$ by $[T_{\rm c}(\tbf E)]_\mu$ and Taylor expand the SE operator. Define $\delta \Sigma_\mu^{-2} \defeq \Sigma_{\mu+1}({\tbf E})^{-2} - \Sigma_\mu({\tbf E})^{-2}$. One can notice from \eqref{eq:defSigma_mu} that $\delta \Sigma_\mu^{-2} = (E_{\mu - w}-E_{\mu+w+1})/(\Delta(2w+1))$, where $E_{\mu - w}-E_{\mu+w+1} \le 1)$. Call $K=\mathcal{O}(1)$ some constant. We assume that the coupled SE operator is Lipshitz continuous with Lipshitz constant $K_T$ independent of the coupling window $w$. Then we obtain
%
\begin{align} \label{eq:deltamstar}
|\delta E_{\mu+1}| &= |[T_{\rm{c}}({\tbf E})]_{\mu +1} - [T_{\rm{c}}({\tbf E})]_{\mu}| \le K \delta \Sigma_\mu^{-2} \Big|\frac{\partial [T_{\rm{c}}({\tbf E})]_{\mu}}{\partial \Sigma_\mu^{-2}}\Big| \le K^*/w \eqdef \delta E^* \ \forall\ \mu.
\end{align}
%
% which is the desired result. Thus ${\tbf E}$ is smooth in the sense that its closeby variations are getting smaller as $w$ increases.
%
\end{proof}
%
Let us now study the second term of \eqref{eq:hessian_explicit} (without considering the boundaries for sake of simplicity, despite they can be included easily)
%
\begin{align}
-&\frac{1}{2\Delta^2(2w+1)^2} \sum_{\mu, \mu'} \delta E_\mu \delta E_{\mu '} \sum_{\nu \in \mu^w\cap {\mu'}^w} \frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \Sigma_{\nu}^{-2}} \nonumber\\ 
%
\le \ &\frac{K_T \delta E^*}{2\Delta^2(2w+1)^2} \sum_{\mu} \delta E_\mu \sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mu^w\cap {\mu'}^w). \label{eq:last_secondTerm_boudHessian}
\end{align}
%
Now, it is easy to show that for a fixed $\mu$, $\sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mu^w\cap {\mu'}^w) = (2w+1)^2$. Thus \eqref{eq:last_secondTerm_boudHessian} can be upper bounded, using (\ref{eq:deltamstar}), by $K_T \delta E^* |E_L-E_0|/(2\Delta^2) = K'/w$ for some $K'=\mathcal{O}(1)$. From this analysis and using the triangle inequality for the last step, we get
%
\begin{align}
\frac{1}{2}\Big| \sum_{\mu,\mu'=1}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 F_{{\rm c}}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}\Big| \le U / w, \quad U=\mathcal{O}(1).
\end{align}
%
Combining this inequality with Lemma~\ref{leminterp}, we can assert the next Lemma.
%
\begin{lemma} \label{lemma:dF_ge_Uoverw}
For a saturated profile $\tbf E$, $|F_{{\rm c}}(\text{S}({\tbf E})) -F_{{\rm c}}({\tbf E})|\le U / w$, where $U=\mathcal{O}(1)$ is independent of $w,L$.
\end{lemma}
%
The second main step in the proof is based on a direct evaluation of the free energy change when shifting the saturated profile. We will need the following Lemmas.
%
\begin{lemma}
Let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_0$. Then $ E_{\rm max} \notin \mathcal{V}_0$.
\label{lemma:outside_basin}
\end{lemma}
%
\begin{proof}
The non decreasing error profile and the assumption that ${\tbf E} \succ {\tbf E}_0$ imply that $E_{\rm max} > E_{0}$. Moreover,
%
$E_{\rm max} \le [T_\text{c}({\tbf E})]_{\mu_{\rm max}} \le T_\text{s}(E_{\rm max})$
%
where the first inequality follows from $\tbf E\succ \tbf E^*$ and the monotonicity of $T_\text{c}$, while the second comes from the fact that $\tbf E$ is non decreasing. Combining these with the 
monotonicity of $T_\text{s}$ gives $T_{\text s}(E_{\rm max}) \ge  E_{\rm max} \Rightarrow T_{\text s}^{(\infty)}( E_{\rm max}) \ge  E_{\rm max}> E_0 \Rightarrow  E_{\rm max} \notin \mathcal {V}_0$.
\end{proof}
%
\begin{lemma}\label{lemma:FcSE_minus_FcE_le_deltaF}
Let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_0$. Then $|F_{\rm{c}}(S(\tbf{E})) - F_{\rm{c}}(\tbf{E})| \ge \delta F_{\rm{u}}$, where $\delta F_{\rm{u}}$ is the free energy gap, see Definition~\ref{def:fgap}.
\end{lemma}
%
\begin{proof}
Call $I(\Sigma) \defeq \mathbb{E}\ln\int P_0(x)\exp\big(\frac{\Sigma^{-2}}{2}(2 xs - x^2) + \Sigma^{-1} zx\big)dx$. Then we have from \eqref{def:RSf_SC} that $F_{\rm{c}}(S(\tbf{E})) - F_{\rm{c}}(\tbf{E})$ is equal to
\begin{align}
% \delta F_{\rm{c}}&=\sum_{\mu=1}^L \Big[\sum_{\nu \in \mu^{w}} \frac{(v-E_{\mu-1}) (v-m_{\nu-1}) }{4\Delta(2w+1)} - I(\hat \Sigma_{\mu-1})\Big] - \sum_{\mu=1}^L \Big[\sum_{\nu \in \mu^{w}} \frac{(v-E_{\mu})(v- E_{\nu})}{4\Delta(2w+1)} - I(\hat \Sigma_{\mu}) \Big] \nonumber \\
%
\sum_{\nu \in 0^{w}} \frac{(v-E_{0}) (v-E_{\nu}) }{4\Delta(2w+1)} - I(\Sigma_{0}) - \sum_{\nu \in L^{w}} \frac{(v-E_{L})(v-E_{\nu}) }{4\Delta(2w+1)} + I(\Sigma_{L}), \label{eq:lastFcSE_minus_FcE}
\end{align}
%
using the telescoping nature of the sum. Now notice that thanks to the saturation of the saturated profile at the boundaries, one gets from \eqref{eq:effNoise} and \eqref{eq:defSigma_mu} that $\Sigma_{0}({\tbf E}) = \Sigma(E_0)$, $\Sigma_{L}({\tbf E}) = \Sigma(E_L)$ where $E_L = E_{\rm{max}}$. So finally, we can write from \eqref{eq:lastFcSE_minus_FcE} that
%
\begin{align}
F_{\rm{c}}(S(\tbf{E})) - F_{\rm{c}}(\tbf{E}) &= \Big[\frac{(v-E_{0})^2 }{4\Delta} - I(\Sigma(E_0)) \Big] - \Big[\frac{(v-E_{L})^2 }{4\Delta} - I(\Sigma(E_L)) \Big] \nonumber\\
%
&= F_{\rm{u}}(E_0) - F_{\rm{u}}(E_L) \le -\delta F_{\rm{u}},
\end{align}
%
where we recognized \eqref{eq:RSf} and the last inequality is a direct application of Lemma~\ref{lemma:outside_basin}. Finally, using the positivity of $\delta F_{\text{u}}$ as $\Delta<\Delta_{\txt{pot}}$, we obtain the desired result.
\end{proof}
%
Combining these results, we can now prove the threshold saturation Theorem.
%
\begin{theorem} \label{th:mainth_thsat}
Assume a spatially coupled instance of rank one matrix estimation is to be solved. Fix $\Delta<\Delta_{\rm{pot}}$, $w>U/\delta F_{\rm{u}}$ ($U=\mathcal{O}(1)$ is independent of $w,L$) and $L>2w$ (such that the problem is well defined, due to the pinning condtition). Then any fixed point profile ${\tbf{E}^*}$ of the coupled state evolution satisfies ${\tbf{E}}^* \prec {\tbf{E}}_0$.
\end{theorem}
%
\begin{proof}
Assume that, under these hypotheses, there exists 
a saturated profile $\tbf E$ associated to $\tbf E^*$ such 
that $\tbf E\succ {\tbf{E}}_0$. Combining Lemma~\ref{lemma:dF_ge_Uoverw} and \ref{lemma:FcSE_minus_FcE_le_deltaF} we get $\delta F_{\text{u}}\le U/w \Rightarrow w \le U/\delta F_{\text{u}}$, a contradiction. 
Hence, ${\tbf{E}} \preceq {\tbf{E}}_0$. Since $\tbf E \succ {\tbf E}^*$ we have ${\tbf E}^* \prec {\tbf{E}}_0$.
\end{proof}
%
The Lemma follows from the last Theorem and Definition~\ref{def:AMPcoupled}. It says that the AMP threshold for the coupled codes saturates the potential threshold.
%
\begin{corollary}\label{cor:maincorollary_thsat}
By first taking $L \to \infty$ and then $w\to\infty$, the AMP threshold of the coupled ensemble satisfies $\Delta_{\rm c}\geq \Delta_{\rm{pot}}$.
\end{corollary}

==> v5 arxiv/sections/1_intro_setting.tex <==
\section{Introduction}
%
We consider the following probabilistic rank-one matrix estimation (or rank-one matrix factorization) problem: one has access to noisy observations
${\bf w} = (w_{ij})_{i,j=1}^n\in \mathbb{R}^{n,n}$ of the pair-wise product of the
components of a vector ${\bf s}=(s_i)_{i=1}^n \in \mathbb{R}^n$
where the components are i.i.d random variables distributed according to $S_i\sim P_0$,
$i=1,\dots, n$. The matrix elements of ${\bf w}$ are observed through a noisy
element-wise (possibly non-linear) output probabilistic channel
$P_{\rm out}(w_{ij}|s_is_j)$, with $i,j=1,\dots,n$. The goal 
is to estimate the vector ${\bf s}$ from ${\bf w}$, up to a global flip of sign in general, assuming that both distributions $P_0$ and $P_{\rm out}$ are 
known. We assume the noise to be symmetric so that $w_{ij}=w_{ji}$. There are many important problems
in statistics and machine learning that can be expressed in this way, among which:
%
\begin{itemize}
\item \emph{Sparse PCA}: Sparse principal component analysis (PCA) is a dimensionality reduction technique where one looks for a 
low-rank representation of a data matrix with sparsity constraints [\cite{zou2006sparse}]. The following is the simplest probabilistic 
symmetric version where one estimates a rank-one matrix. 
Consider a sparse random vector $\tbf{S}$, for instance
 drawn from a Gauss-Bernoulli distribution, and take an additive white Gaussian noise (AWGN) channel
 where the observations are 
  $W_{ij} = S_iS_j/\sqrt{n} + \Delta Z_{ij}$ whith $Z_{ij}\sim\mathcal{N}(0,1)$. Here\footnote{In this paper 
 $\mathcal{N}(x|m, \sigma^2) = (2\pi\sigma^2)^{-1/2}\exp(-(x-m)^2/2\sigma^2))$} 
  $P_{\rm out}(w_{ij}|s_is_j) = \mathcal{N}(w_{ij}|s_is_j/\sqrt{n}, \Delta)$.
\item \emph{Spiked Wigner model}: In this model the noise is still Gaussian, but the vector $\tbf{S}$ is assumed to be a Bernoulli random
  vector with i.i.d components $S_i \sim {\rm Ber}(\rho)$. This formulation is a particular
  case of the spiked covariance model in statistics introduced
  by [\cite{johnstone2004sparse,johnstone2012consistency}]. It has also
  attracted a lot of attention in the framework of random matrix theory
   (see for instance [\cite{baik2005phase}] and references therein).
\item \emph{Community detection}: In its simplest setting, one uses a Rademacher
  vector $\tbf{S}$ where each variable take values $S_i\in \{-1,1\}$
  depending on the ``community'' it belongs to. The observation model
  then introduces missing information and errors such that, for
  instance, $P_{\rm out}(w_{ij}|s_is_j)=p_1 \delta(w_{ij} - s_is_j) + p_2 \delta(w_{ij} +s_is_j) + (1-p_1-p_2) \delta(w_{ij})$, 
  where $\delta(\cdot)$ is the Delta dirac function. 
  These models have recently attracted a lot of attention both in statistics and machine learning contexts
  (see e.g. [\cite{bickel2009nonparametric,decelle2011asymptotic,karrer2011stochastic,saade2014spectral,massoulie2014community,ricci2016performance}]).
\item \emph{Sub-matrix localization}: This is the problem of finding a
  submatrix with an elevated mean in a large noisy matrix, as in
  [\cite{hajek2015submatrix,chen2014statistical}].
\item \emph{Matrix completion}: A last example is the matrix completion
  problem where a part of the information (the matrix elements) is hidden, while the rest is
  given with noise. For instance, a classical model is $P_{\rm out}(w_{ij}|s_is_j) = p\delta(w_{ij}) + (1-p) \mathcal{N}(w_{ij}|s_is_j,\Delta)$. Such problems have been extensively discussed over the last decades, in particular because of their connection to collaborative filtering (see for instance [\cite{candes2009exact,cai2010singular,keshavan2009matrix,saade2015matrix}]).
\end{itemize}

Here we shall consider the probabilistic formulation of these
problems and focus on estimation in the mean square
error (MSE) sense. We rigorously derive an 
explicit formula for the mutual information 
in the asymptotic limit, and for the
information theoretic minimal mean square error (MMSE).
Our results imply that in a large region of parameters, the
posterior expectation of the underlying signal, a quantity often
assumed intractable to compute, can be obtained using a
polynomial-time scheme via the approximate message-passing (AMP) 
framework [\cite{rangan2012iterative,matsushita2013low,6875223,deshpande2015asymptotic,lesieur2015phase}]. 
We also demonstrate the existence of a region where no
{\it known} tractable algorithm is able to find a solution
correlated with the ground truth. Nevertheless, we prove 
explicitly that it is information theoretically possible to do so (even in this region), and 
discuss the implications in terms of computational complexity.

The crux of our analysis rests on an "auxiliary" spatially coupled (SC) system. The hallmark of SC models is that one can tune them so that 
the gap between the algorithmic and information theoretic limits is eliminated, while at the same time the mutual information is maintained unchanged for the coupled and original models. Roughly speaking, this means that it is possible to algorithmically compute 
the information theoretic limit of the original model because a
suitable algorithm is optimal on the coupled system. 

Our proof technique has an interest by its own as it combines recent rigorous results in coding theory
along the study of capacity-achieving SC
codes [\cite{hassani2010coupled,kudekar2011threshold,yedla2014maxwell,
giurgiu2016,BDM_trans2017,DiaThesis}]
with other progress coming from developments in mathematical
physics of spin glass
theory [\cite{guerra2005introduction}].
%putting on a rigorous basis predictions of spin glass
%theory [\cite{guerra2005introduction}].
Moreover, our proof exploits the ``threshold saturation'' phenomenon of the AMP algorithm and uses spatial coupling as a proof technique. From this point of view, we believe that the
theorem proven in this paper is relevant in a broader context going
beyond low-rank matrix estimation and can be applied for a wide range of inference problems where message-passing algorithm and spatial coupling can be applied. Furthermore, our work provides important results on the exact formula for the MMSE and on the optimality of the AMP algorithm. 

Hundreds of papers have been
published in statistics, machine learning or information theory using
the non-rigorous statistical physics approach. We believe that our
result helps setting a rigorous foundation of a broad line of
work. While we focus on rank-one symmetric matrix estimation, our
proof technique is readily extendable to more generic low-rank
symmetric matrix or low-rank symmetric tensor estimation. We also
believe that it can be extended to other problems of interest in
machine learning and signal processing. It has already been extended to linear estimation and compressed sensing [\cite{BDMK_alerton2016,BMDK_trans2017}].

% , such as generalized linear
% regression, features/dictionary learning, compressed sensing or
% multi-layer neural networks [\cite{BDMK_alerton2016,BMDK_trans2017}].

We conclude this introduction by giving a few pointers to the recent literature  
on rigorous results.
For rank-one symmetric matrix estimation problems, AMP has been
introduced by [\cite{rangan2012iterative}], who also computed the
state evolution formula to analyze its performance, generalizing
techniques developed by [\cite{BayatiMontanari10}] and
[\cite{Montanari-Javanmard}]. State evolution was further studied by
[\cite{6875223}] and [\cite{deshpande2015asymptotic}]. In
[\cite{lesieur2015mmse,lesieur2015phase}], the generalization to
larger rank was also considered.
The mutual information was already computed in the special case when
$S_i\!=\!\pm 1\!\sim\! {\rm Ber}(1/2)$ in
[\cite{KoradaMacris}] where an equivalent spin glass model was analyzed.
The results of [\cite{KoradaMacris}] were first generalized in [\cite{krzakala2016mutual}] 
who, notably, obtained a generic matching upper
bound. The same formula was also rigorously computed following
the study of AMP in [\cite{6875223}] for spike models (provided,
however, that the signal was not {\it too} sparse) and in
[\cite{deshpande2015asymptotic}] for strictly symmetric community
detection. The general formula proposed by [\cite{lesieur2015mmse}] for the
conditional entropy and the MMSE on the basis of the heuristic cavity
method from statistical physics was first demonstrated in full
generality by the current authors in [\cite{barbierNIPS2016}]. 
This paper represents an extended version of [\cite{barbierNIPS2016}] that includes all the proofs and derivations along with more detailed discussions.
All preexisting proofs could not reach the more
interesting regime where a gap between the algorithmic and information
theoretic performances appears (i.e. in the presence of ``first order'' phase transition), leaving a gap with the statistical physics conjectured formula. Following the work of [\cite{barbierNIPS2016}], the replica formula for rank-one symmetric matrix estimation has been proven again several times using totally different techniques that involve the concentration's proof of the overlaps [\cite{lelarge2017,BM_stochastic2017}]. Our proof strategy does not require any concentration and it uses AMP and spatial coupling as proof techniques. Hence, our result has more practical implications in terms of proving the range of optimality of the AMP algorithm for both the underlying (uncoupled) and spatially coupled models.

This paper is organized as follows: the problem statement and the main results are given in Section \ref{sec:settings_results} along with a sketch of the proof, two applications for symmetric rank-one matrix estimation are presented in Section \ref{sec:examples}, the threshold saturation phenomenon and the relation between the underlying and spatially coupled models are proven in Section \ref{sec:thresh-sat} and Section \ref{sec:subadditivitystyle} respectively, the proof of the main results follows in Section \ref{sec:proof_theorem} and Section \ref{sec:proof_coro}.

A word about notations: in this paper, we use capital letters for random variables, and small 
letters for fixed realizations. Matrices and vectors are bold while scalars are not. 
Components of vectors or matrices are identified by the presence of lower indices.



==> v5 arxiv/sections/2_results.tex <==
\section{Setting and main results}\label{sec:settings_results}

\subsection{Basic underlying model}

A standard and natural setting is to consider an additive white gausian noise (AWGN) channel with variance $\Delta$ assumed to be known. The model reads
%
\begin{align} \label{eq:mainProblem}
w_{ij} = \frac{s_i s_j}{\sqrt{n}} + \sqrt{\Delta} z_{ij},
\end{align}
%
where ${\bf z} = (z_{ij})_{i,j=1}^n$ is a symmetric matrix with
$Z_{ij} \sim \mathcal{N}(0,1)$, $1\leq i\leq j\leq n$, and ${\bf s} = (s_i)_{i=1}^n$ has i.i.d components
$S_i\sim P_0$. We set $\mathbb{E}[S^2] = v$. Precise hypothesis on $P_0$ are given later.

Perhaps surprisingly, it turns out that the study of this Gaussian setting is 
sufficient to completely characterize all the problems discussed in the introduction, even 
if we are dealing with more complicated (noisy) observation models. This 
is made possible by a theorem of channel universality. Essentially, the theorem states that for any output channel $P_{\rm out}(w|y)$
such that at $y= 0$ the function $y\mapsto \log P_{\rm out}(w|y)$ is three times differentiable
with bounded second and third derivatives, then the
mutual information satisfies
%
\begin{equation}
  I(\tbf{S};\tbf{W}) = I (\tbf{S}\tbf{S}^{\intercal}; \tbf{S}\tbf{S}^{\intercal} + \sqrt{\Delta} \; \tbf{Z}) + O(\sqrt{n} ), 
\end{equation}
%
where $\Delta$ is the
inverse Fisher information (evaluated at $y = 0$) of the output
channel
%
\begin{equation}
  \Delta^{-1} \defeq \int dw P_{\rm out}(w|0) \left( \frac{\partial \log P_{\rm out}(w|y)}{\partial y}\Big|_{y=0}\right)^2\, . 
  \label{FisherInformation}
\end{equation}
This means that the mutual information per variable $ I(\tbf{S};\tbf{W})/n$ is asymptotically equal the mutual information per variable of an AWGN channel. Informally, it implies 
that we only have to compute the mutual
information for an ``effective'' Gaussian channel to take care of a wide range of
problems. The statement was conjectured in [\cite{lesieur2015mmse}] and can be proven by an 
application of the Lindeberg principle [\cite{deshpande2015asymptotic}], [\cite{krzakala2016mutual}].

\subsection{AMP algorithm and state evolution}\label{subsec:AMP_SE}

AMP has been applied for the rank-one symmetric matrix estimation problems by [\cite{rangan2012iterative}], who also computed the
state evolution formula to analyze its performance, generalizing
techniques developed by [\cite{BayatiMontanari10}] and
[\cite{Montanari-Javanmard}]. State evolution was further studied by
[\cite{6875223}] and [\cite{deshpande2015asymptotic}]. AMP is an iterative algorithm that provides an estimate $\hat{\bf s}^{(t)}(\bw)$, at each 
iteration $t \in \mathbb{N}$, of the vector $\bf s$. It turns out that tracking the asymptotic vector and matrix MSE of the AMP algorithm
%\begin{align}
%E^{(t)} = \lim_{n\to +\infty}\frac{1}{n}\| {\bf s} - \hat{\bf s}^{(t)} \|_2^2,
%\end{align}
is equivalent to running a simple recursion called {\it state evolution} (SE).  

The AMP algorithm reads
%
\begin{align}
\begin{cases}
\hat{s}_j^{(t)} = \eta_t((\bw \hat{\bs}^{(t-1)})_j - b^{(t-1)}\hat{\bs}^{(t-2)}_j), 
\\
b^{(t)}= \frac{1}{n}\sum_{i=1}^n \eta_t^\prime((\bw \hat{\bs}^{(t-1)})_i - b^{(t-1)}\hat{s}^{(t-2)}_i)
\end{cases}
\end{align}
%
for $j=1, \cdots, n$, where $\eta_t(y)$ is called the denoiser and $\eta_t^\prime(y)$ is the derivative w.r.t $y$.
The {\it denoiser} is the MMSE estimate associated to an ``equivalent scalar denoising problem''
%
\begin{align}\label{eq:scalarDen}
y = s + \Sigma(E) z,\qquad \Sigma(E)^{-2} \defeq \frac{v-E}{\Delta}\,.
\end{align}
%
with
$Z\sim \mathcal{N}(0,1)$ and
\begin{align}
 \eta(y) = \mathbb{E}[X|Y=y] = \frac{\int dx x P_0(x)e^{-\frac{(x - Y)^2}{2\Sigma(E)^{2}}}}{\int dx P_0(x)
e^{-\frac{(x - Y)^2}{2\Sigma(E)^{2}}}}\, ,
\end{align}
where $E$ is updated at each time instance $t$ according to the recursion \eqref{eq:state-evolution}.

Natural performance measures are the ``vector'' and ``matrix'' MSE's of the AMP estimator defined below.
%
\begin{definition}[Vector and matrix MSE of AMP]\label{def:mse_amp}
The vector and matrix MSE of the AMP estimator $\xhat{\bS}^{(t)}(\bW)$ at iteration $t$ are defined respectively  as follows
%
\begin{align}
{\rm Vmse}_{n, \rm AMP}^{(t)}(\Delta^{-1}) \defeq \frac{1}{n}\mathbb{E}_{\tbf{S}, \bW}\bigl[\| \xhat{\tbf{S}}^{(t)} - \tbf{S}\|_{2}^2\bigr],
\end{align}
\begin{align}
{\rm Mmse}_{n, \rm AMP}^{(t)}(\Delta^{-1}) \defeq \frac{1}{n^2}\mathbb{E}_{\tbf{S}, \bW}\bigl[\|\xhat{\tbf{S}}^{(t)} \xhat{\tbf{S}}^{{(t)}^\intercal} - \tbf{S} \tbf{S}^\intercal\|_{\rm F}^2\bigr],
\end{align}
%
where $\|A\|_{\rm F}^2 = \sum_{i,j} A_{ij}^2$ stands for the Frobenius norm of a matrix $A$.
\end{definition}
%

A remarkable fact that follows from a general theorem of [\cite{BayatiMontanari10}] (see [\cite{deshpande2015asymptotic}] for its use in the matrix case) is that the state evolution sequence tracks these two MSE's and thus allows to assess the performance of AMP. 
Consider the scalar denoising problem \eqref{eq:scalarDen}.
%\begin{align}
%y = s + \Sigma(E) z,\qquad \Sigma(E)^{-2} \defeq \frac{v-E}{\Delta}\, ,
%\end{align}
%with
%$Z\sim \mathcal{N}(0,1)$ and
%\begin{align}
%\mathbb{E}[X|Y=y] = \frac{\int dx x P_0(x)e^{-\frac{(x - y)^2}{2\Sigma(E)^{2}}}}{\int dx P_0(x)
%e^{-\frac{(x - y)^2}{2\Sigma(E)^{2}}}}\,.
%\end{align}
Hence, the (scalar) mmse function associated to this problem reads
%
\begin{align}\label{eq:SE_post}
 {\rm mmse}(\Sigma(E)^{-2}) \defeq \mathbb{E}_{S, Y}[(S - \mathbb{E}[X \vert Y])^2]\, .
\end{align}
%
The {\it state evolution sequence} $E^{(t)}$, $t\in \mathbb{N}$ is defined as 
%
\begin{align}\label{eq:state-evolution}
 E^{(t+1)} = {\rm mmse}(\Sigma(E^{(t)})^{-2}), \qquad E^{(0)} = v.
\end{align}
%
Since the ${\rm mmse}$ function is monotone decreasing (its argument has the dimension of a signal to noise ratio) it is easy to see that that $E^{(t)}$ is a decreasing non-negative sequence. Thus $\lim_{t\to +\infty} E^{(t)} \defeq E^{(\infty)}$ exists. 
One of the basic results of [\cite{BayatiMontanari10}], [\cite{deshpande2015asymptotic}] is 
%
\begin{align}\label{eq:mseampmatriciel}
\lim_{n\to +\infty} {\rm Vmse}_{n, \rm AMP}^{(t)}(\Delta^{-1}) = E^{(t)}, \quad {\rm and} \quad
\lim_{n\to +\infty} {\rm Mmse}_{n, \rm AMP}^{(t)}(\Delta^{-1}) = v^2 - (v- E^{(t)})^2.
\end{align}
%
We note that 
the results in [\cite{BayatiMontanari10}], [\cite{deshpande2015asymptotic}] are stronger in 
the sense that the non-averaged algorithmic mean square errors are tracked by state evolution with probability one.

Note that when $\mathbb{E}[S]=0$ then $v$ is an unstable fixed point, and as such, state evolution ``does not start'', 
in other words we have $E^{(t)} =v$. While this is not really a problem when one runs AMP in practice, for analysis 
purposes one can circumvent this problem by slightly biasing $P_0$ and remove the bias at the end of the analysis. For simplicity, we always assume that $P_0$ is biased so that $\mathbb{E}[S]$ is not zero.

{\bf Assumption 1:} 
In this work we assume that $P_0$ is discrete with bounded support. Moreover, we assume that $P_0$ is biased such that 
$\mathbb{E}[S]$ is non-zero.


A fundamental quantity computed by state evolution is the algorithmic threshold.
\begin{definition}[AMP threshold]\label{amp-thresh}
For $\Delta>0$ small enough, the fixed point equation corresponding to \eqref{eq:state-evolution} has a unique solution for all noise values in $]0, \Delta[$. We define $\Delta_{\rm AMP}$ as the supremum of all such $\Delta$.
\end{definition}
%

\subsection{Spatially coupled model}\label{subsec:SC}

The present spatially coupled construction is similar to the
one used for the coupled Curie-Weiss model [\cite{hassani2010coupled}] and is also similar to mean field spin glass systems 
introduced in [\cite{FranzToninelli,SilvioFranz}]. We consider a chain (or a ring) of underlying systems positioned at
$\mu\!\in\! \{0,\dots, L\}$ and coupled to neighboring blocks
$\{\mu\! -\! w, \dots, \mu\! +\!w\}$. Positions $\mu$ are taken modulo $L\!+\!1$ and the integer $w\!\in\!\{0,\ldots,L/2\}$ equals the size of the {\it coupling window}. The coupled model is
%
\begin{align} \label{eq:def_coupledSyst}
w_{i_\mu j_\nu} = s_{i_\mu} s_{j_\nu}\sqrt{\frac{\Lambda_{\mu\nu}}{n}} + z_{i_\mu j_\nu}\sqrt{\Delta} ,
\end{align}
%
where the index $i_\mu \!\in\! \{1, \dots, n\}$ (resp. $j_\nu$) belongs to the block $\mu$ (resp. $\nu$) along the ring, $\mathbf{\Lambda}$ is an $(L\!+\!1)\!\times\! (L\!+\!1)$ matrix which describes the strength of the coupling between blocks, and $Z_{i_\mu j_\nu}\!\sim \!\mathcal{N}(0,1)$ are i.i.d. For the analysis to work, the matrix elements have to be chosen appropriately. We assume that: 
%
\begin{itemize}
\item[i)] $\mathbf{\Lambda}$ is a doubly stochastic matrix; 
\item[ii)] $\Lambda_{\mu\nu}$ depends on
$\vert \mu \!- \!\nu\vert$; 
\item[iii)] $\Lambda_{\mu\nu}$ is not vanishing for $\vert \mu \!-\!\nu| \leq w$ and vanishes for $\vert \mu \!-\!\nu|\! > \!w$; 
\item[iv)] $\mathbf{\Lambda}$ is {\it smooth} in the sense $\vert \Lambda_{\mu\nu}\! -\! \Lambda_{\mu+1 \nu} \vert\! =\! \mathcal{O}(w^{-2})$ and $\Lambda^{*}\defeq\sup_{\mu, \nu}\Lambda_{\mu\nu} = \mathcal{O}(w^{-1})$; 
\item[v)] $\mathbf{\Lambda}$ has a non-negative Fourier transform. 
\end{itemize}
%
All these conditions can easily be met, the simplest example being a triangle of base $2w\!+\!1$ and height $1/(w\!+\!1)$, more precisely:
\begin{align}\label{triangle}
\Lambda_{\mu\nu} = 
\begin{cases}
\frac{1}{w+1}\biggl(1 - \frac{\vert\mu - \nu\vert}{w+1}\biggr), \qquad \vert\mu-\nu\vert \leq w\\
0, \qquad \vert\mu-\nu\vert > w
\end{cases}
\end{align}
%Note that these conditions imply that the matrix elements, including the largest value $\Lambda^* \defeq {\rm max}\, \Lambda_{\mu, \nu}$, are all $=\mathcal{O}(w^{-2})$. ?????????????? I dont understand this statement and have commented it.
We will always denote by $\mathcal{S}_\mu \defeq \{\nu \,|\, \Lambda_{\mu\nu} \neq 0 \}$ the set of $2w+1$ blocks coupled to block $\mu$.

The construction of the coupled system is completed by introducing a {\it seed} in the ring: we assume 
perfect knowledge of the signal components $\{s_{i_\mu}\}$ for $\mu\! \in \!\mathcal{B}\!\defeq \!\{-w\!-\!1, \dots, w\!-\!1\} \mod L\!+\!1$. 
This seed is what allows to close the gap between the algorithmic and information theoretic limits and therefore plays a crucial role. 
We sometimes refer to the seed as the {\it pinning construction}. 
Note that the seed can also be viewed as an ``opening'' of the chain with fixed boundary conditions.   

AMP has been applied for the rank-one symmetric matrix estimation problems by [\cite{rangan2012iterative}], who also computed the
state evolution formula to analyze its performance, generalizing
techniques developed by [\cite{BayatiMontanari10}] and
[\cite{Montanari-Javanmard}]. State evolution was further studied by
[\cite{6875223}] and [\cite{deshpande2015asymptotic}].

The AMP algorithm and the state evolution recursion [\cite{6875223,deshpande2015asymptotic}] can be easily adapted to the spatially coupled model as done in Section \ref{sec:thresh-sat}. The proof that the state evolution for the symmetric rank-one matrix estimation problem tracks the AMP on a spatially coupled model is an extension of the analysis done in [\cite{6875223,deshpande2015asymptotic}] for the uncoupled model.
%This follows the same lines of [\cite{Montanari-Javanmard}], who provided a rigorous spatially coupled state evolution for the compressed sensing problem [\cite{BayatiMontanari10}].
The full re-derivation of such result would be lengthy and beyond the scope of our analysis. We thus assume that state evolution tracks the AMP performance for our coupled problem. However, we believe that the proof will be similar to the one done for the spatially coupled compressed sensing problem [\cite{Montanari-Javanmard}]. This assumption is vindicated numerically.
%and we strongly believe this claim which is supported by numerical simulations.

{\bf Assumption 2:} We consider the spatially coupled model \eqref{eq:def_coupledSyst} with $P_0$ satisfying Assumption 1. We assume that state evolution tracks the AMP algorithm for this model.

\subsection{Main results: basic underlying model}\label{subsec:results}

One of our central results is a proof of the expression for the asymptotic mutual information per variable via the so-called {\em replica symmetric (RS) potential}. This is the function $E\in [0, v] \mapsto i_{\rm RS}(E; \Delta)\in \mathbb{R}$ defined as
%
\begin{align}\label{eq:potentialfunction}
i_{\rm RS}(E;\Delta) \defeq \frac{(v-E)^2+v^2}{4\Delta} - \mathbb{E}_{S, Z}\biggl[\ln\biggl(\int dx\,P_0(x)
e^{-\frac{x^2}{2\Sigma(E)^{2}} 
+ x\bigl(\frac{S}{\Sigma(E)^{2}} + \frac{Z}{\Sigma(E)}\bigr)}\biggr)\biggr] \, ,
\end{align}
%
with $Z\!\sim\! \mathcal{N}(0,1)$, $S\!\sim\! P_0$. 
%%
%We will see 
%in Section~\ref{subsec:results} that
%$\Sigma(E)^2$ can be interpreted as the variance of an effective 
%scalar AWGN channel and $E$ the associated MSE.
Most of our results will assume that $P_0$ is a discrete distribution over 
a finite bounded real alphabet $P_0(s) \!=\! \sum_{\alpha=1}^\nu p_\alpha \delta(s\! - \! a_\alpha)$ (see Assumption 1). 
Thus the only continuous integral in \eqref{eq:potentialfunction} is the Gaussian over $Z$. The extension to mixtures of continuous and discrete signals 
can be obtained by approximation methods not discussed in this paper (see e.g. the methods in [\cite{lelarge2017}]).

It turns out that both the information theoretic and algorithmic AMP thresholds are determined by the set of stationary points of \eqref{eq:potentialfunction} (w.r.t $E$).
It is possible to show that for all $\Delta > 0$ there always exist at 
least one stationary minimum.\footnote{
Note $E\!=\!0$ is never a stationary 
point (except for the trivial case of $P_0$ a single Dirac mass which we exclude from the discussion) and $E = v$ is stationary only if $\mathbb{E}[S] = 0$.} 
In this contribution 
we suppose that at most three stationary points exist, corresponding to situations with at most one phase transition as depicted in  Fig. \ref{fig:I-AMP} (see Assumption 3 below). 
Situations 
with multiple transitions could also be covered by our techniques.

{\bf Assumption 3:} 
We assume that $P_0$ is such that there exist at most three stationary points for the potential \eqref{eq:potentialfunction}.

To summarize, our main assumptions in this paper are:

\begin{enumerate}[label=(A\arabic*),noitemsep]
	\item The prior $P_0$ is discrete with bounded support. Moreover, we assume that $P_0$ is biased such that $\mathbb{E}[S]$ is non-zero. \label{ass:h1}
	\item We consider the spatially coupled model \eqref{eq:def_coupledSyst} with $P_0$ satisfying Assumption \ref{ass:h1}. We assume that state evolution tracks the AMP algorithm for this model. \label{ass:h2}
	\item  We assume that $P_0$ is such that there exist at most three stationary points for the potential \eqref{eq:potentialfunction}. \label{ass:h3}
\end{enumerate}

\begin{remark}
An important property of the replica symmetric potential is that the stationary points satisfy the state evolution fixed point equation. In other words 
$\partial i_{\rm RS}/\partial E = 0$ implies $E= {\rm mmse}(\Sigma(E)^{-2})$ and conversely. Moreover it is not difficult to see that the 
$\Delta_{\rm AMP}$ is given by the smallest solution of 
$\partial i_{\rm RS}/\partial E\!=\! \partial^2 i_{\rm RS}/\partial E^2 \!=\! 0$.
In other words the AMP threshold is the ``first'' horizontal inflexion point appearing in $i_{\rm RS}(E;\Delta)$ when $\Delta$ increases
from $0$ to $+\infty$.
\end{remark}

One of the main results of this paper is formulated in the following theorem which provides a proof of the conjectured single-letter formula for the asymptotic mutual information per variable.
%in terms of the RS potential \eqref{eq:potentialfunction}.
%
\begin{theorem}[RS formula for the mutual information]\label{thm1}
Fix $\Delta > 0$ and let $P_0$ satisfy Assumptions \ref{ass:h1}-\ref{ass:h3}. Then 
\begin{align}\label{rsform}
 \lim_{n\to \infty} \frac{1}{n}I(\tbf{S} ; \tbf{W}) = \min_{E\in [0, v]}i_{\rm RS}(E;\Delta).
\end{align}
\end{theorem}
%
\begin{proof}
See Section \ref{sec:proof_theorem}.
\end{proof}
The proof of the {\it existence of the limit} does not require the above hypothesis on $P_0$. Also, it was first shown
in [\cite{krzakala2016mutual}] that  
%
\begin{align}\label{eq:guerrabound}
\limsup_{n\to +\infty} \frac{1}{n}I(\tbf{S}; \tbf{W}) \leq \min_{E\in [0, v]}i_{\rm RS}(E;\Delta),
\end{align}
%
an inequality that {\it we will use} in the proof section. 
Note that, interestingly, and perhaps surprisingly, the analysis of [\cite{krzakala2016mutual}] leads to a sharp upper bound on the ``free energy'' for all finite $n$. We will make extensive use of this inequality
and for sake of completeness, we summarize its proof in Appendix~\ref{app:upperBound}. 

%Combining 
%\eqref{eq:guerrabound} with other interpolation ideas borrowed from [\cite{KoradaMacris}], the authors of [\cite{krzakala2016mutual}] where able to 
%show Theorem~\ref{thm1} for the present problem (and another one) for specific noise regimes. These previous works left open the 
%case where a discontinuous first order phase transition is present. Closing this gap is not only a ``technicality" but requires the use of new ideas.
%In the present paper we detail our recent proof technique (sketched in [\cite{NIPS}]) based on an interplay of algorithmic ideas, spatially coupled models and interpolation methods.
%Even more recently purely non-algorithmic proofs have appeared based on rigorous versions of the cavity method [\cite{Leoetal}] and on the so-called ''stochastic interpolation method''
%[\cite{Jean-Nicolas}], [\cite{Jean-Nicolas-Leo-Allerton}].

Theorem \ref{thm1} allows to compute the information theoretic phase transition threshold which we define in the following way.
%
\begin{definition}[Information theoretic or optimal threshold]\label{def-delta-opt} 
Define $\Delta_{\rm opt}$ as the first non-analyticity point of the mutual information as $\Delta$ 
increases. Formally
\begin{align}
 \Delta_{\rm opt} \defeq \sup\{\Delta\vert\lim_{n\to \infty}\frac{1}{n}I(\tbf{S}; \tbf{W}) \ \text{is analytic in} \ ]0, \Delta[\}.
\end{align}
\end{definition}
%
The information theoretic threshold is also called ``optimal threshold" because we expect $\Delta_{\rm AMP} \leq \Delta_{\rm opt}$. This is indeed proven in Lemma \ref{suboptimality}. 

When $P_0$ is s.t \eqref{eq:potentialfunction} has at most three stationary points, then $\min_{E\in [0, v]} i_{\rm RS}(E;\Delta)$ has at most one {\it non-analyticity} point 
denoted $\Delta_{\rm RS}$ (see Fig. \ref{fig:I-AMP}). In case of analyticity over all $\mathbb{R}_+$, we set $\Delta_{\rm RS} \!=\!\infty$. We call $\Delta_{\rm RS}$ the RS or potential threshold. 
Theorem~\ref{thm1} gives us a mean to concretely {\it compute} the information theoretic threshold: $\Delta_{\rm opt} \!=\! \Delta_{\rm RS}$.

%
\begin{figure}[!t]
\centering
\includegraphics[width=1\textwidth]{figs/MUTUAL_INFORMATION_1.pdf}
\vspace*{-18pt}
\caption{The replica symmetric potential $i_{\rm RS}(E)$ for four values of $\Delta$ in the spiked Wigner model with $S_i \sim {\rm Ber}(\rho)$. The normalized mutual information is $\min i_{\rm RS}(E)$ (the black dot, while the black cross corresponds to the local minimum) and the asymptotic MMSE is ${\rm argmin} i_{\rm RS}(E)$, where $v\!=\!\rho$ in this case with $\rho\!=\!0.02$. From top left to bottom right: $i)$ For low noise values, here $\Delta\!=\!0.0008\!<\!\Delta_{\rm AMP}$, there exists a unique ``good'' minimum corresponding to the MMSE and AMP is Bayes optimal. $ii)$ As the noise increases, a second local ``bad'' minimum appears: this is the situation at $\Delta_{\rm AMP}\!<\!\Delta\!=\!0.0012\!<\!\Delta_{\rm RS}$. $iii)$ For $\Delta\!=\!0.00125\!>\!\Delta_{\rm RS}$, the ``bad'' minimum becomes the global one and the MMSE suddenly deteriorates. $iv)$ For larger values of $\Delta$, only the ``bad'' minimum exists. AMP can be seen as a naive minimizer of this curve starting from $E\!=\!v\!=\!0.02$. AMP can reach the global minimum in situations $i)$, $iii)$ and $iv)$. However, in situation $ii)$, when $\Delta_{\rm AMP}\!<\!\Delta\!<\!\Delta_{\rm RS}$, AMP is trapped by the local minimum with large MSE instead of reaching the global one corresponding to the MMSE.}\label{fig:I-AMP}
\end{figure}
%

From Theorem  \ref{thm1} we will also deduce the expressions for the \emph{vector} MMSE and the \emph{matrix} MMSE defined below.
%
\begin{definition}[Vector and matrix MMSE]\label{def:mmse}
The vector and matrix MMSE are defined respectively as follows
%
\begin{align}\label{eq:Vmmse}
 {\rm Vmmse}_n(\Delta^{-1}) \defeq \frac{1}{n}\mathbb{E}_{\tbf{S}, \tbf{W}}\Big[ \bigl\| \tbf{S} - 
 \mathbb{E}[\tbf{X}\vert\tbf{W}]\bigr\|_{2}^2 \Big].
\end{align}
%
%
\begin{align}\label{eq:Mmmse}
 {\rm Mmmse}_n(\Delta^{-1}) \defeq \frac{1}{n^2}\mathbb{E}_{\tbf{S}, \tbf{W}}\Big[ \bigl\| \tbf{S}\tbf{S}^{\intercal} - 
 \mathbb{E}[\tbf{X}\tbf{X}^{\intercal}\vert\tbf{W}]\bigr\|_{\rm F}^2 \Big].
\end{align}
%
\end{definition}
%
The conditional expectation $\mathbb{E}[\,\cdot\,\vert\tbf{W}]$ in Definition \ref{def:mmse} is w.r.t the posterior distribution
%
\begin{align}\label{eq:posterior_dist}
 P(\tbf{x}\vert \tbf{w}) = \frac{1}{\tilde{\mathcal{Z}}(\tbf{w})}e^{-\frac{1}{2\Delta}\sum_{i\leq j}\big(\frac{x_i x_j}{\sqrt n} - w_{ij}\big)^2}\prod_{i=1}^n P_0(x_i),
\end{align}
%
with the normalizing factor depending on the observation given by 
%
\begin{align}
\tilde{\mathcal{Z}}(\tbf{w}) = \int \big\{\prod_{i=1}^n dx_i P_0(x_i)\big\} e^{-\frac{1}{2\Delta}\sum_{i\leq j}\big(\frac{x_i x_j}{\sqrt n} - w_{ij}\big)^2}
\end{align}
%
The expectation $\mathbb{E}_{\tbf{S}, \tbf{W}}[\,\cdot\,]$ is the one w.r.t $P({\bf w})P({\bf s})=\tilde{\mathcal{Z}}(\tbf{w})\prod_{i=1}^{n} P_0(s_i)$. The expressions for the MMSE's in terms of \eqref{eq:potentialfunction} are given in the following corollary.
%
%Once we have the result of Theorem \ref{thm1}, explicit expressions for the MMSE's can be obtained 
%through the I-MMSE relation [\cite{GuoShamaiVerdu}] adapted to this case (see Lemma \ref{lemma:immse}).
%
\begin{corollary}[Exact formula for the MMSE]\label{cor:MMSE}
For all $\Delta\neq \Delta_{\rm RS}$, the 
matrix MMSE  
is asymptotically 
\begin{align}\label{coro1}
\lim_{n\to\infty} {\rm Mmmse}_n(\Delta^{-1}) = v^2-(v-{\rm argmin}_{E\in[0,v]} i_{\rm RS}(E;\Delta))^2.
\end{align}
Moreover, if $\Delta \!<\!\Delta_{\rm AMP}$ or $\Delta\! >\! \Delta_{\rm RS}$, then 
the usual vector MMSE
satisfies 
\begin{align}\label{coro2}
\lim_{n\to \infty}{\rm Vmmse}_n(\Delta^{-1}) = {\rm argmin}_{E\in[0,v]} i_{\rm RS}(E;\Delta).
\end{align}
\end{corollary}
%
\begin{proof}
See Section \ref{sec:proof_coro}.
\end{proof}
It is natural to conjecture that the vector MMSE is given by ${\rm argmin}_{E\in[0,v]} i_{\rm RS}(E;\Delta)$ in the {\it whole} range $\Delta \neq \Delta_{\rm RS}$, but our proof does not quite yield the full statement. 

Another fundamental consequence of Theorem \ref{thm1} concerns the optimality of the performance of AMP. 

\begin{corollary}[Optimality of AMP]\label{perfamp}
For $\Delta <\Delta_{\rm AMP}$ or $\Delta > \Delta_{\rm RS}$, the AMP is asymptotically optimal in the sense that it yields upon convergence the asymptotic vector-MMSE and matrix-MMSE 
of Corollary \ref{cor:MMSE}. Namely, 
%
\begin{align}
\lim_{t\to +\infty}\lim_{n\to +\infty} {\rm Mmse}_{n, \rm AMP}^{(t)}(\Delta^{-1})
&= \lim_{n\to\infty} {\rm Mmmse}_n(\Delta^{-1}).
\label{ampcoro1}
\\
\lim_{t\to +\infty}\lim_{n\to +\infty} {\rm Vmse}_{n, \rm AMP}^{(t)}(\Delta^{-1}) & = \lim_{n\to \infty}{\rm Vmmse}_n(\Delta^{-1}).
\label{ampcoro2}
\end{align}
On the other hand, for $\Delta_{\rm AMP}<\Delta < \Delta_{\rm RS}$ the AMP algorithm is strictly suboptimal, namely 
%
\begin{align}
\lim_{t\to +\infty}\lim_{n\to +\infty} {\rm Mmse}_{n, \rm AMP}^{(t)}(\Delta^{-1})
& > \lim_{n\to\infty} {\rm Mmmse}_n(\Delta^{-1}).
\label{ampsub1}
\\
\lim_{t\to +\infty}\lim_{n\to +\infty} {\rm Vmse}_{n, \rm AMP}^{(t)}(\Delta^{-1}) & > \lim_{n\to \infty}{\rm Vmmse}_n(\Delta^{-1}).
\label{ampsub2}
\end{align}
%
\end{corollary}
%
\begin{proof}
See Section \ref{sec:proof_coro}.
\end{proof}
%

This leaves the region $\Delta_{\rm AMP} < \Delta < \Delta_{\rm RS}$
algorithmically open for efficient polynomial time algorithms. A
natural conjecture, backed up by many results in spin glass theory,
coding theory, planted models and the planted clique problems,
is:
%
\begin{conjecture}
  For $\Delta_{\rm AMP} < \Delta < \Delta_{\rm RS}$, no polynomial time efficient algorithm that outperforms AMP exists.
\end{conjecture}

\subsection{Main results: coupled model}\label{subsec:coupled-results}

In this work, the spatially coupled construction is used for the purposes of the proof. 
However, one can also imagine interesting applications of the spatially coupled estimation problem, specially in view of the fact that
AMP turns out to be optimal for the spatially coupled system.
%(indeed the proof outlined above also shows $\Delta_{\rm AMP, coup} = \Delta_{\rm opt, coup} = \Delta_{\rm opt} =\Delta_{\rm RS}$). 
In coding theory for example, the use of spatially coupled systems as a proof device historically followed their
initial construction which was for engineering purposes and led to the construction of capacity achieving codes.

Our first crucial result states that the mutual information of the coupled and original systems are the same
in a suitable limit. The mutual information of the coupled system of length $L$ and with coupling window $w$ is denoted 
$I_{w, L}(\tbf{S}; \tbf{W})$.

\begin{theorem}[Equality of mutual informations]\label{LemmaGuerraSubadditivityStyle}
For any fixed $w$ s.t. $P_0$ satisfies Assumption \ref{ass:h1}, the following limits exist and are equal
\begin{align}
\lim_{L\to \infty}\lim_{n\to \infty} \frac{1}{n(L+1)}I_{w, L}(\tbf{S}; \tbf{W}) = \lim_{n\to \infty} \frac{1}{n}I(\tbf{S}; \tbf{W}).
\end{align}
\end{theorem}
\begin{proof}
See Section \ref{sec:subadditivitystyle}.
\end{proof}
An immediate corollary is that the non-analyticity points (w.r.t $\Delta$) of the mutual informations
are the same in the coupled and underlying models.
In particular, defining 
$\Delta^{\rm c}_{\rm opt}\! \defeq \!
\sup\{\Delta\mid \lim_{L\to \infty}\lim_{n\to \infty} I_{w, L}(\tbf{S}; \tbf{W})/(n(L\!+\!1)) \ \text{is analytic in}\ ]0, \Delta[\}$,
we have 
$\Delta^{\rm c}_{\rm opt} \!= \!\Delta_{{\rm opt}}$.

The second crucial result states that the AMP threshold of the spatially coupled system is at least as good as $\Delta_{\rm RS}$ (threshold saturation result of Theorem \ref{thres-sat-lemma}). The analysis of
AMP applies to the coupled system as well
[\cite{BayatiMontanari10,Montanari-Javanmard}] and it can be shown that
the performance of AMP is assessed by SE. Let 
\begin{align}
E_{\mu}^{(t)} \!\defeq\!\lim_{n\to\infty}\frac{1}{n}\mathbb{E}_{{\tbf S}, {\tbf Z}}[\|{\tbf S}_{\mu} \!-\! \hat{\tbf S}_{\mu}^{(t)}\|_2^2]
\end{align}
 be the asymptotic average vector-MSE of the AMP estimate
$\hat{\tbf{S}}_\mu^{(t)}$ at time $t$ for the $\mu$-th ``block'' of ${\tbf S}$. We associate to each position $\mu\!\in\! \{0, \ldots, L\}$ an \emph{independent} scalar system with AWGN of the form $y\!=\!s\!+\!\Sigma_\mu({\tbf E}; \Delta)z$, with 
\begin{align}
\Sigma_\mu({\tbf E})^{-2} \defeq \frac{v\!-\! \sum_{\nu=0}^L\Lambda_{\mu\nu} E_\nu}{\Delta}
\end{align}
and $S\!\sim\! P_0$, $Z\!\sim \!\mathcal{N}(0,1)$. Taking into account knowledge of the signal components in the seed 
$\mathcal{B}$, SE reads
\begin{align}\label{coupled-state-evolution}
\begin{cases}
 E_{\mu}^{(t+1)} = {\rm mmse}(\Sigma_\mu({\tbf E}^{(t)}; \Delta)^{-2}), ~ E_\mu^{(0)} = v ~\text{for}~ \mu\in \{0,\ldots, L\}\setminus\mathcal{B}, 
 \\
 E_\mu^{(t)} = 0 ~\text{for}~ \mu\in \mathcal{B}, t\geq 0
 \end{cases}
\end{align}
where the mmse function is defined as in \eqref{eq:SE_post}. 

From the monotonicity of the mmse function we have 
 $E_\mu^{(t+1)} \leq E_\mu^{(t)}$ for all $\mu \in \{0, \ldots, L\}$, a partial order 
 which implies that $\lim_{t\to\infty} {\tbf E}^{(t)} = {\tbf E}^{(\infty)}$ exists. 
 This allows to define an algorithmic threshold for the coupled system on a finite chain:
$$
\Delta_{{\rm AMP}, w,L} \defeq \sup\{\Delta|E^{(\infty)}_\mu\!\le\! E_{\rm good}(\Delta) \ \forall \ \mu\}
$$
where $E_{\rm good}(\Delta)$ is the trivial fixed point solution of the SE starting with the initial condition $E^{(0)} = 0$. A more formal but equivalent definition of $\Delta_{{\rm AMP}, w,L}$ is given in Section \ref{sec:thresh-sat}. 

\begin{theorem}[Threshold saturation]\label{thres-sat-lemma} 
Let $\Delta^{\rm c}_{\rm AMP}$ be the algorithmic threshold on an infinite chain, $\Delta^{\rm c}_{\rm AMP} \!\defeq \!\liminf_{w\to \infty}\liminf_{L\to \infty} \Delta_{{\rm AMP}, w, L}$, s.t. $P_0$ satisfies Assumptions \ref{ass:h1} and \ref{ass:h2}.
%be the AMP threshold of the spatially coupled ensemble (see Definition \ref{def:AMPcoupled}).
We have $\Delta^{\rm c}_{\rm AMP} \!\geq \!\Delta_{\rm RS}$. 
\end{theorem}
\begin{proof}
See Section \ref{sec:thresh-sat}.
\end{proof}
Our techniques also allow to prove the equality $\Delta^{\rm c}_{\rm AMP} = \Delta_{\rm RS}$, but this is not directly needed.

\subsection{Road map of the proof of the replica symmetric formula}

Here we give a road map of the proof of Theorem \ref{thm1} that will occupy Sections \ref{sec:thresh-sat}--\ref{sec:proof_theorem}. A fruitful idea is to concentrate on the question whether $\Delta_{\rm opt} = \Delta_{\rm RS}$. The proof of this 
equality automatically generates the proof of Theorem \ref{thm1}. 
%The proof of Corollary \ref{cor:MMSE} and Corollary \ref{perfamp} follows in Section \ref{sec:proof_coro}.

We first prove in Section \ref{sec:delta-less-delta-opt} that $\Delta_{\rm opt}\leq \Delta_{\rm RS}$. This proof is based on a joint use of the I-MMSE relation (Lemma \ref{lemma:immse}), the replica bound \eqref{eq:guerrabound} and the suboptimality of the AMP algorithm. 
In the process of proving $\Delta_{\rm opt}\leq \Delta_{\rm RS}$, we in fact get as a direct bonus the proof of Theorem \ref{thm1} for $\Delta < \Delta_{\rm opt}$.  

The proof of $\Delta_{\rm opt}\geq \Delta_{\rm RS}$ requires the use of spatial coupling. The main strategy is to show
\begin{align}\label{eq:chain_delta}
\Delta_{\rm RS} \le \Delta^{\rm c}_{\rm AMP} \leq \Delta^{\rm c}_{\rm opt} = \Delta_{\rm opt}.
\end{align}
The first inequality in \eqref{eq:chain_delta} is proven in Section \ref{sec:thresh-sat} using methods first invented in coding theory: The algorithmic AMP
threshold of the spatially coupled system $\Delta^{\rm c}_{\rm AMP}$ saturates (tends in a suitable limit) towards $\Delta_{\rm RS}$, i.e. 
$ \Delta_{\rm RS} \le \Delta^{\rm c}_{\rm AMP}$ (Theorem \ref{thres-sat-lemma}). 
To prove the (last) equality we show in Section \ref{sec:subadditivitystyle} that the free energies, and hence the mutual informations, of the underlying and spatially coupled systems are equal in a suitable asymptotic limit (Theorem \ref{LemmaGuerraSubadditivityStyle}). This implies that their non-analyticities occur at the same 
point and hence $\Delta^{\rm c}_{\rm opt} = \Delta_{\rm opt}$. This is done through an interpolation which, although similar in spirit, is different than the one used 
to prove replica bounds (e.g. \eqref{eq:guerrabound}). In the process of showing 
$\Delta^{\rm c}_{\rm opt} = \Delta_{\rm opt}$, we will also derive the existence of the limit for $I(\tbf{S}; {\tbf W})/n$.
Finally, the second inequality is due the suboptimality of the AMP algorithm. This follows by a direct extension of the SE analysis of [\cite{6875223,deshpande2015asymptotic}] to the spatially coupled case as done in [\cite{Montanari-Javanmard}]. 

Once $\Delta_{\rm opt} = \Delta_{\rm RS}$ is established it is easy to put everything together 
and conclude the proof of Theorem \ref{thm1}. In fact all that remains is to prove Theorem \ref{thm1} for $\Delta >\Delta_{\rm opt}$.
This follows by an easy argument in section \ref{sec:everything-together} which combines  $\Delta_{\rm opt} = \Delta_{\rm RS}$, the replica bound \eqref{eq:guerrabound} and the suboptimality of the AMP algorithm. Note that in the proof sections that follow, we assume that Assumptions \ref{ass:h1}-\ref{ass:h3} hold.

\subsection{Connection with the planted Sherrington-Kirkpatrick spin glass model} 

Let us briefly discuss the connection of the matrix factorization problem \eqref{eq:mainProblem} with a statistical mechanical spin glass model which is a variant of the classic Sherrington-Kirkpatrick (SK) model. This is also the occasion to express the mutual information as a ``free energy" through a simple relation that will be used in various guises later on. 

Replacing $w_{ij} = n^{-1/2}s_is_j + \sqrt{\Delta} z_{ij}$ in \eqref{eq:posterior_dist} and simplifying the fraction after expanding the squares, the posterior distribution can be expressed in terms of $\bs, \bz$ as follows
\begin{align}\label{gibbsi}
P(\bx \vert \bs, \bz) = \frac{1}{\mathcal{Z}} e^{-\mathcal{H}(\bx\vert \bs, \bz)} \prod_{i=1}^n P_0(x_i),
\end{align}
where 
\begin{align}\label{hami}
\mathcal{H}(\bx\vert \bs, \bz) = \sum_{i\leq j=1}^n \Big(\frac{x_i^2 x_j^2}{2n\Delta} - \frac{s_i s_j x_i x_j}{n\Delta} - \frac{z_{ij} x_ix_j}{\sqrt{n \Delta}}\Big)
\end{align}
and 
\begin{align}\label{parti}
\mathcal{Z} = \int \Big\{\prod_{i=1}^n dx_i P_0(x_i)\Big\} e^{-\mathcal{H}(\bx\vert \bs, \bz)}.
\end{align}
In the language of statistical mechanics, \eqref{hami} is the ``Hamiltonian", \eqref{parti} the ``partition function", and \eqref{gibbsi} is the Gibbs distribution.
This distribution is random since it depends on the realizations of $\bS$, $\bZ$. Conditional expectations with respect to \eqref{gibbsi}
are denoted by the Gibbs ``bracket" $\langle - \rangle$. More precisely
\begin{align}
\mathbb{E}_{\bX\vert \bS, \bZ}\big[A(\bX) \vert \bS= \bs, \bZ=\bz\big] = \langle A(\bX) \rangle.
\end{align}
The free energy is defined as 
\begin{align}
f_n = -\frac{1}{n} \mathbb{E}_{\bS, \bZ}[ \ln \mathcal{Z}].
\end{align}
Notice the difference between $\tilde{\mathcal{Z}}$ in \eqref{eq:posterior_dist} and $\mathcal{Z}$ in \eqref{gibbsi}. The former is the partition function with a complete square, whereas the latter is the partition function that we obtain after expanding the square and simplifying the posterior distribution. 


In Appendix \ref{app:freeEnergy}, we show that mutual information and free energy are essentially the same object up to a trivial term. For the present model
\begin{align}\label{eq:energy_MI}
\frac{1}{n} I(\tbf{S}; \bW) = -\frac{1}{n} \mathbb{E}_{\bS, \bZ}[ \ln \mathcal{Z}] + \frac{v^2}{4\Delta} + \frac{1}{4 \Delta n} (2\mathbb{E}[S^4] - v^2),
\end{align}
where recall $v = \mathbb{E}[S^2]$. This relationship turns out to be very practical and will be used several times.

For binary signals we have $s_i$ and $ x_i\in \{-1, +1\}$, so the model is a binary spin glass model. The first term in the Hamiltonian is a trivial constant,  the last term corresponds exactly to the SK model with random Gaussian interactions, and the second term can be interpreted as an external random field that biases the spins. This is sometimes called a ``planted" SK model.

The rest of the paper is organized as follows.
In Section \ref{sec:examples} we provide two examples of the symmetric rank-one matrix estimation problem. %The spatially coupled system is defined in Section \ref{subsec:scsystem}.
Threshold saturation and the invariance of the mutual information due the spatial coupling are shown in Section \ref{sec:thresh-sat} and \ref{sec:subadditivitystyle} respectively. The proof of Theorem \ref{thm1} follows in Section \ref{sec:proof_theorem}. Section \ref{sec:proof_coro} is dedicated to the proof of Corollary \ref{cor:MMSE} and Corollary \ref{perfamp}.

%%%%%%%%%%%%%%%%%%%%KEEP FOR THE MOMENT%%%%%%%%%%%%%%%%%%%%%

% here

% In this paper we prove, for a large
% class of signal distributions $P_0$, an explicit single-letter formula for the mutual information 
% per variable $I(\tbf{S}; \tbf{W})/n$ 
%   in the
% asymptotic limit $n\to +\infty$ of the AWGN case. This expression was already conjectured to be true in
% [\cite{lesieur2015mmse}] where the authors used the replica and cavity 
% methods of statistical physics for its derivation. Informally the result states that
% \begin{align}\label{eq:RSformula}
%  \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^{\intercal};\tbf{W})  = \min_{E\in [0, v]} i_{\rm RS}(E; \Delta),
% \end{align}
% %
% where $i_{RS}(E; \Delta)$ is called the {\em replica symmetric (RS) potential function}
% %
% \begin{align}\label{eq:potentialfunction}
% i_{\rm RS}(E;\Delta) \defeq \frac{(v-E)^2+v^2}{4\Delta} - \mathbb{E}_{S, Z}\Big[\ln\Big(\int dx\,P_0(x)
% e^{-\frac{x^2}{2\Sigma(E,\Delta)^{2}} 
% + x\bigl(\frac{S}{\Sigma(E,\Delta)^{2}} + \frac{Z}{\Sigma(E,\Delta)}\bigr)}\Big)\Big],
% \end{align}
% %
% with $Z\sim \mathcal{N}(0,1)$, $v= \mathbb{E}[S^2]$ and $\Sigma(E,\Delta)^2\defeq \Delta/ (v - E)$. 
% We will see 
% in Section~\ref{subsec:results} that
% $\Sigma(E,\Delta)^2$ can be interpreted as the variance of an effective 
% scalar AWGN channel and $E$ the associated MSE. 
% % $E\in [0,v]$ as it cannot be larger 
% % than the signal variance, which correponds to a purely random guess of the signal ${\bf s}$ knowing its distribution $P_0(\cdot)$.
% This formula allows to determine the information
% theoretical phase transition points where the function $\min_{E\in [0, v]} i_{\rm RS}(E; \Delta)$ is non-analytic (in the sense that its Taylor series does not converge). 
% In this paper we explicitly prove
% \eqref{eq:RSformula} for the class of distributions $P_0$ 
% %which are discrete with a finite number of atoms and 
% such that $i_{\rm RS}(E;\Delta)$ has at most three stationary points. As we will see, the second hypothesis implies that 
% $\min_{E\in [0, v]} i_{\rm RS}(E; \Delta)$ has at most one non-analyticity point, i.e. there is at most one phase transition. 
% Presumably one could extend our analysis to cases with more than one phase transition and cases where $P_0$ is a mixture 
% of a discrete and absolutely continuous distributions ({\bf is discrete an assumption in our proof???}).


%An important application of \eqref{eq:RSformula} is an exact formula for the MMSE, here defined as 
%%
%\begin{align}\label{eq:Mmmse}
% {\rm Mmmse}_n(\Delta^{-1}) \defeq \frac{1}{n^2}\mathbb{E}_{\tbf{S}, \tbf W}\Big[ \bigl\| \tbf{S}\tbf{S}^{\intercal} - 
% \mathbb{E}[\tbf{X}\tbf{X}^{\intercal}\vert\tbf{W}]\bigr\|_{\rm F}^2 \Big].
%\end{align}
%%
%Here, $\|A\|_{\rm F}^2 = \sum_{i,j} A_{ij}^2$ stands for the Frobenius norm of a matrix $A$, and ${\rm Mmmse}$ stands for ``matrix-mmse''. Moreover in the MMSE estimator, the expectation $\mathbb{E}[\tbf{X}\tbf{X}^{\intercal}\vert\tbf{w}]$ is w.r.t the conditional distribution
%%
%\begin{align}
% P(\tbf{x}\vert \tbf{w}) = \frac{1}{Z(\tbf{w})}e^{-\frac{1}{2\Delta}\sum_{i\leq j}\big(\frac{x_i x_j}{\sqrt n} - w_{ij}\big)^2}\prod_{i=1}^n P_0(x_i),
%\end{align}
%%
%$Z(\tbf{w})$ a normalizing factor depending on the observation and equal to the $n$ dimensional integral over the components of $\tbf{x}=(x_i)^n_{i=1}$ and $\mathbb{E}_{\tbf{S}, \tbf{W}}[\cdot]$ is the expectation w.r.t $P({\bf w})P({\bf s})=Z(\tbf{w})\prod_{i=1}^{n} P_0(s_i)$. 
%
%Once we have \eqref{eq:RSformula}, the matrix-mmse can be computed through a well known relation sometimes refered a the I-MMSE theorem [\cite{GuoShamaiVerdu}]. Adapting it to the matrix case (see Appendix~\ref{app:immse} for the proof), we find
%%
%\begin{align}\label{eq:GSV}
%\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^{\intercal}; \tbf{W}) }{d\Delta^{-1}} &= 
%\frac{1}{2n^2}\mathbb{E}_{\tbf{S}, \tbf {W}}\Big[\sum_{i\leq j} \big(S_iS_j - \mathbb{E}[X_iX_j\vert \tbf{W}]\big)^2\Big] 
%\nonumber \\ 
%%
%&= \frac{1}{4n^2}\mathbb{E}_{\tbf{S}, \tbf {W}}\Big[ \bigl\| \tbf{S}\tbf{S}^{\intercal} - \mathbb{E}[\tbf{X}\tbf{X}^{\intercal}\vert\tbf{W}]\bigr\|_{\rm F}^2 \Big]
%+\frac{1}{4n^2}\sum_{i=1}^n (\mathbb{E}[S_i^4] - \mathbb{E}[S_i^2]^2)
%\nonumber \\ 
%&= \frac{1}{4} {\rm Mmmse}_n(\Delta^{-1}) + \mathcal{O}(1/n),
%\end{align}
%%
%where the last equality is obtained thanks to the assumed boundedness of the second and fourth moments of the prior distribution $P_0(\cdot)$. Given any estimator $\hat{\tbf{T}}(\tbf{w})$ for the matrix ${\tbf{s}}{\tbf s}^{\intercal}$ we define a ``matrix mean square error'' as 
% %
%\begin{align}\label{eq:mse-amp-mmse}
% {\rm MSE}_n(\hat{\tbf{T}}(\tbf{w})) \defeq \frac{1}{n^2}\| \tbf{s} \tbf{s}^{\intercal} - \hat{\tbf{T}}(\tbf{w})\|_{\rm F}^2.
%\end{align}
%%
%This is minimized by the MMSE estimator, so clearly
%%
%\begin{align}\label{eq:subopt}
%\mathbb{E}_{\tbf{S}, \tbf{W}}[{\rm MSE}_n(\hat{\tbf{T}}(\tbf{W}))] \geq {\rm Mmmse}_n(\Delta^{-1}).
%\end{align}
%%
%We say that an estimator is {\it optimal} when the equality is reached. Similarly we say that it is 
%\emph{suboptimal} when the inequality is strict.
%
%The AMP estimator, which estimates a vector $\hat{\tbf{s}}$ and sets
%$\hat{\tbf{T}}(\tbf{w}) = \hat{\tbf{s}} \hat{\tbf{s}}^{\intercal}$,
%plays a major role in the proof of \eqref{eq:RSformula}. An important by-product of the proof
%is that it settles the question of determining exactly the noise regimes where the AMP estimator is optimal and those where it is 
%suboptimal. Quite remarquably, this information is entirely contained in the replica symmetric potential function \eqref{eq:potentialfunction}. 
%%
%\begin{algorithm}
% \caption{Symmetric Bayes-optimal AMP}
% \label{alg:ampsym}
%   {\bf Input:} Data $W$ as in eq.(\ref{eq:mainProblem}) and initial
% condition $\hat s^{0}, \hat v^{0}$.  Define the function $f(A,B)$ as
% the expectation with respect to the distribution
% $P(x) \propto P_0(x)e^{B^T x-x^TAx/2}$.  For $t\ge 0$ compute
%   \begin{eqnarray}
%     A^t &=& \frac 1{n\Delta} \hat s^t(\hat s^t)^T,~~~~\text{and} ~~~           B^t = \frac 1{\sqrt n} W \hat s^t - \frac {v^t}{\Delta} \hat s^{t-1}\\
%     \hat s^{t+1} &=& f(A^t,B^t) ~~\text{and}~~ \hat v^t = \frac 1n  \sum_{i=1}^n  \frac {\partial f}{\partial B} (A^t,B^t). 
%   \end{eqnarray}
%\end{algorithm}
%%


%%%%%%%%%%STRUCTURE OF POTENTIAL%%%%%%%%%%%%%%%%%%%%%%%%%%

%
% As we will see the information theoretical as well as the algorithmic approximate message-passing phase transitions, are controlled 
% by the set of critical points of the RS potential function \eqref{eq:potentialfunction}. This set depends 
% on the signal's prior distribution $P_0(\cdot)$ and can be arbitrarily complicated. Here we limit ourselves to the simplest possible situations
% which capture the essence of the problem.
% 
% We assume that $P_0(\cdot)$ is such that the set of solutions $\mathcal{S}_{\Delta}=\{E \, |\, d i_{\rm RS}(E;\Delta)/d E = 0\}$ satisfies the following. There exist two noise variance values $\Delta_\star < \Delta^\prime$ (possibly infinite) such that:
% \begin{enumerate}
% \item[1.] 
% For $0 < \Delta < \Delta_{\star}$ the set $\mathcal{S}_{\Delta}$ contains a \emph{unique} solution
% $E_{\rm good}(\Delta)\in \,]0, v[$ which is a minimum. $E_{\rm good}(\Delta)$ is analytic in $\Delta$. 
% If $\Delta_{\star} = +\infty$ this completely describes the set of solutions. 
% \item[2.] 
% For $\Delta \in\, ]\Delta_\star, \Delta^{\prime}[$ 
% the set $\mathcal{S}_{\Delta}$ contains \emph{three} continuously differentiable extrema which are
% $E_{\rm good}(\Delta) < E_{\rm unstable}(\Delta) < E_{\rm bad}(\Delta)$ contained in $]0, v[$.  One of them, $E_{\rm good}(\Delta)$, is 
% the analytic continuation of the branch found for $\Delta < \Delta_{\star}$ (hence we use the same notation).
% We assume $E_{\rm bad}(\Delta)$ is at least once continuously differentiable.
% Note that necessarily
% $E_{\rm good}(\Delta)$ and $E_{\rm bad}(\Delta)$ are locally minima and $E_{\rm unstable}(\Delta)$ is locally a maximum. 
% \item[3.]
% If $\Delta^{\prime} < +\infty$, for $\Delta > \Delta^\prime$ there exists a \emph{unique} minimum in $]0, v[$ which is a differentiable continuation
% of $E_{\rm bad}(\Delta)$. 
% \item[4.]
% The function $i_{\rm RS}(E_{\rm good}(\Delta);\Delta)$ is analytic for all $\Delta \in\, ]0, \Delta^\prime[$. 
% \end{enumerate}
% %
% These hypothesies are satisfied for all the examples discussed in this paper and many more. In fact all branches of critical points are not only continuously differentiable but are analytic functions (on their domain of definition) and one can then check the analyticity of $i_{\rm RS}(E_{\rm good}(\Delta);\Delta)$ and $i_{\rm RS}(E_{\rm bad}(\Delta);\Delta)$.
% %
% \begin{remark}
% In practice, there are two ways in which the two extra solutions
% may appear at $\Delta_\star$. 
% They may branch of $E_{\rm good}(\Delta_{\star})$ continuously, i.e. $E_{\rm good}(\Delta_{\star})
% = E_{\rm unstable}(\Delta_{\star}) = E_{\rm bad}(\Delta_{\star})$, or they may pop out discontinuously $E_{\rm good}(\Delta_{\star})
% < E_{\rm unstable}(\Delta_{\star}) = E_{\rm bad}(\Delta_{\star})$. The reader familiar with statistical mechanics or bifurcation theory will recognize that the first way 
% corresponds to a continuous (second order) phase transition and the second scenario to a discontinuous (first order) transition. When $\Delta_{\star} = +\infty$ the solution is unique for all $\Delta$ and there is no phase transition.
% \end{remark}
% %
% \begin{remark}
% We will show that $\Delta_{\star}$ can be identified with $\Delta_{\rm AMP}$, the algorithmic threshold of AMP (see Definition
% \ref{amp-thresh}). 
% \end{remark}
% %
% %\begin{remark}
% %We will show that 
% %under the above hypothesies the equation
% %$i_{\rm RS}(E_{\rm good}(\Delta);\Delta)=i_{\rm RS}(E_{\rm bad}(\Delta);\Delta)$ has a unique solution in
% %$[\Delta_\star, \Delta^{\prime}]$ (the solution is set to infinity when $\Delta_\star=+\infty$). 
% %This solution will play a major role and is later defined as 
% %the ``potential threshold" $\Delta_{\rm RS}$ (possibly infinite). One of our important results is that $\Delta_{\rm RS} = \Delta_{\rm opt}$ where $\Delta_{\rm opt}$ is the information theoretic threshold
% %defined as the point where the asymptotic mutual information per variable is not analytic (see definition \ref{Deltaopt}).
% %\end{remark}
% %%
% \begin{remark}
% The value $\Delta^\prime$ is not 
% a threshold that plays a role in our analysis. In coding theory typically it is infinite, but here or in compressed sensing it is finite. 
% \end{remark}
% %

%%%%%%%%%%%ABOUT AMP

%Let us now discuss algorithmic implications. We begin with a short description of the AMP algorithm and state evolution. 
%Consider the simple scalar 
%denoising problem $y = s + \Sigma(E) z$ where $s\sim P_0$ and 
%$z\sim \mathcal{N}(0,1)$. The ``scalar mmse function'' 
%associated to this problem is by definition 
%\begin{align}
% {\rm Smmse}(\Sigma(E)^{-2}) \equiv \mathbb{E}_{s, Y}[(s - \mathbb{E}[x \vert Y])^2]
%\end{align}
%and the {\it state evolution sequence} $E_t$, $t\in \mathbb{N}$ is defined as 
%\begin{align}\label{eq:state-evolution}
% E_{t+1} = {\rm Smmse}(\Sigma(E_{t})^{-2}), \qquad E_0 = v.
%\end{align}
%The AMP algorithm provides an estimate $\hat{s}^t$ according to the iterations
%\begin{align}
%\hat{s}^{t} = \eta_t(W \hat{s}^{t-1} - b_{t-1}\hat{s}^{t-2}), 
%\qquad b_{t}= \frac{1}{n}\sum_{i=1}^n \eta_{t}^\prime(W \hat{s}^{t-1} - b_{t-1}\hat{s}^{t-2})
%\end{align}
%where the denoiser is defined as  
%$\eta_t(y) = \mathbb{E}[x \vert {\rm express~with~} E_t]$. 
%
%The performance measure is the ``matrix MSE" of the AMP estimator, defined as 
%\begin{align}
% {\rm MSE}_{n, \rm AMP}^t(\Delta^{-1}) \equiv \frac{1}{n^2}\|\hat{s}^t (\hat{s}^t)^\intercal - s s^\intercal\|_{\rm F}^2.
%\end{align}
%A remarquable fact that follows from a general theorem of \cite{BayatiMontanari10} (see \cite{deshpande2015asymptotic} for its use in the matrix case) 
%is that the state evolution sequence tracks 
%${\rm MSE}_{n, \rm AMP}^t$ and thus allows to assess the performance of the algorithm. 
%Namely, with probability one,
%\begin{align}\label{eq:mseampmatriciel}
%\lim_{n\to +\infty} {\rm MSE}_{n, \rm AMP}^t(\Delta^{-1}) = v^2 - (v- E_t)^2.
%\end{align}
%%
%The most important quantity computed by state evolution is the algorithmic threshold.
%\begin{definition}[AMP threshold]\label{amp-thresh}
%Let $E_t, t\in \mathbb{N}$ be the state evolution sequence {\it initialised with} $E_0=v$. This is a decreasing sequence 
%and is positive thus $\lim_{t\to +\infty} E_t \equiv E_{\infty}$ exists (see Appendix). The threshold of the 
%AMP algorithm is by definition
%%
%\begin{align}
%\Delta_{\rm AMP} = \sup\,\{\Delta > 0 \ \! | \ \! E_{\infty} = E_{\rm good}(\Delta)\}.
%\end{align}
%\end{definition}
%%

%%%%%%%%%%%%Miscellaneous%%%%%%%%%%%%%%%%%%%%%%

%
%
%compute these partial derivatives more explicitly ? 
%
%\begin{proof}
%We first take the limit $n\to +\infty$ on both sides of \eqref{eq:GSV}. 
%For $\Delta \neq \Delta_{\rm opt}$ (equal to $\Delta_{\rm RS}$, see Lemma~\ref{cor:equality-of-deltas}) it is allowed to exchange the limit and the derivative
% (CITE GOOD ANALYSIS BOOK), so thanks to \eqref{eq:replicaformula},
%\begin{align}\label{mmseirs}
%\lim_{n\to + \infty}{\rm Mmmse}_n(\Delta^{-1}) =  4
%\frac{d}{d\Delta^{-1}}\Big(\min_{E\in[0,v]}i_{\rm RS}(E; \Delta)\Big).
%\end{align}
%Let $E_0(\Delta)$ denote the (global) minimum of the replica symmetric potential. Since this global minimum is $E_{\rm good}(\Delta)$ for $\Delta<\Delta_{\rm RS}$ 
%or $E_{\rm bad}(\Delta)$ for $\Delta >\Delta_{\rm RS}$ and these are continuously differentiable branches on their domain of definition, 
%for $\Delta\neq \Delta_{\rm RS}$ the global minimum $E_0(\Delta)$ is continuously differentiable and locally bounded. Thus
%\begin{align}\label{first}
%\frac{d}{d\Delta^{-1}}\Big(\min_{E\in[0,v]}i_{\rm RS}(E; \Delta)\Big)
%& =
%\frac{di_{\rm RS}}{d\Delta^{-1}}(E_{0}(\Delta); \Delta) 
%\nonumber \\ &
%= 
% \frac{\partial i_{\rm RS}}{\partial E}(E_{0}(\Delta); \Delta) \frac{d E_{0}}{d\Delta^{-1}}
% + \frac{\partial i_{\rm RS}}{\partial\Delta^{-1}}(E_{0}(\Delta) ; \Delta)
% \nonumber \\ &
%=  \frac{\partial i_{\rm RS}}{\partial\Delta^{-1}}(E_{0} ; \Delta).
%\end{align}
%To compute the partial derivative with respect to 
%$\Delta$ we first note that $\frac{\partial i_{\rm RS}}{\partial E}\vert_{E_0} = 0$  implies
%\begin{align}\label{second}
% 0 = -\frac{v-E_0}{2\Delta} - \frac{\partial \mathbb{E}_{s, z}[\cdots]}{\partial \Sigma^{-2}}\Big\vert_{E_0} \frac{\partial\Sigma^{-2}}{\partial E_0} 
%\end{align}
%which immediately gives $\frac{\partial \mathbb{E}_{s, z}[\cdots]}{\partial \Sigma^{-2}}\Big\vert_{E_0} = (v-E_0)/2$.
%Thus
%\begin{align}\label{third}
%\frac{\partial i_{\rm RS}}{\partial\Delta^{-1}}(E_{0} ; \Delta) = \frac{(v-E_0)^2 +v^2}{4}
%- \frac{\partial \mathbb{E}_{s, z}[\cdots]}{\partial \Sigma^{-2}}\Big\vert_{E_0}\frac{\partial\Sigma^{-2}}{\partial\Delta^{-1}} = \frac{v^2 - (v-E_0)^2}{4} 
%\end{align}
%In view of \eqref{mmseirs} and \eqref{first} this ends the proof.
%\end{proof}
%%




==> v5 arxiv/sections/3_examples.tex <==
\section{Two Examples: spiked Wigner model and community detection} \label{sec:examples}
%
In order to illustrate our results, we shall present them here in the
context of two examples: the spiked Wigner model, where we close a
conjecture left open by [\cite{6875223}], and the case of asymmetric
community detection. 
%
\subsection{Spiked Wigner model}
%
\begin{figure}[!t]
\centering
\includegraphics[width=0.49\textwidth]{figs/SPIKEMODEL_PHASEDIAGRAM.pdf}
\includegraphics[width=0.49\textwidth]{figs/SPIKE_MMSE.pdf}
\vspace*{-5pt}
\caption{Left: close up of the phase diagram in the density $\rho$
  (where $P_0(s)=\rho \delta(s-1) + (1-\rho)\delta(x)$) versus noise
  $\Delta$ plane for the rank-one spiked Wigner model (data from
  [\cite{lesieur2015phase}]). In [\cite{6875223}], the authors proved that AMP achieves
  the information theoretic MMSE for all noise as long as
  $\rho>0.041(1)$. We show that AMP is actually achieving the optimal
  reconstruction in the whole phase diagram except in the small region
  between the blue and red line. Notice the large gap with spectral
  methods (dotted black line).  Right: MMSE (red) at $\rho=0.02$ as a
  function of the noise variance $\Delta$. AMP (dashed blue) provably
  achieve the MMSE except in the region
  $\Delta_{\rm AMP}<\Delta<\Delta_{\rm opt}$. We conjecture that no
  polynomial-time algorithm will do better than AMP in this region.}
\label{fig:SPIKEMODEL}
\end{figure}
%
The first model is defined as follows: we are given data distributed
according to the spiked Wigner model where the vector $\tbf{s}$ is
assumed to be a Bernoulli $0/1$ random variable with probability
$\rho$. Data then consists of a sparse, rank-one matrix observed
through a Gaussian noise. In [\cite{6875223}], the authors proved that, for
$\rho>0.041$, AMP is a computationally efficient algorithm that
asymptotically achieves the information theoretically optimal mean-square error for {\it any} value of the noise $\Delta$.  

For very small densities (i.e. when $\rho$ is $o(1)$), there is a well
known large gap between what is information theoretically possible and
what is tractable with current algorithms in support recovery
[\cite{amini2008high}]. This gap is actually related to the planted
clique problem [\cite{d2007direct,barak2016nearly}], where it is
believed that no polynomial algorithm is able to achieve information
theoretic performances. It is thus perhaps not surprising that the
situation for $\rho<0.041$ becomes a bit more complicated. This is
summarized in Fig. \ref{fig:SPIKEMODEL} and discussed in
[\cite{lesieur2015phase}] on the basis of statistical physics
consideration which we now prove.

For such values of $\rho$, as $\Delta$ changes there is a region when
two local minima appears in $i_{\rm RS}(E; \Delta)$ (see the RS formula \eqref{eq:potentialfunction}). In particular for
$\Delta_{\rm AMP}<\Delta<\Delta_{\rm opt}$, the global minimum differs from the
AMP one and a computational gap appears (see right panel in Fig.
\ref{fig:SPIKEMODEL}). Interestingly, in this problem, the region
where AMP is Bayes optimal is still quite large.

The region where AMP is not Bayes optimal is perhaps the most
interesting one.  While this is by no means evident, statistical
physics analogies with actual phase transition in nature suggest that
this region will be hard for a very large class of algorithms. A fact
that add credibility to this prediction is the following: when looking
to small $\rho$ regime, we find that both the information
theoretic threshold {\it and} the AMP one corresponds to what has been
predicted in sparse PCA for sub-extensive values of $\rho$ [\cite{amini2008high}].

Finally, another interesting line of work for such probabilistic
models has appeared in the context of random matrix theory (see for
instance [\cite{baik2005phase}] and references therein). The focus is to
analyze the limiting distribution of the eigenvalues of the observed
matrix. The typical picture that emerges from this line of work is
that a sharp phase transition occurs at a well-defined critical value
of the noise. Above the threshold an outlier eigenvalue (and the
principal eigenvector corresponding to it) has a positive correlation
with the hidden signal. Below the threshold, however, the spectral
distribution of the observation is indistinguishable from that of the
pure random noise. In this model, this happens at
$\Delta_{\rm{spectral}} =\rho^2$. Note that for $\Delta>\Delta_{\rm{spectral}}$
spectral methods are not able to distinguish data coming from the model from
random ones, while AMP is able to sort (partly) data from noise for
any values of $\Delta$ and $\rho$.
%           
%%%%%
%
\subsection{Asymmetric community detection}
%                                                    
\begin{figure}[!t]
\centering
\includegraphics[width=0.49\textwidth]{figs/CS_PHASEDIAGRAM.pdf}
\includegraphics[width=0.49\textwidth]{figs/CS_MMSE.pdf}
\vspace*{-5pt}
\caption{Left: Phase diagram in the density $\rho$ (where
  $P_0(s)=\rho \delta(s-\sqrt{1-\rho/\rho}) +
  (1-\rho)\delta(s+\sqrt{\rho/1-\rho})$)
  corresponding to an asymmetric community detection problem with two
  communities. For $\rho>1-\sqrt{1/12}$ (black point), it is
  information theoretically impossible when $\Delta>1$ to find any
  overlap with the true communities and the optimal MMSE is equal $1$,
  while it is possible for $\Delta<1$.  AMP is again always achieving
  the MMSE, and spectral method can find a non-trivial overlap with
  the truth starting from $\Delta<1$. For $\rho<1-\sqrt{1/12}$,
  however, it is information theoretically possible to find
  information on the hidden assignment (below the blue line), but
  both AMP and spectral methods misses this information: Right:MMSE
  (red) at $\rho=0.05$ as a function of the noise variance
  $\Delta$. AMP (dashed blue) provably achieve the MMSE except in the
  region
  $\Delta_{\rm{spectral}}=\Delta_{\rm AMP}<\Delta<\Delta_{\rm opt}$. }\label{fig:CSMODEL}
\end{figure}
%
The second model is a problem of detecting two communities (groups) with
different sizes $\rho n$ and $(1\!-\!\rho) n$, that generalizes the one considered in
[\cite{deshpande2015asymptotic}]. 
One is given a graph
where the probability to have a link between nodes in the first group
is $p\!+\! \mu (1\!-\!\rho)/(\rho\sqrt{n})$, between those in the second
group is $p\!+\!\mu\rho/(\sqrt{n}(1\!-\!\rho))$, while interconnections appear
with probability $p\!-\!\mu/\sqrt{n}$. With this peculiar ``balanced''
setting, the nodes in each group have the same degree distribution with
mean $pn$, making them harder to distinguish.

According to the universality property described in Section \ref{sec:settings_results}, this is equivalent to the AWGN model \eqref{eq:mainProblem} with variance $\Delta\!=\!p(1\!-\!p)/\mu^2$ where each variable $s_i$ is chosen according to 
%
\begin{align}
P_0(s) = \rho \delta(s - \sqrt{(1 - \rho)/\rho}) +
(1 - \rho)\delta(s + \sqrt{\rho/(1 - \rho)}).
\end{align}

Our results for this problem\footnote{Note that here since $E = v = 1$ is an extremum of $i_{\rm RS}(E;\Delta)$,
one must introduce a small bias in $P_0$ and let it then tend to zero at the end of the proofs.} 
are
summarized in Fig. \ref{fig:CSMODEL}. For
$\rho\!>\rho_c\!=\!1/2\!-\!\sqrt{1/12}$ (black point), it is
asymptotically information theoretically {\it possible} to get an
estimation better than chance if and only if $\Delta\!<\!1$. When
$\rho\!<\!\rho_c$, however, it becomes possible for much larger values
of the noise. Interestingly, AMP and spectral methods have the same
transition and can find a positive correlation with the hidden
communities for $\Delta\!<\!1$, regardless of the value of $\rho$.

==> v5 arxiv/sections/4_threshold_saturation_genericCouplingChain.tex <==
\section{Threshold saturation}\label{sec:thresh-sat}
%
The main goal of this section is to  prove that for a proper spatially coupled (SC) system, threshold saturation 
occurs (Theorem \ref{thres-sat-lemma} ), that is $\Delta_{\rm RS} \le \Delta^{\rm c}_{\rm AMP}$.
We begin with some preliminary formalism in Sec. \ref{stateuncoupled}, \ref{statecoupled} on state evolution for the underlying and coupled systems. 

%
\subsection{State evolution of the underlying system}\label{stateuncoupled}
%
First, define the following posterior average
%
\begin{align}
\langle A \rangle \defeq \frac{\int dx A(x) P_0(x)e^{-\frac{x^2}{2\Sigma(E,\Delta)^{2}} + x\big(\frac{s}{\Sigma(E,\Delta)^{2}} + \frac{z}{\Sigma(E,\Delta)} \big)} }{\int dx P_0(x)
e^{-\frac{x^2}{2\Sigma(E,\Delta)^{2}} + x\big(\frac{s}{\Sigma(E,\Delta)^{2}} + \frac{z}{\Sigma(E,\Delta)} \big)}}, \label{eq:defBracket_posteriorMean}
\end{align}
%
where $S\sim P_0$, $Z\sim\mathcal{N}(0,1)$. The dependence on these variables, as well as on $\Delta$ and $E$ is implicit and dropped from the notation of $\langle A \rangle$. 
Let us define the following operator.
%
\begin{definition}[SE operator] 
The state evolution operator associated with the underlying system is
%
\begin{align}
T_{\rm u}(E) \defeq {\rm mmse}(\Sigma(E)^{-2}) = \mathbb{E}_{S,Z}[(S - \langle X\rangle)^2], \label{def:SEop_underlying}
\end{align}
%
where $S \sim P_0$, $Z\sim \mathcal{N}(0,1)$.
%and ${\rm Smmse}$ stands for ``scalar MMSE''.
%
\end{definition}
%
The fixed points of this operator play an important role. They can be viewed as the stationary points of the replica symmetric potential function $E\in [0,v] \mapsto i_{\rm RS}(E;\Delta)\in \mathbb{R}$
or equivalently of $f_{\rm RS}^{\rm u}: E\in [0,v]\mapsto f_{\rm RS}^{\rm u}(E)\in \mathbb{R}$ where 
\begin{align}
f_{\rm RS}^{\rm u}(E) \defeq i_{\rm RS}(E;\Delta) - \frac{v^2}{4\Delta}.
\end{align}
It turns out to be more convenient to work with $f_{\rm RS}^{\rm u}$ instead of $i_{\rm RS}$. We have 
%
\begin{lemma}\label{lemma:fixedpointSE_extPot_underlying}
Any fixed point of the SE corresponds to a stationary point of $f_{\rm RS}^{\rm u}$:
% If $\mathring{E}$ is a fixed point of \eqref{eq:SEiteration}, i.e., $T_{{\rm u}}(\mathring E) = \mathring E$, then $\frac{\partial F_{{\rm u}}(E)}{\partial E}\big|_{\mathring E} =0$ and vice-versa.
\begin{align}
 E = T_{{\rm u}}(E) \Leftrightarrow \frac{\partial f_{\rm RS}^{\rm u}(E;\Delta)}{\partial E}\big|_{E} =0.
\end{align}
\end{lemma} 
%
\begin{proof}
See Appendix~\ref{app:nishi}.
\end{proof}
%

The asymptotic performance of the AMP algorithm can be tracked by iterating the SE recursion as follows (this is the same as equation \eqref{eq:state-evolution} expressed here with the help of 
$T_{\rm u}$)
%
\begin{align} \label{eq:SEiteration}
E^{(t+1)}=T_{\rm u}(E^{(t)}), \quad t\geq 0, \quad E^{(0)} = v, 
\end{align}
%
where the iteration is initialized without any knowledge about the signal other than its prior distribution 
(in fact, both the asymptotic vector and matrix MSE of the AMP are tracked by the previous recursion as reviewed in Section \ref{subsec:AMP_SE}). 
Let $E_{\rm good}(\Delta) = T_{\rm u}^{(\infty)}(0)$, the fixed point reached by initializing iterations at $E=0$. With our hypothesis on $P_0$ it is not difficult to see that
definition \ref{amp-thresh} is equivalent to 
%
\begin{align}\label{equivDeltaAMP}
\Delta_{{\rm AMP}} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm u}}^{(\infty)}(v) = E_{\rm good}(\Delta)\}\,.
\end{align}
%
The following definition is handy
%
% \begin{definition}[scalar MSE Floor] The scalar MSE floor $E_{\rm good}(\Delta)$ is defined as the fixed point reached from the initial condition $E^{(0)} = 0$. In other words $E_{\rm good}(\Delta) = T_{\rm u}^{(\infty)}(0)$. 
% \end{definition}
%
\begin{definition}[Bassin of attraction]
The basin of attraction of the good solution $E_{\rm good}(\Delta)$ is 
$\mathcal{V}_{\rm good} \defeq \{ E \ \! |\ \! T_{\rm u}^{(\infty )}(E) = E_{\rm good}(\Delta) \}$.
\end{definition}

Finally, we introduce the notion of {\it potential gap}. This is a function $\delta f_{\rm RS}^{\rm u}: \Delta\in \mathbb{R}_+\mapsto \delta f_{\rm RS}^{\rm u}(\Delta)\in \mathbb{R}$ defined as follows:
\begin{definition}[Potential gap] \label{def:fgap}
Define 
\begin{align}
 \delta f_{\rm RS}^{\rm u}(\Delta) \defeq {\rm inf} _{E \notin \mathcal{V}_{\rm good} } (f_{\rm RS}^{\rm u}(E)-f_{\rm RS}^{\rm u} (E_{\rm good}))
\end{align}
 as 
the potential gap, with the convention that the infimum over the empty set is $\infty$ (this happens for $\Delta < \Delta_{{\rm AMP}}$ where the complement of $\mathcal{V}_{\rm good}$ is the empty set).
\end{definition}
%
Our hypothesis on $P_0$ imply that 
\begin{align}
 \Delta_{\rm RS} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! \delta f_{\rm RS}^{\rm u}(\Delta) > 0\}
\end{align}

%
\subsection{State evolution of the coupled system}\label{statecoupled}
%
For the SC system, the performance of the AMP decoder is tracked by an \emph{MSE profile} (or just \emph{profile}) $\tbf{E}^{(t)}$, defined componentwise by 
%
\begin{align}
E^{(t)}_\mu = \lim_{n\to +\infty}\frac{1}{n}\mathbb{E}_{\tbf S, \tbf W}\| {\tbf S}_\mu - \hat{\tbf S}_{\mu}^{(t)}(\tbf W) \|_2^2.
%E^{(t)}_\mu \defeq \mathbb{E}_{S,Z}[n^{-1}\sum_{i_\mu=1}^n(S_{i_\mu} - \hat S_{i_\mu}^{(t)})^2].
\end{align}
%
It has $L+1$ components and describes the scalar MSE in each block $\mu$. Let us introduce the SE associated with the AMP algorithm for the inference over this SC system. First, denote the following posterior average at fixed $s,z$ and $\Delta$.
%
%
\begin{align}
\langle A \rangle_\mu  \defeq \frac{\int dx A(x) P_0(x)e^{-\frac{x^2}{2\Sigma_\mu ({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu ({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu ({\tbf E},\Delta)} \big)} }{\int dx P_0(x)
e^{-\frac{x^2}{2\Sigma_\mu ({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu ({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu ({\tbf E},\Delta)} \big)}}. \label{def:posterior_coupled}
\end{align}
%
%\begin{align}
%P(x|\Sigma_\mu(\tbf{E},\Delta)) &\defeq \frac{P_0(x)e^{-\frac{x^2}{2\Sigma_\mu({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu({\tbf E},\Delta)} \big)} }{\int dx P_0(x)
%e^{-\frac{x^2}{2\Sigma_\mu({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu({\tbf E},\Delta)} \big)}}, \label{def:posterior_coupled}\\  
%\langle A \rangle_\mu &\defeq \int dx A(x)P(x|\Sigma_\mu(\tbf{E},\Delta)), \label{def:posteriorMean_coupled}
%%
%% \langle A \rangle_\mu \defeq \frac{\int dx A(x) P_0(x)e^{-\frac{x^2}{2\Sigma_\mu({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu({\tbf E},\Delta)} \big)} }{\int dx P_0(x)
%% e^{-\frac{x^2}{2\Sigma_\mu({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu({\tbf E},\Delta)} \big)}}, 
%\end{align}
%%
where the \emph{effective noise variance} of the SC system is defined as
%
\begin{align} \label{eq:defSigma_mu}
\Sigma_\mu(\tbf{E})^{-2} \defeq \frac{v-\sum_{\nu \in \mathcal{S}_\mu} \Lambda_{\mu\nu}E_\nu}{\Delta},
\end{align}
%
where we recall $\mathcal{S}_\mu \defeq \{\nu \,|\, \Lambda_{\mu\nu} \neq 0 \}$ is the set of $2w+1$ blocks coupled to block $\mu$.
%
\begin{definition}[SE operator of the coupled system]
The state evolution operator associated with the coupled system (\ref{eq:def_coupledSyst}) is defined component-wise as
%
\begin{align}
[T_{\rm c}({\tbf E})]_\mu \defeq \mathbb{E}_{S,Z}[(S - \langle X\rangle_\mu)^2]. \label{def:SEop_SC}
\end{align}
%
$T_{\rm c}({\tbf E})$ is vector valued and here we have written its $\mu$-th component. 
\end{definition}
%
We assume perfect knowledge of the 
variables $\{s_{i_\mu}\}$ inside the blocks $\mu \in\mathcal{B}\defeq \{0:w-1\}\cup\{L-w:L\}$ as mentioned 
in Section \ref{subsec:SC}, that is $x_{i_\mu} = s_{i_\mu}$ for all $i_\mu$ such that $\mu\in\mathcal{B}$. This 
implies $E_\mu=0 \ \forall \ \mu \in \mathcal{B}$. We refer to this as the {\it pinning condition}. 
The SE iteration tracking the scalar MSE profile of the SC system reads for $\mu\notin \mathcal{B}$
%
\begin{equation}\label{equ:statevolutioncoupled}
E_\mu^{(t+1)} = [T_{\rm c}({\tbf E}^{(t)})]_\mu \quad \forall \ t\geq 0,
\end{equation}
%
with the initialization $E^{(0)}_\mu = v$. For $\mu\in \mathcal{B}$, the pinning condition forces $E_\mu^{(t)} = 0 \ \forall \ t$. This equation is the same as \eqref{coupled-state-evolution} but is expressed here in terms of 
the operator $T{\rm c}$.

Let us introduce a suitable notion of degradation that will be very useful for the analysis.
%
\begin{definition}[Degradation] \label{def:degradation}
A profile ${\tbf{E}}$ is degraded (resp. strictly degraded) w.r.t another one ${\tbf{G}}$, denoted as ${\tbf{E}} \succeq {\tbf{G}}$ (resp. ${\tbf{E}} \succ {\tbf{G}}$), if $E_\mu \ge  G_\mu \ \forall \ \mu$ 
(resp. if ${\tbf{E}} \succeq {\tbf{G}}$ and there exists some $\mu$ such that $E_\mu > G_\mu$).
\end{definition}
%
Define an error profile $\tbf{E}_{\rm good}(\Delta)$ as the vector with all $L+1$ components equal to $E_{\rm good}(\Delta)$.
%
\begin{definition} [AMP threshold of coupled ensemble]\label{def:AMPcoupled}
The AMP threshold of the coupled system is defined as 
\begin{align}
 \Delta^{\rm c}_{\rm AMP} \defeq {\liminf}_{w, L\to \infty}\, {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm c}}^{(\infty)}(\boldsymbol{v}) \prec \tbf{E}_{\rm good}(\Delta)\}
\end{align}
where $\boldsymbol{v}$ is the all $v$ vector. The ${\liminf}_{w, L \to \infty}$ is taken along sequences where {\it first} $L \to \infty$ and {\it then} $w\to\infty$. We also set for a finite system $\Delta_{{\rm AMP}, w, L} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm c}}^{(\infty)}(\boldsymbol{v}) \prec \tbf{E}_{\rm good}(\Delta)\}$.
\end{definition}
%
% Define the ensemble $\mu^{w} \defeq \{\mu - w,\ldots, \mu + w\} = \{\mu - w : \mu + w\}$. 
% The replica symmetric free energy for the SC system \eqref{eq:def_coupledSyst} can be computed by the replica symmetric replica method. It gives
% %
% \begin{align} 
% f_{\rm{c}}(\{E_\mu, \hat m_\mu\}) = &\sum_{\mu=0}^{L}\frac{v - E_\mu}{2} \Big(\hat m_\mu - \sum_{\nu \in \mu^{w}} \frac{v - E_\nu}{2\Delta(2w+1)} \Big) \nonumber \\
% -&\sum_{\mu=0}^L \mathbb{E}_{S,Z}\Big[\ln\Big(\int P_0(x)e^{-x^2\frac{\hat m_\mu}{2} + x \big(S\hat m_\mu + Z\sqrt{\hat m_\mu} \big)}\Big)\Big], \label{eq:coupledF}
% \end{align}
% %
% where $Z\sim \mathcal{N}(z|0,1)$ and $S \sim P_0(s)$. We define the \emph{effective noise variance} of the SC system as
% %
% \begin{align} \label{eq:defSigma_mu}
% \Sigma_\mu(\tbf{E},\Delta)^2 \defeq \Delta \Big(v-\sum_{\nu \in \mu^w} \frac{E_\nu}{2w+1}\Big)^{-1}.
% \end{align}
% %
% The fixed point conditions giving the extrema of this potential are
% %
% \begin{align}
% 0=\frac{\partial f_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {\hat m_\mu}} &\Rightarrow E_\mu = \mathbb{E}[(s - \langle x\rangle_\mu)^2] = [T_{\rm c}({\tbf E})]_\mu, \label{eq:fixedPointPotSC_isSE}\\
% %
% 0=\frac{\partial f_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {E_\mu}} &\Rightarrow \hat m_\mu = \Sigma_\mu({\tbf E})^{-2}.
% \end{align}
% %
% Plugging these relations with (\ref{eq:defSigma_mu}) in (\ref{eq:coupledF}), we obtain the RS free energy for the SC system. 
%

The proof presented in the next subsection uses extensively the following monotonicity properties of the SE operators. 
%
\begin{lemma}
The SE operator of the SC system maintains degradation in space, 
i.e. ${\tbf E} \succeq  {\tbf G} \Rightarrow T_{\rm{c}}({\tbf E}) \succeq T_{\rm{c}}({\tbf{G}})$. This property is verified by $T_{\rm{u}}(E)$ for a scalar error as well.
\label{lemma:spaceDegrad}
\end{lemma}
%
\begin{proof}
From \eqref{eq:defSigma_mu} one can immediately see that ${\tbf E} \succeq  {\tbf G} \Rightarrow \Sigma_\mu({\tbf E}) \geq \Sigma_\mu({\tbf G})\ \forall \ \mu$. 
Now, the SE operator \eqref{def:SEop_SC} can be interpreted as the mmse function associated to the Gaussian channel
$y = s +\Sigma_\mu(\tbf E, \Delta) z$.
This is an increasing function of  the noise intensity $\Sigma_\mu^2$: this is intuitively clear but we provide an explicit formula for the 
derivative below. Thus $[T_{{\rm c}}( {\tbf E})]_\mu \geq [T_{{\rm c}}( {\tbf G})]_\mu \ \forall \ \mu$, which means $T_{{\rm c}}({\tbf E}) \succeq T_{{\rm c}}({\tbf{G}})$.

The derivative of the mmse function of the Gaussian channel can be computed as 
%
\begin{align}
 \frac{d \,{\rm mmse}(\Sigma^{-2})}{d\,\Sigma^{-2}} = - 2\, \mathbb{E}_{X,Y}\Big[\|X - \mathbb{E}[X\vert Y]\|_2^2 \, {\rm Var}[X\vert Y]\Big].
\end{align}
%
This formula explicitly confirms that $T_{\rm u}(E)$ (resp. $[T_{{\rm c}}(\tbf E)]_\mu$) is an increasing function of $\Sigma^2$ (resp. $\Sigma_\mu^2$).
\end{proof}
%
\begin{corollary}
\label{cor:timeDegrad}
The SE operator of the coupled 
system maintains degradation in time, 
i.e., $T_{{\rm c}}({\tbf E}^{(t)}) \preceq  {\tbf E}^{(t)}\Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \preceq  {\tbf E}^{(t+1)}$. 
Similarly $T_{{\rm c}}({\tbf E}^{(t)}) \succeq  {\tbf E}^{(t)} \Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \succeq  {\tbf E}^{(t+1)}$. 
Furthermore, the limiting error profile ${\tbf E}^{(\infty)} \defeq T_{{\rm c}}^{(\infty)}({\tbf E}^{(0)})$
exists. These properties are verified by $T_{{\rm u}}(E)$ as well.
\end{corollary}
%
\begin{proof}
The degradation statements are a consequence of Lemma~\ref{lemma:spaceDegrad}. The existence 
of the limits follows from the monotonicity of the operator and boundedness of the scalar MSE.
\end{proof}
%

Finally we will also need the following generalization of the (replica symmetric) potential function to a spatially coupled system:
%
%
\begin{align}
f_{\rm RS}^{\rm{c}}(\tbf{E}) = &\sum_{\mu=0}^L\sum_{\nu \in \mathcal{S}_\mu} \frac{\Lambda_{\mu\nu}}{4\Delta}(v-E_\mu) (v-E_\nu) \nonumber \\
- &\sum_{\mu=0}^L \mathbb{E}_{S,Z}\Big[\ln\Big(\int dx P_0(x)
 e^{-\frac{1}{2\Sigma_\mu(\tbf E)^{2}}\big(x^2 - 2 xS + xZ\Sigma_\mu(\tbf E,\Delta)\big)} \Big)\Big], \label{def:RSf_SC}
\end{align}
%
where $Z\sim \mathcal{N}(z|0,1)$ and $S \sim P_0(s)$.
%
As for the underlying system, the following Lemma links the SE and RS formulations.
%
\begin{lemma}\label{lemma:fixedpointSE_extPot}
If ${\tbf E}$ is a fixed point of \eqref{equ:statevolutioncoupled}, 
i.e. $ E_\mu = [T_{\rm c}({\tbf E})]_\mu \Rightarrow \frac{\partial f_{\rm RS}^{\rm{c}}({\tbf E})}{\partial E_\mu}\big|_{{{\tbf E}}} = 0 \ \forall \ \mu\in \mathcal{B}^{\rm c}=\{w:L-w-1\}$.
\end{lemma}
%
\begin{proof}
The proof is similar to the proof of Lemma \ref{lemma:fixedpointSE_extPot_underlying} in Appendix~\ref{app:nishi}. We skip the details for brevity.
\end{proof}

%
Now that we have settled the required definitions and properties, we can prove threshold saturation. 
%
\subsection{Proof of Theorem \ref{thres-sat-lemma}}
%
The proof will proceed by contradiction. Let ${\tbf E}^*$ a fixed point profile of
the SE iteration \eqref{equ:statevolutioncoupled}.
We suppose that ${\tbf E}^*$ {\it does not} satisfy ${\tbf E}^* \prec {\tbf E}_{\rm good}(\Delta)$, and exhibit a contradiction for $\Delta < \Delta_{\rm RS}$ and $w$ large enough
(but independent of $L$). Thus we must have ${\tbf E}^* \prec {\tbf E}_{\rm good}(\Delta)$. This is the statement of Theorem \ref{th:mainth_thsat} in Sec. \ref{endsat} and directly implies Theorem \ref{thres-sat-lemma}.

The pinning condition together with the monotonicity properties of the coupled SE operator (Lemma \ref{lemma:spaceDegrad} and Corollary \ref{cor:timeDegrad}) ensure that any fixed point 
profile ${\tbf E}^*$ which does not satisfy ${\tbf E}^* \prec {\tbf E}_{\rm good}(\Delta)$ necessarily has a shape as described in Fig.~\ref{fig:errorProfile}. We construct an associated \emph{saturated profile} $\tbf E$ as described in Fig.~\ref{fig:errorProfile}. 
From now on we work with a \emph{saturated profile} $\tbf E$ which verifies ${\tbf E} \succeq {\tbf E}^{*}$ and 
${\tbf E} \succeq {\tbf E}_{\rm good}(\Delta)$. In the following we will need the following operator.
%
\begin{figure}[!t]
\centering
\includegraphics[width=0.75\textwidth]{figs/profile_E_3.pdf}
\caption{A fixed point profile $\tbf{E}^{*}$ of the coupled SE iteration (solid line) is necessarily null
$\forall \ \mu \in \{0: w-1\}$
because of the pinning condition, and then it increases to reach $E_{{\rm max}} \in [0,v]$ at some $\mu_{\rm max}\in \{w:L-w-1\}$ (for a symmetric coupling matrix $\mu_{\rm max} = L/2$). 
Then, it starts decreasing and it is again null $\forall \ \mu \in \{L-w:L\}$. By definition, the associated \emph{saturated} profile $\tbf E$ (dashed line) starts 
at $E_{\rm good}(\Delta) \ \forall \ \mu \le \mu_*$, where $\mu_*$ is such that: $E^{*}_{\mu}\le E_{\rm good}(\Delta) \ \forall \ \mu\in\{0: \mu_*\}$ 
and $E^{*}_{\mu'} > E_{\rm good}(\Delta) \ \forall \ \mu'\in\{ \mu_*+1:L\}$. Then, ${\bf E}$ matches $\tbf E^{*} \ \forall \ \mu \in\{\mu_*:\mu_{\rm max}\}$ 
and saturates at $E_{{\rm max}} \ \forall \ \mu \ge \mu_{\rm max}$. The saturated profile is extended for $\mu <0$ and $\mu >L$ indices. The green (resp. red) branch 
shows that when the block indices of ${\bf E}$ are $\mu <0$ (resp. $\mu> L$), then $E_\mu$ equals to $E_{\rm good}(\Delta)$ (resp. $E_{\rm max}$). 
By construction, ${\tbf E}$ is non decreasing in $\mu$ and is degraded w.r.t the fixed point profile ${\tbf E} \succeq {\tbf E}^{*}$.}
\label{fig:errorProfile}
\end{figure}
%
\begin{definition}[Shift operator]
% The shift operator is defined componentwise as $[{\rm S}({\tbf E})]_0 \defeq E_{\rm good}(\Delta), \ [{\rm S}({\tbf E})]_\mu \defeq  E_{\mu-1}$.
The shift operator ${\rm S}$ is defined componentwise as $[{\rm S}({\tbf E})]_\mu \defeq  E_{\mu-1}$.
\end{definition}
%
\subsubsection{Upper bound on the potential variation under a shift}
%
The first step in the proof of threshold saturation is based on the Taylor expansion of the RS free energy of the SC system. 
%
\begin{lemma}\label{leminterp}
Let ${\tbf E}$ be a saturated profile. 
Set ${\tbf E}_\lambda \defeq (1-\lambda) {\tbf E} + \lambda {\rm S}({\tbf E})$ for $\lambda\in [0,1]$ and $\delta {E}_{\mu} \defeq {E}_{\mu} -{E}_{\mu-1}$. There exists some $\lambda\in[0,1]$ such that
%
\begin{align}
f_{\rm RS}^{\rm{c}}({\rm S}({\tbf E})) &-f_{\rm RS}^{\rm{c}}({\tbf E}) = \frac{1}{2} \sum_{\mu,\mu'=0}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 f_{\rm RS}^{\rm{c}}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}. \label{eq:lemma_secondDerivativeFsc}
\end{align}
%
\label{lemma:Fdiff_quadraticForm}
\end{lemma}
%
\begin{proof}
%
Using the remainder Theorem, the free energy difference can be expressed as
%
\begin{align}
f_{\rm RS}^{\rm{c}}({\rm S}({\tbf E})) -f_{\rm RS}^{\rm{c}}({\tbf E}) 
= 
- \sum_{\mu=0}^{L} \delta {E}_{\mu} \frac{\partial f_{\rm RS}^{\rm{c}}({\tbf E})}{\partial  E_\mu}\Big|_{{\tbf E}}
+
\frac{1}{2}\sum_{\mu,\mu'=0}^{L} \delta {E}_{\mu} \delta {E}_{\mu'}  
\frac{\partial^2 f_{\rm RS}^{\rm{c}}({\tbf E})}{\partial E_{\mu}\partial  E_{\mu'}}\Big|_{ {\tbf E}_\lambda} 
. \label{eq:expFbsminusFb}
\end{align}
%
for some $\lambda\in [0,1]$.
By definition of the saturated profile $\tbf E$, we have $\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{0:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$ 
and $E_\mu=[T_{\rm c}(\tbf E)]_\mu$ for $r\notin\mathcal{A}$. Recalling Lemma~\ref{lemma:fixedpointSE_extPot} we see that the
derivative in the first sum cancels for $r\notin\mathcal{A}$. Hence the first sum in (\ref{eq:expFbsminusFb}) vanishes.
\end{proof}
%
\begin{lemma} \label{lemma:smooth}
The saturated profile ${\tbf E}$ is smooth, i.e. $\delta E^* \defeq \underset{\mu}{\rm{max}} \,|\delta E_\mu| = \mathcal{O}(1/w)$ uniformly in $L$.
\end{lemma}
%
\begin{proof}
By definition of the saturated profile $\tbf E$ we have
$\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{0:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$. For $\mu \notin\mathcal{A}$, we can replace 
the fixed point profile component $E_\mu$ by $[T_{\rm c}(\tbf E)]_\mu$ so that $\delta E_\mu = [T_{\rm c}(\tbf E)]_\mu - [T_{\rm c}(\tbf E)]_{\mu-1}$.
We will Taylor expand the SE operator. To this end, we define $\delta \Sigma_\mu^{-2} \defeq \Sigma_{\mu}({\tbf E})^{-2} - \Sigma_{\mu-1}({\tbf E})^{-2}$ for 
$\mu \in\{\mu^* +1:\mu_{\rm max}\}$. Recall that $\Lambda_{\mu-1,\nu-1} = \Lambda_{\mu\nu}$, $\Lambda_{\mu\nu} \geq 0$ and $\Lambda^{*}\defeq\sup_{\mu,\nu}\Lambda_{\mu\nu} = \mathcal{O}(1/w)$. Thus from \eqref{eq:defSigma_mu} we get 
%
\begin{align}
|\delta \Sigma_\mu^{-2} | = & \frac{1}{\Delta} \Big|\sum_{\nu \in \mathcal{S}_\mu} \Lambda_{\mu\nu} (E_{\nu} -E_{\nu-1})\Big| 
\nonumber \\ &
\leq 
\frac{\Lambda^{*}}{\Delta} \sum_{\nu \in \mathcal{S}_\mu} (E_{\nu} -E_{\nu-1})
\nonumber \\ &
\leq 
\frac{2v \Lambda^{*}}{\Delta} = \mathcal{O}(\frac{1}{w})
\label{eq:boundSigma_minus2}
%
% &= \sum_{\nu \in \mathcal{S}_\mu\cap \mathcal{S}_{\mu-1}} 
%\frac{E_{\nu}(\Lambda_{\mu,\nu} - \Lambda_{\mu-1,\nu})}{\Delta} + \mathcal{O}(1/w) \le \frac{CK_{\Lambda}v(2w+1)}{\Delta w^2} = C'/w \ \forall \ \mu, \label{eq:boundSigma_minus2}
\end{align}
%
where we have used $E_{\nu} -E_{\nu-1} \geq 0$ to get  rid of the absolute value.
Note that the first and second derivatives of the SE operator \eqref{def:SEop_SC} w.r.t $\Sigma_\mu^{-2}$ 
are bounded as long as the five first moments of the posterior \eqref{def:posterior_coupled} exist and are 
bounded (which is true under our assumptions). Then by Taylor expansion at first 
order in $\delta \Sigma_\mu^{-2}$ and using the remainder theorem, we obtain
%
\begin{align} \label{eq:deltamstar}
|\delta E_{\mu}| &= |[T_{\rm{c}}({\tbf E})]_{\mu} - [T_{\rm{c}}({\tbf E})]_{\mu-1}| 
\le |\delta \Sigma_\mu^{-2}| \Big|\frac{\partial [T_{\rm{c}}({\tbf E})]_{\mu}}{\partial \Sigma_\mu^{-2}}\Big| + \mathcal{O}(\delta \Sigma_\mu^{-4}) \le \mathcal{O}(\frac{1}{w}),
\end{align}
%
where the last inequality follows from \eqref{eq:boundSigma_minus2}.
%
\end{proof}

\begin{proposition} \label{lemma:dF_ge_Uoverw}
Let $\tbf E$ be a saturated profile. Then for all $\Delta > 0$ there exists a constant $0 < C(\Delta) < +\infty$ independent of $L$ such that 
\begin{align}
|f^{\rm c}_{\rm RS}({\rm S}({\tbf E})) -f^{\rm c}_{\rm RS}({\tbf E})| \leq \frac{C(\Delta)}{w} .
\end{align}
\end{proposition}
%
\begin{proof}
From Lemma~\ref{leminterp}, in order to compute the free energy difference between the shifted and non-shifted profiles, we need to compute the Hessian associated with this free energy. We have
%
\begin{align}
\frac{\partial f_{\rm RS}^{\rm{c}}({\tbf E})}{\partial {E_\mu}} &= \sum_{\nu \in \mathcal{S}_\mu} \frac{\Lambda_{\mu, \nu} E_\nu}{2\Delta} -\frac{1}{2} \sum_\nu \frac{\partial \Sigma_\nu(\tbf E)^{-2}}{\partial E_\mu} [T_{\rm{c}}({\tbf E})]_\nu - \frac{v}{2\Delta} 
\nonumber \\
&= \frac{1}{2\Delta}\Big(\sum_{\nu \in \mathcal{S}_\mu} \Lambda_{\mu, \nu}E_\nu+\sum_{\nu \in\mathcal{S}_\mu}\Lambda_{\mu, \nu} [T_{\rm{c}}({\tbf E})]_\nu-v\Big)
\end{align}
%
and 
%
\begin{align}
\frac{\partial^2 f_{\rm RS}^{\rm{c}}({\tbf E})}{\partial {E_\mu}\partial {E_{\mu'}}} &= \frac{1}{2\Delta}\Big( \Lambda_{\mu,\mu'}\mathbb{I}(\mu' \in \mathcal{S}_\mu) - \frac{1}{\Delta}\sum_{\nu \in \mathcal{S}_\mu\cap \mathcal{S}_{\mu'}} \Lambda_{\mu ,\nu}\Lambda_{\mu',\nu}\frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \, \Sigma_\nu^{-2}} \Big). 
\label{eq:hessian_explicit}
\end{align}
%
We can now estimate the sum in the Lemma~\ref{leminterp}. The contribution of the first term on the r.h.s of \eqref{eq:hessian_explicit} can be bounded as
%
\begin{align}
\frac{1}{2\Delta} \Big|\sum_{\mu=0}^L\sum_{\mu'\in \mathcal{S}_\mu}\Lambda_{\mu,\mu'}\delta E_{\mu}\delta E_{\mu'}\Big| \le \frac{\delta E^*\Lambda^*(2w+1)}{2\Delta} \Big|\sum_{\mu=0}^L\delta E_{\mu}\Big| \le \mathcal{O}(\frac{1}{w}), \label{eq:firstTermbound}
\end{align}
%
where we used the facts: $\delta E_\mu \geq 0$, the sum over $\mu=0, \cdots, L$ is telescopic, $E_\mu\in[0,v]$, $\Lambda^* = \mathcal{O}(1/w)$ and $\delta E^{*} = \mathcal(w^{-1})$ (Lemma~\ref{lemma:smooth}). We now bound the contribution of the second term on the r.h.s of \eqref{eq:hessian_explicit}. Recall the first derivative w.r.t $\Sigma_{\nu}^{-2}$ of the SE operator is bounded uniformly in $L$. Call this bound $K=\mathcal{O}(1)$. We obtain
%
\begin{align}
&\frac{1}{2\Delta^2} \Big|\sum_{\mu, \mu'=1}^L \delta E_\mu \delta E_{\mu '} \sum_{\nu \in \mathcal{S}_\mu\cap \mathcal{S}_{\mu'}}\Lambda_{\mu ,\nu}\Lambda_{\mu',\nu} \frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \Sigma_{\nu}^{-2}}\Big| \nonumber\\ 
%
\le \ &\frac{K\Lambda^{*2}\delta E^*}{2\Delta^2} \Big|\sum_{\mu=1}^L \delta E_\mu \sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mathcal{S}_\mu\cap \mathcal{S}_{\mu'})\Big| \le \mathcal{O}(\frac{1}{w}). \label{eq:last_secondTerm_boudHessian}
\end{align}
%
The last inequality follows from the following facts: the sum over $\mu=1, \cdots, L$ is telescopic, $\Lambda^* = \mathcal{O}(1/w)$, Lemma~\ref{lemma:smooth}, and for any fixed $\mu$ the following holds
\be
\sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mathcal{S}_\mu\cap \mathcal{S}_{\mu'}) = (2w+1)^2.
\ee
Finally, from \eqref{eq:firstTermbound}, \eqref{eq:last_secondTerm_boudHessian} and the triangle inequality we obtain
%
\begin{align}
\frac{1}{2}\Big| \sum_{\mu,\mu'=1}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 f^{\rm c}_{\rm RS}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}\Big| = \mathcal{O}(\frac{1}{w})
\end{align}
%
uniformly in $L$. Combining this result with Lemma~\ref{leminterp} ends the proof.
\end{proof}
%
%
\subsubsection{Lower bound on the potential variation under a shift}
%
The second step in the proof is based on a direct evaluation of $f_{\rm RS}^{\rm c}({\rm S}(E)) - f_{\rm RS}^{\rm c}(E)$.
We first need the Lemma:
%
\begin{lemma}
Let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_{\rm good}(\Delta)$. Then $ E_{\rm max} \notin \mathcal{V}_{\rm good}$.
\label{lemma:outside_basin}
\end{lemma}
%
\begin{proof}
The fact that the error profile is non decreasing and the assumption that ${\tbf E} \succ {\tbf E}_{\rm good}(\Delta)$ imply that $E_{\rm max} > E_0 =E_{\rm good}(\Delta)$. Moreover,
%
$E_{\rm max} \le [T_{\rm c}({\tbf E})]_{\mu_{\rm max}} \le T_{\rm u}(E_{\rm max})$
%
where the first inequality follows from $\tbf E\succ \tbf E^*$ and the monotonicity of $T_{\rm c}$, while the second comes from the fact that $\tbf E$ is non decreasing. Combining these with the 
monotonicity of $T_{\rm u}$ gives $T_{\rm u}(E_{\rm max}) \ge  E_{\rm max}$ which implies $T_{\rm u}^{(\infty)}( E_{\rm max}) \ge  E_{\rm max}> E_{\rm good}(\Delta)$ which means $E_{\rm max} \notin \mathcal {V}_{\rm good}$.
\end{proof}
%
\begin{proposition}\label{lemma:FcSE_minus_FcE_le_deltaF}
Fix $\Delta < \Delta_{\rm RS}$ and let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_{\rm good}(\Delta)$. Then 
\begin{align}
|f^{\rm c}_{\rm RS}(S(\tbf{E})) - f^{\rm c}_{\rm RS}(\tbf{E})| \ge \delta f^{\rm u}_{\rm RS}(\Delta)
\end{align}
where $\delta f^{\rm u}_{\rm RS}(\Delta)$ is the potential gap (Definition~\ref{def:fgap}).
\end{proposition}
%
\begin{proof}
Set 
\begin{align*}
\mathcal{I}(\Sigma) \defeq \mathbb{E}_{S,Z}\Big[\ln\Big(\int dxP_0(x) e^{- \frac{1}{2\Sigma^2}\big(x^2 -2 Sx - 2\Sigma Zx\big)}\Big)\Big]\, .
\end{align*}
By \eqref{def:RSf_SC} 
%
\begin{align}
f^{\rm c}_{\rm RS}({\rm S}(\tbf{E})) - f^{\rm c}_{\rm RS}(\tbf{E})=&\sum_{\mu = -1}^{L-1} \sum_{\nu \in \mathcal{S}_{\mu}} \frac{\Lambda_{\mu+1\nu+1} }{4\Delta}(v\!-\!E_{\mu}) (v\!-\!E_{\nu}) - \sum_{\mu = 0}^{L} \sum_{\nu \in \mathcal{S}_{\mu}} \frac{\Lambda_{\mu\nu} }{4\Delta}(v\!-\!E_{\mu}) (v\!-\!E_{\nu}) \nonumber \\
%
& \quad - \sum_{\mu=0}^L \mathcal{I}(\Sigma_{\mu}({\rm S}({\bf E}))) + \sum_{\mu=0}^L \mathcal{I}(\Sigma_{\mu}(\bf E))\nonumber\\
%
= &\sum_{\nu \in \mathcal{S}_{-1}} \frac{\Lambda_{\mu\nu} }{4\Delta}(v\!-\!E_{\mu}) (v\!-\!E_{\nu}) - \sum_{\nu \in \mathcal{S}_{L}} \frac{\Lambda_{\mu\nu} }{4\Delta}(v\!-\!E_{\mu}) (v\!-\!E_{\nu}) \nonumber \\
%
& \quad - \mathcal{I}(\Sigma_{-1}({\bf E})) + \mathcal{I}(\Sigma_{L}(\bf E)), \label{eq:lastFcSE_minus_FcE}
\end{align}
%
where we used $\Lambda_{\mu+1\nu+1}=\Lambda_{\mu\nu}$ implying also $\Sigma_{\mu}({\rm S}({\bf E})) = \Sigma_{\mu-1}({\bf E})$ as seen from \eqref{eq:defSigma_mu}. Recall $\Sigma(E)^{-2}= (v - E)/\Delta$. Now looking at \eqref{eq:defSigma_mu}, one notices that thanks to the saturation of ${\tbf E}$, $\Sigma_{-1}({\tbf E}) = \Sigma(E_0)$ where $E_0=E_{\rm good}(\Delta)$ (see the green branch in Fig.~\ref{fig:errorProfile}), while $\Sigma_{L}({\tbf E}) = \Sigma(E_L)$ where $E_L = E_{\rm{max}}$ (see the red branch Fig.~\ref{fig:errorProfile}). Finally from \eqref{eq:lastFcSE_minus_FcE}, using that the coupling matrix is (doubly) stochastic and the saturation of ${\bf E}$
%
\begin{align}
f^{\rm c}_{\rm RS}({\rm S}(\tbf{E})) - f^{\rm c}_{\rm RS}(\tbf{E}) &= \Big[\frac{(v\!-\!E_{0})^2 }{4\Delta} - \mathcal{I}(\Sigma(E_{\rm good}(\Delta))) \Big] - \Big[\frac{(v\!-\!E_{L})^2 }{4\Delta} - \mathcal{I}(\Sigma(E_L)) \Big] \nonumber\\
%
&= f^{\rm u}_{\rm RS}(E_{\rm good}) - f^{\rm u}_{\rm RS}(E_{\rm max}) \le -\delta f^{\rm u}_{\rm RS}(\Delta),
\end{align}
%
where we recognized the potential function of the underlying system $f_{\rm RS}^{\rm u}(E;\Delta) = i_{\rm RS}(E;\Delta) - \frac{v^2}{4\Delta}$ and the last inequality is a direct application of Lemma~\ref{lemma:outside_basin} and Definition \ref{def:fgap}. Finally, using the positivity of $\delta f^{\rm u}_{\rm RS}(\Delta)$ for $\Delta<\Delta_{\rm{RS}}$, we obtain the desired result.
\end{proof}
%

\subsubsection{End of proof of threshold saturation}\label{endsat}

We now have the necessary ingredients in order to prove threshold saturation.
%
\begin{theorem}[Asymptotic performance of AMP for the coupled system] \label{th:mainth_thsat}
Fix $\Delta<\Delta_{\rm{RS}}$. Take a spatially coupled system with $w>C(\Delta)/\delta f^{\rm u}_{\rm RS}(\Delta)$ where $C(\Delta)$ is the constant in 
Proposition \ref{lemma:dF_ge_Uoverw}. Then any fixed point profile ${\tbf{E}^*}$ of the coupled state evolution iteration \eqref{equ:statevolutioncoupled} must satisfy ${\tbf{E}}^* \prec {\tbf{E}}_{\rm good}(\Delta)$.
\end{theorem}
%
\begin{proof}
The proof is by contradiction. Fix $\Delta < \Delta_{\rm RS}$ and $w \ge C(\Delta)/\delta f^{\rm u}_{\rm RS}(\Delta)$.
We assume there exists a fixed point profile which does not satisfy $\tbf E^*\prec {\tbf{E}}_{\rm good}(\Delta)$. Then we construct
the associated saturated profile ${\tbf E}$. This profile satisfies both statements 
of Propositions ~\ref{lemma:dF_ge_Uoverw} and \ref{lemma:FcSE_minus_FcE_le_deltaF}. Therefore we must have
$\delta f^{\rm u}_{\rm RS}(\Delta)\le C(\Delta)/w$ which contradicts the choice  $w > C(\Delta)/\delta f^{\rm u}_{\rm RS}(\Delta)$.
We conclude that ${\tbf E}^* \prec {\tbf{E}}_{\rm good}(\Delta)$ must be true.
\end{proof}
%
%\begin{corollary}[Threshold saturation]\label{cor:maincorollary_thsat}
%By first taking $L \to \infty$ and then $w\to\infty$, the AMP threshold of the coupled ensemble satisfies $\Delta_{\rm AMP, coup}\geq \Delta_{\rm{RS}}$.
%\end{corollary}
%

Theorem \ref{thres-sat-lemma} is a direct corollary of Theorem~\ref{th:mainth_thsat} and Definition~\ref{def:AMPcoupled}. Take 
some $\Delta_* < \Delta_{\rm RS}$ and choose $w > C(\Delta_*)/\delta f^{\rm u}_{\rm RS}(\Delta_*)$. Then we have 
$\Delta_{{\rm AMP}, w, L} \geq \Delta_*$. Note that $\delta f^{\rm u}_{\rm RS}(\Delta_*) \to 0_+$ for $\Delta_*\to \Delta_{\rm RS}$. Thus  
Taking $L\to +\infty$ first and $w\to +\infty$ second we can make $\Delta_*$ as close to $\Delta_{\rm RS}$ as we wish. Therefore we obtain $\Delta_{\rm AMP}^{\rm c} \defeq\liminf_{L, w\to +\infty} \Delta_{{\rm AMP}, w, L} \geq \Delta_{\rm RS}$ where the limit is taken in the specified order. 




==> v5 arxiv/sections/5_interpolation_subadditivity_jeanRevision.tex <==
\section{Invariance of the mutual information under spatial coupling}\label{sec:subadditivitystyle}
%
In this section we prove that the mutual information remains unchanged under spatial coupling in a suitable asymptotic limit 
(Theorem \ref{LemmaGuerraSubadditivityStyle}). 
We will compare the mutual informations of the four following variants of \eqref{eq:def_coupledSyst}. In each case, the signal $\bs$ has $n(L+1)$ i.i.d components.
%
\begin{itemize}
\item \emph{The fully connected:} If we choose $w = L/2$ and a homogeneous coupling matrix with elements $\Lambda_{\mu,\nu} = (L+1)^{-1}$ in \eqref{eq:def_coupledSyst}. This yields a homogeneous fully connected system equivalent to \eqref{eq:mainProblem} with $n(L+1)$ instead of $n$ variables. The associated mutual information per variable for fixed $L$ and $n$ is denoted by $i_{n, L}^{\rm con}$.
%
\item \emph{The SC pinned system:} This is the system studied in Section~\ref{sec:thresh-sat} to prove threshold saturation, with the pinning condition. In this case we choose $0<w < L/2$. The coupling matrix $\boldsymbol{\Lambda}$ is any matrix that fulfills the requirements in Section~\ref{subsec:SC} (the concrete example given there will do). The associated mutual information per variable is here denoted $i_{n, w, L}^{\rm cou}$. Note that $i_{n, w, L}^{\rm cou} = (n(L+1))^{-1} I_{w,L}(\tbf{S}; \bW)$
%
\item \emph{The periodic SC system:} This is the same SC system (with same coupling window and coupling matrix) but without the pinning condition. The associated mutual information per variable at fixed $L,w, n$ is denoted $i_{n, w, L}^{\rm per}$.
%
\item \emph{The decoupled system:} This corresponds simply to $L+1$ identical and independent systems of the form \eqref{eq:mainProblem} with $n$ variables each. This is equivalent to periodic SC system with $w = 0$. The associated mutual information per variable is  denoted $i_{n, L}^{\rm dec}$. Note that $i_{n, L}^{\rm dec} = n^{-1} I(\tbf{S}; \bW)$.
\end{itemize}
%
Let us outline the proof strategy.
In a first step, we use an interpolation method twice: first interpolating between the fully connected and periodic SC systems, and then between the decoupled and periodic SC systems. This will allow to sandwich the mutual information of the periodic SC system by those of the fully connected and decoupled systems respectively (see Lemma~\ref{lemma:freeEnergy_sandwich}). 
In the second step, using again a similar interpolation and Fekete's theorem for superadditive sequences, we prove that the decoupled and fully connected systems have asymptotically the same mutual information (see Lemma \ref{lemma:superadditivity} for the existence of the limit). From these results we deduce the proposition:
%
\begin{proposition}\label{lemma:freeEnergy_sandwich_limit} 
For any $0\leq w \leq L/2$ 
\begin{align}
\lim_{n\to +\infty} i_{n, w, L}^{\rm per}= \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \bW)
\end{align}
\end{proposition}
%
\begin{proof}
Lemma \ref{lemma:superadditivity} implies that $\lim_{n\to +\infty} i_{n, L}^{\rm con} = \lim_{n\to +\infty} i_{n, L}^{\rm dec}$. One also notes that $i_{n, L}^{\rm dec} = \frac{1}{n} I(\tbf{S}; \bW)$. Thus the result follows from Lemma \ref{lemma:freeEnergy_sandwich}.
\end{proof}
%
In a third step an easy argument shows
%
\begin{proposition}\label{lemma:openVSclosed} 
Assume $P_0$ has finite first four moments. For any $0\leq w \leq L/2$ 
%
\begin{align}
\vert i_{n, w, L}^{\rm per} - i_{n, w, L}^{\rm cou} \vert = \mathcal{O}(\frac{w}{L})
\end{align}
%
\end{proposition}
%
\begin{proof}
See Appendix \ref{appendix-pinfree}.
\end{proof}
%
Since $i_{n, w, L}^{\rm cou} = (n(L+1))^{-1} I_{w,L}(\tbf{S}; \bW)$, Theorem \ref{LemmaGuerraSubadditivityStyle} is an immediate consequence of Propositions \ref{lemma:freeEnergy_sandwich_limit} and \ref{lemma:openVSclosed}. 
%
\subsection{A generic interpolation}\label{generic}
%
Let us consider two systems of same total size $n(L+1)$ with coupling matrices $\bold{\Lambda}^{(1)}$ and $\bold{\Lambda}^{(0)}$ supported on coupling windows $w_1$ and $w_0$ respectively. 
Moreover, we assume that the observations associated with the first system are corrupted by an AWGN equals to $\sqrt{\Delta / t}\bz$ while the 
AWGN corrupting the second system is $\sqrt{\Delta / (1 - t)}\bz^{\prime}$, where $Z_{ij}$ and $Z^{\prime}_{ij}$ are two i.i.d. 
standard Gaussians and $t\in[0,1]$ is the \emph{interpolation parameter}. The interpolating inference problem has the form
\begin{align}
 \begin{cases}
  w_{i_\mu j_\nu} & = s_{i_\mu} s_{j_\nu}\sqrt{\frac{\Lambda_{\mu\nu}^{(1)}}{n}} + z_{i_\mu j_\nu}\sqrt{\frac{\Delta}{t}},\\
  w_{i_\mu j_\nu} & = s_{i_\mu} s_{j_\nu}\sqrt{\frac{\Lambda_{\mu\nu}^{(0)}}{n}} + z_{i_\mu j_\nu}^\prime\sqrt{\frac{\Delta}{1-t}}
 \end{cases}
\end{align}
In this setting, at $t=1$ the interpolated system corresponds to the first system as the 
noise is infinitely large in the second one and no information is available about it, while at $t=0$ the opposite happens. 
The associated interpolating posterior distribution can be expressed
as 
\begin{align}\label{post-interp-d}
 P_{t}(\bx\vert \bs, \bz, \bz^\prime) = \frac{1}{\mathcal{Z}_{\rm int}(t)} e^{-\mathcal{H}(t, \bold{\Lambda}^{(1)},\bold{\Lambda}^{(0)}))}\prod_{\mu=0}^{L}\prod_{i_\mu=1}^n P_0(x_{i_\mu})
\end{align}
where the ``Hamiltonian'' is
 $\mathcal{H}_{\rm int}(t,\bold{\Lambda}^{(1)},\bold{\Lambda}^{(0)}) \defeq 
\mathcal{H}(t,\bold{\Lambda}^{(1)}) + \mathcal{H}(1-t,\bold{\Lambda}^{(0)})$ with\footnote{Note that since the SC system is defined on a ring, we can express the Hamiltonian in terms of forward coupling only.} 
%
\begin{align}
\mathcal{H}(t,\bold{\Lambda}) \defeq &\frac{t}{\Delta} \sum_{\mu=0}^L \Lambda_{\mu,\mu} \sum_{i_\mu\le j_\mu}\bigg( \frac{x_{i_\mu}^2x_{j_\mu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\mu}x_{i_\mu}x_{j_\mu}}{n} - \frac{x_{i_\mu}x_{j_\mu}z_{i_\mu j_\mu} \sqrt{\Delta}}{\sqrt{n t\Lambda_{\mu,\mu}}}\bigg)\nonumber\\
%
+&\frac{t}{\Delta} \sum_{\mu=0}^L\sum_{\nu=\mu+1}^{\mu+w}\Lambda_{\mu,\nu}\sum_{i_\mu,j_\nu=1}^{n}\bigg( \frac{x_{i_\mu}^2x_{j_\nu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n} - \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu} \sqrt{\Delta}}{\sqrt{nt\Lambda_{\mu,\nu}}}\bigg).
\end{align}
%
and $\mathcal{Z}_{\rm int}(t)$ is the obvious normalizing factor, the ``partition function''. The posterior average with respect to \eqref{post-interp-d} is denoted by the bracket notation $\langle - \rangle_t$. It is easy to see
that the mutual information per variable (for the interpolating inference problem) can be expressed as 
%
\begin{align}
i_{\rm int}(t) \defeq - \frac{1}{n(L+1)}\mathbb{E}_{{\bf S}, {\bf Z}, {\bf Z}^{\prime}}[\ln \mathcal{Z}_{\rm int}(t)] + \frac{v^2}{4\Delta} + \frac{1}{4 \Delta n(L+1)} (2\mathbb{E}[S^4] - v^2)
\end{align}

The aim of the interpolation method in the present context is to compare the mutual informations of the systems at $t=1$ and $t=0$. To do so, 
one uses the fundamental theorem of calculus
%
\begin{align}\label{calc}
i_{\rm int}(1) - i_{\rm int}(0) = \int_{0}^1 dt \, \frac{di_{\rm int}(t)}{dt}\,.
\end{align}
%
and tries to determine the sign of the integral term. 

We first prove that
%
\begin{align} 
& \frac{di_{\rm int}(t)}{dt} = \nonumber\\
%
&\frac{1}{4\Delta(L+1)} \mathbb{E}_{\bf S, \bf Z,{\bf Z}^{\prime}}\Big[\Big\la 
-\frac{1}{n^2}\Big(\sum_{\mu=0}^L\sum_{\nu=\mu-w_1}^{\mu + w_1} \Lambda_{\mu\nu}^{(1)} 
\sum_{i_\mu, j_\nu=1}^n X_{i_\mu}X_{j_\nu}S_{i_\mu}S_{j_\nu} + \sum_{\mu=0}^L \Lambda_{\mu\mu}^{(1)} \sum_{i_\mu=1}^n X_{i_\mu}^2 S_{i_\mu}^2\Big) \nonumber \\
%
&+ \frac{1}{n^2}\Big(\sum_{\mu=0}^L\sum_{\nu = \mu-w_0}^{\mu+w_0} \Lambda_{\mu\nu}^{(0)} \sum_{i_\mu, j_\nu=1}^n X_{i_\mu}X_{j_\nu}S_{i_\mu}S_{j_\nu} 
+ \sum_{\mu=0}^L \Lambda_{\mu\mu}^{(0)} \sum_{i_\mu=1}^n X_{i_\mu}^2 S_{i_\mu}^2 \Big) \Big\ra_{t} \Big],
\label{eq:derivative_interpolation}
\end{align}  
%
where $\la - \ra_t$ denotes the expectation over the posterior distribution associated with the interpolated Hamiltonian $\mathcal{H}_{\rm int}(t,\bold{\Lambda}^{(1)},\bold{\Lambda}^{(0)})$.
We start with a simple differentiation of the Hamiltonian w.r.t. $t$ which yields
\begin{align*}
\frac{d}{dt}\mathcal{H}_{\rm int}(t,\bold{\Lambda}^{(1)},\bold{\Lambda}^{(0)}) = \frac{1}{\Delta} \big( \mathcal{A}(t,\bold{\Lambda^{(1)}}) - \mathcal{B}(t,\bold{\Lambda}^{(0)}) \big),
\end{align*}
where
\begin{align*}
\mathcal{A}(t,\bold{\Lambda}^{(1)}) = & \sum_{\mu=0}^L \Lambda_{\mu\mu}^{(1)} \sum_{i_\mu\le j_\mu}\bigg( \frac{x_{i_\mu}^2x_{j_\mu}^2}{2n} 
-  \frac{s_{i_\mu}s_{j_\mu}x_{i_\mu}x_{j_\mu}}{n} - \frac{x_{i_\mu}x_{j_\mu}z_{i_\mu j_\mu} \sqrt{\Delta}}{2\sqrt{n t\Lambda_{\mu\mu}^{(1)}}}\bigg)\nonumber\\
%
+& \sum_{\mu=0}^L\sum_{\nu=\mu+1}^{\mu+w_1}\Lambda_{\mu\nu}^{(1)}\sum_{i_\mu,j_\nu=1}^{n}\bigg( \frac{x_{i_\mu}^2x_{j_\nu}^2}{2n} 
-  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n} - \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu} \sqrt{\Delta}}{2\sqrt{nt\Lambda_{\mu\nu}^{(1)}}}\bigg)\nonumber \\
%
\mathcal{B}(t,\bold{\Lambda}^{(0)}) = &\sum_{\mu=0}^L \Lambda^{(0)}_{\mu\mu} \sum_{i_\mu\le j_\mu}\bigg( \frac{x_{i_\mu}^2x_{j_\mu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\mu}x_{i_\mu}x_{j_\mu}}{n} - \frac{x_{i_\mu}x_{j_\mu}z^{\prime}_{i_\mu j_\mu} \sqrt{\Delta}}{2\sqrt{n (1-t)\Lambda^{(0)}_{\mu\mu}}}\bigg)\nonumber\\
%
& \sum_{\mu=0}^L\sum_{\nu=\mu+1}^{\mu+w_0}\!\Lambda^{(0)}_{\mu\nu}\!\sum_{i_\mu,j_\nu=1}^{n}\!\bigg( \frac{x_{i_\mu}^2x_{j_\nu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n} - \frac{x_{i_\mu}x_{j_\nu}z^{\prime}_{i_\mu j_\nu} \sqrt{\Delta}}{2\sqrt{n(1-t)\Lambda^{(0)}_{\mu\nu}}}\bigg) .
\end{align*}
%
%Note that for a prior $P_0$ with finite support, both $ A(\bx,t,\bold{\Lambda})$ and $ B(\bx,t,\bold{\Lambda}^0) $ are dominated by functions integrable w.r.t. the posterior distribution associated to $\mathcal{H}_{\rm int}(\bx,t,\bold{\Lambda},\bold{\Lambda}^0)$. Hence, by the dominated convergence theorem we get
%\begin{align*}
%\frac{d\ln (\mathcal{Z}_{\rm int}(t))}{dt} 
%= -\int \frac{d\bx P_0(\bx) e^{-\mathcal{H}_{\rm int}}}{\mathcal{Z}_{\rm int}(t)}\partial_t \mathcal{H}_{\rm int}
%= -\langle \partial_t \mathcal{H}_{\rm int}\rangle_{t}  = -\frac{1}{\Delta} \langle  \mathcal{A}(\bX,t,\bold{\Lambda}) - \mathcal{B}(\bX,t,\bold{\Lambda}^0) \rangle_{t}, 
%\end{align*}
%Similarly, one can apply the dominated convergence theorem on $\langle A(\bx,t,\bold{\Lambda})\rangle_t$ and $\langle B(\bx,t,\bold{\Lambda}^0)  \rangle_t$ to get
%\begin{align}\label{eq:derivative_freeEnergy_interpolation}
%\frac{df_{\rm int}(t)}{dt} 
%= \frac{-1}{n(L+1)} \mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}\Big[\frac{d\ln (\mathcal{Z}_{\rm int}(t))}{dt} \Big]
%= \frac{1}{\Delta n(L+1)}\mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}[\langle \mathcal{A}(\bX,t,\bold{\Lambda}) - \mathcal{B}(\bX,t,\bold{\Lambda}^0)\rangle_{t}].
%\end{align}
%We then compute $\mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}[Z_{i_\mu j_\nu} \langle X_{i_\mu} X_{j_\nu}  \rangle_{t}]$ and $\mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}[Z^{\prime}_{i_\mu j_\nu} \langle X_{j_\mu} X_{j_\nu}\rangle_{t}]$ using Gaussian integration by part. For instance, we have that $\mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}[Z_{i_\mu j_\nu} \langle X_{i_\mu} X_{j_\nu}  \rangle_{t}] = \mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}[ \partial_{Z_{i_\mu j_\nu}} \langle X_{i_\mu} X_{j_\nu}  \rangle_{t}]$. Furthermore, by using the dominated convergence theorem twice, one obtains
%\begin{align*}
%&\partial_{z_{i_\mu j_\nu}} \mathcal{Z}_{\rm int}(t) =  -\int d\bx P_0(\bx) e^{-\mathcal{H}_{\rm int}}\partial_{z_{i_\mu j_\nu}} \mathcal{H}_{\rm int}= \sqrt{\frac{t\Lambda_{\mu,\nu}}{n\Delta}} \mathcal{Z}_{\rm int}(t) \langle X_{i_\mu} X_{j_\nu}  \rangle_{t} \nonumber \\
%%
%&\partial_{z_{i_\mu j_\nu}} \langle X_{i_\mu} X_{j_\mu}  \rangle_{t} = \sqrt{\frac{t\Lambda_{\mu,\nu}}{n\Delta}} \bigg( \langle X_{i_\mu}^2 X_{j_\nu}^2  \rangle_{t} - \langle X_{i_\mu} X_{j_\nu}  \rangle_{t}^2 \bigg).
%\end{align*}
Using integration by parts with respect to the Gaussian variables $Z_{ij}$, $Z_{ij}^\prime$, one gets
%
\begin{align}
&\mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}[Z_{i_\mu j_\nu} \langle X_{i_\mu} X_{j_\nu}  \rangle_{t}] =  \sqrt{\frac{t\Lambda_{\mu,\nu}}{n\Delta}}  \mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}\Big[ \langle X_{i_\mu}^2 X_{j_\nu}^2  \rangle_{t} - \langle X_{i_\mu} X_{j_\nu}  \rangle_{t}^2 \Big]
\label{intfirst}
\\
%
&\mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}[Z^{\prime}_{i_\mu j_\nu} \langle X_{i_\mu} X_{j_\nu}  \rangle_{t}] =  \sqrt{\frac{(1-t)\Lambda^0_{\mu,\nu}}{n\Delta}}  \mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}\Big[ \langle X_{i_\mu}^2 X_{j_\nu}^2  \rangle_{t} - \langle X_{i_\mu} X_{j_\nu}  \rangle_{t}^2 \Big].
\label{eq:derivative_freeEnergy_integrationByPart}
\end{align}
Moreover an application of the Nishimori identity \eqref{eq:nishCond} shows
\begin{align}\label{eq:derivative_freeEnergy_nishimori}
\mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}[ \langle X_{i_\mu} X_{j_\nu}  \rangle_{t}^2 ] = \mathbb{E}_{\bf S, \bf Z, \bf Z^{\prime}}[ \langle X_{i_\mu} X_{j_\nu}  S_{i_\mu} S_{j_\nu} \rangle_{t} ].
\end{align}
Combining \eqref{eq:derivative_interpolation}-\eqref{eq:derivative_freeEnergy_nishimori} and using the fact that the SC system defined on a ring satisfies
\begin{align*}
&\sum_{\mu=0}^L \Lambda_{\mu\mu} \sum_{i_\mu\le j_\mu} x_{i_\mu} x_{j_\mu}s_{i_\mu} s_{j_\mu} + \sum_{\mu=0}^L\sum_{\nu=\mu+1}^{\mu+w}\Lambda_{\mu\nu}\sum_{i_\mu,j_\nu=1}^{n} x_{i_\mu} x_{j_\nu} s_{i_\mu} s_{j_\nu} = \\
%
&\frac{1}{2} \sum_{\mu=0}^L\sum_{\nu=\mu-w}^{\mu+w}\Lambda_{\mu\nu}\sum_{i_\mu,j_\nu=1}^{n} x_{i_\mu} x_{j_\nu} s_{i_\mu} s_{j_\nu} + \frac{1}{2} \sum_{\mu=0}^L \Lambda_{\mu\mu} x_{i_\mu}^2 s_{i_\mu}^2,
\end{align*}
we obtain \eqref{eq:derivative_interpolation}.

%
Now, define the {\it overlaps} associated to each block $\mu$ as 
%
\begin{align}
q_\mu \defeq \frac{1}{n} \sum_{i_\mu=1}^n X_{i_\mu}S_{i_\mu}, \qquad \tilde{q}_\mu \defeq \frac{1}{n} \sum_{i_\mu=1}^n X_{i_\mu}^2 S_{i_\mu}^2.
\end{align}
%
Hence, (\ref{eq:derivative_interpolation}) can be rewritten as
%
\begin{align} \label{eq:derivative_interpolation_overlap}
 \frac{di_{\rm int}(t)}{dt} = \frac{1}{4\Delta(L+1)} \mathbb{E}_{{\bf S}, {\bf Z},{\bf Z}^{\prime}} \Big[\Big\la\mathbf{q}^{\intercal} \mathbf{\Lambda}^{(0)} \, \mathbf{q} -\mathbf{q}^{\intercal} 
 \mathbf{\Lambda}^{(1)} \, \mathbf{q} + \frac{1}{n} \, \Big(\tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}}^{(0)}) - \tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}^{(1)}}) \Big) \Big\ra_t \Big],
\end{align} 
%
where $\mathbf{q}^\intercal = [q_0\cdots q_L]$, $\tilde{\mathbf{q}}^\intercal = [\tilde{q}_0\cdots \tilde{q}_L]$ are row vectors and 
${\rm diag} ({\mathbf{\Lambda}})$ represents the column vector with entries $\{\Lambda_{\mu\mu}\}_{\mu=0}^L$.
The coupling matrices $\mathbf{\Lambda}^{(1)}, \mathbf{\Lambda}^{(0)}$ are real, symmetric, circulant (due to the periodicity of the ring) and thus can be diagonalized in the same Fourier basis. 
% Call $\mathbf{U}$ ($\mathbf{U}^0$) the orthogonal matrix which rows forms the eigenbasis of $\mathbf{\Lambda}$ ($\mathbf{\Lambda}^0$ resp.) and $\mathbf{D}$ ($\mathbf{D}^0$ resp.) the diagonal matrix with the associated eigenvalues. 
%
% \begin{align} \label{eq:derivative_interpolation_diagonalization}
% 4\Delta \frac{df_n(t)}{dt} = \mathbb{E} \Big[({\mathbf{U}^0\mathbf{q}})^{\intercal} \mathbf{D}^0 \, (\mathbf{U}^0\mathbf{q}) - (\mathbf{Uq})^{\intercal}\mathbf{D} \, (\mathbf{Uq}) + \frac{1}{n} \, \Big(\tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}}^0) - \tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}}) \Big) \Big].
% \end{align}
%
We have
%
\begin{align} \label{eq:derivative_generic_Fourier}
\frac{di_{\rm int}(t)}{dt} = \frac{1}{4\Delta (L+1)} \mathbb{E}_{{\bf S}, {\bf Z},{\bf Z}^{\prime}} \Big[ \Big\la \hat{\mathbf{q}}^{\intercal} 
\big(\mathbf{D}^{(0)} - \mathbf{D}^{(1)}\big) \, \hat{\mathbf{q}} + \frac{1}{n} \, \Big(\tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}}^{(0)}) 
- \tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}^{(1)}}) \Big)\Big\ra_t \Big],
\end{align}
%
where $\widehat{\mathbf{q}}$ is the discrete Fourier transfrom of $\mathbf{q}$ and $\mathbf{D}^{(1)}, \mathbf{D}^{(0)}$ are 
the diagonal matrices with the eigenvalues of $\mathbf{\Lambda}^{(1)},\mathbf{\Lambda}^{(0)}$. Since the coupling matrices are stochastic with non-negative Fourier transform, their
largest eigenvalue equals $1$ (and is associated to the $0$-th Fourier mode) while the remaining eigenvalues are non-negative. These properties will be essential in the following paragraphs. 
%
\subsection{Applications}\label{appli}
%
Our first application is
%
\begin{lemma}\label{lemma:freeEnergy_sandwich} 
Let the coupling matrix $\Lambda$ verify the requirements (i)-(v) in Sec. \ref{subsec:SC}.
The mutual informations of the decoupled, periodic SC and fully connected systems verify 
\begin{align}
 i_{n, L}^{\rm{dec}} \le i_{n, w, L}^{\rm per} \le i_{n, L}^{\rm con}.
\end{align}
\end{lemma}
%
\begin{proof}
We start with the second inequality. We choose $\Lambda_{\mu\nu}^{(1)} = (L+1)^{-1}$ for the fully connected system at $t=1$. This matrix 
has a unique eigenvalue equal to $1$ and $L$ degenerate eigenvalues equal to $0$. Therefore it is clear 
that $\mathbf{D}^{(0)} - \mathbf{D}^{(1)}$ is positive semi-definite and 
$\hat{\mathbf{q}}^{\intercal} \big(\mathbf{D}^{(0)} - \mathbf{D}^{(1)}\big)\hat{\mathbf{q}}\geq 0$.
Moreover notice that $\Lambda_{\mu\mu}^{(0)} = \Lambda_{00}$ is independent of $L$. Therefore for $L$ large enough
\begin{align}
\tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}}^{(0)}) - \tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}^{(1)}}) = 
\Big(\Lambda_{00}-\frac{1}{L+1}\Big) \sum_{\mu=0}^L\tilde{q}_{\mu} \geq 0.
\end{align}
Therefore we conclude that \eqref{eq:derivative_generic_Fourier} is positive and from \eqref{calc} $i_{n,L}^{\rm con} - i_{n, w, L}^{\rm per} \geq 0$. 
For the first inequality we proceed similarly, but this time we choose $\Lambda_{\mu\nu}^{(1)} = \delta_{\mu\nu}$ for the decoupled system which has all eigenvalues equal to $1$. Therefore 
$\mathbf{D}^{(0)} - \mathbf{D}^{(1)}$ is negative semidefinite so $\hat{\mathbf{q}}^{\intercal} \big(\mathbf{D}^{(0)} - \mathbf{D}^{(1)}\big)\hat{\mathbf{q}}\leq 0$. Moreover this time
\begin{align}
\tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}}^{(0)}) - \tilde{\mathbf{q}}^{\intercal} {\rm diag} ({\mathbf{\Lambda}^{(1)}}) = 
\Big(\Lambda_{00}-1\Big) \sum_{\mu=0}^L\tilde{q}_{\mu} \leq 0
\end{align}
because we necessarily have $0\leq \Lambda_{00}^{(0)} \leq 1$. We conclude that \eqref{eq:derivative_generic_Fourier} is 
negative and from \eqref{calc} $i_{n, L}^{\rm{dec}} - i_{n, w, L}^{\rm per}\leq 0$.
\end{proof}
 
The second application is 

%
\begin{lemma}\label{lemma:superadditivity}
Consider the mutual information of system \eqref{eq:mainProblem} and set  $i_n = n^{-1}I(\tbf{S}; \bW)$. Consider also $i_{n_1}$ and $i_{n_2}$ the mutual informations 
of two systems of size $n_1$ and $n_2$ with $n= n_1 +n_2$.
The sequence $n i_n$ is superadditive in the sense that  
\begin{align}
 n_1 i_{n_1} + n_2 i_{n_2} \leq n i_n.
\end{align}
Fekete's lemma then implies that $\lim_{n\to +\infty} i_n$ exists. 
\end{lemma}
%
\begin{proof}
The proof is easily obtained by following the generic interpolation method of Sec. \ref{generic} for a coupled system with two spatial positions (i.e. $L+1=2$). We choose 
$\Lambda_{\mu\nu}^{(0)}=\delta_{\mu\nu}$, $\mu,\nu\in{0,1}$ for the ''decoupled`` system and $\Lambda_{\mu\nu}^{(1)}=1/2$ for $\mu,\nu\in{0,1}$ for the ''fully connected`` system.
This analysis is essentially identical to [\cite{guerraToninelli}] were the existence of the thermodynamic limit of the free energy for the Sherrington-Kirkpatrick mean field spin glass is proven. 
\end{proof}
% We use again the interpolation method but this time between an underlying system with $N$ 
% variables (system $1$) and another system made of two decoupled underlying subsystems with 
% respective sizes $N_1$ and $N_2$ such that $N=N_1+N_2$ (system $2$). 
% 
% The Hamiltonian of the interpolated system we are interested in is $\tilde{\mathcal{H}}(\bx,t) = \tilde{\mathcal{H}}_N(\bx,t) + \tilde{\mathcal{H}}_{N_1+N_2}(\bx,1-t)$, where the Hamiltonians of system $1$ and system $2$ are respectively
% %
% \begin{align}
% \tilde{\mathcal{H}}_N(\bx,t) &= \frac{t}{\Delta} \sum_{1 \le i\le j\le N}\bigg[ \frac{x_{i}^2x_{j}^2}{2N} -  \frac{s_{i}s_{j}x_{i}x_{j}}{N} - \frac{x_{i}x_{j}z_{i j} \sqrt{\Delta}}{\sqrt{tN}}\bigg], \\
% \tilde{\mathcal{H}}_{N_1+N_2}(\bx,t) &= \frac{t}{\Delta}  \sum_{1 \le i\le j\le N_1}\bigg[ \frac{x_{i}^2x_{j}^2}{2N_1} -  \frac{s_{i}s_{j}x_{i}x_{j}}{N_1} - \frac{x_{i}x_{j}z^{\prime}_{i j} \sqrt{\Delta}}{\sqrt{tN_1}}\bigg]\nonumber \\
% &+\frac{t}{\Delta}  \sum_{N_1+1 \le i\le j\le N_2}\bigg[ \frac{x_{i}^2x_{j}^2}{2N_2} -  \frac{s_{i}s_{j}x_{i}x_{j}}{N_2} - \frac{x_{i}x_{j}z^{\prime}_{i j} \sqrt{\Delta}}{\sqrt{tN_2}}\bigg]. \label{eq:ham_twoSubs}
% \end{align}
% %
% When the interpolation parameter $t\in[0,1]$ is $1$ we recover system $1$, while at $t=0$ we recover system $2$. As previously done, we study the sign of the derivative w.r.t the interpolation parameter $t$ of the interpolated system's free energy $\tilde{f}(t) = -\mathbb{E}_{{\bf S}, {\bf Z},{\bf Z}^{\prime}}[\ln(\tilde{\mathcal{Z}}(t))]/N$, where $\tilde{\mathcal{Z}}(t)$ is the partition function associated with $\tilde{\mathcal{H}}(\bx,t)$, see \eqref{eq:posterior_partition}. With a slight abuse of notation, we define the overlaps $q \defeq \sum_{i=1}^{N}X_i S_i/N$, $q_1 \defeq \sum_{i=1}^{N_1}X_i S_i/N_1$ and $q_2 \defeq \sum_{i=N_1+1}^{N}X_i S_i/N_2$. Moreover, we denote by $\la \cdot \ra_t$ the posterior expectation associated with $\tilde{\mathcal{H}}(\bx,t)$. Hence, by similar arguments used in the proof of \eqref{eq:derivative_interpolation}, we obtain
% %
% \begin{align}
% 4\Delta\frac{d\tilde{f}(t)}{dt} &= \mathbb{E}_{{\bf S}, {\bf Z},{\bf Z}^{\prime}}\Big[ \Big\la\frac{N_1}{N} q_1^2 + \frac{N_2}{N} q_2^2 -q^2 \Big\ra_t\Big] \nonumber\\
% %
% &= \mathbb{E}_{{\bf S}, {\bf Z},{\bf Z}^{\prime}}\Big[ \Big\la \frac{N_1}{N} q_1^2 + \frac{N_2}{N} q_2^2-\Big( \frac{N_1}{N} q_1 + \frac{N_2}{N} q_2\Big)^2 \Big\ra_t \Big] \ge 0, \label{eq:ineq_last_convexLimit}
% \end{align}
% %
% where the inequality is due to the convexity of $g:x\to x^2$. 
% 
% Now notice that as the two subsystems composing system $2$ are independent (which is reflected by the fact that the Hamiltonian \eqref{eq:ham_twoSubs} is simply the sum of the Hamiltonians of the two subsystems), the free energy of system $2$ is just the weighted sum of the individual free energies of the two subsystems. More formally, define $f_{N_1+N_2}^{\rm u} = -\mathbb{E}_{{\bf S}, {\bf Z},{\bf Z}^{\prime}}[\ln(\mathcal{Z}_{N_1+N_2}(t))]/N$ the free energy of system $2$, where $\mathcal{Z}_{N_1+N_2}(t)$ is the partition function associated with \eqref{eq:ham_twoSubs}. Furthermore, define $f_{N_i}^{\rm u}=-\mathbb{E}_{{\bf S}, {\bf Z},{\bf Z}^{\prime}}[\ln(\mathcal{Z}_{N_i}(t))]/N_i$ the free energy of the subsytem $i\in\{1,2\}$, which is associated to the $i^{th}$ term of the overall Hamiltonian $\eqref{eq:ham_twoSubs}$. Then we have $Nf_{N_1+N_2}^{\rm u} = N_1f_{N_1}^{\rm u} + N_2f_{N_2}^{\rm u}$. Moreover \eqref{eq:ineq_last_convexLimit} proves that $Nf_{N}^{\rm u} \ge Nf_{N_1+N_2}^{\rm u}$. Hence, Lemma \ref{lemma:superadditivity} follows.
% \end{proof}
%


==> v5 arxiv/sections/6_proof.tex <==
\section{Proof of the replica symmetric formula (Theorem \ref{thm1})} \label{sec:proof_theorem}
%
In this section we provide the proof of the RS formula for the mutual information of the underlying model (Theorem \ref{thm1})
for $0 < \Delta \leq \Delta_{\rm opt}$ (Proposition \ref{cor:delta-low-regime}) and then for $\Delta \geq \Delta_{\rm opt}$ (Proposition \ref{for:above-delta-opt}). For $0 < \Delta  \leq \Delta_{\rm opt}$ the proof directly follows form the I-MMSE relation Lemma \ref{lemma:immse}, the replica bound \eqref{eq:guerrabound} and the suboptimality of the AMP algorithm. In this interval the proof doesn't require spatial coupling.
For $\Delta \geq  \Delta_{\rm opt}$ the proof uses the results of Sections \ref{sec:thresh-sat} and \ref{sec:subadditivitystyle} on the spatially coupled model. 

Let us start with two preliminary lemmas.
The first is an I-MMSE relation [\cite{GuoShamaiVerdu}] adapted to the current matrix estimation problem.
%
\begin{lemma}\label{lemma:immse}
Let $P_0$ has finite first four moments.
The mutual information and the matrix-MMSE are related by
\begin{align}\label{eq:GSV}
\frac{1}{n}\frac{d I(\tbf{S}; \tbf{W}) }{d\Delta^{-1}} 
= \frac{1}{4} {\rm Mmmse}_n(\Delta^{-1}) + \mathcal{O}(1/n).
\end{align}
%
\end{lemma}
%
\begin{proof}
\begin{align}
\frac{1}{n}\frac{d I(\tbf{S}; \tbf{W}) }{d\Delta^{-1}} &= 
\frac{1}{2n^2}\mathbb{E}_{\tbf{S}, \tbf {W}}\Big[\sum_{i\leq j} \big(S_iS_j - \mathbb{E}[X_iX_j\vert \tbf{W}]\big)^2\Big] 
\nonumber \\ 
%
&= \frac{1}{4n^2}\mathbb{E}_{\tbf{S}, \tbf {W}}\Big[ \bigl\| \tbf{S}\tbf{S}^{\intercal} - \mathbb{E}[\tbf{X}\tbf{X}^{\intercal}\vert\tbf{W}]\bigr\|_{\rm F}^2 \Big]
+\frac{1}{4n^2}\sum_{i=1}^n \mathbb{E}_{\tbf{S}, \tbf {W}}[(S_i^2 - \mathbb{E}[X_i^2 \vert \bW])^2]
\nonumber \\ 
&= \frac{1}{4} {\rm Mmmse}_n(\Delta^{-1}) + \mathcal{O}(1/n),
\end{align}
%
The proof details for first equality are in Appendix~\ref{app:immse}. The second equality is obatined by completing the sum and accounting for the diagonal terms. The last equality is obtained from 
\begin{align}
\mathbb{E}_{\tbf{S}, \tbf {W}}[(S_i^2 - \mathbb{E}[X_i^2 \vert \bW])^2]& 
= \mathbb{E}[S_i^4] - 2 \mathbb{E}_{S_i, \tbf {W}}[ S_i^2 \mathbb{E}[X_i^2 \vert \bW]] + 
\mathbb{E}_{\bW}[\mathbb{E}[X_i^2 \vert \bW]^2]
\nonumber \\ &
= 
 \mathbb{E}[S_i^4] - \mathbb{E}_{\bW}[\mathbb{E}[X_i^2 \vert \bW]^2]
 \nonumber \\ &
 \leq 
 \mathbb{E}[S_i^4].
\end{align}
where we have used the Nishimori identity 
$\mathbb{E}_{S_i, \tbf {W}}[ S_i^2 \mathbb{E}[X_i^2 \vert \bW]] = \mathbb{E}_{\bW}[\mathbb{E}[X_i^2 \vert \bW]^2]$ in the second equality (Appendix \ref{app:nishi}).
\end{proof}
%
%
\begin{lemma}\label{existence-thermo-limit}
The limit $\lim_{n\to +\infty}n^{-1}I(\tbf{S};\tbf{W})$ exists 
and is a concave, continuous, function of $\Delta$. 
\end{lemma}
%
\begin{proof}
The existence of the limit is the statement of Lemma \ref{lemma:superadditivity} in Sec. \ref{sec:subadditivitystyle}. The continuity follows from the concavity of the mutual information with respect to $\Delta^{-1}$: because the limit of a sequence of concave functions remains concave, and thus it is continuous. To see the concavity notice that the first derivative of the mutual information w.r.t $\Delta^{-1}$ equals the matrix-MMSE (Lemma \ref{lemma:immse}) and that the later cannot increase as a function of $\Delta^{-1}$.
\end{proof}

\subsection{Proof of Theorem \ref{thm1} for $0<\Delta  \leq \Delta_{\rm opt}$}\label{sec:delta-less-delta-opt}
%
\begin{lemma}\label{small-noise-lemma}
Assume $P_0$ is a discrete distribution. Fix $\Delta < \Delta_{\rm AMP}$. The mutual information per variable  is asymptotically given by the RS formula \eqref{rsform}.
\end{lemma}
%
\begin{proof}
By the suboptimality of the AMP algorithm we have
% 
\begin{align}\label{startingpoint}
{\rm Mmse}_{n, \rm AMP}^{(t)}(\Delta^{-1}) \geq {\rm Mmmse}_n(\Delta^{-1}).
\end{align}
%
Taking limits in the order $\lim_{t\to +\infty}\limsup_{n\to +\infty}$ and using \eqref{eq:mseampmatriciel} we find
%
\begin{align}
v^2 - (v-E^{(\infty)})^2 \geq \limsup_{n\to +\infty}{\rm Mmmse}_n(\Delta^{-1}).
\end{align}
%
Furthermore, by applying Lemma \ref{lemma:immse} we obtain 
%
\begin{align}\label{thisineq}
\frac{v^2 - (v-E^{(\infty)})^2}{4} \geq \limsup_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}; \tbf{W}) }{d\Delta^{-1}}.
\end{align}
%
Now, for $\Delta < \Delta_{\rm AMP}$ we have $E^{(\infty)} = E_{\rm good}(\Delta)$ which is the unique and hence {\it global} minimum of $i_{\rm RS}(E; \Delta)$ over $E\in [0,v]$. Moreover, for $\Delta < \Delta_{\rm AMP}$ we have that $E^{(\infty)}(\Delta)$ is continuously differentiable $\Delta^{-1}$ with locally bounded derivative. Thus
\begin{align}\label{first_1}
\frac{d}{d\Delta^{-1}}\Big(\min_{E\in[0,v]}i_{\rm RS}(E; \Delta)\Big)
& =
\frac{di_{\rm RS}}{d\Delta^{-1}}(E^{(\infty)}; \Delta) 
\nonumber \\ &
= 
 \frac{\partial i_{\rm RS}}{\partial E}(E^{(\infty)}; \Delta) \frac{d E^{(\infty)}}{d\Delta^{-1}}
 + \frac{\partial i_{\rm RS}}{\partial\Delta^{-1}}(E^{(\infty)} ; \Delta)
 \nonumber \\ &
=  \frac{\partial i_{\rm RS}}{\partial\Delta^{-1}}(E^{(\infty)} ; \Delta) \nonumber \\
&= \frac{(v-E^{(\infty)})^2 +v^2}{4}
- \frac{\partial \mathbb{E}_{S, Z}[\cdots]}{\partial \Sigma^{-2}}\bigg\vert_{E^{(\infty)}}\frac{\partial\Sigma^{-2}}{\partial\Delta^{-1}}\bigg\vert_{E^{(\infty)}} 
\nonumber \\
&= \frac{v^2 - (v-E^{(\infty)})^2}{4},
\end{align}
where $\mathbb{E}_{S, Z}[\cdots]$ is the expectation that appears in the RS potential \eqref{eq:potentialfunction}. The third equality is obtained from 
%
\begin{align}
\frac{\partial\Sigma^{-2}}{\partial\Delta^{-1}}\bigg\vert_{E^{(\infty)}}  = v -E^{(\infty)}
\end{align}
%
and 
%
\begin{align}
\frac{\partial \mathbb{E}_{S, Z}[\cdots]}{\partial \Sigma^{-2}}\Big\vert_{E^{(\infty)}} = \frac{1}{2}(v-E^{(\infty)}).
\end{align}
%
This last identity immediately follows from
$\frac{\partial i_{\rm RS}}{\partial E}\Big\vert_{E^{(\infty)}} = 0$.
From \eqref{thisineq} and \eqref{first_1}
% $$
% \frac{d}{d\Delta^{-1}}(\min_{E}i_{\rm RS}(E; \Delta)).
% $$
\begin{align}
\frac{d}{d\Delta^{-1}}(\min_{E\in [0,v]}i_{\rm RS}(E; \Delta)) \geq 
\limsup_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}; \tbf{W}) }{d\Delta^{-1}}, \nonumber\\
\end{align}
which is equivalent to 
\begin{align}
\frac{d}{d\Delta}(\min_{E\in [0,v]}i_{\rm RS}(E; \Delta)) \leq 
\liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S};\tbf{W}) }{d\Delta}. 
\label{middlepoint}
\end{align}
%
We now integrate inequality \eqref{middlepoint} over an interval 
$[0, \Delta] \subset [0, \Delta_{\rm AMP}[$
%
\begin{align}
\min_{E\in [0,v]}i_{\rm RS}(E; \Delta) - \min_{E\in [0,v]}i_{\rm RS}(E; 0) 
& \leq 
\int_0^\Delta d\tilde{\Delta}\,\liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}; \tbf{W}) }{d\tilde{\Delta}}
\nonumber \\ &
\leq 
\liminf_{n\to +\infty}\int_0^\Delta d\tilde{\Delta}\,\frac{1}{n}\frac{d I(\tbf{S}; \tbf{W}) }{d\tilde{\Delta}}
\nonumber \\ &
= \liminf_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W}) - H(S).
\end{align}
%
The second inequality uses Fatou's Lemma and the last equality uses that for a discrete prior 
\begin{align}
\lim_{\Delta\to 0_+}I(\tbf{S}; \tbf{W}) = H(\tbf{S}) - \lim_{\Delta\to 0_+}H(\tbf{S}\vert \tbf{W}) =  nH(S).
\end{align}
In Appendix \ref{appendix_smallnoise} an explicit calculation shows that $\min_{E}i_{\rm RS}(E; 0) = H(S)$.  Therefore
%
\begin{align}\label{eq:lower_bound_small}
\min_{E\in [0,v]}i_{\rm RS}(E; \Delta) \leq \liminf_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W}).
\end{align}
%
The final step combines inequality \eqref{eq:lower_bound_small} with the replica bound \eqref{eq:guerrabound} to obtain
%
\begin{align}
\min_{E\in [0,v]}i_{\rm RS}(E; \Delta) & \leq 
\liminf_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W})
\leq 
\limsup_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W})
\leq 
\min_{E\in [0,v]}i_{\rm RS}(E; \Delta).
\end{align}
%
This shows that the limit of the mutual information exists and is equal to the RS formula for $\Delta <\Delta_{\rm AMP}$.
Note that in this proof we did not need the a-priori existence of the limit.
\end{proof}
%
%\begin{remark}
%This proof already shows the existence of the thermodynamic limit for 
%$\Delta < \Delta_{\rm AMP}$. In hindsight this is perhaps not so surprising. Indeed it crucially uses the replica bound \eqref{eq:guerrabound} which itself is based on an interpolation which does not per se show the existence of this limit, but which is quite similar to another interpolation used for showing the existence of the limit for {\it all} $\Delta$ (this other type of interpolation is used in Section~\ref{sec:subadditivitystyle}). 
%\end{remark}
%
\begin{remark}
One can try to apply the same proof idea to the regime $\Delta > \Delta_{\rm RS}$. 
Equations \eqref{startingpoint}-\eqref{middlepoint} work out exactly in the same way
because the AMP fixed point $E^{(\infty)}$ is a {\it global} minimum of $i_{\rm RS}(E; \Delta)$. Then when integrating on $]\Delta, +\infty[\subset [\Delta_{\rm RS}, +\infty[$, one finds 
%
\begin{align}
\limsup_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W}) \leq \min_{E\in [0, v]}i_{\rm RS}(E; \Delta).
\end{align}
%
This essentially gives an alternative proof of \eqref{eq:guerrabound} for $\Delta > \Delta_{\rm RS}$.
\end{remark}
%

\begin{lemma}\label{suboptimality}
We necessarily have $\Delta_{\rm AMP} \leq \Delta_{\rm opt}$.
\end{lemma}
%
\begin{proof}
Notice first that it not possible to have $\Delta_{\rm RS} < \Delta_{\rm AMP}$ because in the range $]0, \Delta_{\rm AMP}[$, as a function of $E$, the function $i_{\rm RS}(E;\Delta)$ has a unique stationary point. Since $\min_{E\in [0,v]} i_{\rm RS}(E; \Delta)$ is analytic
for $\Delta < \Delta_{\rm RS}$, it is analytic for $\Delta <\Delta_{\rm AMP}$. Now we proceed by contradiction: suppose we would have $\Delta_{\rm AMP} \geq \Delta_{\rm opt}$. Lemma \ref{small-noise-lemma} asserts 
that $\lim_{n\to +\infty} n^{-1} I(\tbf{S}; \bW) = \min_{E\in [0,v]} i_{\rm RS}(E; \Delta)$ for $\Delta < \Delta_{\rm AMP}$ thus we would have 
$\lim_{n\to +\infty} n^{-1} I(\tbf{S}; \bW)$ analytic at $\Delta_{\rm opt}$. This is a contradiction by definition of $\Delta_{\rm opt}$.
\end{proof}

%
\begin{lemma}\label{analyticity-argument-lemma}
We necessarily have $\Delta_{\rm RS} \geq \Delta_{\rm opt}$. 
\end{lemma}
%
\begin{proof}
If $\Delta_{\rm RS} =+\infty$ then we are done, so we suppose it is finite. The proof 
proceeds by contradiction: suppose $\Delta_{\rm RS} < \Delta_{\rm opt}$.  So we assume $\Delta_{\rm RS}\in [\Delta_{\rm AMP}, \Delta_{\rm opt}[$ (in the previous lemma we showed that this must be the case). For $\Delta \in \, ]0, \Delta_{\rm RS}[$ we have $\min_{E\in [0, v]}i_{\rm RS}(E; \Delta) = i_{\rm RS}(E_{\rm good}(\Delta); \Delta)$ which is an analytic function  in this interval. By definition of $\Delta_{\rm opt}$, the function 
$\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W})$ is analytic in $]0, \Delta_{\rm opt}[$. Therefore {\it both functions are analytic on} $]0, \Delta_{\rm RS}[$ and since by Lemma~\ref{small-noise-lemma} they are equal for $]0, \Delta_{\rm AMP}[\subset ]0, \Delta_{\rm RS}[$, {\it they must 
be equal on the whole range} $]0, \Delta_{\rm RS}[$. This implies that the two functions are equal at $\Delta_{\rm RS}$ because they are continuous. Explicitly,
%
\begin{align}\label{eq:equalityatpoint}
\min_{E}i_{\rm RS}(E; \Delta) = \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W})\vert_{\Delta} \qquad  \forall \ \Delta \in \, ]0, \Delta_{\rm RS}].
\end{align}
%
Now, fix some $\Delta \in \, ]\Delta_{\rm RS}, \Delta_{\rm opt}[$. Since this $\Delta$ is greater than $\Delta_{\rm RS}$ the fixed point of state evolution $E^{(\infty)}$ is also the global minimum of $i_{\rm RS}(E;\Delta)$. Hence 
exactly as in \eqref{startingpoint}-\eqref{middlepoint} we can show that for 
$\Delta \in \, ]\Delta_{\rm RS}, \Delta_{\rm opt}[$, \eqref{middlepoint} is verified.
% %
% \begin{align}\label{contra}
% \frac{d}{d\Delta}(\min_{E}i_{\rm RS}(E; \Delta)) \leq 
% \liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^\intercal; \tbf{W}) }{d\Delta}.
% \end{align}
% %
This time, combining \eqref{eq:guerrabound}, \eqref{middlepoint} and the assumption $\Delta_{\rm RS}\in [\Delta_{\rm AMP}, \Delta_{\rm opt}[$, leads to a 
contradiction, and hence we must have $\Delta_{\rm RS} \geq \Delta_{\rm opt}$. To see explicitly how the contradiction appears, integrate \eqref{middlepoint} 
on $]\Delta_{\rm RS}, \Delta[\subset ]\Delta_{\rm RS}, \Delta_{\rm opt}[$, and use Fatou's Lemma, to obtain
%
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) - \min_{E}i_{\rm RS}(E; \Delta_{\rm RS})
\leq & \liminf_{n\to +\infty}\Big(\frac{1}{n}I(\tbf{S}; \tbf{W})\vert_{\Delta} - \frac{1}{n}I(\tbf{S}; \tbf{W})\vert_{\Delta_{\rm RS}}\Big)
\nonumber \\
=& 
\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W})\vert_{\Delta} - 
\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W})\vert_{\Delta_{\rm RS}}.
\end{align}
%
From \eqref{eq:equalityatpoint} and \eqref{eq:guerrabound} we obtain 
$\min_{E}i_{\rm RS}(E; \Delta) = \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}; \tbf{W})$ 
{\it when} $\Delta_{\rm AMP} \leq \Delta_{\rm RS} < \Delta < \Delta_{\rm opt}$. But from \eqref{eq:equalityatpoint}, this equality is also true for $0 < \Delta \leq \Delta_{\rm RS}$. So the equality is valid in the whole interval $]0, \Delta_{\rm opt}[$ and therefore $\min_{E}i_{\rm RS}(E; \Delta)$ is analytic at $\Delta_{\rm RS}$. But this is impossible by the definition of $\Delta_{\rm RS}$. 
\end{proof} 
%
\begin{proposition}\label{cor:delta-low-regime}
Assume $P_0$ is a discrete distribution. Fix $\Delta \leq \Delta_{\rm opt}$. The mutual information per variable  is asymptotically given by the RS formula \eqref{rsform}.
\end{proposition}
%
\begin{proof}
Lemma~\ref{small-noise-lemma} says that the two functions, $\lim_{n\to +\infty} n^{-1}I(\tbf{S}; \bW)$ and $\min_{E\in [0, v]} i_{\rm RS}(E; \Delta)$, are equal for $\Delta <\Delta_{\rm AMP}$ and Lemma~\ref{analyticity-argument-lemma} implies that {\it both} functions are analytic for $\Delta <\Delta_{\rm opt}$. Thus they must be equal on the whole range $\Delta < \Delta_{\rm opt}$. Since we also know they are continuous, then they are equal also at $\Delta =\Delta_{\rm opt}$.
\end{proof}
%
\subsection{Proof of Theorem \ref{thm1} for $\Delta \geq  \Delta_{\rm opt}$}\label{sec:everything-together}
%
We first need the following lemma where spatial coupling comes into the play.

\begin{lemma}\label{cor:equality-of-deltas}
The optimal threshold is given by the potential threshold: $\Delta_{\rm opt} = \Delta_{\rm RS}$.
\end{lemma}

\begin{proof}
It suffices to see that 
\begin{align}
\Delta_{\rm RS}\leq \Delta^{\rm c}_{\rm AMP}\leq \Delta^{\rm c}_{\rm opt} = \Delta_{\rm opt} \leq \Delta_{\rm RS}.
\end{align}
The first inequality is the threshold saturation result of Theorem \ref{thres-sat-lemma} in Section \ref{sec:thresh-sat}. The second inequality is due the suboptimality of the AMP algorithm.\footnote{More precisely one shows by the same methods Lemmas \ref{small-noise-lemma} and \ref{suboptimality} for the spatially coupled system.}
%This inequality holds because 
%we know that state evolution tracks the AMP algorithm for the spatially coupled system (see {\bf NEW SECTION/LEMMA TO ADD ???}).
The equality is a consequence of Theorem \ref{LemmaGuerraSubadditivityStyle} in Section \ref{sec:subadditivitystyle}. Indeed, equality of asymptotic mutual informations of the coupled and underlying system implies that they must be non-analytic at the same value of $\Delta$. 
Finally, the last inequality is the statement of Lemma \ref{analyticity-argument-lemma} in Section \ref{sec:delta-less-delta-opt}.
\end{proof}

\begin{proposition}\label{for:above-delta-opt}
Assume $P_0$ is a discrete distribution. Fix $\Delta \geq \Delta_{\rm opt}$. The mutual information per variable  is asymptotically given by the RS formula \eqref{rsform}.
\end{proposition}

\begin{proof}
We already remarked in section \ref{sec:delta-less-delta-opt} that for $\Delta > \Delta_{\rm RS}$,
\begin{align}
\frac{d}{d\Delta}(\min_{E}i_{\rm RS}(E; \Delta)) \leq 
\liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S};\tbf{W}) }{d\Delta}. 
\end{align}
Now we integrate on an interval $]\Delta_{\rm RS}, \Delta]$ both sides of the inequality. 
Since from Lemma \ref{cor:equality-of-deltas} we have that $\Delta_{\rm RS} = \Delta_{\rm opt}$, it is equivalent to integrate from 
$\Delta_{\rm opt}$ upwards\footnote{This is the point we did not yet know in section \ref{sec:delta-less-delta-opt}.}
\begin{align}
\int_{\Delta_{\rm opt}}^{\Delta}d\tilde{\Delta}\, \frac{d}{d\tilde{\Delta}}(\min_{E}i_{\rm RS}(E; \tilde{\Delta})) \leq 
\int_{\Delta_{\rm opt}}^{\Delta} d\tilde{\Delta}\, \liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S};\tbf{W}) }{d\tilde{\Delta}}.
\end{align}
By Fatou's lemma the inequality is preserved if we bring the $\liminf$ outside of the integral, thus
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) - \min_{E}i_{\rm RS}(E; \Delta_{\rm RS}) & \leq \liminf_{n\to +\infty}\biggl\{
\frac{1}{n}I(\tbf{S};\tbf{W})\Big\vert_{\Delta} -  \frac{1}{n}I(\tbf{S};\tbf{W})\Big\vert_{\Delta_{\rm opt}}\biggr\}
\nonumber \\ &
= \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S};\tbf{W})\Big\vert_{\Delta} -  
\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S};\tbf{W})\Big\vert_{\Delta_{\rm opt}}.
\end{align}
To get the last line we have used the existence of the thermodynamic limit (see Lemma \ref{existence-thermo-limit}).
But we already know from Proposition \ref{cor:delta-low-regime} that 
$\min_{E}i_{\rm RS}(E; \Delta_{\rm opt}) = \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S};\tbf{W})\Big\vert_{\Delta_{\rm opt}}$. Therefore
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) \leq \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S};\tbf{W}),
\end{align}
which together with \eqref{eq:guerrabound} ends the proof.
\end{proof}


==> v5 arxiv/sections/7_proof_corollaries.tex <==
\section{Proof of corollaries \ref{cor:MMSE} and \ref{perfamp}} \label{sec:proof_coro}
%
In this section, we provide the proofs of Corollary \ref{cor:MMSE} and Corollary \ref{perfamp} concerning the MMSE formulae and the optimality of the AMP algorithm.
We first show the following result about the matrix and vector MMSE's in Definition \ref{def:mmse}.
%
\begin{lemma}\label{lemma:Mmmse}
Assume the prior $P_0$ has finite first four moments and recall the second moment is called $v$. The matrix and vector MMSE verify
%
\begin{align}
{\rm Mmmse}_n
\le \big( v^2-(v - {\rm Vmmse}_n)^2 \big) + \mathcal{O}(\frac{1}{n}).
\end{align}
%
\end{lemma}
%
\begin{proof}
For this proof we denote $\langle \cdot \rangle $ the expectation w.r.t the posterior distribution \eqref{eq:posterior_dist}. The matrix and vector MMSE then read
%
\begin{align}
{\rm Mmmse}_{n} &\defeq \frac{1}{n^2}\mathbb{E}_{\bS, \bW}\Big[ \bigl\| \bS\bS^{\intercal} - \langle\bX\bX^{\intercal}\rangle \bigr\|_{\rm F}^2 \Big], \label{eq:matrix_mmse}\\ 
{\rm Vmmse}_{n} &\defeq \frac{1}{n}\mathbb{E}_{\bS, \bW}\Big[ \bigl\| \bS - \langle\bX\rangle \bigr\|_{2}^2 \Big]. \label{eq:vector_mmse}
\end{align}
%
Expanding the Frobenius norm in (\ref{eq:matrix_mmse}) yields
%
\begin{align}
{\rm Mmmse}_{n} &= \frac{1}{n^2}\mathbb{E}_{\bS, \bW}\Big[ \sum_{i,j=1}^n ( S_i S_j - \langle X_i X_j\rangle)^2 \Big] =\frac{1}{n^2}\mathbb{E}_{\bS, \bW}\Big[ \sum_{i,j=1}^n  S_i^2 S_j^2 - \langle X_i X_j\rangle^2 \Big] \nonumber \\
&= \mathbb{E}_{\bS}\Big[\Big(\frac{1}{n}\sum_{i=1}^n S_i^2\Big)^2 \Big] - \frac{1}{n^2} \sum_{i,j=1}^n \mathbb{E}_{\bS, \bW}[\langle X_i X_j \rangle^2], 
\end{align}
%
where the second equality follows from $\mathbb{E}_{\bS, \bW}[\langle X_i X_j\rangle^2]=\mathbb{E}_{\bS, \bW}[ S_i S_j \langle X_i X_j\rangle]$, implied by the Nishimori 
identity \eqref{eq:nishCond}. Similarly, using $\mathbb{E}_{\bS, \bW} [\langle X_i \rangle^2] = \mathbb{E}_{\bS, \bW} [S_i \langle X_i\rangle]$ implied by the Nishimori identity, 
(\ref{eq:vector_mmse}) simplifies to
%
\begin{align}
{\rm Vmmse}_{n} = v - \frac{1}{n}\sum_{i=1}^n \mathbb{E}_{\bS, \bW}[\langle X_i\rangle^2 ].
\end{align}
%
Hence,
\begin{align}
{\rm Mmmse}_n
-  \big( v^2-(v - {\rm Vmmse}_n)^2 \big) = \mathcal{A}_{n} - \mathcal{B}_{n},
\end{align}
with
%
\begin{align}
\mathcal{A}_{n} &\defeq  \mathbb{E}_{\bS}\Big[\Big(\frac{1}{n}\sum_{i=1}^n S_i^2\Big)^2 \Big] - v^2, \\
\mathcal{B}_{n} &\defeq \frac{1}{n^2} \sum_{i,j=1}^n \Big(\mathbb{E}_{\bS, \bW}[ \langle X_i X_j \rangle^2 ] - \mathbb{E}_{\bS, \bW}[\langle X_i \rangle^2 ]\mathbb{E}_{\bS, \bW}[\langle X_j \rangle^2 ]\Big).\label{eq:Mmmse_Vmmse_diff_1}
\end{align}
%
Since the signal components $\{S_i\}$ are i.i.d and $P_0$ has finite first four moments, $\mathcal{A}_n = \mathcal{O}(1/n)$. 
It remains to show that $\mathcal{B}_n \geq 0$. This is most easily seen as follows. By defining the {\it overlap}
\begin{align}
 q(\bX,\bS) \defeq \frac{1}{n}\sum_{i=1}^n S_iX_i
\end{align}
and using the Nishimori identities
$\mathbb{E}_{\bS, \bW}[\langle X_i \rangle^2 ] = \mathbb{E}_{\bS, \bW}[S_i\langle X_i \rangle ]$ and $\mathbb{E}_{\bS, \bW}[\langle X_i X_j\rangle^2]=\mathbb{E}_{\bS, \bW}[ S_i S_j \langle X_i X_j\rangle]$, 
we observe that 
%
\begin{align}
\mathcal{B}_{n} & = \mathbb{E}_{\bS, \bW}[ \langle q^2\rangle ] -  \mathbb{E}_{\bS, \bW}[\langle q \rangle]^2 
\nonumber \\ &
=
\mathbb{E}_{\bS, \bW}[ (q - \mathbb{E}_{\bS, \bW}[\langle q \rangle])^2]
% \nonumber \\
% %
% &=  (\mathbb{E}_{\bS, \bW}[ \langle q^2\rangle ] - \mathbb{E}_{\bS, \bW}[ \langle q\rangle^2 ]) + (\mathbb{E}_{\bS, \bW}[\langle q \rangle^2 ] - \mathbb{E}_{\bW}[\mathbb{E}_{\bS}[ \langle q\rangle ]^2] )\nonumber \\
% &\ \ \ +  ( \mathbb{E}_{\bW}[\mathbb{E}_{\bS}[ \langle q\rangle ]^2] -\mathbb{E}_{\bS, \bW}[\langle q \rangle ]^2  )  \nonumber\\
% %
% &=   \mathbb{E}_{\bS,\bW}[ \langle (q - \langle q \rangle )^2\rangle ] + \mathbb{E}_{\bS,\bW}[ ( \langle q\rangle -\mathbb{E}_{\bS}[\langle q\rangle])^2] + \mathbb{E}_{\bW}[(\mathbb{E}_{\bS}[\langle q \rangle ] - \mathbb{E}_{\bS,\bW}[\langle q \rangle ])^2 ]   \nonumber \\
% %
% &\eqdef  \mathcal{B}_{n}^{(1)} + \mathcal{B}_{n}^{(2)} + \mathcal{B}_{n}^{(3)}.
\end{align}
which is non-negative.
%
%All the quadratic terms $\mathcal{B}_{n}^{(i)}$ are positive and the inequality holds. 
\end{proof}
%
\begin{remark}
Using ideas similar to [\cite{KoradaMacris}] to prove concentration of overlaps in inference problems suggest that Lemma \ref{lemma:Mmmse} holds with an equality
when suitable ``side observations'' are added. 
\end{remark}
%
\subsection{Proof of Corollary \ref{cor:MMSE}} \label{sec:proof_coro_1}
%
We first show how to prove the expression \eqref{coro1} for the asymptotic ${\rm Mmmse}_n$ by taking the limit $n\to +\infty$ on both sides of \eqref{eq:GSV}. 
First notice that since $n^{-1} I({\tbf S}; \bW)$ is a sequence of concave functions with respect to $\Delta^{-1}$, the limit when $n\to +\infty$ is also concave 
and differentiable for almost all $\Delta^{-1}$ and at all differentiability points we have (by a standard theorem of real analysis on convex functions)
%
\begin{align}\label{limderexchg}
\lim_{n\to + \infty} \frac{1}{n}\frac{d}{d\Delta^{-1}} I(\tbf{S}; \tbf{W})
= 
 \frac{1}{n}\frac{d}{d\Delta^{-1}}\lim_{n\to + \infty} I(\tbf{S}; \tbf{W})\,.
\end{align}
%
Thus from Lemma \ref{lemma:immse} and Theorem \ref{thm1} we have for all $\Delta \neq \Delta_{\rm RS}$
%
\begin{align}\label{mmseirs}
\lim_{n\to + \infty}{\rm Mmmse}_n(\Delta^{-1}) = 
4 \frac{d}{d\Delta^{-1}}\min_{E\in[0,v]}i_{\rm RS}(E; \Delta).
\end{align}
%
It remains to compute the right hand side. 
Let $E_0(\Delta)$ denote the (global) minimum of $i_{\rm RS}(E; \Delta)$. For $\Delta \neq \Delta_{\rm RS}$ this is a differentiable function of $\Delta$ with locally bounded derivative. 
Hence using a similar calculation to the one done in \eqref{first_1}, we obtain
%
\begin{align}\label{first}
\frac{d}{d\Delta^{-1}}\Big(\min_{E\in[0,v]}i_{\rm RS}(E; \Delta)\Big)
& =
\frac{di_{\rm RS}}{d\Delta^{-1}}(E_{0}; \Delta) 
\nonumber \\ &
= 
 \frac{\partial i_{\rm RS}}{\partial E}(E_{0}; \Delta) \frac{d E_{0}}{d\Delta^{-1}}
 + \frac{\partial i_{\rm RS}}{\partial\Delta^{-1}}(E_{0}; \Delta)
 \nonumber \\ &
=  \frac{\partial i_{\rm RS}}{\partial\Delta^{-1}}(E_{0} ; \Delta).
\end{align}
%
To compute the partial derivative with respect to 
$\Delta$ we first note that $\frac{\partial i_{\rm RS}}{\partial E}\Big\vert_{E_0} = 0$  implies
\begin{align}\label{second}
 0 = -\frac{v-E_0}{2\Delta} - \frac{\partial \mathbb{E}_{S, Z}[\cdots]}{\partial \Sigma^{-2}}\bigg\vert_{E_0} \frac{\partial\Sigma^{-2}}{\partial E}\bigg\vert_{E_0}, 
\end{align}
where $\mathbb{E}_{S, Z}[\cdots]$ is the expectation that appears 
in the RS potential \eqref{eq:potentialfunction}.
This immediately gives 
%
\begin{align}
 \frac{\partial \mathbb{E}_{S, Z}[\cdots]}{\partial \Sigma^{-2}}\Big\vert_{E_0} = \frac{1}{2}(v-E_0)
\end{align}
%
Thus
%
\begin{align}\label{third}
\frac{\partial i_{\rm RS}}{\partial\Delta^{-1}}(E_{0} ; \Delta) & = \frac{(v-E_0)^2 +v^2}{4}
- \frac{\partial \mathbb{E}_{S, Z}[\cdots]}{\partial \Sigma^{-2}}\bigg\vert_{E_0}\frac{\partial\Sigma^{-2}}{\partial\Delta^{-1}}\bigg\vert_{E_0} 
\nonumber \\ &
= \frac{v^2 - (v-E_0)^2}{4}. 
\end{align}
%
From \eqref{mmseirs}, \eqref{first}, \eqref{third} we obtain the desired result, formula \eqref{coro1}.

We now turn to the proof of \eqref{coro2} for the 
expression of the asymptotic vector-MMSE. 
From Lemma \ref{lemma:Mmmse} and the suboptimality of the AMP algorithm (here $E_0(\Delta)$ is the global minimum of $i_{\rm RS}(E;\Delta)$ and 
$E^{(\infty)}$ the fixed point of state evolution)
%
\begin{align}
v^2-(v - E_0)^2 & = \lim_{n\rightarrow\infty} {\rm Mmmse}_n
\nonumber \\ & 
\le \liminf_{n\rightarrow\infty} \big( v^2-(v - {\rm Vmmse}_n)^2 \big) 
\nonumber \\ &
\le 
\limsup_{n\rightarrow\infty} \big( v^2-(v - {\rm Vmmse}_n)^2 \big)
\nonumber \\ &
\le v^2-(v - E^{(\infty)})^2 ,
\end{align}
%
For $\Delta \notin [\Delta_{\rm AMP},\Delta_{\rm RS}]$, we have that $E_0 = E^{(\infty)}$ which ends the proof.   
% 
\subsection{Proof of Corollary \ref{perfamp}} \label{sec:proof_coro_1}
%
In view of \eqref{eq:mseampmatriciel} we have
%
\begin{align}
\lim_{t\to +\infty}\lim_{n\to +\infty} {\rm Vmse}_{n, \rm AMP}^{(t)}(\Delta^{-1}) &= E^{(\infty)},
\label{eq:proofCorollaryAMP_1}
\\
\lim_{t\to +\infty}\lim_{n\to +\infty} {\rm Mmse}_{n, \rm AMP}^{(t)}(\Delta^{-1})
&= v^2 - (v - E^{(\infty)})^2.
\label{eq:proofCorollaryAMP_2}
\end{align}
%
For $\Delta \notin [\Delta_{\rm AMP},\Delta_{\rm RS}]$ we have $E^{(\infty)} = {\rm{argmin}}_{E\in [0, v]} i_{\rm RS}(E; \Delta)$ and also the two formulas of Corrolary \ref{cor:MMSE}
hold. This directly implies the formulas \eqref{ampcoro1} and \eqref{ampcoro2}.  

On the other hand for $\Delta \in [\Delta_{\rm AMP},\Delta_{\rm RS}]$ we have $E^{(\infty)} > {\rm{argmin}}_{E\in [0, v]} i_{\rm RS}(E; \Delta)$, 
so
using the monotonicity of $E^{(t)}$ leads to strict inequalities in \eqref{eq:proofCorollaryAMP_1} and \eqref{eq:proofCorollaryAMP_2} and thus to \eqref{ampsub1} and \eqref{ampsub2}.


==> v5 arxiv/sections/concentration_jean.tex <==
\section{Concentration} \label{app:concentration}
%
In this appendix we prove a concentration equality that is necessary to show formula ?? linking the signal and matrix MMSE.

\section{Concentration of the overlap w.r.t the posterior}
%
In order to show the connection between the matrix-mmse and the vector-mmse, it turns out that we need some concentration properties on the overlap $q \defeq 1/n \sum_i x_i^{(1)}x_i^{(2)}$ between the two independent replicas $x_i^{(1)}$ and $x_i^{(2)}$. For this end, we consider a \emph{perturbed} system with the following Hamiltonian
\begin{align}\label{eq:perturbed_hamiltonian}
\mathcal{H}(\bx,h) &= \frac{1}{\Delta} \sum_{1 \le i\le j\le n}\bigg[ \frac{x_{i}^2x_{j}^2}{2n} -  \frac{s_{i}s_{j}x_{i}x_{j}}{n} - \frac{x_{i}x_{j}z_{i j} \sqrt{\Delta}}{\sqrt{n}} \bigg] + h \sum_i x_i^{(1)}x_i^{(2)},
\end{align}
where a perturbation term $h \sum_i x_i^{(1)}x_i^{(2)}$ is added to the original Hamiltonian (again, the dependence of the Hamiltonian on $\bs,\bz,\Delta$ and $n$ is implicit and dropped from the notation of $\mathcal{H}(\bx,h)$ for readability). Note that $\mathcal{H}(\bx,0)$ corresponds to the Hamiltonian of the original system. However, for some technical reasons that will become clear in the sequel, we work with the perturbed system (\ref{eq:perturbed_hamiltonian}) and then let $h \rightarrow 0$ at the end of the analysis.

Let $Z(h)$ be the partition function associated with $\mathcal{H}(\bx,h)$ and denote by $f_{h,n}$ the free energy of the perturbed system at fixed signal and noise realization with $f_{h,n} =  - \ln \big( Z(h) \big)/n$. Moreover, we denote by $\langle \cdot \rangle_{h}$ the expectation over the posterior distribution associated with $\mathcal{H}(\bx, h)$. Note the the perturbation term has been chosen so that the following lemma holds.
\begin{lemma}\label{lemma:pertubed_energy_concave}
$f_{h,n}$ is concave in $h$.
\end{lemma}
\begin{proof}
By using the dominated convergence theorem, one obtains the following
\begin{align}
\label{eq:perturbed_energy_derivative1}
\frac{d}{dh} f_{h,n} &=  \langle q \rangle_{h} \\
\label{eq:perturbed_energy_derivative2}
\frac{d^2}{dh^2} f_{h,n} &= - n \Big( \langle q^2 \rangle_{h} - \langle q \rangle_{h}^2 \Big) \le 0. 
\end{align}
\end{proof}
Furthermore, it turns out the the overlap $q$ satisfies some concentration properties.
\begin{lemma}\label{lemma:concentration_q}
Concentration of $q$: For any $a >\epsilon>0$ fixed
\begin{align*}
\int_{\epsilon}^{a} dh \mathbb{E} \Big[ \Big\langle \big(q - \langle q \rangle_{h} \big)^2 \Big\rangle_{h} \Big] = \mathcal{O}\Big(\frac{1}{n}\Big).
\end{align*}
\end{lemma}
\begin{proof}
\begin{align*}
\int_{\epsilon}^{a} dh \mathbb{E} \Big[ \Big\langle \big(q - \langle q \rangle_{h} \big)^2 \Big\rangle_{h} \Big]
&= \int_{\epsilon}^{a} dh \mathbb{E} \big[ \langle q^2 \rangle_{h} - \langle q \rangle_{h}^2 \big]
= - \int_{\epsilon}^{a} dh \frac{1}{n} \frac{d^2}{dh^2} \mathbb{E} \big[f_{h,n} \big]\\
&= \frac{1}{n} \Big( \frac{d}{dh} \mathbb{E} \big[f_{\epsilon,n}\big] - \frac{d}{dh} \mathbb{E} \big[f_{a,n}\big] \Big) = \mathcal{O}\Big(\frac{1}{n}\Big),
\end{align*}
where the second equality follows from (\ref{eq:perturbed_energy_derivative2}) and the dominated convergence theorem. The last equality uses the fact that the derivative of $\mathbb{E} \big[f_{h,n}\big]$ is $\mathcal{O}(1)$ for $h\ge\epsilon$, which is valid, by Nishimori condition, for all signal's prior distribution with bounded second moment
\begin{align*}
\frac{d}{dh} \mathbb{E} \big[f_{h,n}\big] =  \frac{1}{n} \sum_i \mathbb{E} \big[ \langle x_i^{(1)}x_i^{(2)} \rangle_{h} \big] = \mathbb{E} \big[ \langle s_i x_i \rangle_{h} \big] \le \mathbb{E} \big[  s_i^2 \big] = v. 
\end{align*} 
\end{proof} 
%
\subsection{Concentration of the overlap w.r.t the disorder}
%
Call the perturbed signal $\tilde \bs = [\tilde s_1, s_2, \ldots,s_n]$, where the first signal component is modified w.r.t $\bs$. It is easy to show that the difference between the Hamiltonian evaluated at $\bs$ and $\tilde\bs$ is simply
%
\begin{align}
\delta \mathcal{H}(\bx,\tilde \bs, \bs) \defeq \mathcal{H}(\bx,\bs, \bz) - \mathcal{H}(\bx,\tilde \bs,\bz) = \frac{x_1(\tilde s_1 - s_1)}{\Delta n}\sum_{j=1}^n s_jx_j \label{eq:deltaH_concentration}
\end{align}
%
Call $\mathcal{Z}(\bs,\bz)=\int d\bx P_0(\bx)\exp(-\mathcal{H}(\bx,\bs,\bz))$ the partition associated with $\mathcal{H}(\bx,\bs)$, and $f(\bs,\bz) = -\ln(\mathcal{Z}(\bs,\bz) )/n$ the associated free energy at fixed signal and noize realizations. We now use similar steps as in Section~\ref{sec:subadditivitystyle} in order to evaluate the difference between the free energy associated with $\mathcal{H}(\bx,\bs, \bz)$ and $\mathcal{H}(\bx,\tilde \bs,\bz)$. Exactly as we obtained \eqref{eq:Z_openVSclosed}, \eqref{eq:Z_openVSclosed_2}, we get
%
\begin{align}
f(\bs,\bz) &= f(\tilde \bs,\bz) - \frac{1}{n}\ln(\langle e^{-\delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)}\rangle_{\mathcal{H}}),\\ 
f(\tilde \bs,\bz) &= f(\bs,\bz) - \frac{1}{n}\ln(\langle e^{\delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)}\rangle_{\tilde{\mathcal{H}}}),
\end{align}
%
where $\langle A(\mathbf{X}) \rangle_{\mathcal{H}} \defeq \mathcal{Z}(\bs,\bz)^{-1}\int d\bx A(\bx) P_0(\bx)\exp(-\mathcal{H}(\bx,\bs,\bz))$ is the expectation w.r.t the posterior associated with $\mathcal{H}(\bx,\bs,\bz)$, and similarly, $\langle A(\mathbf{X}) \rangle_{\tilde{\mathcal{H}}}$ is the the expectation w.r.t the posterior associated with $\mathcal{H}(\bx,\tilde \bs,\bz)$. Combining these two identites and using the convexity of the exponential, we get
%
\begin{align}
f(\tilde \bs,\bz) + \frac{\langle \delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)\rangle_{\mathcal{H}}}{n} \le f(\bs,\bz) \le f(\tilde \bs,\bz) + \frac{\langle \delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)\rangle_{\tilde{\mathcal{H}}}}{n}.
\end{align}
%
Let us now estimate $\langle \delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)\rangle_{\mathcal{H}}/n$. From \eqref{eq:deltaH_concentration} we get
%
\begin{align}
\frac{\langle \delta \mathcal{H}(\mathbf{X},\tilde \bs, \bs)\rangle_{\mathcal{H}}}{n} = \frac{(\tilde s_1-s_1)}{\Delta n^2} \sum_{j=1}^n s_j \langle X_1 X_j\rangle_{\mathcal{H}}
\end{align}
%


==> v5 arxiv/sections/interpolation_subadditivity_style.tex <==
\section{Invariance of the optimal threshold under spatial coupling}\label{sec:subadditivitystyle}
%
In this section, we prove that the Bayesian optimal threshold (defined in (\ref{Deltaopt}) in terms of the mutual information) remains intact under spatial coupling, i.e. $\Delta_{\rm opt}^{\rm c} = \Delta_{\rm opt}$. Note that for a Gaussian noise, the normalized mutual information of the underlying system is equal to the free energy $f^{\rm u}_n$, a fundamental quantity in statistical physics, up to a trivial term
\begin{align}\label{eq:mutual_Information_free_Energy}
\frac{1}{n} I(\tbf{S} \tbf{S}^T ; \tbf{W}) = f^{\rm u}_n + \frac{v^2}{4\Delta}.
\end{align}
Therefore, we will perform our analysis for this section in terms of the free energy.

In statistical physics language, for an underlying system with a given Hamiltonian $\mathcal{H^{\rm u}}$, the posterior probability distribution $p(\bx\vert \bs,\bz)$ and the corresponding partition function $Z$ are
%
\begin{align}\label{eq:posterior_partition}
&p(\bx\vert \bs,\bz) = \frac{P_0(\bx) e^{-\mathcal{H}_{\rm u}}}{Z},\nonumber \\
%
&Z = \int d\bx P_0(\bx) e^{-\mathcal{H}_{\rm u}}.
\end{align}
%
The free energy is then defined as
\begin{align}
f_{n}^{\rm u} = \frac{-\mathbb{E} [\ln (Z)]}{n},
\end{align}
where $\mathbb{E}[\cdot]$ is the average over all the disorders.
In order to prove that $\Delta_{\rm opt}^{\rm c} = \Delta_{\rm opt}$, we introduce four systems of the form (\ref{eq:def_coupledSyst}) having all the same size $n(L+1)$:
\begin{itemize}
\item $S_1$: the fully connected (homogeneous) system having the optimal threshold $\Delta_{\rm opt}^{\rm h}$ and the free energy $f_{ L,n}^{\rm h} = \frac{-\mathbb{E} [\ln (Z_1)]}{n(L+1)}$, where $Z_1$ is the partition function associated to $S_1$, with  coupling window $w_1 = L/2$.
\item $S_2$: the SC system, previously used to show threshold saturation with pinning conditions at the boundaries, having $\Delta_{\rm opt}^{\rm c}$ and $f_{ L,n}^{\rm c}$ with $1<w_2<L/2$. We will refer to this system as the actual SC system.
\item $S_3$: the unpinned SC system (similar to $S_2$ but without pinning conditions) having $\Delta_{\rm opt}^{\rm p}$ and $f_{L,n}^{\rm p}$ with $1<w_3<L/2$.
\item $S_4$: the decoupled system having $\Delta_{\rm opt}^{\rm dec}$ and $f_{L,n}^{\rm dec}$ with $w_4 = 0$.
\end{itemize}
By using the interpolation method twice, between $S_1$ and $S_3$ then between $S_4$ and $S_3$, and knowing that $S_1$ and $S_4$ have the same asymptotic free energy $f^{\rm u} = \lim_{n \rightarrow \infty}f_{n}^{\rm u}$ as the underlying system (and thus the same threshold $\Delta_{\rm opt}$), we prove that $\lim_{n \rightarrow \infty}f_{L,n}^{\rm p} = f^{\rm u}$. Furthermore, we show that pinning the closed chain in $S_2$ results in an energy loss that vanishes with $L$. Therefore, one can deduce that $f_{L,n}^{\rm c} = f_{L,n}^{\rm p}$ by taking $n \rightarrow \infty$ then $L \rightarrow \infty$. Hence, the results $\lim_{L,n \rightarrow \infty}f_{L,n}^{\rm c} = f^{\rm u}$ and $\Delta_{\rm opt}^{\rm c} = \Delta_{\rm opt}$ follow directly. Note that the reason why we used $S_3$ as an intermediate step to proof the result for $S_2$ is because the former is more convenient to perform the interpolation method.
        
In full generality, let us consider two SC systems of size $n(L+1)$ with coupling windows $w$ and $w_0$ respectively. Furthermore, we assume that the two systems are coupled using the matrices $\bold{\Lambda}$ and $\bold{\Lambda}^0$ respectively. We consider that the noise of the first and second SC systems are respectively $\Delta / t$ and $\Delta / (1 - t)$ and we define an interpolated system which Hamiltonian is just the sum of those of the two SC systems, $\mathcal{H}_{\rm int}(t,\bold{\Lambda},\bold{\Lambda}^0) = \mathcal{H}(t,\bold{\Lambda}) + \mathcal{H}(1-t,\bold{\Lambda}^0)$, with
\begin{align*}
\mathcal{H}(t,\bold{\Lambda}) &= \frac{t}{\Delta} \sum_{\mu} \Lambda_{\mu,\mu} \sum_{i_\mu\le j_\mu}\bigg[ \frac{x_{i_\mu}^2x_{j_\mu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\mu}x_{i_\mu}x_{j_\mu}}{n} - \frac{x_{i_\mu}x_{j_\mu}z_{i_\mu j_\mu} \sqrt{\Delta}}{\sqrt{n t\Lambda_{\mu,\mu}}}\bigg]\nonumber\\
%
&+ \frac{t}{\Delta} \sum_{\mu}\sum_{\nu\in \{\mu+1:\mu+w\}}\Lambda_{\mu,\nu}\sum_{i_\mu\le j_\nu}\bigg[ \frac{x_{i_\mu}^2x_{j_\nu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n} - \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu} \sqrt{\Delta}}{\sqrt{nt\Lambda_{\mu,\nu}}}\bigg]\nonumber\\
%
&+ \frac{t}{\Delta} \sum_{\mu}\sum_{\nu\in \{\mu-w:\mu-1\}}\Lambda_{\mu,\nu}\sum_{j_\nu < i_\mu}\bigg[ \frac{x_{i_\mu}^2x_{j_\nu}^2}{2n} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n} - \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu} \sqrt{\Delta}}{\sqrt{nt\Lambda_{\mu,\nu}}}\bigg].
\end{align*}
In this setting, at $t=1$ the interpolated system is the first SC one as the noise is infinitely large in the second SC one and no information is available about it, while at $t=0$ the opposite happens. 
In order to compare any two systems, one is normally interested in computing the derivative of $\mathbb{E}[\ln \big(Z(t)\big)]$ w.r.t. the interpolation parameter $t$. Following the lines of [\cite{krzakala2016mutual}], we obtain
\begin{align} \label{eq:derivative_interpolation}
\partial_t \mathbb{E}[\ln \big(Z(t)\big)] &= \frac{1}{4\Delta n} \Big( \sum_{\mu}\sum_{\nu\in \mathcal{S}_{\mu}^{w}} \Lambda_{\mu,\nu} \sum_{i_\mu, j_\nu}\mathbb{E}[x_{i_\mu}x_{j_\nu}s_{i_\mu}s_{j_\nu}] + \sum_{\mu} \Lambda_{\mu,\mu} \sum_{ i_\mu} \mathbb{E}[x_{i_\mu}^2 s_{i_\mu}^2] \Big) \nonumber \\
&- \frac{1}{4\Delta n} \Big( \sum_{\mu}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} \Lambda_{\mu,\nu}^0 \sum_{i_\mu, j_\nu}\mathbb{E}[x_{i_\mu}x_{j_\nu}s_{i_\mu}s_{j_\nu}] + \sum_{\mu} \Lambda_{\mu,\mu}^0 \sum_{ i_\mu} \mathbb{E}[x_{i_\mu}^2 s_{i_\mu}^2] \Big),
\end{align}  
%
where $\mathcal{S}_{\mu}^{w} = \{\mu-w:\mu+w\}$. We define the overlaps per block as $q_\mu \defeq \frac{1}{n} \sum_{i_\mu} x_{i_\mu}s_{i_\mu}$ and $\tilde{q}_\mu \defeq \frac{1}{n} \sum_{i_\mu} x_{i_\mu}^2 s_{i_\mu}^2$. Hence, (\ref{eq:derivative_interpolation}) can be rewritten as
\begin{align} \label{eq:derivative_interpolation_overlap}
\frac{4\Delta}{ n} \partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E} \Big[ \mathbf{q}^{\intercal} \mathbf{\Lambda} \, \mathbf{q} + \frac{1}{n} \, \tilde{\mathbf{q}}^{\intercal} diag ({\mathbf{\Lambda}})
- \mathbf{q}^{\intercal} \mathbf{\Lambda}^0 \, \mathbf{q} - \frac{1}{n} \, \tilde{\mathbf{q}}^{\intercal} diag ({\mathbf{\Lambda}}^0)
\Big],
\end{align} 
where $\mathbf{q}^{\intercal}  = [q_0:q_L]$, $\tilde{\mathbf{q}}^{\intercal}  = [\tilde{q}_0:\tilde{q}_L]$ and $diag ({\mathbf{\Lambda}})$ represents the column vector with entries $\Lambda_{\mu,\mu}$.  Moreover, the symmetry of the coupling matrix rewrites (\ref{eq:derivative_interpolation_overlap}) as 
\begin{align} \label{eq:derivative_interpolation_diagonalization}
\frac{4\Delta}{ n} \partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E} \Big[ (\mathbf{Uq})^{\intercal}\mathbf{D} \, (\mathbf{Uq}) + \frac{1}{n} \, \tilde{\mathbf{q}}^{\intercal} diag ({\mathbf{\Lambda}})
- ({\mathbf{U}^0\mathbf{q}})^{\intercal} \mathbf{D}^0 \, (\mathbf{U}^0\mathbf{q}) - \frac{1}{n} \, \tilde{\mathbf{q}}^{\intercal} diag ({\mathbf{\Lambda}}^0)
\Big],
\end{align}
where $\mathbf{U}$ and $\mathbf{U}^0$ are the orthogonal matrices obtained by eigenvalue decomposition of $\mathbf{\Lambda}$ and $\mathbf{\Lambda}^0$ respectively, while $\mathbf{D}$ and $\mathbf{D}^0$ are the  corresponding diagonal matrices. Furthermore, since the coupling matrices are doubly-stochastic, the leading eigenvalue in $\mathbf{D}$ and $\mathbf{D}^0$ is always equal to $1$ while the remaining eigenvalues are $\le 1$ in absolute value.

\subsection{The homogeneous VS the coupled systems}
%
We interpolate between $S_1$ (recovered at $t=1$) and $S_3$ (recovered at $t=0$). We represent $S_1$ by setting $w = w_1=L/2$  in (\ref{eq:derivative_interpolation_diagonalization}) and taking a homogeneous coupling matrix with elements $\Lambda_{\mu,\nu} = \frac{1}{L+1}$ for $\nu\in \mathcal{S}_{\mu}^{w}$. $S_3$ is represented by setting $1<w_0=w_3<L/2$ and taking a triangular shape coupling window wiht $\Lambda_{\mu,\nu}^0 = \frac{(w_0+1) - |\mu - \nu|}{(w_0+1)^2}$ for $\nu\in \mathcal{S}_{\mu}^{w_0}$. 

Due to the periodicity of the closed-chain, the coupling matrices are also circulant. Hence, the corresponding eigenvalue decomposition in (\ref{eq:derivative_interpolation_diagonalization}) is nothing but the Discrete Fourier Transform (DFT) given by
\begin{align} \label{eq:derivative_homogeneousVScoupled}
\frac{4\Delta}{ n} \partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E} \Big[ \hat{\mathbf{q}}^{\intercal} \mathbf{D} \, \hat{\mathbf{q}} + \frac{1}{n(L+1)} \sum_{\mu}\tilde{q}_{\mu}
- \hat{\mathbf{q}}^{\intercal} \mathbf{D}^0 \, \hat{\mathbf{q}} - \frac{1}{n(w_0+1)} \sum_{\mu}\tilde{q}_{\mu}
\Big],
\end{align}
where $\hat{\mathbf{q}}$ is the DFT of $\mathbf{q}$. Notice that the fully connected system $S_1$ yields a diagonal matrix $\mathbf{D}$ with a single non-zero eigenvalue (which is the unity one). For $\mathbf{D}^0$, beside the unity leading eigenvalue, all the remaining eigenvalues are non-negative. This is because of the triangular shape coupling window used in the construction of $S_3$. The triangular window corresponds to a discrete-time convolution between two rectangular windows, and thus a quadratic value in the DFT domain.
%Following the lines of [\cite{krzakala2016mutual}], we obtain
%%
%\begin{align}  \label{eq:derivative_homogeneousVScoupled}
%\partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \frac{1}{4\Delta} \Big[ \frac{1}{n(L+1)} \sum_{\mu,\nu, i_\mu, j_\nu} \mathbb{E}[x_{i_\mu}x_{j_\nu}s_{i_\mu}s_{j_\nu}] -  \frac{1}{ n(2w_0+1)} \sum_{\mu}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} \sum_{i_\mu, j_\nu}\mathbb{E}[x_{i_\mu}x_{j_\nu}s_{i_\mu}s_{j_\nu}] \Big]
%\end{align}
%%
%where  $\mathbb{E}[\cdot]$ is the average over all the disorders. We define the overlap per block as $q_\mu \defeq \frac{1}{n} \sum_{i_\mu} x_{i_\mu}s_{i_\mu}$. Note that due to the periodic boundary condition of the closed-chain SC system of length $L+1$, any quantity $U_\mu$ indexed by the spatial index satisfies $U_\mu = U_{\bar{\mu}}$, with $\bar{\mu} = \text{mod}(\mu -1, L+1) +1$. This induces the following identities
%%
%\begin{align} \label{eq:periodicBound}
%\sum_{\mu} U_\mu &= \sum_{\mu} \frac{1}{l+1}\sum_{\nu \in \bar{\mathcal{S}}_{\mu}} U_\nu, \nonumber \\
%\sum_{\mu} U_{\mu} \sum_{\nu \in \bar{\mathcal{S}}_{\mu}\backslash \mu} U_\nu &= \sum_{\mu} \frac{1}{l+1}\sum_{\underset{\eta \neq \nu }{\eta , \nu \in \bar{\mathcal{S}}_{\mu}}} U_{\eta}  U_\nu,
%\end{align}
%%
%where $\bar{\mathcal{S}}_{\mu}=\{k+\mu:k+\mu+l\}$ and $\forall k,l \in \mathbb{N}$. Furthermore, the periodicity at the boundaries yields the following property
%\begin{align}\label{eq:periodicBound_2}
%\sum_{\mu} U_\mu\sum_{\nu \in \bar{\mathcal{S}}_{\mu}} U_{\nu} = \sum_{\mu} \frac{1}{l+1}  \Big(\sum_{\nu\in \bar{\mathcal{S}}_{\mu}} U_\nu\Big)^2 .
%\end{align}
%\begin{proof}
%\textbf{(\ref{eq:periodicBound_2}):} By combining the two identities in (\ref{eq:periodicBound}), one obtains
%\begin{align*}
%\sum_{\mu} \frac{1}{l+1}\sum_{\underset{\eta \neq \nu }{\eta , \nu \in \bar{\mathcal{S}}_{\mu}}} U_{\eta}  U_\nu = \sum_{\mu} \frac{1}{l+1}\sum_{\eta \in \bar{\mathcal{S}}_{\mu}} U_{\eta} \sum_{\nu \in \bar{\mathcal{S}}_{\eta}\backslash \eta}U_\nu.
%\end{align*}
%Thus, the property (\ref{eq:periodicBound_2}) follows
%\begin{align*}
%&\sum_{\mu} U_\mu\sum_{\nu \in \bar{\mathcal{S}}_{\mu}} U_{\nu} = \sum_{\mu} U_{\mu}^2 + \sum_{\mu} U_{\mu} \sum_{\nu \in \bar{\mathcal{S}}_{\mu}\backslash \mu} U_\nu = \frac{1}{l+1} \Big( \sum_{\mu}  \sum_{\nu\in \bar{\mathcal{S}}_{\mu}} U_\nu^{2} + \sum_{\mu} \sum_{\eta \in \bar{\mathcal{S}}_{\mu}} U_{\eta} \sum_{\nu \in \bar{\mathcal{S}}_{\eta} \backslash \eta} U_\nu \Big) \nonumber \\
%%
%=&\frac{1}{l+1} \Big( \sum_{\mu}  \sum_{\nu\in \bar{\mathcal{S}}_{\mu}} U_\nu^{2} + \sum_{\mu}  \sum_{\underset{\eta \neq \nu }{\eta , \nu \in \bar{\mathcal{S}}_{\mu}}} U_{\eta}  U_\nu \Big) = \frac{1}{l+1}  \sum_{\mu} \Big(\sum_{\nu\in \bar{\mathcal{S}}_{\mu}} U_\nu\Big)^2 . 
%\end{align*}
%\end{proof}
%Hence, (\ref{eq:derivative_homogeneousVScoupled}) can be rewritten as
%%
%\begin{align}  \label{eq:derivativeNeg_homogeneousVScoupled}
%&\frac{4\Delta}{n}\partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E}\Big[\frac{1}{L+1} \sum_{\mu,\nu} q_\mu q_\nu -  \frac{1}{2w_0+1} \sum_{\mu}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} q_\mu q_\nu \Big] \nonumber\\
%%
%&= (L+1) \mathbb{E}\Big[\Big(\frac{1}{L+1} \sum_{\mu} q_\mu\Big)^2 - \frac{1}{L+1}\sum_{\mu} q_\mu\frac{1}{2w_0+1}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} q_\nu \Big]\nonumber \\
%%
%&= (L+1) \mathbb{E}\Big[\Big(\frac{1}{L+1} \sum_{\mu} \frac{1}{2w_0+1}\sum_{\nu\in S{\mu}} q_\nu\Big)^2 - \frac{1}{L+1}\sum_{\mu} \Big(\frac{1}{2w_0+1}\sum_{\nu\in \mathcal{S}_{\mu}^{w_0}} q_\nu \Big)^2 \Big]\le 0,
%\end{align}
%%
%where the inequality is obtained using the convexity of the quadratic function and the last equality using the property (\ref{eq:periodicBound_2}). 
Therefore, we can assert that $\frac{\partial_t \mathbb{E}[\ln \big(Z(t)\big)]}{ n} \le 0$.  Hence, $f_{L,n}^{\rm {p}}\le f_{L,n}^{\rm h}$ as  the interpolated free energy $\frac{-\mathbb{E}[\ln (Z(t))]}{n(L+1)}$ is non-decreasing in $t$.
%
\subsection{The decoupled VS the coupled systems}
%
We now interpolate between $S_4$ (recovered at $t=1$) and $S_3$ (recovered at $t=0$) by setting $w = w_4=0$ and using the same parameters for $S_3$ as before. Using similar arguments as for the previous case, one obtains
\begin{align} \label{eq:derivativeNeg_decoupledVScoupled}
\frac{4\Delta}{ n} \partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E} \Big[ \hat{\mathbf{q}}^{\intercal} \mathbf{D} \, \hat{\mathbf{q}} + \frac{1}{n} \sum_{\mu}\tilde{q}_{\mu}
- \hat{\mathbf{q}}^{\intercal} \mathbf{D}^0 \, \hat{\mathbf{q}} - \frac{1}{n(w_0+1)} \sum_{\mu}\tilde{q}_{\mu}
\Big] \ge 0,
\end{align}
%
%\begin{align}
%\frac{4\Delta}{n}\partial_t \mathbb{E}[\ln \big(Z(t)\big)] &= \mathbb{E}\Big[\sum_{\mu} q_\mu^2 -  \frac{1}{2w_0+1} \sum_{\mu}\sum_{\nu\in\{\mu:\mu+w_0\}} q_\mu q_\nu \Big] \nonumber\\
%%
%&= \mathbb{E}\Big[\sum_{\mu} \frac{1}{2w_0+1}\sum_{\nu\in\{\mu:\mu+w_0\}} q_\nu^2 - \sum_{\mu} \Big(\frac{1}{2w_0+1}\sum_{\nu\in\{\mu:\mu+w_0\}} q_\nu \Big)^2 \Big] \ge 0, \label{eq:derivativeNeg_decoupledVScoupled}
%\end{align}
%
where the inequality is obtained by noticing that $\mathbf{D}$ is the identity matrix in this case. This proves that $f_{L,n}^{\rm{dec}}\le f_{L,n}^{\rm{p}}$. Combining the previous two results, we have that 
%
\begin{lemma}\label{lemma:freeEnergy_sandwich}
$ f_{L,n}^{\rm{dec}} \le f_{L,n}^{\rm{p}}\le f_{L,n}^{\rm h}$.
\end{lemma}
%
\subsection{Existence of the free energy's infinite limit}
%
Consider now the underlying system of the form (\ref{eq:mainProblem}) with size $N$ and free energy $f_N^{\rm u}$. By dividing this system into two similar but independent subsystems of sizes $N_1$ and $N_2$, with $N_1 + N_2 = N$, it turns out that the free energy $f_N^{\rm u}$ is superadditive w.r.t. $N$.
%
\begin{lemma}\label{lemma:superadditivity}
$N f_N^{\rm u} \geq N_1 f_{N_1}^{\rm u} + N_2 f_{N_2}^{\rm u}$.
\end{lemma}
%
\begin{proof}
Using the interpolation method again, as done in [\cite{guerra_toninelli_2008}], between the underlying system and the two subsystems, one gets the following partition function
\begin{align*}
Z(t) =& \int d\bx P_0(\bx) \exp\Bigg(-\frac{t}{\Delta} \sum_{1 \le i\le j\le N}\bigg[ \frac{x_{i}^2x_{j}^2}{2N} -  \frac{s_{i}s_{j}x_{i}x_{j}}{N} - \frac{x_{i}x_{j}z_{i j} \sqrt{\Delta/t}}{\sqrt{N}}\bigg]\\
%
&-\frac{(1-t)}{\Delta}  \sum_{1 \le i\le j\le N_1}\bigg[ \frac{x_{i}^2x_{j}^2}{2N_1} -  \frac{s_{i}s_{j}x_{i}x_{j}}{N_1} - \frac{x_{i}x_{j}z_{i j} \sqrt{\Delta/t}}{\sqrt{N_1}}\bigg] \\
&-\frac{(1-t)}{\Delta}  \sum_{N_1 \le i\le j\le N_2}\bigg[ \frac{x_{i}^2x_{j}^2}{2N_2} -  \frac{s_{i}s_{j}x_{i}x_{j}}{N_2} - \frac{x_{i}x_{j}z_{i j} \sqrt{\Delta/t}}{\sqrt{N_2}}\bigg]\Bigg).
\end{align*}
The derivative of $\mathbb{E}[\ln \big(Z(t)\big)]$ w.r.t. the interpolation parameter $t$ gives
\begin{align*}
\frac{4\Delta}{N}\partial_t \mathbb{E}[\ln \big(Z(t)\big)] = \mathbb{E}\Big[  q^2 -  \frac{N_1}{N} q_1^2 - \frac{N_2}{N} q_2^2 \Big] \le 0
\end{align*}
where $q = \frac{1}{N} \sum_{i=1}^{N}x_i s_i$, $q_1= \frac{1}{N_1} \sum_{i=1}^{N_1}x_i s_i$ and $q_2 = \frac{1}{N_2} \sum_{i=N_1+1}^{N}x_i s_i$. The inequality is due to the convexity of the quadratic. Hence, Lemma \ref{lemma:superadditivity} follows.
\end{proof}
%
Lemma \ref{lemma:superadditivity} implies, by Fekete's Lemma of superadditive sequences, that the asymptotic free energy of the underlying system exists $\lim_{N\rightarrow \infty}\frac{1}{N}f_N^{\rm u} = f^{\rm u}$. Note that the  homogeneous system $S_1$ is nothing but the underlying system at $N= n(L+1)$. Moreover, the decoupled system $S_4$ consists of $L+1$ non-interacting copies of the underlying system.  Therefore, in the limit $n\rightarrow \infty$, the three quantities of Lemma \ref{lemma:freeEnergy_sandwich} exist and the following lemma holds
\begin{lemma}\label{lemma:freeEnergy_sandwich_limit}
$ \lim_{n\rightarrow \infty} f_{L,n}^{\rm{dec}} = \lim_{n\rightarrow \infty} f_{L,n}^{\rm{p}} = \lim_{n\rightarrow \infty} f_{L,n}^{\rm h} = f^{\rm u}$.
\end{lemma}
%
\subsection{The unpinned VS the actual SC systems}
The only difference between the free energy of the unpinned SC system $f_{L,n}^{\rm{p}}$ and that of the actual SC system $f_{L,n}^{\rm{c}}$ comes from the boundary condition (the blocks in $\mathcal{B}= \{0:w\} \cup \{L-w+1:L\}$). In the sequel, we prove that the contribution of the pinned boundary conditions of the actual SC systems to the free energy is $\mathcal{O}(\frac{w}{L})$ for a wide range of parameters. Therefore, by taking the asymptotic limit in the proper order, we have that
\begin{lemma}\label{lemma:openVSclosed}
$\lim_{L,n \rightarrow \infty}f_{L,n}^{\rm{c}} = \lim_{L,n \rightarrow \infty}f_{L,n}^{\rm{p}} = f^{\rm{u}}$ and $\Delta_{\rm opt}^{\rm c} = \Delta_{\rm opt}$.
\end{lemma}
\begin{proof}
The Hamiltonians of the unpinned and the actual SC systems, $\mathcal{H}^{\rm p}$ and $\mathcal{H}^{\rm c}$ respectively, satisfy the identity $\mathcal{H}^{\rm c} = \mathcal{H}^{\rm p} - \delta \mathcal{H}$ with
\begin{align}\label{eq:H_openVSclosed}
\delta \mathcal{H} &=  \sum_{\mu \in \mathcal{B}} \Lambda_{\mu,\mu} \sum_{i_\mu\le j_\mu}\bigg[ \frac{x_{i_\mu}^2x_{j_\mu}^2 + s_{i_\mu}^2s_{j_\mu}^2}{2n\Delta} -  \frac{s_{i_\mu}s_{j_\mu}x_{i_\mu}x_{j_\mu}}{n\Delta} - \frac{(x_{i_\mu}x_{j_\mu}-s_{i_\mu}s_{j_\mu})z_{i_\mu j_\mu}}{\sqrt{n \Delta \Lambda_{\mu,\mu}}}\bigg]\nonumber\\
%
&+ \sum_{\mu \in \mathcal{B}}\sum_{\nu\in \{\mu+1:\mu+w\}\cap \mathcal{B}}\Lambda_{\mu,\nu}\sum_{i_\mu\le j_\nu}\bigg[ \frac{x_{i_\mu}^2x_{j_\nu}^2 + s_{i_\mu}^2s_{j_\nu}^2}{2n\Delta} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n \Delta} - \frac{(x_{i_\mu}x_{j_\nu}-s_{i_\mu}s_{j_\nu})z_{i_\mu j_\nu} }{\sqrt{n \Delta \Lambda_{\mu,\nu}}}\bigg]\nonumber\\
%
&+ \sum_{\mu \in \mathcal{B}}\sum_{\nu\in \{\mu-w:\mu-1\}\cap \mathcal{B}}\Lambda_{\mu,\nu}\sum_{j_\nu < i_\mu}\bigg[ \frac{x_{i_\mu}^2x_{j_\nu}^2 + s_{i_\mu}^2s_{j_\nu}^2}{2n\Delta} -  \frac{s_{i_\mu}s_{j_\nu}x_{i_\mu}x_{j_\nu}}{n\Delta} - \frac{(x_{i_\mu}x_{j_\nu}-s_{i_\mu}s_{j_\mu})z_{i_\mu j_\nu} }{\sqrt{n\Delta\Lambda_{\mu,\nu}}}\bigg]
%
\end{align}
% old $\delta \mathcal{H}$
%\begin{align}
%\delta \mathcal{H} &=  \sum_{\mu \in \mathcal{B}} \sum_{i_\mu\le j_\mu} \frac{x_{i_\mu}x_{j_\mu}z_{i_\mu j_\mu} \sqrt{\Lambda_{\mu,\mu}} }{\sqrt{\Delta n}}
%%
%+ \sum_{\mu \in \mathcal{B}}\sum_{\nu\in \{\mu+1:\mu+w\} \cap \mathcal{B}}\sum_{i_\mu\le j_\nu} \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu}\sqrt{\Lambda_{\mu,\nu}}}{\sqrt{\Delta n}}\nonumber\\
%%
%&+ \sum_{\mu \in \mathcal{B}}\sum_{\nu\in \{\mu-w:\mu-1\} \cap \mathcal{B}}\sum_{j_\nu < i_\mu} \frac{x_{i_\mu}x_{j_\nu}z_{i_\mu j_\nu}\sqrt{\Lambda_{\mu,\nu}}}{\sqrt{ \Delta n}}.
%\end{align}
Let $Z^{\rm p}$ and $Z^{\rm c}$ be the partition functions associated with $\mathcal{H}^{\rm p}$ and $\mathcal{H}^{\rm c}$ (where $Z^{\rm p}=\int d\bx P_0(\bx) e^{- \mathcal{H^{\rm p}}}$ and $Z^{\rm c}= \int d\bx P_0(\bx)e^{- \mathcal{H^{\rm c}}}$). Hence, one obtains the following identities
\begin{align}\label{eq:Z_openVSclosed}
\begin{cases}
\ln(Z^{\rm p}) &= \ln\Big( Z^{\rm c} \int d\bx \frac{P_0(\bx)e^{- \mathcal{H}^{\rm c}}}{Z^{\rm c}} e^{-\delta \mathcal{H}} \Big) \\
\ln(Z^{\rm c}) &= \ln\Big( Z^{\rm p}  \int d\bx \frac{P_0(\bx)e^{- \mathcal{H}^{\rm p}}}{Z^{\rm p}} e^{\delta \mathcal{H}} \Big),
\end{cases}
\end{align}
where the integrals can be seen as expectations over two posterior distributions, of the form (\ref{eq:posterior_partition}), associated to $\mathcal{H}^{\rm c}$ and $\mathcal{H}^{\rm p}$ respectively. Denote by $\langle \cdot \rangle_{\rm c}$ and $\langle \cdot \rangle_{\rm p}$ these expectations. In terms of free energy, (\ref{eq:Z_openVSclosed}) translates to
\begin{equation}\label{eq:energy_openVSclosed}
\begin{cases}
 f_{L,n}^{\rm{p}} = f_{L,n}^{\rm{c}} - \frac{\mathbb{E}\big[\ln \big( \langle e^{ -\delta \mathcal{H}} \rangle_{\rm c} \big)\big]}{n(L+1)}\\
  f_{L,n}^{\rm{c}} = f_{L,n}^{\rm{p}} - \frac{\mathbb{E}\big[\ln \big( \langle e^{ \delta \mathcal{H}} \rangle_{\rm p} \big)\big]}{n(L+1)}.
 \end{cases}
\end{equation}
Using the convexity of exponential, we get
%where the left-hand side inequality is obtained by noticing that the extra energy term is non-negative for a Hamiltonian with complete square, while the right-hand side inequality is due to the convexity of exponential. Furthermore, for bounded second and forth moments of the signal's prior distribution, $\frac{\mathbb{E} [ \langle \delta \mathcal{H} \rangle_{\rm c} ]}{n(L+1)}=\mathcal{O}(\frac{w}{L})$.
\begin{equation}\label{eq:openVSclosed_sandwich}
f_{L,n}^{\rm{c}} + \frac{\mathbb{E}\big[ \langle \delta \mathcal{H} \rangle_{\rm p} \big]}{n(L+1)} \le f_{L,n}^{\rm{p}} \le f_{L,n}^{\rm{c}} + \frac{\mathbb{E}\big[ \langle \delta \mathcal{H} \rangle_{\rm c} \big]}{n(L+1)}.
\end{equation}
Recall that due to the pinning condition used in the construction of the SC system in section \ref{sec:thresh-sat} (Remark \ref{remark:pinning}), we assume perfect knowledge of the variables at the boundaries where $x_{i_\mu} = s_{i_\mu}\, \forall \mu \in \mathcal{B}$. Thus, the expectation $\langle \cdot \rangle_{\rm c}$ associated with the actual SC system yields
\begin{align}
\frac{\mathbb{E}[ \langle \delta \mathcal{H} \rangle_{\rm c} ]}{n(L+1)} = 0 . 
\end{align}
Moreover, following the lines of [\cite{krzakala2016mutual}] by using a Gaussian integration by part and Nishimori conditions, we obtain
\begin{align}\label{eq:openVSclosed_order}
\frac{\Big|\mathbb{E}[ \langle \delta \mathcal{H} \rangle_{\rm p} ]\Big|}{n(L+1)} &\le \frac{n(n+1)(2w+1)^2}{n^2(L+1)(w+1)} \Big|\mathbb{E} [\langle x_{i_\mu}^2x_{j_\nu}^2 \rangle_{\rm p}]\Big|  + \frac{n(n-1)(2w+1)}{2n^2(L+1)(w+1)} \Big|\mathbb{E} [\langle x_{i_\mu}^2x_{j_\mu}^2 \rangle_{\rm p}]\Big| \nonumber \\
%
&+ \frac{(2w+1)}{n(L+1)(w+1)}\Big|\mathbb{E} [\langle x_{i_\mu}^4\rangle_{\rm p}]\Big| \nonumber\\
%
&= \mathcal{O}\Big(\frac{w}{L}\Big) \Big|\mathbb{E} [\langle x_{i_\mu}^2x_{j_\nu}^2 \rangle_{\rm p}]\Big|  + \mathcal{O}\Big(\frac{1}{L}\Big)  \Big|\mathbb{E} [\langle x_{i_\mu}^2x_{j_\mu}^2 \rangle_{\rm p}]\Big| + \mathcal{O}\Big(\frac{1}{nL}\Big) \Big|\mathbb{E} [\langle x_{i_\mu}^4\rangle_{\rm p}]\Big|,
\end{align}
for $ \Lambda_{\mu,\nu} \le \frac{1}{w+1}$. Furthermore, for bounded second and fourth moments of the signal's prior distribution, all the expectations in (\ref{eq:openVSclosed_order}) are bounded too (by Nishimori conditions). Therefore, Lemma \ref{lemma:openVSclosed} holds by taking $n\rightarrow \infty$ then $L\rightarrow \infty$ in (\ref{eq:openVSclosed_sandwich}).

\end{proof}
 
%

==> v5 arxiv/sections/low_noise_regime.tex <==
\section{Proof of Theorem \ref{thm1} for $\Delta <\Delta_{\rm opt}$}\label{sec:delta-less-delta-opt}
%
We first show the following Lemma.

\begin{lemma}\label{small-noise-lemma}
Let $\Delta < \Delta_{\rm amp}$. Then the limit of the mutual information per variable exists and is given by the replica symmetric formula \eqref{eq:RSformula}.
\end{lemma}

\begin{proof}
Let us apply \eqref{eq:subopt} to the AMP estimator $\hat{\tbf{s}}^t$. By definition of the MMSE estimator as being optimal in the MSE sense,
% 
\begin{align}\label{startingpoint}
{\rm MSE}_{n, \rm amp}^t(\Delta^{-1}) \geq {\rm MMSE}_n(\Delta^{-1}).
\end{align}
%
Taking limits in the order $\lim_{t\to +\infty}\limsup_{n\to +\infty}$ and using \eqref{eq:mseampmatriciel} we find
\begin{align}
v^2 - (v-E_{\infty})^2 \geq \limsup_{n\to +\infty}{\rm MMSE}_n(\Delta^{-1}),
\end{align}
and in view of \eqref{eq:GSV} we obtain 
\begin{align}\label{thisineq}
\frac{1}{4}(v^2 - (v-E_{\infty})^2) \geq  \limsup_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\Delta^{-1}}.
\end{align}
Now, for $\Delta < \Delta_{\rm amp}$ we have $E_{\infty} = E_{\rm good}(\Delta)$ which is the unique and hence {\it global} minimum of $i_{\rm RS}(E; \Delta)$. Hence, by exactly the same calculation done in equations
\eqref{first} -\eqref{third}, we conclude that the left hand of \eqref{thisineq} is a {\it total derivative}, namely
$$
\frac{d}{d\Delta^{-1}}\{\min_{E}i_{\rm RS}(E; \Delta)\}.
$$
In other words
\begin{align}
\frac{d}{d\Delta^{-1}}\{\min_{E}i_{\rm RS}(E; \Delta)\} \geq 
\limsup_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\Delta^{-1}},
\end{align}
which is also equivalent to 
\begin{align}\label{middlepoint}
\frac{d}{d\Delta}\{\min_{E}i_{\rm RS}(E; \Delta)\} \leq 
\liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\Delta}.
\end{align}
We now integrate this inequality over an interval 
$[0, \Delta] \subset [0, \Delta_{\rm amp}]$
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) - \min_{E}i_{\rm RS}(E; 0) 
& \leq 
\int_0^\Delta d\tilde{\Delta}\,\liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\tilde{\Delta}}
\nonumber \\ &
\leq 
\liminf_{n\to +\infty}\int_0^\Delta d\tilde{\Delta}\,\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\tilde{\Delta}}
\nonumber \\ &
= \liminf_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W}) - H(S).
\end{align}
The second inequality uses Fatou's Lemma and the last equality uses that for zero noise 
$I(\tbf{S}\tbf{S}^T\vert \tbf{W}) = H(\tbf{S}\tbf{S}^T) - H(\tbf{S}\tbf{S}^T\vert \tbf{W}) = H(\tbf{S}\tbf{S}^T) = H(\tbf{S}) = nH(S)$. 
In appendix \ref{appendix_smallnoise} an explicit calculation shows that $\min_{E}i_{\rm RS}(E; 0) = H(S)$.  Therefore
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) \leq \liminf_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W}).
\end{align}
The final step combines this inequality with the interpolation bound \eqref{eq:guerrabound}
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) & \leq 
\liminf_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})
\leq 
\limsup_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})
\leq 
\min_{E}i_{\rm RS}(E; \Delta)
\end{align}
This shows that the limit of the mutual information exists and is equal to the replica symmetric formula for $\Delta <\Delta_{\rm amp}$.
\end{proof}

This proof already shows the existence of the thermodynamic limit for 
$\Delta < \Delta_{\rm amp}$. In hindsight this is perhaps not so surprising. Indeed it crucially uses the interpolation bound \eqref{eq:guerrabound} which itself is based on an interpolation which does not per se show the existence of this limit, but which is quite similar to another interpolation used for showing the existence of the limit for {\it all} $\Delta$ (this other type of interpolation is used in section \ref{sec:subadditivitystyle}). 

One can try to apply the same proof idea to the regime $\Delta > \Delta_{\rm pot}$. 
Equations \eqref{startingpoint} - \eqref{middlepoint} work out exactly in the same way
because the AMP fixed point $E_{\infty} = E_{\rm bad}(\Delta)$ which is the {\it global} minimum of $i_{\rm RS}(E; \Delta)$.
Then when one integrates on $[\Delta, +\infty[$ one finds 
$$
\limsup_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W}) \leq \min_{E}i_{\rm RS}(E; \Delta).
$$
This essentially gives an alternative proof of \eqref{eq:guerrabound} for $\Delta > \Delta_{\rm pot}$. However the result is {\it weaker} because \eqref{eq:guerrabound} is valid at finite size.

For the rest of this section we need the following Lemma. The proof is deferred to section 
\ref{sec:subadditivitystyle} because it uses similar interpolation arguments together with 
standard limiting arguments for sequences of concave/convex functions. 

\begin{lemma}\label{existence-thermo-limit}
The limit $\lim_{n\to +\infty}\frac{1}{n} I(\tbf{S}\tbf{S}^T\vert \tbf{W})$ exists 
and is a continuous function of $\Delta$. 
\end{lemma}

A crucial step in our analysis is the following Lemma.

\begin{lemma}\label{analyticity-argument-lemma}
We necessarily have $\Delta_{\rm pot} \geq \Delta_{\rm opt}$. 
\end{lemma}

\begin{proof}
If $\Delta_{\rm pot} =+\infty$ then we are done; so we suppose it is finite. The proof 
proceeds by contradiction: suppose $\Delta_{\rm pot} < \Delta_{\rm opt}$. Notice first that it not possible to have $\Delta_{\rm pot} < \Delta_{\rm amp}$ because in the range $]0, \Delta_{\rm amp}[$, as a function of $E$, the function $i_{\rm RS}(E;\Delta)$ has a unique critical point. So we assume $\Delta_{\rm pot}\in [\Delta_{\rm amp}, \Delta_{\rm opt}[$. 
For $\Delta \in ]0, \Delta_{\rm pot}[$ we have $\min_{E\in [0, v]}i_{\rm RS}(E; \Delta)
= i_{\rm RS}(E_{\rm good}(\Delta); \Delta)$ which by hypothesis is an analytic function  in this interval. By definition of $\Delta_{\rm opt}$, the function 
$\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})$ is analytic in $]0, \Delta_{\rm opt}[$. Therefore {\it both functions are analytic on} $]0, \Delta_{\rm pot}[$ and since by Lemma~\ref{small-noise-lemma} they are equal for $]0, \Delta_{\rm amp}[\subset ]0, \Delta_{\rm pot}[$, {\it they must 
be equal on the whole range} $]0, \Delta_{\rm pot}[$. This implies that the two functions are equal at $\Delta_{\rm pot}$ because they are continuous. Explicitly,
\begin{align}\label{eq:equalityatpoint}
\min_{E}i_{\rm RS}(E; \Delta_{\rm pot}) = \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta_{\rm pot}}.
\end{align}

Now, fix some $\Delta \in ]\Delta_{\rm pot}, \Delta_{\rm opt}[$. Since this $\Delta$ is greater than $\Delta_{\rm pot}$ the fixed point of state evolution is $E_{\infty} = E_{\rm bad}(\Delta)$ and this is also the global minimum of $i_{\rm RS}(E;\Delta)$. Hence 
exactly as in \eqref{startingpoint} - \eqref{middlepoint} we can show that for 
$\Delta \in ]\Delta_{\rm pot}, \Delta_{\rm opt}[$,
\begin{align}\label{contra}
\frac{d}{d\Delta}\{\min_{E}i_{\rm RS}(E; \Delta)\} \leq 
\liminf_{n\to +\infty}\frac{1}{n}\frac{d I(\tbf{S}\tbf{S}^T\vert \tbf{W}) }{d\Delta}.
\end{align}
This time \eqref{eq:guerrabound}, \eqref{contra} and the assumption $\Delta_{\rm pot}\in [\Delta_{\rm amp}, \Delta_{\rm opt}[$, taken together, lead to a 
contradiction, and hence we must have $\Delta_{\rm pot} \geq \Delta_{\rm opt}$. 

To see explicitly how the contradiction appears, integrate \eqref{contra} 
on $]\Delta_{\rm pot}, \Delta[\subset\Delta \in ]\Delta_{\rm pot}, \Delta_{\rm opt}[$, and use Fatou's Lemma, to obtain
\begin{align}
\min_{E}i_{\rm RS}(E; \Delta) - \min_{E}i_{\rm RS}(E; \Delta_{\rm pot})
& 
\leq \liminf_{n\to +\infty}\biggl\{\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta} - \frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta_{\rm pot}}\biggr\}
\nonumber \\ &
= 
\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta} - 
\lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})\Big\vert_{\Delta_{\rm pot}}
\end{align}
From \eqref{eq:equalityatpoint} and \eqref{eq:guerrabound} we obtain 
$
\min_{E}i_{\rm RS}(E; \Delta) = \lim_{n\to +\infty}\frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W})
$
{\it when} $\Delta_{\rm amp} \leq \Delta_{\rm pot} < \Delta < \Delta_{\rm opt}$. But by 
the previous results this equality is also 
true for $0 < \Delta \leq \Delta_{\rm pot}$. So the equality is valid 
in the whole interval $]0, \Delta_{\rm opt}[$ and therefore $\min_{E}i_{\rm RS}(E; \Delta)$ is analytic at $\Delta_{\rm pot}$. But this is impossible by the definition of 
$\Delta_{\rm pot}$. 
\end{proof} 

\begin{corollary}
Let $\Delta < \Delta_{\rm opt}$. Then the thermodynamic limit of the mutual information per variable is given by the replica symmetric formula \eqref{eq:RSformula}.
\begin{align}
\lim_{n\to +\infty} \frac{1}{n}I(\tbf{S}\tbf{S}^T\vert \tbf{W}) = \min_{E}i_{\rm RS}(E; \Delta)
\end{align}
\end{corollary}

\begin{proof}
Lemma~\ref{small-noise-lemma} says that the two functions are equal  for $\Delta <\Delta_{\rm amp}$ and Lemma~\ref{analyticity-argument-lemma} implies that {\it both} functions are analytic for $\Delta <\Delta_{\rm opt}$. Thus they must be equal on the whole range $\Delta < \Delta_{\rm opt}$.
\end{proof}

==> v5 arxiv/sections/threshold_saturation.tex <==
\section{Threshold saturation}\label{sec:thresh-sat}
%
Let us now prove that for a proper spatially coupled system, threshold saturation occurs, that is $\Delta_{\rm pot} \le \Delta_{\rm amp, c}$, where $\Delta_{\rm amp, c}$ is the algorithmic AMP threshold of the coupled system that we will define in the next. First, define the following average
%
\begin{align}
\langle A \rangle_E \defeq \frac{\int dx A(x) P_0(x)e^{-\frac{x^2}{2\Sigma(E,\Delta)^{2}} + x\big(\frac{s}{\Sigma(E,\Delta)^{2}} + \frac{z}{\Sigma(E,\Delta)} \big)} }{\int dx P_0(x)
e^{-\frac{x^2}{2\Sigma(E,\Delta)^{2}} + x\big(\frac{s}{\Sigma(E,\Delta)^{2}} + \frac{z}{\Sigma(E,\Delta)} \big)}}. \label{eq:defBracket_posteriorMean}
\end{align}
%
where $s,z$ and $\Delta$ are fixed and the dependence in these is implicit for sake of brevity. The AMP algorithm asymptotic perfomance can be tracked thanks to the SE analysis. Let us define the following operator.
%
\begin{definition}[SE operator] 
The state evolution operator associated with the underlying system is
%
\begin{align}
T_{\rm u}(E) \defeq \mathbb{E}_{S,Z}[(S - \langle x\rangle_E)^2], \label{def:SEop_underlying}
\end{align}
%
where $S \sim P_0(s)$, $Z\sim \mathcal{N}(z|0,1)$.
%
\end{definition}
%
Note that this operator is nothing else than the MMSE of a scalar AWGN channel with effective noise variance equal to $\Sigma(E,\Delta)^2$. Call $\hat{\tbf{s}}^{(t)}$ the estimate at iteration $t$ of the signal by the AMP algorithm. The AMP averaged scalar MSE is $E^{(t)}\defeq \mathbb{E}_{S,Z}[n^{-1}\sum_{i=1}^n(s_i - \hat s_i^{(t)})^2]$ is tracked iterating the SE recursion
%
\begin{align} \label{eq:SEiteration}
E^{(t+1)}=T_{\rm u}(E^{(t)}), \quad t\geq 0, \quad E^{(0)} = v, 
\end{align}
%
i.e. initializing the iteration without any knowledge about the signal other than its prior distribution.
%
\begin{remark}
Note that using this operator, $i)$ the good solution is given by $E_{\rm good}(\Delta) = T_{\rm u}^{(\infty)}(0)$ and $ii)$ the AMP threshold of Definition~\ref{amp-thresh} is given by $\Delta_{{\rm amp}} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm u}}^{(\infty)}(v) = E_{\rm good}(\Delta)\}$. 
\end{remark}
%
% In the next we will need the following definition.
%
% \begin{definition}[scalar MSE Floor] The scalar MSE floor $E_{\rm good}(\Delta)$ is defined as the fixed point reached from the initial condition $E^{(0)} = 0$. In other words $E_{\rm good}(\Delta) = T_{\rm u}^{(\infty)}(0)$. 
% \end{definition}
%
\begin{definition}[Bassin of attraction]
The basin of attraction of the good solution $E_{\rm good}(\Delta)$ is 
$\mathcal{V}_{\rm good} \defeq \{ E \ \! |\ \! T_{\rm u}^{(\infty )}(E) = E_{\rm good}(\Delta) \}$.
\end{definition}
%
% \begin{definition} [AMP threshold of the underlying ensemble]
% The AMP threshold of the underlying system is $\Delta_{{\rm u}} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm u}}^{(\infty)}(v) = E_{\rm good}(\Delta)\}$. 
% \end{definition}
%
For this section, it is more convenient to work with the free energy $f_{\rm u}(E)$, simply related to the replica potential \eqref{eq:potentialfunction} by $f_{\rm u}(E;\Delta) = i_{\rm RS}(E;\Delta) - \frac{v^2}{4\Delta}$. In Appendix~\ref{app:nishi}, we show the following Lemma linking the SE and potential analysies.
%
% \begin{align}
% 0=\frac{\partial f_{\rm{u}}(E)}{\partial E}\Big|_{\mathring E} \Leftrightarrow \mathring E = \mathbb{E}[(s - \langle x\rangle_{\mathring E})^2] = T_{\rm{u}}(\mathring E).
% \end{align}
% %
% We recognize the SE operator (\ref{def:SEop_underlying}), so that we can assert the follwing Lemma that links the SE and potential formulations.
%
\begin{lemma}\label{lemma:fixedpointSE_extPot_underlying}
% If $\mathring{E}$ is a fixed point of \eqref{eq:SEiteration}, i.e., $T_{{\rm u}}(\mathring E) = \mathring E$, then $\frac{\partial F_{{\rm u}}(E)}{\partial E}\big|_{\mathring E} =0$ and vice-versa.
$\mathring E = T_{{\rm u}}(\mathring E) \Leftrightarrow \frac{\partial f_{{\rm u}}(E)}{\partial E}\big|_{\mathring E} =0$.
\end{lemma} 
%
\begin{definition}[Free energy gap] \label{def:fgap}
Define $\delta f_{{\rm u}}(\Delta) \defeq {\rm inf} _{E \notin \mathcal{V}_{\rm good} } (f_{{\rm u}}( E) - f_{{\rm u}}(E_{\rm good}(\Delta)))$ as the free energy gap, with the convention that the infimum over the empty set is $\infty$ (this happens for $\Delta < \Delta_{{\rm amp}}$).
\end{definition}
%
\begin{remark}\label{remark:potThresh}
An equivalent definition of the potential threshold, Definition~\ref{def:pot-thresh}, but in terms of the free energy gap is $\Delta_{\rm pot} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! \delta f_{{\rm u}}(\Delta) > 0\}$. (HERE IS $\Delta_{\rm pot}$ is such that $\delta f_{{\rm u}}(\Delta_{\rm pot}) = 0$ BETTER?? TO HOMOGENEIZE WITH Definition~\ref{def:pot-thresh})
\end{remark}
%
In order to prove threshold saturation, formally given by Theorem~\ref{th:mainth_thsat} and Corollary~\ref{cor:maincorollary_thsat}, we need to define a proper spatially coupled (SC) version of the original problem (\ref{eq:mainProblem}). 
%
\subsection{The spatially coupled system}
%
We consider a chain of length $L+1$ where each \emph{block} of the chain, each of size $n$, is coupled to itself and $w \in\{1:L\}$ blocks in front and $w$ blocks before itself, thus to $2w+1$ blocks in total. The SC system is naturally defined, similarly to (\ref{eq:mainProblem}), as
%
\begin{align} \label{eq:def_coupledSyst}
W_{i_\mu j_\nu} = \frac{s_{i_\mu} s_{j_\nu}}{\sqrt{n(2w+1)}} + z_{i_\mu j_\nu} \sqrt{\Delta},
\end{align}
%
where the notation $u_{i_\mu j_\nu}$ means that the index $i_\mu \in \{1:n\}$ (resp. $j_\nu$) belongs to the block $\mu \in \{0:L\}$ (resp. $\nu$) along the coupled chain. In the case $w=L$, one recovers the original (or underlying) problem where the signal $\bf s$ has $n(L+1)$ components. In this construction, the performance of the AMP decoder is tracked by a \emph{scalar MSE profile} (or just \emph{profile}) $\tbf{E}^{(t)}$, defined componentwise by 
%
\begin{align}
E^{(t)}_\mu \defeq \mathbb{E}_{S,Z}[n^{-1}\sum_{i_\mu=1}^n(s_{i_\mu} - \hat s_{i_\mu}^{(t)})^2].
\end{align}
%
It has $L+1$ components and describes the scalar MSE in each block. Let us introduce the SE associated with the AMP algorithm for the inference over this SC system but first, denote the following average at fixed $s,z$ and $\Delta$
%
\begin{align}
% \langle f(x) \rangle_\mu = \frac{\int dx f(x)P_0(x)e^{\frac{\Sigma_\mu({\tbf E})^{-2}}{2} (2 xs - x^2) + \Sigma_\mu({\tbf E})^{-1} zx}}{\int dx P_0(x)e^{\frac{\Sigma_\mu({\tbf E})^{-2}}{2} (2 xs - x^2) + \Sigma_\mu({\tbf E})^{-1} zx}},
\langle A \rangle_\mu \defeq \frac{\int dx A(x) P_0(x)e^{-\frac{x^2}{2\Sigma_\mu({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu({\tbf E},\Delta)} \big)} }{\int dx P_0(x)
e^{-\frac{x^2}{2\Sigma_\mu({\tbf E},\Delta)^{2}} + x\big(\frac{s}{\Sigma_\mu({\tbf E},\Delta)^{2}} + \frac{z}{\Sigma_\mu({\tbf E},\Delta)} \big)}},
\end{align}
%
where the \emph{effective noise variance} of the SC system is defined as
%
\begin{align} \label{eq:defSigma_mu}
\Sigma_\mu(\tbf{E},\Delta)^2 \defeq \Delta \Big(v-\sum_{\nu \in \mu^w} \frac{E_\nu}{2w+1}\Big)^{-1}.
\end{align}
%
\begin{definition}
The state evolution operator associated with the coupled system (\ref{eq:def_coupledSyst}) is defined component-wise as
%
\begin{align}
[T_{\rm c}({\tbf E})]_\mu \defeq \mathbb{E}_{S,Z}[(S - \langle x\rangle_\mu)^2]. \label{def:SEop_SC}
\end{align}
%
$T_{\rm c}({\tbf E})$ is vector valued and here we have written its $\mu$-th component. 
\end{definition}
%
\begin{remark} \label{remark:pinning}
We assume perfect knowledge at the boundaries, i.e. $z_{i_\mu j_\nu} = 0$ if $\mu$ and $\nu$ both belong to $\mathcal{B} \defeq \{0:w\}\cup \{L-w:L\}$ (TO DOUBLE CHECK THIS) or equivalently, $E_\mu=0 \ \forall \ \mu \in \mathcal{B}$. We refer to this as the pinning condition. 
\end{remark}
%
The SE iteration tracking the scalar MSE profile of the SC system then read for $\mu\notin \mathcal{B}$
%
\begin{equation}\label{equ:statevolutioncoupled}
E_\mu^{(t+1)} = [T_{\rm c}({\tbf E}^{(t)})]_\mu, \quad t\geq 0, \quad E^{(0)}_\mu = v \ \forall \ \mu\notin \mathcal{B}.
\end{equation}
%
Let us introduce a suitable notion of degradation that will be useful in the next.
%
\begin{definition}[Degradation] \label{def:degradation}
A profile ${\tbf{E}}$ is degraded (resp. strictly degraded) w.r.t another one ${\tbf{G}}$, denoted as ${\tbf{E}} \succeq {\tbf{G}}$ (resp. ${\tbf{E}} \succ {\tbf{G}}$), if $E_\mu \ge  G_\mu \ \forall \ \mu$ 
(resp. if ${\tbf{E}} \succeq {\tbf{G}}$ and there exists some $\mu$ such that $E_\mu > G_\mu$).
\end{definition}
%
Similarly as for the underlying system, see Definition~\ref{amp-thresh}, we define the AMP threshold for the SC system. Define the good error profile $\tbf{E}_{\rm good}(\Delta)$ as the vector with $L+1$ components equal to $E_{\rm good}(\Delta)$.
%
\begin{definition} [Threshold of coupled ensemble]\label{def:AMPcoupled}
The AMP threshold of the coupled system is defined as $\Delta_{\rm amp, c} \defeq {\liminf}_{L, w\to \infty}\, {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm c}}^{(\infty)}(\boldsymbol{v}) \prec \tbf{E}_{\rm good}(\Delta)\}$
where $\boldsymbol{v}$ is the all $v$ vector. The ${\liminf}_{L, w \to \infty}$ is taken along sequences where {\it first} $L \to \infty$ and {\it then} $w\to\infty$. 
\end{definition}
%
% Define the ensemble $\mu^{w} \defeq \{\mu - w,\ldots, \mu + w\} = \{\mu - w : \mu + w\}$. 
% The replica symmetric free energy for the SC system \eqref{eq:def_coupledSyst} can be computed by the replica symmetric replica method. It gives
% %
% \begin{align} 
% f_{\rm{c}}(\{E_\mu, \hat m_\mu\}) = &\sum_{\mu=0}^{L}\frac{v - E_\mu}{2} \Big(\hat m_\mu - \sum_{\nu \in \mu^{w}} \frac{v - E_\nu}{2\Delta(2w+1)} \Big) \nonumber \\
% -&\sum_{\mu=0}^L \mathbb{E}_{S,Z}\Big[\ln\Big(\int P_0(x)e^{-x^2\frac{\hat m_\mu}{2} + x \big(S\hat m_\mu + Z\sqrt{\hat m_\mu} \big)}\Big)\Big], \label{eq:coupledF}
% \end{align}
% %
% where $Z\sim \mathcal{N}(z|0,1)$ and $S \sim P_0(s)$. We define the \emph{effective noise variance} of the SC system as
% %
% \begin{align} \label{eq:defSigma_mu}
% \Sigma_\mu(\tbf{E},\Delta)^2 \defeq \Delta \Big(v-\sum_{\nu \in \mu^w} \frac{E_\nu}{2w+1}\Big)^{-1}.
% \end{align}
% %
% The fixed point conditions giving the extrema of this potential are
% %
% \begin{align}
% 0=\frac{\partial f_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {\hat m_\mu}} &\Rightarrow E_\mu = \mathbb{E}[(s - \langle x\rangle_\mu)^2] = [T_{\rm c}({\tbf E})]_\mu, \label{eq:fixedPointPotSC_isSE}\\
% %
% 0=\frac{\partial f_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {E_\mu}} &\Rightarrow \hat m_\mu = \Sigma_\mu({\tbf E})^{-2}.
% \end{align}
% %
% Plugging these relations with (\ref{eq:defSigma_mu}) in (\ref{eq:coupledF}), we obtain the RS free energy for the SC system. 
%
\begin{definition}[RS free energy of the coupled system]
%
The replica symmetric free energy of the SC system, or SC potential, is
%
\begin{align}
f_{\rm{c}}(\tbf{E}) = &\sum_{\mu=0}^L\sum_{\nu \in \mu^{w}} \frac{(v\!-\!E_\mu) (v\!-\!E_\nu)}{4\Delta(2w+1)} \nonumber \\
- &\sum_{\mu=0}^L \mathbb{E}_{S,Z}\Big[\ln\Big(\int P_0(x)
 e^{-\frac{x^2}{2\Sigma_\mu(\tbf E,\Delta)^{2}} +x\big(\frac{S}{\Sigma_\mu(\tbf E, \Delta)^{2} } + \frac{Z}{\Sigma_\mu(\tbf E,\Delta)}\big)} dx\Big)\Big], \label{def:RSf_SC}
\end{align}
%
where $\mu^{w} \defeq \{\mu - w,\ldots, \mu + w\} = \{\mu - w : \mu + w\}$, $Z\sim \mathcal{N}(z|0,1)$ and $S \sim P_0(s)$.
\end{definition}
%
As for the underlying system, we obtain from similar relations as in Appendix~\ref{app:nishi} the following Lemma linking SE and potential formulations.
%
\begin{lemma}\label{lemma:fixedpointSE_extPot}
$\mathring E_\mu = [T_{\rm c}(\mathring {\tbf E})]_\mu \Leftrightarrow \frac{\partial f_{{\rm c}}({\tbf E})}{\partial E_\mu}\big|_{\mathring{{\tbf E}}} = 0 \ \forall \ \mu\in \mathcal{B}^{\rm c}=\{w+1:L-w-1\}$.
\end{lemma}
%
The proof presented in the next subsection uses extensively the following monotonicity properties of the SE operators. 
%
\begin{lemma}
The SE operator of the SC system maintains degradation in space, i.e. ${\tbf E} \succeq  {\tbf G} \Rightarrow T_{\rm{c}}({\tbf E}) \succeq T_{\rm{c}}({\tbf{G}})$. This property is verified by $T_{\rm{u}}(E)$ for a scalar error as well.
\label{lemma:spaceDegrad}
\end{lemma}
%
\begin{proof}
From \eqref{eq:defSigma_mu} it is immediately seen that ${\tbf E} \succeq  {\tbf G} \Rightarrow \Sigma_\mu({\tbf E},\Delta) \geq \Sigma_\mu({\tbf G},\Delta)\ \forall \ \mu$. Now, the SE operator \eqref{def:SEop_SC} can be interpreted as an average over the chain blocks of local MMSE's. The local MMSE's are the ones of random variables $S\sim P_0(s)$ sent through AWGN channels with effective noise distributed as $\mathcal{N}(\cdot | 0,\Sigma_\mu^2)$. The MMSE's are increasing functions of $\Sigma_\mu^2$: this is intuitively clear but we provide an explicit formula for the derivative below. Thus $[T_{{\rm c}}( {\tbf E})]_\mu \geq [T_{{\rm c}}( {\tbf G})]_\mu \ \forall \ \mu$, which means $T_{{\rm c}}({\tbf E}) \succeq T_{{\rm c}}({\tbf{G}})$.

The derivative of the scalar MMSE of the Gaussian channel with i.i.d noise $\mathcal{N}(\cdot|0, \Sigma^2)$ can be computed as 
%
\begin{align}
 \frac{d \,{\rm Smmse}(\Sigma^{-2})}{d\,\Sigma^{-2}} = - 2\, \mathbb{E}_{X,Y}\big[\|X - \mathbb{E}[X\vert Y]\|_2^2 \, {\rm Var}[X\vert Y]\big].
\end{align}
%
This formula explicitly confirms that $T_{\rm u}(E)$ (resp. $[T_{{\rm c}}(\tbf E)]_\mu$) is an increasing function of $\Sigma$ (resp. $\Sigma_\mu$).
\end{proof}
%
\begin{corollary}
\label{cor:timeDegrad}
The SE operator of the coupled 
system maintains degradation in time, 
i.e., $T_{{\rm c}}({\tbf E}^{(t)}) \preceq  {\tbf E}^{(t)}\Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \preceq  {\tbf E}^{(t+1)}$. 
Similarly $T_{{\rm c}}({\tbf E}^{(t)}) \succeq  {\tbf E}^{(t)} \Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \succeq  {\tbf E}^{(t+1)}$. 
Furthermore, the limiting error profile ${\tbf E}^{(\infty)} \defeq T_{{\rm c}}^{(\infty)}({\tbf E}^{(0)})$
exists. This property is verified by $T_{{\rm u}}(E)$ for a scalar error as well.
\end{corollary}
%
\begin{proof}
The degradation statements are a consequence of Lemma~\ref{lemma:spaceDegrad}. The existence 
of the limits follows from the monotonicity of the operator and boundedness of the scalar MSE.
\end{proof}
%
Now that we have settled the required definitions and properties, we can prove threshold saturation. 
%
\subsection{Proof of threshold saturation}
%
The pinning condition together with the monotonicity properties of the coupled SE operator ensure that any fixed point point profile ${\tbf E}^*$ of the SE iteration \eqref{equ:statevolutioncoupled} must adopt a shape similar to Fig.~\ref{fig:errorProfile}. From now on we work with a \emph{saturated profile} $\tbf E$, which construction is described in detail in Fig.~\ref{fig:errorProfile}. It verifies ${\tbf E} \succeq {\tbf E}^{*}$ and thus serves as an upper bound in the proof. In the next, we will need the following operator.
%
\begin{figure}[!t]
\centering
\includegraphics[width=0.65\textwidth]{figs/profile_E_2}
\vspace*{-5pt}
\caption{A fixed point profile $\tbf{E}^{*}$ of the coupled SE iteration (solid) is null $\forall \ \mu \le w$ by the pinning condition and increases until $E_{{\rm max}} \in [0,v]$ at $\mu_{\rm max}\in \{w+1:L-w-1\}$. Then it decreases and is again null $\forall \ \mu \ge L-w$. The associated \emph{saturated} profile $\tbf E$ (dashed) starts at $E_{\rm good}(\Delta) \ \forall \ \mu \le \mu_*$, where $\mu_*$ is defined by: $E^{*}_{\mu}\le E_{\rm good}(\Delta) \ \forall \ \mu\le \mu_*$ and $E^{*}_{\mu'} > E_{\rm good}(\Delta) \ \forall \ \mu' > \mu_*$. Then it matches $\tbf E^{*} \ \forall \ \mu \in\{\mu_*:\mu_{\rm max}\}$ and saturates at $E_{{\rm max}} \ \forall \ \mu \ge \mu_{\rm max}$. By construction ${\tbf E}$ is non decreasing and is degraded w.r.t the fixed point profile ${\tbf E} \succeq {\tbf E}^{*}$.}
\label{fig:errorProfile}
\end{figure}
%
\begin{definition}[Shift operator]
The shift operator is defined componentwise as $[{\rm S}({\tbf E})]_1 \defeq E_{\rm good}(\Delta), \ [{\rm S}({\tbf E})]_\mu \defeq  E_{\mu-1}$.
\end{definition}
%
\subsubsection{Taylor expansion of the RS free energy of the SC system}
%
The first main step in the proof of threshold saturation is based on the Taylor expansion of the RS free energy of the SC system. It starts with the following Lemma.
%
\begin{lemma}\label{leminterp}
Let ${\tbf E}$ be a saturated profile. If ${\tbf E}_\lambda \defeq (1-\lambda) {\tbf E} + \lambda {\rm S}({\tbf E})$ and $\delta {E}_{\mu} \defeq {E}_{\mu} -{E}_{\mu-1}$, then for a proper $\lambda\in[0,1]$,
%
\begin{align}
f_{{\rm c}}({\rm S}({\tbf E})) &-f_{{\rm c}}({\tbf E}) = \frac{1}{2} \sum_{\mu,\mu'=1}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 f_{{\rm c}}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}. \label{eq:lemma_secondDerivativeFsc}
\end{align}
%
\label{lemma:Fdiff_quadraticForm}
\end{lemma}
%
\begin{proof}
%
The free energy difference can be expressed as
%
\begin{align}
f_{{\rm c}}({\rm S}({\tbf E})) -f_{{\rm c}}({\tbf E}) = \frac{1}{2}\sum_{\mu,\mu'=1}^{L} \delta {E}_{\mu} \delta {E}_{\mu'}  \frac{\partial^2 f_{{\rm c}}({\tbf E})}{\partial E_{\mu}\partial  E_{\mu'}}\Big|_{ {\tbf E}_\lambda} - \sum_{\mu=1}^{L} \delta {E}_{\mu} \frac{\partial f_{{\rm c}}({\tbf E})}{\partial  E_\mu}\Big|_{{\tbf E}}. \label{eq:expFbsminusFb}
\end{align}
%
By saturation of $\tbf E$ at the boundaries, $\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{1:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$. Moreover for $r\notin\mathcal{A}$, $E_\mu=[T_{\rm c}(\tbf E)]_\mu$, and thus by Lemma~\ref{lemma:fixedpointSE_extPot} the potential derivative cancels at these positions. Hence the last sum in (\ref{eq:expFbsminusFb}) cancels.
\end{proof}
%
From the previous Lemma, in order to compute the free energy difference between those of the shifted and non-shifted profiles, we need to compute the Hessian associated with this free energy.
%
\begin{align}
\frac{\partial f_{\rm{c}}({\tbf E})}{\partial {E_\mu}} &= \sum_{\nu \in \mu^{w}} \frac{E_\nu}{2\Delta(2w+1)} -\frac{1}{2} \sum_\nu \frac{\partial \Sigma_\nu(\tbf E)^{-2}}{\partial E_\mu} [T_{\rm{c}}({\tbf E})]_\nu - \frac{v}{2\Delta} \nonumber\\
%
&= \frac{1}{2\Delta(2w+1)}\Big(\sum_{\nu \in \mu^{w}} E_\nu-\sum_{\nu \in \mu^w} [T_{\rm{c}}({\tbf E})]_\nu\Big)- \frac{v}{2\Delta},\\
%
\Rightarrow\frac{\partial^2 f_{\rm{c}}({\tbf E})}{\partial {E_\mu}\partial {E_{\mu'}}} &= \frac{1}{2\Delta(2w+1)}\Big( \mathbb{I}(\mu' \in \mu^w) - \frac{1}{\Delta(2w+1)}\sum_{\nu \in \mu^w\cap {\mu'}^w} \frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \, \Sigma_\nu^{-2}} \Big). \label{eq:hessian_explicit}
\end{align}
%
We can now compute the r.h.s of \eqref{eq:lemma_secondDerivativeFsc}. Define $\delta E^* \defeq {\rm{max}} \,|\delta E_\mu|$. Due to the indicator function, the first term of the r.h.s of \eqref{eq:hessian_explicit} can be bounded as
%
\begin{align}
\frac{1}{2\Delta(2w+1)} \Big|\sum_{\mu=1}^L\sum_{\mu'\in \mu^w}\delta E_{\mu}\delta E_{\mu'}\Big| \le \frac{\delta E^*}{2\Delta} \Big|\sum_{\mu}\delta E_{\mu}\Big| \le \frac{\delta E^*}{2\Delta} |E_L - E_{\rm good}(\Delta)|,
\end{align}
%
where we have used the fact that the sum is telescopic for the last inequality. Notice now the following important smoothness property verified by the saturated profile.
%
\begin{lemma}
The saturated profile ${\tbf E}$ is smooth, i.e. $\delta E^* \le K^*/w$ for some $K^*=\mathcal{O}(1)$.
\end{lemma}
%
\begin{proof}
By saturation of $\tbf E$, $\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{1:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$. For $\mu \notin\mathcal{A}$, we can replace the fixed point profile component $E_\mu$ by $[T_{\rm c}(\tbf E)]_\mu$ and Taylor expand the SE operator. Define $\delta \Sigma_\mu^{-2} \defeq \Sigma_{\mu+1}({\tbf E})^{-2} - \Sigma_\mu({\tbf E})^{-2}$. From \eqref{eq:defSigma_mu} we get $\delta \Sigma_\mu^{-2} = (E_{\mu - w}-E_{\mu+w+1})/(\Delta(2w+1))$, where $E_{\mu - w}-E_{\mu+w+1} \le v$. We assume that the coupled SE operator is Lipshitz continuous with Lipshitz constant $K_T$ independent of the coupling window $w$. Then we obtain (TO DOUBLE CHECK THIS STEP)
%
\begin{align} \label{eq:deltamstar}
|\delta E_{\mu+1}| &= |[T_{\rm{c}}({\tbf E})]_{\mu +1} - [T_{\rm{c}}({\tbf E})]_{\mu}| \le K \delta \Sigma_\mu^{-2} \Big|\frac{\partial [T_{\rm{c}}({\tbf E})]_{\mu}}{\partial \Sigma_\mu^{-2}}\Big| \le K^*/w \eqdef \delta E^* \ \forall\ \mu,
\end{align}
%
where $K, K^*=\mathcal{O}(1)$ are independent of $w$.
% which is the desired result. Thus ${\tbf E}$ is smooth in the sense that its closeby variations are getting smaller as $w$ increases.
%
\end{proof}
%
Let us now study the second term of the r.h.s of \eqref{eq:hessian_explicit} (without considering the boundaries for sake of simplicity, despite they can be included easily) (TO INCLUDE)
%
\begin{align}
-&\frac{1}{2\Delta^2(2w+1)^2} \sum_{\mu, \mu'=1}^L \delta E_\mu \delta E_{\mu '} \sum_{\nu \in \mu^w\cap {\mu'}^w} \frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \Sigma_{\nu}^{-2}} \nonumber\\ 
%
\le \ &\frac{K_T \delta E^*}{2\Delta^2(2w+1)^2} \sum_{\mu=1}^L \delta E_\mu \sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mu^w\cap {\mu'}^w). \label{eq:last_secondTerm_boudHessian}
\end{align}
%
One can show that for a fixed $\mu$, $\sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mu^w\cap {\mu'}^w) = (2w+1)^2$. Thus \eqref{eq:last_secondTerm_boudHessian} can be upper bounded, using (\ref{eq:deltamstar}), by $K_T \delta E^* |E_L-E_{\rm good}(\Delta)|/(2\Delta^2) = K'/w$ for some constant $K'=\mathcal{O}(1)$ independent of $w$. From this analysis and using the triangle inequality for the last step, we obtain
%
\begin{align}
\frac{1}{2}\Big| \sum_{\mu,\mu'=1}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 f_{{\rm c}}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}\Big| \le U / w, \quad U=\mathcal{O}(1),
\end{align}
%
$U$ independent of $w.$ Combining this inequality with Lemma~\ref{leminterp} proves the following Lemma.
%
\begin{lemma} \label{lemma:dF_ge_Uoverw}
For a saturated profile $\tbf E$, $|f_{{\rm c}}({\rm S}({\tbf E})) -f_{{\rm c}}({\tbf E})|\le U / w$, where $U=\mathcal{O}(1)$ is independent of $w,L$.
\end{lemma}
%
\subsubsection{Direct evalutation of the free energy change}
%
The second main step in the proof is based on a direct evaluation of the free energy change when shifting the saturated profile. For this step, we will need the following Lemmas.
%
\begin{lemma}
Let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_{\rm good}(\Delta)$. Then $ E_{\rm max} \notin \mathcal{V}_{\rm good}$.
\label{lemma:outside_basin}
\end{lemma}
%
\begin{proof}
The fact that the error profile is non decreasing and the assumption that ${\tbf E} \succ {\tbf E}_{\rm good}(\Delta)$ imply that $E_{\rm max} > E_{0}$. Moreover,
%
$E_{\rm max} \le [T_{\rm c}({\tbf E})]_{\mu_{\rm max}} \le T_{\rm u}(E_{\rm max})$
%
where the first inequality follows from $\tbf E\succ \tbf E^*$ and the monotonicity of $T_{\rm c}$, while the second comes from the fact that $\tbf E$ is non decreasing. Combining these with the 
monotonicity of $T_{\rm u}$ gives $T_{\rm u}(E_{\rm max}) \ge  E_{\rm max} \Rightarrow T_{\rm u}^{(\infty)}( E_{\rm max}) \ge  E_{\rm max}> E_{\rm good}(\Delta) \Rightarrow  E_{\rm max} \notin \mathcal {V}_{\rm good}$.
\end{proof}
%
\begin{lemma}\label{lemma:FcSE_minus_FcE_le_deltaF}
Fix $\Delta < \Delta_{\rm pot}$ and let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_0$. Then $|f_{\rm{c}}(S(\tbf{E})) - f_{\rm{c}}(\tbf{E})| \ge \delta f_{\rm{u}}(\Delta)$, where $\delta f_{\rm{u}}(\Delta)$ is the free energy gap, see Definition~\ref{def:fgap}.
\end{lemma}
%
\begin{proof}
Call $\mathcal{I}(\Sigma) \defeq \mathbb{E}_{S,Z}[\ln(\int P_0(x)\exp\big(\frac{\Sigma^{-2}}{2}(2 Sx - x^2) + \Sigma^{-1} Zx\big)dx)]$. Then \eqref{def:RSf_SC} gives
%$f_{\rm{c}}(S(\tbf{E})) - f_{\rm{c}}(\tbf{E})$ is equal to
\begin{align}
% \delta F_{\rm{c}}&=\sum_{\mu=1}^L \Big[\sum_{\nu \in \mu^{w}} \frac{(v-E_{\mu-1}) (v-m_{\nu-1}) }{4\Delta(2w+1)} - I(\hat \Sigma_{\mu-1})\Big] - \sum_{\mu=1}^L \Big[\sum_{\nu \in \mu^{w}} \frac{(v-E_{\mu})(v- E_{\nu})}{4\Delta(2w+1)} - I(\hat \Sigma_{\mu}) \Big] \nonumber \\
%
f_{\rm{c}}({\rm S}(\tbf{E})) - f_{\rm{c}}(\tbf{E})=\sum_{\nu \in 0^{w}} \frac{(v\!-\!E_{0}) (v\!-\!E_{\nu}) }{4\Delta(2w+1)} - \mathcal{I}(\Sigma_{0}) - \sum_{\nu \in L^{w}} \frac{(v\!-\!E_{L})(v\!-\!E_{\nu}) }{4\Delta(2w+1)} + \mathcal{I}(\Sigma_{L}), \label{eq:lastFcSE_minus_FcE}
\end{align}
%
using the fact that the sum is telescoping. Recall $\Sigma(E,\Delta)^2= \Delta/ (v - E)$. Now looking at \eqref{eq:defSigma_mu}, one notices that thanks to the saturation of ${\tbf E}$ at the boundaries, $\Sigma_{0}({\tbf E}) = \Sigma(E_{\rm good}(\Delta))$, $\Sigma_{L}({\tbf E}) = \Sigma(E_L)$ where $E_L = E_{\rm{max}}$. So finally, we can write from \eqref{eq:lastFcSE_minus_FcE} that
%
\begin{align}
f_{\rm{c}}({\rm S}(\tbf{E})) - f_{\rm{c}}(\tbf{E}) &= \Big[\frac{(v\!-\!E_{0})^2 }{4\Delta} - \mathcal{I}(\Sigma(E_{\rm good}(\Delta))) \Big] - \Big[\frac{(v\!-\!E_{L})^2 }{4\Delta} - \mathcal{I}(\Sigma(E_L)) \Big] \nonumber\\
%
&= f_{\rm{u}}(E_{\rm good}(\Delta)) - f_{\rm{u}}(E_L) \le -\delta f_{\rm{u}}(\Delta),
\end{align}
%
where we recognized the free energy of the underlying system $f_{\rm u}(E;\Delta) = i_{\rm RS}(E;\Delta) - \frac{v^2}{4\Delta}$ and the last inequality is a direct application of Lemma~\ref{lemma:outside_basin}. Finally, using the positivity of $\delta f_{\rm{u}}(\Delta)$ as $\Delta<\Delta_{\txt{pot}}$, we obtain the desired result.
\end{proof}
%
We now have all the necessary Lemmas in order to prove threshold saturation.
%
\begin{theorem} \label{th:mainth_thsat}
Assume a spatially coupled instance of rank one matrix estimation is to be solved. Fix $\Delta<\Delta_{\rm{pot}}$, $w>U/\delta f_{\rm{u}}(\Delta)$ ($U$ being independent of $w,L$) and $L>2w$ (such that the problem is well defined, due to the pinning condition, see remark~\ref{remark:pinning}). Then any fixed point profile ${\tbf{E}^*}$ of the coupled state evolution iteration \eqref{equ:statevolutioncoupled} satisfies ${\tbf{E}}^* \prec {\tbf{E}}_{\rm good}(\Delta)$.
\end{theorem}
%
\begin{proof}
Assume that, under these hypotheses, there exists 
a saturated profile $\tbf E$ associated with $\tbf E^*$ such 
that $\tbf E\succ {\tbf{E}}_{\rm good}(\Delta)$. Combining Lemmas~\ref{lemma:dF_ge_Uoverw} and \ref{lemma:FcSE_minus_FcE_le_deltaF} we get $\delta f_{\rm{u}}(\Delta)\le U/w \Rightarrow w \le U/\delta f_{\rm{u}}(\Delta)$, a contradiction. 
Hence, ${\tbf{E}} \preceq {\tbf{E}}_{\rm good}(\Delta)$. Since $\tbf E \succ {\tbf E}^*$, then ${\tbf E}^* \prec {\tbf{E}}_{\rm good}(\Delta)$.
\end{proof}
%
\begin{corollary}\label{cor:maincorollary_thsat}
By first taking $L \to \infty$ and then $w\to\infty$, the AMP threshold of the coupled ensemble satisfies $\Delta_{\rm amp, c}\geq \Delta_{\rm{pot}}$.
\end{corollary}
%
This corollary follows from Theorem~\ref{th:mainth_thsat} and Definition~\ref{def:AMPcoupled}. It says that the AMP threshold of the SC system saturates the potential threshold. 

==> v5 arxiv/sections/threshold_saturation_old.tex <==
\section{Threshold saturation}\label{sec:thresh-sat}
%
%The replica symmetric solution is intimately related to an effective scalar denoising problem given by $y = s + \Sigma(E) z$
%where $s\sim P_0$ and $z\sim \mathcal{N}(0,1)$. Define the function 
%\begin{align}
%{\rm mmse}(\Sigma(E)^{-2}) = \mathbb{E}_{s, y}\bigl[ s - \mathbb{E}[x\vert y]\bigr]
%\end{align}
%where 
%\begin{align}
%\mathbb{E}[x\vert y] = \frac{\int dx\, x P_0(x) e^{-\frac{(y-x)^2}{2\Sigma(E)^2}}}{\int dx\,  P_0(x) e^{-\frac{(y-x)^2}{2\Sigma(E)^2}}}
%\end{align}
%In appendix \ref{appendixA} we show that the critical points of $h_{\rm RS}(E;\Delta)$ satisfy the fixed point equation
%\begin{align}
%E = {\rm mmse}(\Sigma(E)^{-2})
%\end{align}
%On the other hand, this is nothing else than the fixed point equation of state evolution 
%associated to the Approximate Message Passing (AMP) algorithm
%
Let us now introduce the main objects used in this paper, namely the state evolution and potential analysies. First define the \emph{effective noise variance} as
%
\begin{align}
\Sigma(E)^2 = \frac{\Delta}{v-E}. \label{eq:effNoise}
\end{align}
%
Using this definition, we can define the potential of the underlying system.
%
\begin{definition}[RS free energy] \label{def:RSf}
The replica symmetric (RS) free energy for the underlying system, or potential, obtained from the replica method of statistical physics, is
%
\begin{align}
% F_{\rm{u}}(\tilde m) = \frac{{\tilde m}^2}{4\Delta} - \mathbb{E}\Big[\ln\int P_0(x)\exp\Big(-\frac{\tilde m}{2\Delta} x^2+\frac{\tilde m}{\Delta} xs + \sqrt{\frac{\tilde m}{\Delta}} zx\Big)dx\Big],\\
%
% F_{\rm{u}}(\tilde E) = \frac{(v-\tilde E)^2}{4\Delta} - \mathbb{E}\ln\Big(\mathbb{E}_x\exp\Big(-\frac{v-\tilde E}{2\Delta}(x^2+ 2xs) + \sqrt{\frac{v-\tilde E}{\Delta}} zx\Big)\Big),
%
F_{\rm{u}}(E) = \frac{(v-E)^2}{4\Delta} - \mathbb{E}\ln\int P_0(x)\exp\Big(\frac{\Sigma(E)^{-2}}{2}(2xs -x^2) + \Sigma(E)^{-1} zx\Big)dx, \label{eq:RSf}
\end{align}
%
where the expectation $\mathbb{E}[\cdot]$ is w.r.t $z\sim \mathcal{N}(z|0,1)$ and $s \sim P_0(s)$.
\end{definition}
%
Define $\langle\cdot\rangle_E$ as the average w.r.t 
%
\begin{align}
\langle f(x) \rangle_E \defeq \frac{\int dx f(x) P_0(x)e^{\frac{\Sigma(E)^{-2}}{2}(2xs - x^2) + \Sigma(E)^{-1} zx} }{\int dx P_0(x)e^{\frac{\Sigma(E)^{-2}}{2}(2xs - x^2) + \Sigma(E)^{-1} zx}}. \label{eq:defBracket_posteriorMean}
\end{align}
%
Keep in mind that this distribution depends on $s$, $z$ too. The inference of the signal is performed by approximate message passing (AMP), which asymptotic perfomance can be tracked thanks to the state evolution (SE) analysis.
%
\begin{definition}[SE operator] 
The state evolution operator associated with the underlying system is
%
\begin{align}
T_{\rm u}(E) \defeq \mathbb{E}[(s - \langle x\rangle_E)^2]. \label{def:SEop_underlying}
\end{align}
%
\end{definition}
%
Call $\hat{\tbf{s}}^{(t)}$ the estimate at iteration $t$ of the signal by the AMP algorithm. The AMP averaged mean squarre error (MSE) is $E^{(t)}\defeq \mathbb{E}[n^{-1}\sum_{i=1}^n(s_i - \hat s_i^{(t)})^2]$, where $\mathbb{E}[\cdot]$ is the average w.r.t the observation $W$, i.e. w.r.t the noise and signal instances. It can then be tracked iterating the SE recursion
%
\begin{align} \label{eq:SEiteration}
E^{(t+1)}=T_{\rm u}(E^{(t)}), \qquad t\geq 0,
\end{align}
%
with initialization $E^{(0)} = v$, that is without any knowledge about the signal other than its prior distribution.
%
\begin{definition}[MSE Floor] The MSE floor $E_0$ is defined as the fixed point reached from the initial condition $E^{(0)} = 0$. In other words $E_0 = T_{\rm u}^{(\infty)}(0)$. 
\end{definition}
%
\begin{definition}[Bassin of attraction]
The basin of attraction of the MSE floor $E_0$ is 
$\mathcal{V}_0 \defeq \{ E \ \! |\ \! T_{\rm u}^{(\infty )}(E) = E_0 \}$.
\end{definition}
%
\begin{definition} [AMP threshold of the underlying ensemble]
The AMP threshold is $\Delta_{{\rm u}} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! T_{{\rm u}}^{(\infty)}(v) = E_0\}$. 
\end{definition}
%
The replica method suggests that the free energy is the minimum of (\ref{eq:RSf}). Using an integration by part for $z$ and the so-called Nishimori conditions (TO PROVE??) $v = \mathbb{E}[\langle x^2\rangle_E]$, $\mathbb{E}[s \langle x \rangle_E] = \mathbb{E}[\langle x\rangle_E^2]\ \forall \ E$, one obtains
%
\begin{align}
0=\frac{\partial F_{\rm{u}}(E)}{\partial E}\Big|_{\mathring E} \Rightarrow \mathring E = \mathbb{E}[(s - \langle x\rangle_{\mathring E})^2] = T_{\rm{u}}(\mathring E).
\end{align}
%
We recognize the SE operator (\ref{def:SEop_underlying}), so that we can assert the follwing Lemma that links the SE and potential formulations.
%
\begin{lemma}\label{lemma:fixedpointSE_extPot_underlying}
% If $\mathring{E}$ is a fixed point of \eqref{eq:SEiteration}, i.e., $T_{{\rm u}}(\mathring E) = \mathring E$, then $\frac{\partial F_{{\rm u}}(E)}{\partial E}\big|_{\mathring E} =0$ and vice-versa.
$\mathring E = T_{{\rm u}}(\mathring E) \Leftrightarrow \frac{\partial F_{{\rm u}}(E)}{\partial E}\big|_{\mathring E} =0$.
\end{lemma} 
%
\begin{definition}[Free energy gap] \label{def:fgap}
The free energy gap is $\delta F_{{\rm u}} \defeq {\rm inf} _{E \notin \mathcal{V}_0 } (F_{{\rm u}}( E) - F_{{\rm u}}(E_0))$, with the convention that the infimum over the empty set is $\infty$ (this happens for $\Delta < \Delta_{{\rm u}}$).
\end{definition}
%
\begin{definition}[Potential threshold] \label{def:potThresh}
The potential threshold is defined as $\Delta_{\rm pot} \defeq {\rm sup}\,\{\Delta>0\ \! |\ \! \delta F_{{\rm u}} > 0\}$. 
\end{definition} 

THIS ENDS THE DEFINITIONS THAT I MOVED, N

THE PROOF OF THRSHOLD SATURATION STARTS HERE.

%
A fundamental step in the proof is based on the Theorem~\ref{th:mainth_thsat} and Corollary~\ref{cor:maincorollary_thsat}. Let us now prove this Theorem. It starts by defining a proper spatially coupled (SC) version of the original problem (\ref{eq:mainProblem}). 
%
\subsection{The spatially coupled system}
%
We consider a chain of length $L+1$ where each \emph{block} of size $n$ is connected to itself and $w \in\{1:L\}$ blocks in front and before itself, thus to $2w+1$ blocks in total. The SC system is naturally defined similarly to (\ref{eq:mainProblem}) as
%
\begin{align} \label{eq:def_coupledSyst}
W_{i_\mu j_\nu} = \frac{s_{i_\mu} s_{j_\nu}}{\sqrt{n(2w+1)}} + z_{i_\mu j_\nu} \sqrt{\Delta},
\end{align}
%
where the notation $x_{i_\mu j_\nu}$ means that the index $i$ (resp. $j$) belongs to the block $\mu$ (resp. $\nu$) along the $1$-d spatial dimension, i.e. along the coupled chain. In the case $w=L$, one recovers the original (or homogeneous) problem with $n(L+1)$ variables. In this construction, the performance of the AMP decoder is tracked by an \emph{MSE profile} (or just \emph{profile}) $\tbf{E}$ with $L+1$ components, describing the MSE in each block.

Let us introduce the state evolution associated with the AMP algorithm for the inference over this SC system. First, define the \emph{effective noise variance} of the SC system as
%
\begin{align} \label{eq:defSigma_mu}
\Sigma_\mu(\tbf{E})^2 \defeq \Delta \Big(v-\sum_{\nu \in \mu^w} \frac{E_\nu}{2w+1}\Big)^{-1},
\end{align}
%
and denote
%
\begin{align}
\langle f(x) \rangle_\mu = \frac{\int dx f(x)P_0(x)e^{\frac{\Sigma_\mu({\tbf E})^{-2}}{2} (2 xs - x^2) + \Sigma_\mu({\tbf E})^{-1} zx}}{\int dx P_0(x)e^{\frac{\Sigma_\mu({\tbf E})^{-2}}{2} (2 xs - x^2) + \Sigma_\mu({\tbf E})^{-1} zx}},
\end{align}
%
than depends on $z, s$. Before defining the SE operator associated with the AMP algorithm for this SC system, we introduce a suitable notion of degradation that will be useful in the next.
%
\begin{definition}[Degradation] \label{def:degradation}
A profile ${\tbf{E}}$ is degraded (resp. strictly degraded) w.r.t another one ${\tbf{G}}$, denoted as ${\tbf{E}} \succeq {\tbf{G}}$ (resp. ${\tbf{E}} \succ {\tbf{G}}$), if $E_\mu \ge  G_\mu \ \forall \ \mu$ 
(resp. if ${\tbf{E}} \succeq {\tbf{G}}$ and there exists some $\mu$ such that $E_\mu > G_\mu$).
\end{definition}
%
\begin{definition}
The state evolution operator associated with the coupled system (\ref{eq:def_coupledSyst}) is defined component-wise as
%
\begin{align}
[T_{\rm c}({\tbf E})]_\mu \defeq \mathbb{E}[(s - \langle x\rangle_\mu)^2]. \label{def:SEop_SC}
\end{align}
%
$T_{\rm c}({\tbf E})$ is vector valued and here we have written its $\mu$-th component. 
\end{definition}
%
We assume perfect knowledge at the boundaries, i.e. $E_\mu=0 \ \forall \ \mu \in \mathcal{B} \defeq \{0:w\}\cup \{L-w:L\}$. We refer to this as the \emph{pinning condition}. The SE iterations for the SC system then read for $\mu\notin \mathcal{B}$
%
\begin{equation}\label{equ:statevolutioncoupled}
E_\mu^{(t+1)} = [T_{\rm c}({\tbf E}^{(t)})]_\mu, \qquad t\geq 0,
\end{equation}
%
with initialization $E^{(0)}_\mu = v \ \forall \ \mu\notin \mathcal{B}$. Similarly for the underlying system, we define an AMP threshold for the SC system.
%
\begin{definition} [Threshold of coupled ensemble]\label{def:AMPcoupled}
The AMP threshold of the coupled system is defined as $\Delta_{\text c} \defeq {\liminf}_{L, w\to \infty} {\rm sup}\,\{\Delta>0\ \! |\ \! T_{\text{c}}^{(\infty)}(\boldsymbol{1}) \prec \tbf E_0\}$
where $\boldsymbol{1}$ is the all ones vector. The ${\liminf}_{L, w \to \infty}$ is taken along sequences where {\it first} $L \to \infty$ and {\it then} $w\to\infty$. 
\end{definition}
%
Define the ensemble $\mu^{w} \defeq \{\mu - w,\ldots, \mu + w\}\eqdef \{\mu - w : \mu + w\}$. The RS free energy under the Nishimori conditions for this SC system can be computed by the replica symmetric replica method, which gives
%
\begin{align} 
F_{\rm{c}}(\{E_\mu, \hat m_\mu\}) = &\sum_{\mu=0}^{L}\frac{v - E_\mu}{2} \Big(\hat m_\mu - \sum_{\nu \in \mu^{w}} \frac{v - E_\nu}{2\Delta(2w+1)} \Big) \nonumber \\
-&\sum_{\mu=0}^L \mathbb{E}\ln\int P_0(x)\exp\Big(\frac{\hat m_\mu}{2} (2xs - x^2) + \sqrt{\hat m_\mu} zx\Big)dx, \label{eq:coupledF}
\end{align}
%
where the expectation $\mathbb{E}[\cdot]$ is w.r.t $z\sim \mathcal{N}(z|0,1)$ and $s \sim P_0(s)$. The fixed point conditions givieng the extrema of this potential are
%
\begin{align}
0=\frac{\partial F_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {\hat m_\mu}} &\Rightarrow E_\mu = \mathbb{E}[(s - \langle x\rangle_\mu)^2] = [T_{\rm c}({\tbf E})]_\mu, \label{eq:fixedPointPotSC_isSE}\\
%
0=\frac{\partial F_{\rm{c}}(\{E_\mu, \hat m_\mu\})}{\partial {E_\mu}} &\Rightarrow \hat m_\mu = \Sigma_\mu({\tbf E})^{-2}.
\end{align}
%
Plugging these relations with (\ref{eq:defSigma_mu}) in (\ref{eq:coupledF}), we obtain the RS free energy for the SC system.
%
\begin{definition}[RS free energy of the coupled system]
%
The replica symmetric free energy of the SC system, or SC potential, is
%
\begin{align}
F_{\rm{c}}(\tbf{E}) = &\sum_{\mu=0}^L\sum_{\nu \in \mu^{w}} \frac{(v-E_\mu) (v-E_\nu)}{4\Delta(2w+1)} \nonumber \\
- &\sum_{\mu=0}^L \mathbb{E}\ln\int P_0(x)\exp\Big(\frac{\Sigma_\mu(\tbf E)^{-2}}{2}(2 xs - x^2) + \Sigma_\mu(\tbf E)^{-1} zx\Big)dx. \label{def:RSf_SC}
\end{align}
\end{definition}
%
As for the underlying system, we obtain from (\ref{eq:fixedPointPotSC_isSE}) the following Lemma linking SE and potential formulations.
%
\begin{lemma}\label{lemma:fixedpointSE_extPot}
$\mathring E_\mu = [T_{\rm c}(\mathring {\tbf E})]_\mu \Leftrightarrow \frac{\partial F_{{\rm c}}({\tbf E})}{\partial E_\mu}\big|_{\mathring{{\tbf E}}} = 0 \ \forall \ \mu\in \mathcal{B}^{\rm c}=\{w+1:L-w-1\}$.
\end{lemma}
%
\subsection{Proof of threshold saturation}
%
The next monotonicity properties of the SE operators are essential in the proof. 
%
\begin{lemma}
The SE operator of the SC system maintains degradation in space, i.e. ${\tbf E} \succeq  {\tbf G} \Rightarrow T_{\rm{c}}({\tbf E}) \succeq T_{\rm{c}}({\tbf{G}})$. This property is verified by $T_{\rm{u}}(E)$ for a scalar error as well.
\label{lemma:spaceDegrad}
\end{lemma}
%
\begin{proof}
From \eqref{eq:defSigma_mu} it is immediately seen that ${\tbf E} \succeq  {\tbf G} \Rightarrow \Sigma_\mu({\tbf E}) \geq \Sigma_\mu({\tbf G})\ \forall \ \mu$. Now, the SE operator \eqref{def:SEop_SC} can be interpreted as an average over the spatial dimension of local MMSE's. The local MMSE's are the ones of random variables $s\sim P_0(s)$ sent through AWGN channels with effective noise $\mathcal{N}(\cdot | 0,\Sigma_\mu^2)$. The MMSE's are increasing functions of $\Sigma_\mu^2$: this is intuitively clear but we provide an explicit formula for the derivative below. Thus $[T_{{\rm c}}( {\tbf E})]_\mu \geq [T_{{\rm c}}( {\tbf G})]_\mu \ \forall \ \mu$, which means $T_{{\rm c}}({\tbf E}) \succeq T_{{\rm c}}({\tbf{G}})$.

The derivative of the MMSE of the Gaussian channel with i.i.d noise $\mathcal{N}(\cdot|0, \Sigma^2)$ can be computed as 
%
\begin{align}
 \frac{d \ \! {\rm mmse}(\Sigma)}{d(\Sigma^{-2})} = - 2 \mathbb{E}_{X,Y}\big[\|X - \mathbb{E}[X\vert Y]\|_2^2 \, {\rm Var}[X\vert Y]\big].
\end{align}
%
This formula explicitly confirms that $T_{\rm u}(E)$ (resp. $[T_{{\rm c}}(\tbf E)]_\mu$) is an increasing function of $\Sigma$ (resp. $\Sigma_\mu$).
\end{proof}
%
\begin{corollary}
\label{cor:timeDegrad}
The SE operator of the coupled 
system maintains degradation in time, 
i.e., $T_{{\rm c}}({\tbf E}^{(t)}) \preceq  {\tbf E}^{(t)}\Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \preceq  {\tbf E}^{(t+1)}$. 
Similarly $T_{{\rm c}}({\tbf E}^{(t)}) \succeq  {\tbf E}^{(t)} \Rightarrow T_{{\rm c}}({\tbf E}^{(t+1)}) \succeq  {\tbf E}^{(t+1)}$. 
Furthermore, the limiting error profile ${\tbf E}^{(\infty)} \defeq T_{{\rm c}}^{(\infty)}({\tbf E}^{(0)})$
exists. This property is verified by $T_{{\rm u}}(E)$ for the underlying system as well.
\end{corollary}
%
\begin{figure}[!t]
\centering
\includegraphics[width=0.65\textwidth]{figs/profile_E}
\vspace*{-5pt}
\caption{A fixed point profile $\tbf{E}^{*}$ of the coupled SE (solid) is null $\forall \ \mu \le w$ and increases until $E_{{\rm max}} \in [0,v]$ at $\mu_{\rm max}\in \{w+1:L-w-1\}$. Then it decreases and is again null $\forall \ \mu \ge L-w$. The associated \emph{saturated} profile $\tbf E$ (dashed) starts at $E_0 \ \forall \ \mu \le \mu_*$, where $\mu_*$ is defined by: $E^{*}_{\mu}\le E_0 \ \forall \ \mu\le \mu_*$ and $E^{*}_{\mu'} > E_0 \ \forall \ \mu' > \mu_*$. Then it matches $\tbf E^{*} \ \forall \ \mu \in\{\mu_*:\mu_{\rm max}\}$ and saturates $E_{{\rm max}} \ \forall \ \mu \ge \mu_{\rm max}$. By construction ${\tbf E}$ is non decreasing and ${\tbf E} \succeq {\tbf E}^{*}$.}
\label{fig:errorProfile}
\end{figure}
%
\begin{proof}
The degradation statements are a consequence of Lemma~\ref{lemma:spaceDegrad}. The existence 
of the limits follows from the monotonicity of the operator and boundedness of the MSE.
\end{proof}
%
The pinning condition together with the monotonicity properties of the coupled SE operator ensures that any fixed point point profile ${\tbf E}^*$ must adopt a shape similar to Fig.~\ref{fig:errorProfile}. 
From now on we work with a \emph{saturated profile} $\tbf E$, which construction is described in detail in Fig.~\ref{fig:errorProfile}. The associated saturated profile verifies ${\tbf E} \succeq {\tbf E}^{*}$, where ${\tbf E}^{*}$ is the fixed point profile of the coupled SE operator \eqref{def:SEop_SC}. In the next, we will need the following operator.
%
\begin{definition}[Shift operator]
The shift operator is defined componentwise as $[\text{S}({\tbf E})]_1 \defeq E_0, \ [\text{S}({\tbf E})]_\mu \defeq  E_{\mu-1}$.
\end{definition}
%
The first main step in the proof of threshold saturation is based on the Taylor expansion of the RS free energy of the SC system. It starts with the following Lemma.
%
\begin{lemma}\label{leminterp}
Let ${\tbf E}$ be a saturated profile. If ${\tbf E}_\lambda \defeq (1-\lambda) {\tbf E} + \lambda \text{S}({\tbf E})$ and $\delta {E}_{\mu} \defeq {E}_{\mu} -{E}_{\mu-1}$, then for a proper $\lambda\in[0,1]$,
%
\begin{align}
F_{{\rm c}}(\text{S}({\tbf E})) &-F_{{\rm c}}({\tbf E}) = \frac{1}{2} \sum_{\mu,\mu'=1}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 F_{{\rm c}}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}. \label{eq:lemma_secondDerivativeFsc}
\end{align}
%
\label{lemma:Fdiff_quadraticForm}
\end{lemma}
%
\begin{proof}
%
$F_{{\rm c}}(\text{S}({\tbf E})) - F_{{\rm c}}({\tbf E})$ can be expressed as
%
\begin{align}
F_{{\rm c}}(\text{S}({\tbf E})) -F_{{\rm c}}({\tbf E}) = \frac{1}{2}\sum_{\mu,\mu'=1}^{L} \delta {E}_{\mu} \delta {E}_{\mu'}  \frac{\partial^2 F_{{\rm c}}({\tbf E})}{\partial E_{\mu}\partial  E_{\mu'}}\Big|_{ {\tbf E}_\lambda} - \sum_{\mu=1}^{L} \delta {E}_{\mu} \frac{\partial F_{{\rm c}}({\tbf E})}{\partial  E_\mu}\Big|_{{\tbf E}}. \label{eq:expFbsminusFb}
\end{align}
%
By saturation of $\tbf E$, $\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{1:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$. Moreover for $r\notin\mathcal{A}$, $E_\mu=[T_{\rm c}(\tbf E)]_\mu$, and thus by Lemma~\ref{lemma:fixedpointSE_extPot} the potential derivative cancels at these positions. Hence the last sum in (\ref{eq:expFbsminusFb}) cancels.
\end{proof}
%
We thus need to compute the Hessian associated with this free energy.
%
\begin{align}
\frac{\partial F_{\rm{c}}({\tbf E})}{\partial {E_\mu}} &= \sum_{\nu \in \mu^{w}} \frac{E_\nu}{2\Delta(2w+1)} -\frac{1}{2} \sum_\nu \frac{\partial \Sigma_\nu(\tbf E)^{-2}}{\partial E_\mu} [T_{\rm{c}}({\tbf E})]_\nu - \frac{v}{2\Delta} \nonumber\\
%
&= \frac{1}{2\Delta(2w+1)}\Big(\sum_{\nu \in \mu^{w}} E_\nu-\sum_{\nu \in \mu^w} [T_{\rm{c}}({\tbf E})]_\nu\Big)- \frac{v}{2\Delta},\\
%
\Rightarrow\frac{\partial^2 F_{\rm{c}}({\tbf E})}{\partial {E_\mu}\partial {E_{\mu'}}} &= \frac{1}{2\Delta(2w+1)}\Big( \mathbb{I}(\mu' \in \mu^w) - \frac{1}{\Delta(2w+1)}\sum_{\nu \in \mu^w\cap {\mu'}^w} \frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \, \Sigma_\nu^{-2}} \Big). \label{eq:hessian_explicit}
\end{align}
%
We can now compute the r.h.s of \eqref{eq:lemma_secondDerivativeFsc}. Define $\delta E^* = {\rm{max}} \,|\delta E_\mu|$. Due to the indicator function, the first term in \eqref{eq:hessian_explicit} can be bounded as
%
\begin{align}
\frac{1}{2\Delta(2w+1)} \Big|\sum_{\mu, \mu'\in \mu^w}\delta E_{\mu}\delta E_{\mu'}\Big| \le \frac{\delta E^*}{2\Delta} \Big|\sum_{\mu}\delta E_{\mu}\Big| \le \frac{\delta E^*}{2\Delta} |E_L - E_0|,
\end{align}
%
where we have used the fact that the sum is telescopic for the last inequality. Notice now the following important smoothness property verified by a saturated profile.
%
\begin{lemma}
A saturated profile ${\tbf E}$ is smooth, i.e. $\delta E^* \le K^*/w$ for some $K^*=\mathcal{O}(1)$.
\end{lemma}
%
\begin{proof}
By saturation of $\tbf E$, $\delta E_\mu=0 \ \forall \ \mu \in\mathcal{A}\defeq\{1:\mu_*\}\cup \{\mu_{\rm max}+1:L\}$. For $\mu \notin\mathcal{A}$, we can replace $E_\mu$ by $[T_{\rm c}(\tbf E)]_\mu$ and Taylor expand the SE operator. Define $\delta \Sigma_\mu^{-2} \defeq \Sigma_{\mu+1}({\tbf E})^{-2} - \Sigma_\mu({\tbf E})^{-2}$. One can notice from \eqref{eq:defSigma_mu} that $\delta \Sigma_\mu^{-2} = (E_{\mu - w}-E_{\mu+w+1})/(\Delta(2w+1))$, where $E_{\mu - w}-E_{\mu+w+1} \le 1)$. Call $K=\mathcal{O}(1)$ some constant. We assume that the coupled SE operator is Lipshitz continuous with Lipshitz constant $K_T$ independent of the coupling window $w$. Then we obtain
%
\begin{align} \label{eq:deltamstar}
|\delta E_{\mu+1}| &= |[T_{\rm{c}}({\tbf E})]_{\mu +1} - [T_{\rm{c}}({\tbf E})]_{\mu}| \le K \delta \Sigma_\mu^{-2} \Big|\frac{\partial [T_{\rm{c}}({\tbf E})]_{\mu}}{\partial \Sigma_\mu^{-2}}\Big| \le K^*/w \eqdef \delta E^* \ \forall\ \mu.
\end{align}
%
% which is the desired result. Thus ${\tbf E}$ is smooth in the sense that its closeby variations are getting smaller as $w$ increases.
%
\end{proof}
%
Let us now study the second term of \eqref{eq:hessian_explicit} (without considering the boundaries for sake of simplicity, despite they can be included easily)
%
\begin{align}
-&\frac{1}{2\Delta^2(2w+1)^2} \sum_{\mu, \mu'} \delta E_\mu \delta E_{\mu '} \sum_{\nu \in \mu^w\cap {\mu'}^w} \frac{\partial [T_{\rm{c}}({\tbf E})]_\nu }{\partial \Sigma_{\nu}^{-2}} \nonumber\\ 
%
\le \ &\frac{K_T \delta E^*}{2\Delta^2(2w+1)^2} \sum_{\mu} \delta E_\mu \sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mu^w\cap {\mu'}^w). \label{eq:last_secondTerm_boudHessian}
\end{align}
%
Now, it is easy to show that for a fixed $\mu$, $\sum_{\mu'\in \{\mu - 2w : \mu + 2w\}} {\rm card}(\mu^w\cap {\mu'}^w) = (2w+1)^2$. Thus \eqref{eq:last_secondTerm_boudHessian} can be upper bounded, using (\ref{eq:deltamstar}), by $K_T \delta E^* |E_L-E_0|/(2\Delta^2) = K'/w$ for some $K'=\mathcal{O}(1)$. From this analysis and using the triangle inequality for the last step, we get
%
\begin{align}
\frac{1}{2}\Big| \sum_{\mu,\mu'=1}^{L} \delta {E}_\mu \delta {E}_{\mu'} \frac{\partial^2 F_{{\rm c}}({\tbf E})}{\partial  E_{\mu}\partial  E_{\mu'}}\Big|_{{\tbf E}_\lambda}\Big| \le U / w, \quad U=\mathcal{O}(1).
\end{align}
%
Combining this inequality with Lemma~\ref{leminterp}, we can assert the next Lemma.
%
\begin{lemma} \label{lemma:dF_ge_Uoverw}
For a saturated profile $\tbf E$, $|F_{{\rm c}}(\text{S}({\tbf E})) -F_{{\rm c}}({\tbf E})|\le U / w$, where $U=\mathcal{O}(1)$ is independent of $w,L$.
\end{lemma}
%
The second main step in the proof is based on a direct evaluation of the free energy change when shifting the saturated profile. We will need the following Lemmas.
%
\begin{lemma}
Let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_0$. Then $ E_{\rm max} \notin \mathcal{V}_0$.
\label{lemma:outside_basin}
\end{lemma}
%
\begin{proof}
The non decreasing error profile and the assumption that ${\tbf E} \succ {\tbf E}_0$ imply that $E_{\rm max} > E_{0}$. Moreover,
%
$E_{\rm max} \le [T_\text{c}({\tbf E})]_{\mu_{\rm max}} \le T_\text{s}(E_{\rm max})$
%
where the first inequality follows from $\tbf E\succ \tbf E^*$ and the monotonicity of $T_\text{c}$, while the second comes from the fact that $\tbf E$ is non decreasing. Combining these with the 
monotonicity of $T_\text{s}$ gives $T_{\text s}(E_{\rm max}) \ge  E_{\rm max} \Rightarrow T_{\text s}^{(\infty)}( E_{\rm max}) \ge  E_{\rm max}> E_0 \Rightarrow  E_{\rm max} \notin \mathcal {V}_0$.
\end{proof}
%
\begin{lemma}\label{lemma:FcSE_minus_FcE_le_deltaF}
Let ${\tbf E}$ be a saturated profile such that ${\tbf E}\succ {\tbf E}_0$. Then $|F_{\rm{c}}(S(\tbf{E})) - F_{\rm{c}}(\tbf{E})| \ge \delta F_{\rm{u}}$, where $\delta F_{\rm{u}}$ is the free energy gap, see Definition~\ref{def:fgap}.
\end{lemma}
%
\begin{proof}
Call $I(\Sigma) \defeq \mathbb{E}\ln\int P_0(x)\exp\big(\frac{\Sigma^{-2}}{2}(2 xs - x^2) + \Sigma^{-1} zx\big)dx$. Then we have from \eqref{def:RSf_SC} that $F_{\rm{c}}(S(\tbf{E})) - F_{\rm{c}}(\tbf{E})$ is equal to
\begin{align}
% \delta F_{\rm{c}}&=\sum_{\mu=1}^L \Big[\sum_{\nu \in \mu^{w}} \frac{(v-E_{\mu-1}) (v-m_{\nu-1}) }{4\Delta(2w+1)} - I(\hat \Sigma_{\mu-1})\Big] - \sum_{\mu=1}^L \Big[\sum_{\nu \in \mu^{w}} \frac{(v-E_{\mu})(v- E_{\nu})}{4\Delta(2w+1)} - I(\hat \Sigma_{\mu}) \Big] \nonumber \\
%
\sum_{\nu \in 0^{w}} \frac{(v-E_{0}) (v-E_{\nu}) }{4\Delta(2w+1)} - I(\Sigma_{0}) - \sum_{\nu \in L^{w}} \frac{(v-E_{L})(v-E_{\nu}) }{4\Delta(2w+1)} + I(\Sigma_{L}), \label{eq:lastFcSE_minus_FcE}
\end{align}
%
using the telescoping nature of the sum. Now notice that thanks to the saturation of the saturated profile at the boundaries, one gets from \eqref{eq:effNoise} and \eqref{eq:defSigma_mu} that $\Sigma_{0}({\tbf E}) = \Sigma(E_0)$, $\Sigma_{L}({\tbf E}) = \Sigma(E_L)$ where $E_L = E_{\rm{max}}$. So finally, we can write from \eqref{eq:lastFcSE_minus_FcE} that
%
\begin{align}
F_{\rm{c}}(S(\tbf{E})) - F_{\rm{c}}(\tbf{E}) &= \Big[\frac{(v-E_{0})^2 }{4\Delta} - I(\Sigma(E_0)) \Big] - \Big[\frac{(v-E_{L})^2 }{4\Delta} - I(\Sigma(E_L)) \Big] \nonumber\\
%
&= F_{\rm{u}}(E_0) - F_{\rm{u}}(E_L) \le -\delta F_{\rm{u}},
\end{align}
%
where we recognized \eqref{eq:RSf} and the last inequality is a direct application of Lemma~\ref{lemma:outside_basin}. Finally, using the positivity of $\delta F_{\text{u}}$ as $\Delta<\Delta_{\txt{pot}}$, we obtain the desired result.
\end{proof}
%
Combining these results, we can now prove the threshold saturation Theorem.
%
\begin{theorem} \label{th:mainth_thsat}
Assume a spatially coupled instance of rank one matrix estimation is to be solved. Fix $\Delta<\Delta_{\rm{pot}}$, $w>U/\delta F_{\rm{u}}$ ($U=\mathcal{O}(1)$ is independent of $w,L$) and $L>2w$ (such that the problem is well defined, due to the pinning condtition). Then any fixed point profile ${\tbf{E}^*}$ of the coupled state evolution satisfies ${\tbf{E}}^* \prec {\tbf{E}}_0$.
\end{theorem}
%
\begin{proof}
Assume that, under these hypotheses, there exists 
a saturated profile $\tbf E$ associated to $\tbf E^*$ such 
that $\tbf E\succ {\tbf{E}}_0$. Combining Lemma~\ref{lemma:dF_ge_Uoverw} and \ref{lemma:FcSE_minus_FcE_le_deltaF} we get $\delta F_{\text{u}}\le U/w \Rightarrow w \le U/\delta F_{\text{u}}$, a contradiction. 
Hence, ${\tbf{E}} \preceq {\tbf{E}}_0$. Since $\tbf E \succ {\tbf E}^*$ we have ${\tbf E}^* \prec {\tbf{E}}_0$.
\end{proof}
%
The Lemma follows from the last Theorem and Definition~\ref{def:AMPcoupled}. It says that the AMP threshold for the coupled codes saturates the potential threshold.
%
\begin{corollary}\label{cor:maincorollary_thsat}
By first taking $L \to \infty$ and then $w\to\infty$, the AMP threshold of the coupled ensemble satisfies $\Delta_{\rm c}\geq \Delta_{\rm{pot}}$.
\end{corollary}

==> v5 arxiv/settings_custom.tex <==
% new commands
\newcommand*\NewPage{\null\thispagestyle{empty}\newpage}
\def \L{{\cal L}}
\def \({\left(}
\def \){\right)}
\def \[{\left[}
\def \]{\right]}
\newcommand{\tbf}[1]{{\textbf{#1}}}
\newcommand{\bsy}[1]{{\boldsymbol{#1}}}
\newcommand{\txt}[1]{\text{#1}}
\newcommand{\defeq}{\vcentcolon=}
\newcommand{\eqdef}{=\vcentcolon}
\newcommand{\cv}[1]{\underline{#1}}
\newcommand{\bQ}{{\textbf{Q}}}
\newcommand{\bq}{{\textbf{q}}}
\newcommand{\bm}{{\textbf{m}}}
\newcommand{\br}{{\textbf{r}}}
\newcommand{\bF}{{\textbf{F}}}
\newcommand{\bff}{{\textbf{f}}}
\newcommand{\bG}{{\textbf{G}}}
\newcommand{\bW}{{\textbf{W}}}
\newcommand{\bZ}{{\textbf{Z}}}
\newcommand{\bY}{{\textbf{Y}}}
\newcommand{\bh}{{\textbf{h}}}
\newcommand{\bw}{{\textbf{w}}}
\newcommand{\bv}{{\textbf{v}}}
\newcommand{\bA}{{\textbf{A}}}
\newcommand{\bB}{{\textbf{B}}}
\newcommand{\bhx}{\hat{\textbf{x}}}
\newcommand{\bX}{{\textbf{X}}}
\newcommand{\bx}{{\textbf{x}}}
\newcommand{\bo}{{\textbf{o}}}
\newcommand{\blambda}{{\boldsymbol{\Lambda}}}
\newcommand{\btau}{{\boldsymbol{\tau}}}
\newcommand{\by}{{\textbf{y}}}
\newcommand{\bz}{{\textbf{z}}}
\newcommand{\bl}{{\textbf{l}}}
\newcommand{\bs}{{\textbf{s}}}
\newcommand{\bS}{{\textbf{S}}}
\newcommand{\bc}{{\textbf{c}}}
\newcommand{\bk}{{\textbf{k}}}
\newcommand{\bR}{{\textbf{R}}}
\newcommand{\beps}{{\boldsymbol{\epsilon}}}
\newcommand{\bxigma}{{\boldsymbol{\Sigma}}}
\newcommand{\bxi}{{\boldsymbol{\xi}}}
\newcommand{\bzero}{{\textbf{0}}}
\newcommand{\ba}{{\textbf{a}}}
\newcommand{\cC}{{\mathcal{C}}}
\newcommand{\cB}{{\mathcal{B}}}
\newcommand{\lab}[1]{\label{#1}}
\newcommand{\bxii}{{\boldsymbol{\xi}}}
\newcommand{\bre}{{\textbf {e}}}
\newcommand{\bytilde}{{\tilde{\textbf{y}}}}
\newcommand{\bxhat}{{\tilde{\textbf{x}}}}
\newcommand{\mc}{\mathcal}
\newcommand{\eps}{\varepsilon}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\s}{\sigma}
\renewcommand{\d}{\text{d}}
\newcommand{\e}{\text {e}}
\newcommand{\ds}{\Delta\sigma}
\newcommand{\hw}{h^{\rm W}}
\newcommand{\sw}{\sigma^{\rm W}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\de}{\partial}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\eq}{\text{ eq}}
\newcommand{\sign}{\text{ sign}}
\newcommand{\ua}{\uparrow}
\newcommand{\da}{\downarrow}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\mE}{\mathbb{E}}
\newcommand*{\xhat}[1]{#1\kern-0.50em\hat{\phantom{#1}}}

% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{\textbf{Lemma}}
% \newtheorem{thm}[theorem]{\textbf{Theorem}}
% \newtheorem{remark}[theorem]{\textbf{Remark}}
% \newtheorem{proposition}[theorem]{\textbf{Proposition}}
% \newtheorem{corollary}[theorem]{\textbf{Corollary}}
% \newtheorem{definition}[theorem]{\textbf{Definition}}
